On the Predictive Accuracy of Neural Temporal Point Process Models for Continuous-time Event Data

Temporal Point Processes (TPPs) serve as the standard mathematical framework for modeling asynchronous event sequences in continuous time. However, classical TPP models are often constrained by strong assumptions, limiting their ability to capture complex real-world event dynamics. To overcome this limitation, researchers have proposed Neural TPPs, which leverage neural network parametrizations to offer more flexible and efficient modeling. While recent studies demonstrate the effectiveness of Neural TPPs, they often lack a unified setup, relying on different baselines, datasets, and experimental configurations. This makes it challenging to identify the key factors driving improvements in predictive accuracy, hindering research progress. To bridge this gap, we present a comprehensive large-scale experimental study that systematically evaluates the predictive accuracy of state-of-the-art neural TPP models. Our study encompasses multiple real-world and synthetic event sequence datasets, following a carefully designed unified setup. We thoroughly investigate the influence of major architectural components such as event encoding, history encoder, and decoder parametrization on both time and mark prediction tasks. Additionally, we delve into the less explored area of probabilistic calibration for neural TPP models. By analyzing our results, we draw insightful conclusions regarding the significance of history size and the impact of architectural components on predictive accuracy. Furthermore, we shed light on the miscalibration of mark distributions in neural TPP models. Our study aims to provide valuable insights into the performance and characteristics of neural TPP models, contributing to a better understanding of their strengths and limitations.

==> alpha_plots.tex <==
\newgeometry{left=2cm,bottom=0.5cm,right=2cm, top=1.5cm}

\subsection{Github}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_github_filtered_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_github_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{MOOC}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_mooc_filtered_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_mooc_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{MIMIC2}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_mimic2_filtered_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_mimic2_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{LastFM}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_lastfm_filtered_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_lastfm_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Wikipedia}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_wikipedia_filtered_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_wikipedia_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hawkes Exponential Dependent}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_hawkes_exponential_mutual_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_hawkes_exponential_mutual_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hawkes Sum Exponential Dependent}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_hawkes_sum_exponential_mutual_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_hawkes_sum_exponential_mutual_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Twitter}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_twitter_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_twitter_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Taxi}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_taxi_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_taxi_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reddit Submissions}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_reddit_politics_submissions_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_reddit_politics_submissions_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PUBG}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_pubg_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_pubg_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Yelp Toronto}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_yelp_toronto_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_yelp_toronto_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Yelp Mississauga}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_yelp_mississauga_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_yelp_mississauga_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reddit Comments}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_reddit_askscience_comments_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_reddit_askscience_comments_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Yelp Airport}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_yelp_airport_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/coefficients/coefficients_yelp_airport_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\restoregeometry

==> base_tabular.tex <==
\begin{table}[!t]
\setlength\tabcolsep{1.2pt}
%\centering
\centering
\tiny
%\setlength\tabcolsep{1.3pt}
\caption{Average, median, and worst scores, as well as average ranks per decoder, with and without a base intensity term, for marked datasets. Refer to Section \ref{result_aggregation} for details on the aggregation procedure. Best results are highlighted in bold.}
\begin{tabular}{ccccccccccccccccccccc}
\toprule
& \multicolumn{20}{c}{Marked Datasets} \\ \\
               & \multicolumn{4}{c}{NLL-T} & \multicolumn{4}{c}{NLL-M} & \multicolumn{4}{c}{PCE} & \multicolumn{4}{c}{ECE} & \multicolumn{4}{c}{F1-score} \\ \\
               &            Mean & Median & Worst & Rank &     Mean & Median & Worst & Rank &      Mean & Median & Worst & Rank &      Mean & Median & Worst & Rank &     Mean & Median & Worst & Rank \\ \\
\midrule \\

       EC-B &            0.32 &           0.34 &           0.82 &          1.75 &           0.11 &          -0.04 &           1.23 &           2.0 & \textbf{0.19} & \textbf{0.19} &           0.4 & \textbf{1.38} &           0.4 &          0.37 &           0.5 &           2.0 &          0.24 &          0.22 &           0.0 & \textbf{1.75} \\
         EC-NB &   \textbf{0.28} &  \textbf{0.21} &  \textbf{0.79} & \textbf{1.25} & \textbf{-0.36} & \textbf{-0.34} &  \textbf{0.05} &  \textbf{1.0} &          0.19 &          0.19 & \textbf{0.39} &          1.62 & \textbf{0.37} & \textbf{0.34} & \textbf{0.49} &  \textbf{1.0} & \textbf{0.25} & \textbf{0.24} & \textbf{0.01} &          1.25 \\ \\

 
         LNM-B &            0.22 &           0.24 &           1.09 &           2.0 &           0.67 &           0.54 &           1.73 &           2.0 &          0.11 &          0.08 &          0.35 &           2.0 &          0.46 &          0.46 &           0.5 &           2.0 &          0.17 &          0.19 &           0.0 &  \textbf{2.0} \\
        LNM-NB &  \textbf{-0.64} & \textbf{-0.72} & \textbf{-0.24} &  \textbf{1.0} & \textbf{-0.88} & \textbf{-0.48} & \textbf{-0.19} &  \textbf{1.0} & \textbf{0.02} & \textbf{0.02} & \textbf{0.06} &  \textbf{1.0} & \textbf{0.36} & \textbf{0.34} & \textbf{0.44} &  \textbf{1.0} & \textbf{0.27} & \textbf{0.24} & \textbf{0.03} &           1.0 \\ \\
         RMTPP-B &  \textbf{-0.01} &  \textbf{-0.0} &  \textbf{0.17} & \textbf{1.38} &          -0.54 &          -0.23 &           0.12 &  \textbf{1.5} & \textbf{0.12} &  \textbf{0.1} & \textbf{0.27} & \textbf{1.12} & \textbf{0.35} &          0.33 & \textbf{0.45} &  \textbf{1.5} &          0.26 & \textbf{0.24} & \textbf{0.03} &          1.38 \\
      RMTPP-NB &            0.05 &           0.06 &           0.24 &          1.62 & \textbf{-0.67} & \textbf{-0.37} & \textbf{-0.14} &           1.5 &          0.13 &          0.13 &          0.27 &          1.88 &          0.35 & \textbf{0.32} &          0.45 &           1.5 & \textbf{0.27} &          0.24 &          0.03 & \textbf{1.62} \\ \\
            NH &   \textbf{0.87} &   \textbf{0.9} &  \textbf{1.42} & \textbf{1.38} &  \textbf{0.16} &           0.24 &           0.54 &  \textbf{1.5} & \textbf{0.24} & \textbf{0.32} &  \textbf{0.4} &          1.88 & \textbf{0.48} & \textbf{0.47} &  \textbf{0.5} & \textbf{1.25} & \textbf{0.17} & \textbf{0.16} &  \textbf{0.0} & \textbf{1.75} \\
          NH-B &            0.87 &            0.9 &           1.42 &          1.62 &           0.18 &  \textbf{0.23} &  \textbf{0.51} &           1.5 &          0.24 &          0.32 &           0.4 & \textbf{1.12} &          0.48 &          0.47 &           0.5 &          1.75 &          0.17 &          0.16 &           0.0 &          1.25 \\ \\
\bottomrule
\end{tabular}
\label{averageranks_baseline}
\end{table}

==> c_calibration.tex <==
\newgeometry{left=2cm,bottom=0.5cm,right=2cm, top=1.5cm}
\subsection{Github}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_gru_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_unmarked_gru.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_selfattention_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{MOOC}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_gru_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_unmarked_gru.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_selfattention_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mooc_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Wikipedia}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_gru_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_unmarked_gru.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_selfattention_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_wikipedia_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{MIMIC2}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_gru_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_unmarked_gru.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_selfattention_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_mimic2_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{LastFM}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_gru_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_unmarked_gru.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_selfattention_base_fc.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_lastfm_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Hawkes Exponential Dependent}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_exponential_mutual_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_exponential_mutual_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_exponential_mutual_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-1cm}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_exponential_mutual_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_exponential_mutual_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_exponential_mutual_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-1cm}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hawkes Sum of Exponential Mutual}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_sum_exponential_mutual_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_sum_exponential_mutual_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_sum_exponential_mutual_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-1cm}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_sum_exponential_mutual_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_sum_exponential_mutual_selfattention_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_hawkes_sum_exponential_mutual_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-1cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Twitter}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_twitter_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_twitter_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_twitter_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_twitter_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_twitter_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_twitter_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Taxi}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_taxi_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_taxi_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_taxi_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_taxi_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_taxi_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_taxi_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\subsection{Reddit Submissions}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_politics_submissions_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_politics_submissions_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_politics_submissions_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_politics_submissions_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_politics_submissions_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_politics_submissions_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{PUBG}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_pubg_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_pubg_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_pubg_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_pubg_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_pubg_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_pubg_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Yelp Mississauga}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_mississauga_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_mississauga_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_mississauga_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_mississauga_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_mississauga_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_mississauga_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Yelp Toronto}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_toronto_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_toronto_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_toronto_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_toronto_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_toronto_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_toronto_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Reddit Comments}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_askscience_comments_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_askscience_comments_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_askscience_comments_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_askscience_comments_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_askscience_comments_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_reddit_askscience_comments_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Yelp Airport}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_airport_stub.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_airport_gru_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_airport_gru_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_airport_selfattention.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_airport_selfattention_base.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_yelp_airport_selfattention_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}



\restoregeometry

==> cd_diagrams_body.tex <==
\begin{figure}[t!]
\centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_NLLTime_marked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{Time NLL on marked datasets.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_NLLTime_unmarked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{Time NLL on unmarked datasets.}
     \end{subfigure}
    \vfill
    %\vspace{-1cm}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_TimeCal._marked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{TCE on marked datasets.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_TimeCal._unmarked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{TCE on unmarked datasets.}
     \end{subfigure}
     
     %\vspace{-1cm}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_NLLMark_marked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{Mark NLL.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_MarkCal._marked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{ECE.}
     \end{subfigure}
     %\vfill\vspace{-1cm}
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/cd_diag/stat_tests_holm_F1-score_marked_CPLNMLNK1MLPCMMLPMCRMTPPSACMSAMCHawkesPoisson.json.png}
     \vspace{-1.5cm}
     \caption{F1-score.}
     \end{subfigure}
     \vfill
\label{fig:class_reddit_lasftm}
\caption{Critical Distance (CD) diagrams per metric at the $\alpha=0.05$ significance level for all decoders. Each model's average rank is displayed on top, and a bold line joins models variations that are not statistically different.}
\label{cd_diagramsbody}
\end{figure}


==> d_calibration.tex <==

\newgeometry{left=2cm,bottom=0cm,right=2cm, top=0.5cm}
\subsection{Github}



\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_github_filtered_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{MOOC}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mooc_filtered_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Wikipedia}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_wikipedia_filtered_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{LastFM}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_lastfm_filtered_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{MIMIC2}


\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_mimic2_filtered_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\subsection{Reddit}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Hawkes Exponential Dependent}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_exponential_mutual_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Hawkes Sum of Exponential Dependent}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_conditional-poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_conditional-poisson.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_conditional-poisson_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_log-normal-mixture.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_log-normal-mixture.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_log-normal-mixture_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_mlp-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_mlp-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_mlp-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_mlp-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_mlp-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_mlp-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_rmtpp.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_rmtpp.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_rmtpp_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_selfattention-cm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_selfattention-cm.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_selfattention-cm_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\clearpage
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_gru_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_gru_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\vspace{-45pt}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_selfattention-mc.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_poisson_selfattention_selfattention-mc.png}
     \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_selfattention_selfattention-mc_base_fc.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_identity_poisson.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calD_hawkes_sum_exponential_mutual_stub_hawkes.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


All models assign probabilities between 0.2 and 0.3 to the predicted class. This was due to the simulated process having extremely similar realizations along all five dimensions, and so were also the mark-wise intensities estimated by the model. As $p^\ast(K = k) = \frac{\lambda_k^\ast(t)}{\lambda^\ast(t)})$, the predicted probability naturally falls around 0.2, i.e. the model randomly guesses the mark. \textbf{Generate processes that display quite different realizations along each dimension.}  

\restoregeometry

==> decoder_tabular.tex <==

\begin{table}[!t]
\centering
\tiny
\setlength\tabcolsep{1.3pt}
\caption{Average, median, and worst scores, as well as average ranks per decoder for marked datasets. Refer to Section \ref{result_aggregation} for details on the aggregation procedure. Best results are highlighted in bold.}
\begin{tabular}{ccccccccccccccccccccc}
\toprule
& \multicolumn{20}{c}{Marked Datasets} \\ \\
    & \multicolumn{4}{c}{NLL-T} & \multicolumn{4}{c}{NLL-M} & \multicolumn{4}{c}{PCE} & \multicolumn{4}{c}{ECE} & \multicolumn{4}{c}{F1-score} \\ \\
    &            Mean & Median & Worst &  Rank &     Mean & Median & Worst &  Rank &      Mean & Median & Worst &  Rank &      Mean & Median & Worst &  Rank &     Mean & Median & Worst & Rank \\ \\
\midrule \\ 
 EC &             0.3 &          0.27 &          0.81 &          6.62 &          -0.13 &           -0.2 &           0.64 &          4.12 &          0.19 &          0.19 &          0.39 &          8.12 &          0.39 &          0.36 &          0.49 &         5.25 &          0.24 &          0.23 &          0.01 &          5.12 \\
    LNM &  \textbf{-0.21} & \textbf{-0.2} &           0.4 & \textbf{3.38} &           -0.1 &          -0.01 &           0.73 &           5.5 & \textbf{0.07} & \textbf{0.06} &          0.18 &          3.88 &          0.41 &           0.4 &          0.47 &          6.0 &          0.22 &          0.23 &          0.02 &          5.25 \\
   LNK1 &            0.29 &           0.2 &          1.53 &          6.25 &            0.2 &           0.14 &           1.71 &          7.12 &          0.14 &          0.13 &          0.25 &          6.62 &          0.42 &          0.41 &          0.48 &         6.38 &          0.21 &          0.22 &          0.01 &          6.62 \\
    FNN &            0.39 &          0.38 &          0.63 &          7.88 &           0.03 &           0.02 &            0.4 &          6.88 &          0.15 &          0.21 &          0.24 &          6.88 &          0.43 &          0.44 &          0.49 &          8.0 &           0.2 &          0.19 &          0.01 &          7.25 \\
 MLP/MC &            0.12 &          0.01 &          0.42 &          5.25 &           0.02 &           -0.0 &           1.04 &           6.0 &          0.14 &          0.14 &          0.32 &          5.12 &          0.36 &          0.34 &          0.47 &         3.38 &          0.25 &          0.24 &          0.02 &          3.88 \\
  RMTPP &            0.02 &         -0.02 & \textbf{0.19} &          4.62 &          -0.61 &          -0.28 & \textbf{-0.01} & \textbf{2.12} &          0.13 &          0.12 &          0.27 &          4.62 &          0.35 &          0.33 &          0.45 &         2.62 &          0.27 &          0.24 &          0.03 &          2.62 \\
  SA/CM &            2.03 &         -0.19 &         17.62 &          3.38 &           0.23 &           0.11 &           1.04 &          7.62 &          0.08 &          0.09 & \textbf{0.17} & \textbf{3.25} &          0.42 &          0.43 &           0.5 &         7.88 &          0.19 &          0.16 &           0.0 &          8.75 \\
  SA/MC &            0.05 &          0.07 &          0.25 &          4.62 &          -0.03 &          -0.06 &           0.33 &          5.75 &          0.13 &          0.14 &          0.31 &          4.38 &          0.37 &          0.37 &          0.49 &          4.5 &          0.23 &          0.23 &          0.01 &           5.5 \\
 Hawkes &            0.73 &         -0.07 &          4.32 &           4.5 & \textbf{-4.73} & \textbf{-0.69} &           2.33 &           2.5 &          0.11 &          0.11 &          0.23 &          3.25 & \textbf{0.15} & \textbf{0.15} & \textbf{0.34} & \textbf{1.0} & \textbf{0.44} & \textbf{0.42} & \textbf{0.26} &           1.0 \\
Poisson &            1.16 &          1.08 &          1.69 &         10.38 &           1.27 &           0.84 &           4.15 &         10.88 &          0.24 &          0.34 &           0.4 &          9.88 &          0.48 &          0.48 &           0.5 &        10.62 &          0.16 &          0.15 &           0.0 & \textbf{11.0} \\
     NH &            0.87 &           0.9 &          1.42 &          9.12 &           0.16 &           0.24 &           0.54 &           7.5 &          0.24 &          0.32 &           0.4 &          10.0 &          0.48 &          0.47 &           0.5 &        10.38 &          0.17 &          0.16 &           0.0 &          10.5 \\
  
MRC &    \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &   \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &  \textbackslash &   \textbackslash &     0.16 &          0.16 &           0.0 &          10.38 \\ \\
\bottomrule
\end{tabular}

\label{averageranks_decoder_marked}
\end{table}








==> encoding_update.tex <==






==> history_plots.tex <==
\newgeometry{left=1cm,bottom=0cm,right=1cm, top=0.5cm}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{images/history/history_lastfm_filtered_gru-fixed.png}
    \includegraphics[width=1\linewidth]{images/history/history_mooc_filtered_gru-fixed.png}
    \includegraphics[width=1\linewidth]{images/history/history_wikipedia_filtered_gru-fixed.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \includegraphics[width=1\linewidth]{images/history/history_github_filtered_gru-fixed.png}
    \includegraphics[width=1\linewidth]{images/history/history_mimic2_filtered_gru-fixed.png}
    \includegraphics[width=1\linewidth]{images/history/history_hawkes_exponential_mutual_gru-fixed.png}
    \label{fig:my_label}
\end{figure}





\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_taxi_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_taxi_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}



\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_twitter_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_twitter_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}



\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_reddit_politics_submissions_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_reddit_politics_submissions_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_reddit_askscience_comments_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_reddit_askscience_comments_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_pubg_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_pubg_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_yelp_toronto_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_yelp_toronto_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_yelp_airport_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_yelp_airport_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.34\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_yelp_mississauga_selfattention-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.56\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_yelp_mississauga_gru-fixed.png}
     \end{subfigure}
\end{figure}
\end{center}



\begin{comment}
\begin{center} 
\begin{figure}[h!]
\centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/history/history_github_filtered_gru-fixed.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/calibration/calC_github_filtered_gru_base.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}
\end{comment}

\restoregeometry

==> historyencoder_update.tex <==
\begin{table}[!t]
\setlength\tabcolsep{1.2pt}
%\centering
\centering
\tiny
%\setlength\tabcolsep{1.3pt}
\caption{\textcolor{blue}{Average and median scores, as well as average ranks per decoder and variation of history encoder, for relevant marked datasets. Refer to Section \ref{result_aggregation} for details on the aggregation procedure. Best results are highlighted in bold.}}
 \begin{tabular}{ccccc@{\hspace{10\tabcolsep}}cccc@{\hspace{10\tabcolsep}}cccc@{\hspace{10\tabcolsep}}cccc@{\hspace{10\tabcolsep}}ccc}
\toprule \\
 & \multicolumn{19}{c}{Marked Datasets} \\ \\
               & \multicolumn{3}{c}{NLL-T} && \multicolumn{3}{c}{PCE} && \multicolumn{3}{c}{NLL-M} && \multicolumn{3}{c}{ECE} && \multicolumn{3}{c}{F1-score} \\ \\
               &            Mean &         Median &          Rank &&          Mean &        Median &          Rank &&           Mean &         Median &          Rank &&          Mean &        Median &          Rank &&          Mean &        Median &          Rank \\ \\
\midrule \\

CONS-EC &            1.83 &           1.28 &           3.0 &&          0.24 &          0.33 &          2.88 & &          0.98 &            0.6 &          2.75 &&          0.48 &          0.47 &           3.0 &&          0.16 &          0.15 &  \textbf{3.0} \\
SA-EC &            0.61 &           0.43 &          1.88 & &          0.2 &          0.22 &           2.0 &&          -0.07 &          -0.16 &          1.88 &&          0.41 &          0.39 &           2.0 & &         0.24 &          0.23 &          1.75 \\
GRU-EC &   \textbf{0.31} &  \textbf{0.15} & \textbf{1.12} & &\textbf{0.17} & \textbf{0.14} & \textbf{1.12} && \textbf{-0.26} & \textbf{-0.37} & \textbf{1.38} && \textbf{0.36} & \textbf{0.32} &  \textbf{1.0} && \textbf{0.25} & \textbf{0.24} &          1.25 \\\\
CONS-LNM &            0.02 &          -0.24 &          2.88 && \textbf{0.02} & \textbf{0.01} &          2.25 &&           0.94 &            0.6 &           3.0 &&          0.47 &          0.47 &           3.0 &&          0.16 &          0.15 &  \textbf{3.0} \\
SA-LNM &           -0.69 &          -0.66 &          1.88 &   &       0.02 &          0.02 &          2.12 & &         -0.74 &          -0.44 &          1.75 & &         0.38 &          0.35 &          1.88 &&          0.27 &          0.24 &          1.75 \\
GRU-LNM &  \textbf{-1.12} & \textbf{-0.92} & \textbf{1.25} &   &       0.02 &          0.01 & \textbf{1.62} && \textbf{-1.23} & \textbf{-0.89} & \textbf{1.25} && \textbf{0.33} & \textbf{0.32} & \textbf{1.12} && \textbf{0.28} & \textbf{0.26} &          1.25 \\\\
CONS-FNN &            1.24 &           0.79 &           3.0 &   &       0.16 &          0.22 &          2.75 &&           1.02 &            0.5 &           3.0 &&          0.46 &          0.47 &          2.75& &          0.18 &          0.16 &  \textbf{3.0} \\
SA-FNN &            0.56 &           0.29 &          1.88 && \textbf{0.15} &          0.21 &           2.0 & &          0.11 &           0.09 &          1.88 & &         0.43 & \textbf{0.44} &          1.75 &&          0.19 & \textbf{0.19} &          1.75 \\
GRU-FNN &   \textbf{0.36} &  \textbf{0.08} & \textbf{1.12} &&          0.15 & \textbf{0.18} & \textbf{1.25} && \textbf{-0.17} & \textbf{-0.08} & \textbf{1.12} && \textbf{0.41} &          0.45 &  \textbf{1.5} &&  \textbf{0.2} &          0.18 &          1.25 \\\\
CONS-MLP/MC &            0.82 &           0.66 &          2.88 &&          0.15 &          0.16 &          2.25 &&           1.14 &           0.61 &          2.75 &&          0.44 &          0.45 &           3.0 &&          0.19 &          0.16 &  \textbf{3.0} \\
SA-MLP/MC &            0.09 &           0.15 &          2.12 & &         0.14 &          0.14 &          2.38 &&           0.09 &          -0.04 &          1.75 &&          0.37 &          0.37 &           2.0 && \textbf{0.25} &          0.23 &          1.75 \\
GRU-MLP/MC &  \textbf{-0.28} & \textbf{-0.29} &  \textbf{1.0} && \textbf{0.13} & \textbf{0.11} & \textbf{1.38} &&  \textbf{0.02} & \textbf{-0.12} &  \textbf{1.5} && \textbf{0.33} & \textbf{0.32} &  \textbf{1.0} &&          0.24 & \textbf{0.24} &          1.25 \\\\
CONS-RMTPP &            1.12 &            0.8 &           3.0 &&          0.14 &          0.16 &           2.5 &&           1.47 &           0.67 &          2.75 &&          0.47 &          0.47 &           3.0 &&          0.15 &          0.15 &  \textbf{3.0} \\
SA-RMTPP &            0.11 &            0.1 &          1.88 &  &        0.13 &          0.13 &           2.0 & &         -0.46 &          -0.41 &          2.12 & &         0.37 &          0.34 &          1.88 & &         0.27 &          0.24 &          1.88 \\
GRU-RMTPP &  \textbf{-0.28} & \textbf{-0.22} & \textbf{1.12} & &\textbf{0.12} &  \textbf{0.1} &  \textbf{1.5} && \textbf{-1.05} & \textbf{-0.74} & \textbf{1.12} && \textbf{0.31} & \textbf{0.29} & \textbf{1.12} && \textbf{0.29} & \textbf{0.27} &          1.12 \\\\
CONS-SA/CM &           11.92 &           0.02 &           2.5 && \textbf{0.09} &           0.1 &          2.12 &&           1.24 &            0.5 &          2.75 &&          0.44 & \textbf{0.45} &          2.25 && \textbf{0.18} & \textbf{0.14} &          1.88 \\
SA-SA/CM &           10.28 &          -0.01 & \textbf{1.75} &  &        0.09 & \textbf{0.06} &          2.12 & &          0.53 &           0.13 &          1.88 & &\textbf{0.43} &          0.45 & \textbf{1.88} & &         0.18 &          0.12 &          1.88 \\
GRU-SA/CM &   \textbf{7.52} & \textbf{-0.07} &          1.75 & &         0.09 &          0.07 & \textbf{1.75} &&  \textbf{0.51} &   \textbf{0.1} & \textbf{1.38} &&          0.43 &          0.45 &          1.88 &&          0.18 &          0.13 & \textbf{2.25} \\ \\
CONS-SA/MC &            1.09 &           0.75 &           3.0 &&          0.17 &          0.22 &          2.62 &&           1.04 &           0.53 &           3.0 &&          0.45 &          0.46 &           3.0 &&          0.18 &          0.16 &  \textbf{3.0} \\
SA-SA/MC &            0.22 &           0.23 &          1.75 & &\textbf{0.15} & \textbf{0.15} &          1.88 & &          0.06 &           0.12 &          1.75 & &         0.41 &          0.42 &           2.0 & &\textbf{0.21} &           0.2 &          1.62 \\
GRU-SA/MC &   \textbf{0.16} &  \textbf{0.22} & \textbf{1.25} &&          0.15 &          0.15 &  \textbf{1.5} &&   \textbf{0.0} &  \textbf{0.04} & \textbf{1.25} &&  \textbf{0.4} & \textbf{0.41} &  \textbf{1.0} &&          0.21 & \textbf{0.21} &          1.38 \\\\
\bottomrule
\end{tabular}
\label{averageranks_historyencoder_update}
\end{table}

==> intensities_up.tex <==
\begin{figure}[!t]
\centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=0.98\textwidth]{images/intensities/LastFM-GRU-EC_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-GRU-LNM_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-GRU-FNN_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-GRU-MLP_MC_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-GRU-RMTPP_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-GRU-SA_CM_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-GRU-SA_MC_long.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intensities/LastFM-Hawkes_long.png}
     \end{subfigure}
\caption{Evolution of $\lambda^\ast(t)$ (red first event, orange second event) and $f(t|\mathcal{H}_t)$ (blue first event, green second event) between two events on the LastFM dataset. \textcolor{blue}{Arrival times correspond to 2.0975 and 2.0986, respectively.}}
\label{intensities_plot}
\end{figure}


==> intensity_plots.tex <==

\newgeometry{left=2cm,bottom=0cm,right=2cm, top=0.5cm}
\subsection{Hawkes Exponential Dependent}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_conditional-poisson.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_conditional-poisson.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_log-normal-mixture.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_log-normal-mixture.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_mlp-cm.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_mlp-cm.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_mlp-mc.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_mlp-mc.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_rmtpp.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_rmtpp.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_selfattention-cm.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_selfattention-cm.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_gru_selfattention-mc.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_selfattention_selfattention-mc.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_identity_poisson.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_exponential_mutual_stub_hawkes.png}
    \label{fig:my_label}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Hawkes Sum Exponential Dependent }

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_conditional-poisson.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_conditional-poisson.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_log-normal-mixture.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_log-normal-mixture.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_mlp-cm.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_mlp-cm.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_mlp-mc.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_mlp-mc.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_rmtpp.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_rmtpp.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_selfattention-cm.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_selfattention-cm.png}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_gru_selfattention-mc.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_selfattention_selfattention-mc.png}
    \label{fig:my_label}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_identity_poisson.png}
    \includegraphics[width=\textwidth]{images/intensity/intensity_hawkes_sum_exponential_mutual_stub_hawkes.png}
    \label{fig:my_label}
\end{figure}

\restoregeometry

==> losses.tex <==
\subsection{Github}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_github_filtered_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_github_filtered_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\subsection{Github Unmarked}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_github_filtered_unmarked_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_github_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{MOOC Unmarked}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_mooc_filtered_unmarked_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_mooc_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}




\clearpage
\subsection{MOOC}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_mooc_filtered_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_mooc_filtered_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\subsection{Wikipedia}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_wikipedia_filtered_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_wikipedia_filtered_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\subsection{Wikipedia Unmarked}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_wikipedia_filtered_unmarked_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_wikipedia_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{MIMIC2 Unmarked}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_mimic2_filtered_unmarked_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_mimic2_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}



\clearpage
\subsection{MIMIC2}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_mimic2_filtered_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_mimic2_filtered_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}



\clearpage
\subsection{LastFM}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_lastfm_filtered_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_lastfm_filtered_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\clearpage
\subsection{LastFM Unmarked}


\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_lastfm_filtered_unmarked_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_lastfm_filtered_unmarked_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Reddit Unmarked}

\clearpage
\subsection{Reddit}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Hawkes Exponential Mutual}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_hawkes_exponential_mutual_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_hawkes_exponential_mutual_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Hawkes Sum of Exponential Mutual}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_hawkes_sum_exponential_mutual_gru.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\begin{center} 
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{images/losses/loss_hawkes_sum_exponential_mutual_selfattention.png}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\subsection{Taxi}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_taxi_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_taxi_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Twitter}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_twitter_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_twitter_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\subsection{Reddit Submissions}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_reddit_politics_submissions_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_reddit_politics_submissions_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Reddit Comments}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_reddit_askscience_comments_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_reddit_askscience_comments_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\subsection{PUBG}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_pubg_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_pubg_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Yelp Mississauga}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_yelp_mississauga_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_yelp_mississauga_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\subsection{Yelp Airport}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_yelp_airport_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_yelp_airport_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

\subsection{Yelp Toronto}

\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_yelp_toronto_gru.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/losses/loss_yelp_toronto_selfattention.png}
     \end{subfigure}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}

==> notes.tex <==


%\listoftodos

\dobox{Differences in terms of datasets, methods, metrics, etc? New observations?}
\dobox{" Unfortunately, a thorough and fair comparison between different methods is difficult due to lack of standardized implementations and benchmarks."}

\dobox{Exploring Generative Neural Temporal Point Process (TMLR paper). Focus on predictive accuracy of generative models (MAPE, CRPS, QQplot-deviation, Top-1 accuracy). Weird results on CRPS.  Only report a single number for the QQplots (calibration). SEE COMMENTS APPENDIX A.}

\dobox{Start citing all TPP related papers. IN PROGRESS AS WRITING PROGRESSES.}


\dobox{Discuss weaknesess of existing review (architecture, granger causality, metrics (NLL, MAPE, Mark Accuracy), datasets (MOOC, stack overflow only) + Stack overflow (discuté comme non-adapté)). SEE COMMENTS APPENDIX A.}


\dobox{  * See comments in "user-dependent paper" on heterogeneity (see expression (9))}

\dobox{Regarder le commentaire openreview de lognormmix sur les différences entre les loss de la densité et des marks.}


\dobox{* Compare methods on computational complexity}

\dobox{Evaluation 1: LogS (time) + AUC (already implemented), MAE, MSE, calibration (on time and mark, we have both a regression and classification task)(rare to have both in ML)}

\textbf{Experiments}

\doTB{Evaluate models on Reddit. Create pertinent split of the dataset (in two) to lower runtime.}
\doTB{Evaluate Neural Hawkes model.}
\doTB{Assess impact of history size on models' performance.}
\begin{itemize}
    \item Done for GRU and SA without base term. 
    \item Runs in progress for GRU and SA with baseline. 
\end{itemize}
\doTB{Consider additional metrics, espicially the ones employed in \citep{lin2021empirical} and \citep{LinGenerative} (CRPS, ...)}
\doTB{Generate better looking figures.}
\doTB{Use carefully designed statistical tests to properly compare models' performance, i.e Adjusted Friedman test and Nemenyi post-hoc tests \citep{Demsar}.}
\begin{itemize}
    \item Done Friedmann + Schafer's post-hoc test. 
    \item Diagram implemented. 
\end{itemize}
\doTB{Implement sampling.}
\doTB{Consider additional encoder (LSTM?) and alternative event encodings (i.e. no encodings).}
\doTB{Search for complementary datasets. }

\doTB{Retrain LNM with one mixture. IN PROGRESS}
\begin{itemize}
    \item Done
\end{itemize}
\doTB{Retrain all modular models without softmax on coefficients. IN PROGRESS.}

\doTB{Continue cleaning code.}


\textbf{Writing}

\doTB{Add optimzation subsection in background and notation section. Make the decomposition in term of time NLL, mark NLL, and window NLL explicit.}
\doTB{Add 'Metrics' section in Result and Discussion section.}
\doTB{Add figures to text.}
\doTB{Update Pipeline figure.}
\doTB{Rework Results and Discussion section (i.e. make it more structured and readable).}

- Make $\lambda$ explicitely function of $\theta$.
- Changer les noms des méthodes. 
- Décomposition $\lambda_k = \lambda p(k|t)$ dans background et notation. 

\clearpage
\section{Notes}


\begin{center} 
\begin{figure}[h]
\centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/distlastfm.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/distreddit.png}
     \end{subfigure}
\caption{Distributions of the 3150 marks of LastFM (left) and of the 984 marks of Reddit (right). Classes are sorted on the horizontal axis according to their occurrence. The most represented classes account for 0.006\% and 0.087\% of events respectively.}
\label{fig:class_reddit_lasftm}
\end{figure}
\end{center}


\dobox{Add key points}

\textbf{Continuous calibration}. At the exception of LogNormMix, all models used in this experimental study appear to be poorly (marginally) calibrated on all datasets. More specifically, all models tend to assign too little probability mass to the observed arrival times, as illustrated by the calibration curve being systematically above the baseline. This means that the modeled marginal distributions tend to be shifted to the right of the continuous time domain with respect to the observed marginal distribution of arrival times. Consequently, under the modeled distributions, high probability mass gets assigned to high arrival times, although the latter do not form the bulk of the observed distribution. A notable expection concerns the mlp-mc and selfattention-mc decoders equipped with a self-attention encoder on the MIMIC2 dataset, both displaying a completely opposite behaviour. Indeed, for these models, the modeled CDF is systematically close to 1 when evaluated on the arrival times. This could indicate that almost all the probability mass is assigned to arrival times close to 0. \textbf{Check calibration analysis in litterature to better write this section}. \textbf{Add comment explaining why the inductive biases of LogNormMix make it better calibrated.}


On the time NLL, LogNormMix performs the best across all datasets (only tie with RMTPP on MIMIC2), with an impressive gain in performance when a base intensity term is added to the model (not on MOOC, Wikipedia, MIMIC2, PUBG only SA). Same conclusion for the calibration of the inter-arrival times, with more impressive differences regarding other models on marked datasets (at the exception of MIMIC2).

On the Mark NLL, LogNormMix is often amongst the top performing models, but when a base intensity term is added to the model, the performance drops drastically (only not observed on MOOC). The drop is often proportional to the increase in time NLL. 




\begin{itemize}
    \item Overall, LogNormMix performs the best accross all datasets, significantly outperforming all other baselines on the negative log-likelihood.
    \item On Wikipedia, the conditional Poisson decoders perform worst, indicating that a piece-wise constant intensity is a too strong modeling assumption, i.e. the inter-arrival times do not seem to follow an exponential distribution. Their poor performance is mostly explained by their inability to correctly model the mark distribution, which forms by a high margin the greatest contribution to the overall loss. \textbf{What does the conditional Poisson model tell us regarding the mark distribution ?}
    \item Most of the time, the greatest contributions to the total negative log-likelihood comes from the mark loss terms. Conversely, the density term tends to drive the loss downward for most datasets, indicating that the models struggle less at modeling the arrival time distributions than the mark distributions. 
    \item The window term corresponds to the log-probability of observing no events between $t_n$ and $T$, meaning that the lowest achievable score for this term is 0. For most models, this term contributes to a small proportion of the overall loss, meaning that the models tend to correctly assign a quasi-null probability to observe an event in [$t_n, T$]. However, for decoders that estimate the window term using Monte Carlo integration, the opposite behaviour is observed. Indeed, for such models and on all datasets at the exception of Github, the window integral window actually contributes to the loss by a significant margin. This may indicate that estimating the integral term in the negative log-likelihood using Monte Carlo integration can lead to high approximation errors. \textbf{Can it be linked to the average length of the window interval ? To be checked. Previous results were obtained using an ill-defined window boundary , and hence, they were not trustworthy. Updated results do not include a window term anymore, so this comment is not relevant.}
    
    
    \item \citep{EHR} also evaluated these models on MIMIC2, and found the Self-attention/MC decoder to perform well with respect to other baselines on the negative log-likelihood. However, for each sequence, they considered the window boundary as its last observed event, this way discarding the window integral in the loss computation. However, considering this integral term completely changes the performance of the model, as it constitutes the highest loss contribution. 
    \item The SA-SA/MC model achieves 0 Precision, Recall and F1 score on the MIMIC2 dataset. This is in clear contrast with the results of \citep{EHR}, in which they found this model to be amongst the top performing baselines. \textbf{Check if no issue}.
    \item No clear winner stands out between GRU or self-attention encoders. 
    \item Although making the explicit assumption of a mark distribution independent of the time given the history of the process, LogNormMix and RMTPP often achieve best performance in modeling the mark distribution (best two with respect to the negative log-likelihood on MOOC, MIMIC2 and Github). This observation is further confirmed by their Precision, Recall and F1 scores on all but the Github dataset, for which they significantly outperform all baselines. \textbf{Is the best score explained by the hypothesis of LogNormMix and RMTPP (are marks indeed conditionally independent of the time given the history of the proces ?) or is it because separately parametrizing the arrival time distribution and the mark distribution makes the model easier to train ?}
    \item As argued in \citep{UserDep}, most TPP models typically assume that all realized sequences come from the same underlying data distribution. In practice however, such hypothesis is not systematically met, as sequences may arise from different sources, and hence, show significant heterogeneity among themselves. They further hypothesized that the mark distribution across sequences was likely to be responsible for the most part of this heterogeneity. In our experiments, the greatest contribution to the loss can be directly associated to the estimated mark distributions, an observation that tends to support this argument. 
    \item Important observation made in \citep{IntensityFree}. The negative log-likelihood is actually very sensitive to the scale of the data. Assume $\tau$ is distributed according to $p(\tau)$ and we are interested in the distribution of $y = a\tau$. According to the change of variable formula, $q(y=a\tau) = \frac{1}{a}p(\tau)$, which means that $-\text{log}~q(y=a\tau) = -\text{log}~p(\tau) + \text{log}~(a)$. Consequently, the negative log-likelihood can shifted arbitrarily by choosing different values of $a$. In this context, we cannot directly compare the time density NLL to the mark distribution NLL, as the former can be made arbitrarily low or large by scaling the inter-arrival times. However, as $\nabla_\theta~\mathcal{L}(\theta) = \nabla_\theta\big(-\text{log}~p(\tau;\theta) + \text{log}~(a)\big) = \nabla_\theta \big(-\text{log}~p(\tau;\theta)\big)$, the gradient of the negative log-likelihood is not influenced by the scale of the inter-arrival times, and hence, neither should be the training process. 
\end{itemize}    


\textbf{Independence of sequences}. During training and at inference time, all sequences are processed independently of one another. This protocol explicitly assumes such sequences to be independent realizations of the same underlying process. While this assumption might be suitable in certain scenarios, it may as well be to constraining in many other cases. For instance, consider the MOOC dataset that records students activity on an online course system (watching a video, solving a quiz, ...). The actions performed by a student are often solemnly isolated, but rather influenced by the actions his fellow students carried out previously. A student might decide to take on a quiz because he heard that his friend already took it. Similarly, on an online shopping platform, we might decide to purchase a specific item because other people got it previously. In this sense, the course of actions of an individual directly influences others. 



\clearpage
\section{Strengths and weaknesses of previous experimental study}

\subsection{\citep{lin2021empirical}}

\textbf{Strengths}. 
\begin{itemize}
    \item Considers a greater number of neural architectures than me. 
    \item Application of TTP to causal discovery. 
    \item Next event time predicition. Does not mention in the paper how it is actually done. 
    \item They say that the time distirbution and the mark distribution are independent in the learning process, which is incorrect in the general case. 
\end{itemize}

\textbf{Weaknesses}. 
\begin{itemize}
    \item Does not consider statistical TPP models. 
    \item Number of datasets limited (Only MOOC and Stackoverflow)
\end{itemize}

\subsection{\citep{LinGenerative}}

\textbf{Proposed contributions.}
\begin{itemize}
    \item Focus on predictive performance of deep generative models (i.e. in terms of MAPE) rather than "goodness-of-fit". Transfer of deep generative models to the field of TPP (Diffusion denoising, Variational Autoencoder, conditional GAN, Normalizing flows, Noise score network).
    \item Modification of the self-attentive encoder by making the attention weights "time aware", such that the relative position in time of arrival-times in the history is taken into account. Attention weights are now also influenced by the similarity between two event types. However, experimental results showed marginal gain in performance for the modified attention architectures. 
    \item Performance comparison of probabilistic decoders:
    \begin{itemize}
        \item RMTPP, LogNorMix, \textbf{ERTPP}, \textbf{WeibMix}, Self-attentive Hawkes Process, Transformer Hawkes Process. 
    \end{itemize}
    \item Metrics employed for model comparison:
    \begin{itemize}
        \item MAPE on event time prediction. (time predicted through sampling or estimation of the expectation ?).
        \item CRPS
        \item QQP-Dev : Comparison of the distribution of the cumulative intensity to a an exponential distribution of rate 1. This is equivalent to comparing the distribution of the cumulative density to a uniform distribution in [0,1] (as I have done so far). They simply report the absolute deviation with respect to the baseline line. 
        \item Top 1 and top 3 accuracy in mark prediction. 
    \end{itemize}
    \item Datasets used:
    \begin{itemize}
        \item Real-word datasets: MOOC, Retweet, Stack Overflow, Yelp (which one ?). 
        \item Synthetic data: Hawkes process with different kernels. 
    \end{itemize}
    \item Complexity comparison in term of single epoch time and memory. 
    consumption.
    \item Sensitivity analysis.
\end{itemize}

\textbf{Differences with current paper}. 
\begin{itemize}
    \item My focus is on goodness of fit of probabilistic decoders, and not on predictive ability of deep generative models. 
    \item Other decoders considered : Conditional Poisson, MLP-CM, Selfattention-CM. 
    \item Considering non Neural baselines (Hawkes)
    \item Other datasets considered :
    \begin{itemize}
        \item Marked : Reddit, Wikipedia, LastFM, MIMIC2, Github
        \item Unmarked : Taxi, Twitter, PUBG, Yelp Toronto, Yelp Mississauga, Yelp airport, Reddit Submissions, Reddit Comments. 
        \item Synthetic : Gaussian, Poisson, Inhomogeneous Poisson. 
    \end{itemize}
    \item Influence of the mark on the estimated intensity/density.
    \item Study of the influence of the different terms in the NLL. 
    \item Discrete calibration (+ plots) and continuous calibration (+ plots), not only single metric.
    \item Other discrete metrics : Precision, Recall, F1 score
    \item Visualisation of the estimated intensities for synthetic datasets. 
    \item \textbf{Possible additions :} 
    \begin{itemize}
        \item Additional decoders: Neural Hawkes, ERTPP, WeibMix ? 
        \item Additional encoders: LSTM ? 
    \end{itemize}
\end{itemize}

\textbf{Strengths.}
\begin{itemize}
    
\end{itemize}

\textbf{Weaknesses.}
\begin{itemize}
    \item No real discussion as per why some architectures perform favorably compared to others. 
\end{itemize}


==> results_tabular.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newgeometry{left=2cm,bottom=2cm,right=2cm, top=1cm}
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
                models & \multicolumn{12}{c}{NLL Time} \\
                       & \multicolumn{2}{c}{lastfm_filtered} & \multicolumn{2}{c}{mooc_filtered} & \multicolumn{2}{c}{wikipedia_filtered} & \multicolumn{2}{c}{github_filtered} & \multicolumn{2}{c}{mimic2_filtered} & \multicolumn{2}{c}{hawkes_exponential_mutual} \\
                       &               R &          Val &             R &         Val &                  R &         Val &               R &         Val &               R &         Val &                         R &         Val \\
\midrule
             GRU-CP-TO &              93 & -1114.927416 &            99 & -109.662049 &                 54 & -158.654091 &              72 & -294.601884 &               8 &    0.900263 &                        28 &  -78.051052 \\
            GRU-CP-LTO &             112 & -1067.340163 &           125 &  -86.944348 &                 56 & -155.288788 &              70 & -294.878666 &              60 &    1.722404 &                        33 &  -78.031711 \\
         GRU-CP-CONCAT &             101 & -1097.298704 &            97 & -113.641853 &                 64 & -145.319318 &              73 & -293.806189 &              18 &    1.184996 &                        34 &  -78.017722 \\
        GRU-CP-LCONCAT &             107 & -1085.792296 &           108 & -101.328590 &                 65 & -145.243119 &              68 & -295.257662 &              70 &    1.914378 &                        37 &  -77.996941 \\
            GRU-CP-TEM &             115 & -1060.320485 &           109 & -101.287690 &                 83 & -130.598666 &              94 & -273.115839 &              28 &    1.350319 &                        35 &  -78.000888 \\
          GRU-CP-TEMWL &             114 & -1060.320485 &           110 & -101.287690 &                 82 & -130.598666 &              93 & -273.115839 &              29 &    1.350319 &                        36 &  -78.000888 \\
             GRU-CP-LE &             105 & -1090.060246 &           103 & -105.476865 &                 60 & -149.005591 &              84 & -277.090697 &              12 &    1.043077 &                        29 &  -78.044421 \\
           GRU-CP-LEWL &             111 & -1077.674725 &           102 & -105.723955 &                 66 & -144.225984 &             111 & -263.601510 &              17 &    1.175433 &                        32 &  -78.033979 \\
              SA-CP-TO &             167 &  -788.543925 &           128 &  -76.641160 &                107 & -102.185018 &             159 & -167.705597 &              62 &    1.733512 &                       158 &  -72.524217 \\
             SA-CP-LTO &             168 &  -787.126618 &           129 &  -76.635914 &                109 &  -99.425426 &             158 & -168.622201 &              61 &    1.732948 &                       157 &  -72.527680 \\
          SA-CP-CONCAT &             121 & -1042.282862 &           119 &  -93.517013 &                 70 & -139.471897 &              97 & -272.381202 &              76 &    1.984611 &                        90 &  -76.582159 \\
         SA-CP-LCONCAT &             124 & -1036.760908 &           118 &  -93.654371 &                 68 & -144.050328 &              92 & -273.368924 &              75 &    1.974352 &                        89 &  -76.624317 \\
             SA-CP-TEM &             144 &  -948.603389 &           115 &  -96.244678 &                 77 & -134.733416 &             129 & -254.179001 &              90 &    2.134666 &                        85 &  -76.674977 \\
           SA-CP-TEMWL &             143 &  -948.603389 &           114 &  -96.244678 &                 78 & -134.733416 &             130 & -254.179001 &              91 &    2.134666 &                        86 &  -76.674977 \\
              SA-CP-LE &             120 & -1043.486442 &           126 &  -86.559238 &                 69 & -141.481969 &             105 & -268.253860 &              66 &    1.864267 &                        97 &  -76.070877 \\
            SA-CP-LEWL &             129 & -1026.192303 &           120 &  -92.438419 &                 81 & -131.506507 &             127 & -256.485480 &              79 &    1.997498 &                        96 &  -76.090251 \\
               C-CP-TO &             175 &  -782.775225 &           145 &  -51.746319 &                114 &  -75.884176 &             171 & -148.076161 &             104 &    2.992702 &                       165 &  -71.603209 \\
               C-CP-TO &             174 &  -782.775225 &           144 &  -51.746319 &                115 &  -75.884176 &             172 & -148.076161 &             103 &    2.992702 &                       164 &  -71.603209 \\
         GRU-CP-TO + B &             234 &          NaN &           234 &         NaN &                234 &         NaN &             234 &         NaN &             234 &         NaN &                       234 &         NaN \\
        GRU-CP-LTO + B &             233 &          NaN &           233 &         NaN &                233 &         NaN &             233 &         NaN &             233 &         NaN &                       233 &         NaN \\
     GRU-CP-CONCAT + B &             232 &          NaN &           232 &         NaN &                232 &         NaN &             232 &         NaN &             232 &         NaN &                       232 &         NaN \\
    GRU-CP-LCONCAT + B &             231 &          NaN &           231 &         NaN &                231 &         NaN &             231 &         NaN &             231 &         NaN &                       231 &         NaN \\
        GRU-CP-TEM + B &             133 & -1022.669053 &           116 &  -94.317542 &                 94 & -119.278889 &             103 & -270.287097 &              46 &    1.631002 &                        31 &  -78.044360 \\
      GRU-CP-TEMWL + B &             132 & -1022.669053 &           117 &  -94.317542 &                 93 & -119.278889 &             102 & -270.287097 &              47 &    1.631002 &                        30 &  -78.044360 \\
         GRU-CP-LE + B &             230 &          NaN &           230 &         NaN &                230 &         NaN &             230 &         NaN &             230 &         NaN &                       230 &         NaN \\
       GRU-CP-LEWL + B &             229 &          NaN &           229 &         NaN &                229 &         NaN &             229 &         NaN &             229 &         NaN &                       229 &         NaN \\
          SA-CP-TO + B &             228 &          NaN &           228 &         NaN &                228 &         NaN &             228 &         NaN &             228 &         NaN &                       228 &         NaN \\
         SA-CP-LTO + B &             227 &          NaN &           227 &         NaN &                227 &         NaN &             227 &         NaN &             227 &         NaN &                       227 &         NaN \\
      SA-CP-CONCAT + B &             226 &          NaN &           226 &         NaN &                226 &         NaN &             226 &         NaN &             226 &         NaN &                       226 &         NaN \\
     SA-CP-LCONCAT + B &             225 &          NaN &           225 &         NaN &                225 &         NaN &             225 &         NaN &             225 &         NaN &                       225 &         NaN \\
         SA-CP-TEM + B &             142 &  -962.071219 &           121 &  -92.382329 &                102 & -111.685072 &             112 & -263.153322 &              78 &    1.988042 &                        92 &  -76.566816 \\
       SA-CP-TEMWL + B &             141 &  -962.071219 &           122 &  -92.382329 &                101 & -111.685072 &             113 & -263.153322 &              77 &    1.988042 &                        91 &  -76.566816 \\
          SA-CP-LE + B &             224 &          NaN &           224 &         NaN &                224 &         NaN &             224 &         NaN &             224 &         NaN &                       224 &         NaN \\
        SA-CP-LEWL + B &             223 &          NaN &           223 &         NaN &                223 &         NaN &             223 &         NaN &             223 &         NaN &                       223 &         NaN \\
           C-CP-TO + B &             170 &  -782.876487 &           147 &  -51.743351 &                118 &  -73.125930 &             169 & -148.536579 &             105 &    2.998080 &                       163 &  -71.606678 \\
           C-CP-TO + B &             171 &  -782.876487 &           148 &  -51.743351 &                119 &  -73.125930 &             170 & -148.536579 &             106 &    2.998080 &                       162 &  -71.606678 \\
            GRU-LNM-TO &               8 & -1369.579080 &            18 & -296.549876 &                 19 & -273.636576 &               8 & -380.377581 &               1 &   -0.634690 &                         9 &  -78.566933 \\
           GRU-LNM-LTO &               7 & -1382.813971 &            16 & -299.777613 &                  5 & -290.020356 &               9 & -379.353677 &              35 &    1.494437 &                        21 &  -78.453960 \\
        GRU-LNM-CONCAT &              10 & -1367.236437 &             9 & -304.557098 &                 13 & -284.996340 &               7 & -383.357037 &               2 &   -0.075882 &                        10 &  -78.566455 \\
       GRU-LNM-LCONCAT &               9 & -1369.004724 &            13 & -303.712306 &                  3 & -290.667020 &              12 & -377.198747 &              10 &    0.929319 &                         8 &  -78.593116 \\
           GRU-LNM-TEM &              22 & -1327.631315 &             4 & -307.545878 &                 23 & -265.493409 &              15 & -374.489032 &              30 &    1.362320 &                        16 &  -78.536594 \\
         GRU-LNM-TEMWL &              21 & -1327.631315 &             3 & -307.545878 &                 24 & -265.493409 &              14 & -374.489032 &              31 &    1.362320 &                        15 &  -78.536594 \\
            GRU-LNM-LE &              12 & -1355.954168 &            19 & -295.281497 &                 22 & -268.143117 &              16 & -374.063074 &               3 &    0.069749 &                        12 &  -78.555078 \\
          GRU-LNM-LEWL &              16 & -1345.230854 &            12 & -303.767042 &                 20 & -272.296299 &              13 & -375.643165 &               4 &    0.422391 &                        11 &  -78.555790 \\
             SA-LNM-TO &              23 & -1327.124673 &            21 & -284.130456 &                 14 & -280.537787 &              22 & -362.477876 &               5 &    0.799618 &                       122 &  -74.616318 \\
            SA-LNM-LTO &              27 & -1318.372398 &            22 & -283.869934 &                 21 & -268.656365 &              23 & -360.871942 &              14 &    1.137080 &                       121 &  -74.632452 \\
         SA-LNM-CONCAT &              14 & -1352.238612 &            15 & -302.561331 &                  4 & -290.213141 &              17 & -372.481877 &              23 &    1.296199 &                        58 &  -77.513494 \\
        SA-LNM-LCONCAT &              13 & -1355.697674 &            14 & -303.527028 &                  9 & -285.441578 &              10 & -379.183951 &              36 &    1.509052 &                        67 &  -77.459959 \\
            SA-LNM-TEM &              24 & -1325.242305 &             8 & -305.612299 &                  7 & -288.893279 &              19 & -371.985258 &              22 &    1.270280 &                        60 &  -77.485827 \\
          SA-LNM-TEMWL &              25 & -1325.242305 &             7 & -305.612299 &                  6 & -288.893279 &              18 & -371.985258 &              21 &    1.270280 &                        61 &  -77.485827 \\
             SA-LNM-LE &              15 & -1350.110785 &            20 & -292.956004 &                 10 & -285.251309 &              21 & -370.213728 &              13 &    1.096419 &                        80 &  -77.063471 \\
           SA-LNM-LEWL &              17 & -1343.267552 &            17 & -298.687769 &                  8 & -286.901513 &              20 & -371.779557 &              38 &    1.543966 &                        75 &  -77.138985 \\
              C-LNM-TO &              18 & -1329.534035 &            23 & -279.272211 &                 18 & -275.732187 &              25 & -358.754496 &              93 &    2.392370 &                       137 &  -73.988845 \\
              C-LNM-TO &              19 & -1329.534035 &            24 & -279.272211 &                 17 & -275.732187 &              26 & -358.754496 &              94 &    2.392370 &                       138 &  -73.988845 \\
        GRU-LNM-TO + B &             222 &          NaN &           222 &         NaN &                222 &         NaN &             222 &         NaN &             222 &         NaN &                       222 &         NaN \\
        GRU-LNM-TO + B &             221 &          NaN &           221 &         NaN &                221 &         NaN &             221 &         NaN &             221 &         NaN &                       221 &         NaN \\
    GRU-LNM-CONCAT + B &             235 &          NaN &           235 &         NaN &                235 &         NaN &             235 &         NaN &             235 &         NaN &                       235 &         NaN \\
   GRU-LNM-LCONCAT + B &             220 &          NaN &           220 &         NaN &                220 &         NaN &             220 &         NaN &             220 &         NaN &                       220 &         NaN \\
       GRU-LNM-TEM + B &               1 & -1740.429967 &             5 & -305.885598 &                 11 & -285.223350 &               6 & -509.589412 &              20 &    1.232513 &                         4 & -101.070487 \\
     GRU-LNM-TEMWL + B &               2 & -1740.429967 &             6 & -305.885598 &                 12 & -285.223350 &               5 & -509.589412 &              19 &    1.232513 &                         3 & -101.070487 \\
        GRU-LNM-LE + B &             218 &          NaN &           218 &         NaN &                218 &         NaN &             218 &         NaN &             218 &         NaN &                       218 &         NaN \\
      GRU-LNM-LEWL + B &             217 &          NaN &           217 &         NaN &                217 &         NaN &             217 &         NaN &             217 &         NaN &                       217 &         NaN \\
         SA-LNM-TO + B &             216 &          NaN &           216 &         NaN &                216 &         NaN &             216 &         NaN &             216 &         NaN &                       216 &         NaN \\
        SA-LNM-LTO + B &             215 &          NaN &           215 &         NaN &                215 &         NaN &             215 &         NaN &             215 &         NaN &                       215 &         NaN \\
     SA-LNM-CONCAT + B &             214 &          NaN &           214 &         NaN &                214 &         NaN &             214 &         NaN &             214 &         NaN &                       214 &         NaN \\
    SA-LNM-LCONCAT + B &             213 &          NaN &           213 &         NaN &                213 &         NaN &             213 &         NaN &             213 &         NaN &                       213 &         NaN \\
        SA-LNM-TEM + B &               6 & -1527.562519 &            11 & -303.990567 &                 16 & -277.083662 &               4 & -603.173822 &              16 &    1.165442 &                         5 &  -99.626613 \\
      SA-LNM-TEMWL + B &               5 & -1527.562519 &            10 & -303.990567 &                 15 & -277.083662 &               3 & -603.173822 &              15 &    1.165442 &                         6 &  -99.626613 \\
         SA-LNM-LE + B &             212 &          NaN &           212 &         NaN &                212 &         NaN &             212 &         NaN &             212 &         NaN &                       212 &         NaN \\
       SA-LNM-LEWL + B &             211 &          NaN &           211 &         NaN &                211 &         NaN &             211 &         NaN &             211 &         NaN &                       211 &         NaN \\
          C-LNM-TO + B &               3 & -1601.226459 &             2 & -376.168667 &                  2 & -296.194367 &               2 & -625.777589 &              80 &    2.015728 &                         1 & -121.840197 \\
          C-LNM-TO + B &               4 & -1601.226459 &             1 & -376.168667 &                  1 & -296.194367 &               1 & -625.777589 &              81 &    2.015728 &                         2 & -121.840197 \\
         GRU-MLP/CM-TO &              80 & -1145.956620 &            91 & -142.841424 &                 88 & -121.904310 &              91 & -274.631966 &              32 &    1.408367 &                       101 &  -75.883007 \\
        GRU-MLP/CM-LTO &              11 & -1361.097529 &            26 & -268.451235 &                 28 & -232.295476 &              11 & -378.149476 &             113 &    3.304127 &                        93 &  -76.548984 \\
     GRU-MLP/CM-CONCAT &              98 & -1102.673004 &            65 & -211.612829 &                100 & -113.550178 &             108 & -266.271724 &              92 &    2.181381 &                        94 &  -76.166716 \\
    GRU-MLP/CM-LCONCAT &             108 & -1084.397130 &            64 & -213.427546 &                 91 & -120.084467 &             106 & -268.025966 &              86 &    2.105602 &                       114 &  -75.396276 \\
         GRU-MLP/CM-LE &             113 & -1062.031991 &            85 & -155.927991 &                 95 & -118.734085 &             104 & -269.510654 &              63 &    1.740694 &                       104 &  -75.717223 \\
       GRU-MLP/CM-LEWL &             102 & -1096.254680 &            54 & -228.564385 &                 92 & -119.862397 &             109 & -265.603626 &              54 &    1.677261 &                        95 &  -76.123713 \\
          SA-MLP/CM-TO &             163 &  -795.524699 &           132 &  -75.012795 &                113 &  -87.442528 &             160 & -167.599290 &              87 &    2.123611 &                       175 &  -70.545987 \\
         SA-MLP/CM-LTO &              56 & -1204.010938 &            25 & -270.903826 &                 30 & -225.012602 &              31 & -334.426483 &              95 &    2.739430 &                       156 &  -72.562471 \\
      SA-MLP/CM-CONCAT &             158 &  -816.113699 &           136 &  -70.457056 &                108 &  -99.441026 &             155 & -175.207461 &              83 &    2.095027 &                       147 &  -73.644896 \\
     SA-MLP/CM-LCONCAT &             159 &  -815.495294 &           133 &  -73.547183 &                111 &  -94.444606 &             154 & -175.481448 &              84 &    2.099929 &                       151 &  -72.807674 \\
          SA-MLP/CM-LE &             161 &  -812.780610 &           101 & -109.071746 &                112 &  -92.598445 &             156 & -173.196753 &              85 &    2.100798 &                       153 &  -72.750527 \\
        SA-MLP/CM-LEWL &             157 &  -818.118486 &            95 & -115.445913 &                110 &  -99.066229 &             157 & -172.938048 &              82 &    2.065708 &                       155 &  -72.747229 \\
           C-MLP/CM-TO &             164 &  -794.153984 &            72 & -195.358917 &                125 &  -60.467138 &             166 & -150.220841 &             119 &    3.451486 &                       172 &  -70.773452 \\
          C-MLP/CM-LTO &              28 & -1300.138019 &            30 & -265.848739 &                 27 & -234.402539 &              28 & -352.766445 &             124 &    3.709337 &                       160 &  -71.874418 \\
       C-MLP/CM-CONCAT &             165 &  -793.721390 &            98 & -113.384889 &                123 &  -61.571278 &             161 & -161.120772 &             123 &    3.525102 &                       173 &  -70.618712 \\
      C-MLP/CM-LCONCAT &             166 &  -789.577912 &            75 & -189.596387 &                124 &  -61.556001 &             162 & -160.092412 &             122 &    3.487203 &                       174 &  -70.548532 \\
           C-MLP/CM-LE &             160 &  -813.106295 &            78 & -162.673303 &                133 &  -52.594233 &             165 & -152.800000 &             118 &    3.400326 &                       171 &  -70.915217 \\
         C-MLP/CM-LEWL &             169 &  -787.022563 &            76 & -179.199316 &                130 &  -57.064994 &             163 & -158.134640 &             117 &    3.394913 &                       161 &  -71.733835 \\
     GRU-MLP/CM-TO + B &             210 &          NaN &           210 &         NaN &                210 &         NaN &             210 &         NaN &             210 &         NaN &                       210 &         NaN \\
    GRU-MLP/CM-LTO + B &             209 &          NaN &           209 &         NaN &                209 &         NaN &             209 &         NaN &             209 &         NaN &                       209 &         NaN \\
 GRU-MLP/CM-CONCAT + B &             208 &          NaN &           208 &         NaN &                208 &         NaN &             208 &         NaN &             208 &         NaN &                       208 &         NaN \\
GRU-MLP/CM-LCONCAT + B &             207 &          NaN &           207 &         NaN &                207 &         NaN &             207 &         NaN &             207 &         NaN &                       207 &         NaN \\
     GRU-MLP/CM-LE + B &             146 &  -912.221494 &           124 &  -91.992734 &                 87 & -122.689186 &             117 & -261.249235 &              39 &    1.549479 &                       116 &  -75.261813 \\
   GRU-MLP/CM-LEWL + B &             147 &  -912.221494 &           123 &  -91.992734 &                 86 & -122.689186 &             116 & -261.249235 &              40 &    1.549479 &                       115 &  -75.261813 \\
      SA-MLP/CM-TO + B &             206 &          NaN &           206 &         NaN &                206 &         NaN &             206 &         NaN &             206 &         NaN &                       206 &         NaN \\
     SA-MLP/CM-LTO + B &             205 &          NaN &           205 &         NaN &                205 &         NaN &             205 &         NaN &             205 &         NaN &                       205 &         NaN \\
  SA-MLP/CM-CONCAT + B &             219 &          NaN &           219 &         NaN &                219 &         NaN &             219 &         NaN &             219 &         NaN &                       219 &         NaN \\
 SA-MLP/CM-LCONCAT + B &             236 &          NaN &           236 &         NaN &                236 &         NaN &             236 &         NaN &             236 &         NaN &                       236 &         NaN \\
      SA-MLP/CM-LE + B &             156 &  -826.119095 &            93 & -142.269234 &                 97 & -116.173636 &             152 & -175.500602 &              68 &    1.889283 &                       119 &  -74.754677 \\
    SA-MLP/CM-LEWL + B &             155 &  -826.119095 &            92 & -142.269234 &                 96 & -116.173636 &             153 & -175.500602 &              67 &    1.889283 &                       120 &  -74.754677 \\
       C-MLP/CM-TO + B &             237 &          NaN &           237 &         NaN &                237 &         NaN &             237 &         NaN &             237 &         NaN &                       237 &         NaN \\
      C-MLP/CM-LTO + B &             238 &          NaN &           238 &         NaN &                238 &         NaN &             238 &         NaN &             238 &         NaN &                       238 &         NaN \\
   C-MLP/CM-CONCAT + B &             256 &          NaN &           256 &         NaN &                256 &         NaN &             256 &         NaN &             256 &         NaN &                       256 &         NaN \\
  C-MLP/CM-LCONCAT + B &             257 &          NaN &           257 &         NaN &                257 &         NaN &             257 &         NaN &             257 &         NaN &                       257 &         NaN \\
       C-MLP/CM-LE + B &             172 &  -782.866823 &           150 &  -51.662351 &                117 &  -73.362574 &             174 & -143.895369 &             109 &    3.019282 &                       170 &  -71.595293 \\
     C-MLP/CM-LEWL + B &             173 &  -782.866823 &           149 &  -51.662351 &                116 &  -73.362574 &             173 & -143.895369 &             110 &    3.019282 &                       169 &  -71.595293 \\

\bottomrule
\end{tabular}
\end{table}


\newgeometry{left=2cm,bottom=2cm,right=2cm, top=1cm}
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
                models & \multicolumn{12}{c}{NLL Time} \\
                       & \multicolumn{2}{c}{lastfm_filtered} & \multicolumn{2}{c}{mooc_filtered} & \multicolumn{2}{c}{wikipedia_filtered} & \multicolumn{2}{c}{github_filtered} & \multicolumn{2}{c}{mimic2_filtered} & \multicolumn{2}{c}{hawkes_exponential_mutual} \\
                       &               R &          Val &             R &         Val &                  R &         Val &               R &         Val &               R &         Val &                         R &         Val \\
\midrule
         GRU-MLP/MC-TO &              85 & -1138.032752 &           139 &  -66.146060 &                149 &  -17.112733 &              77 & -283.467390 &             133 &   67.407375 &                        38 &  -77.976058 \\
        GRU-MLP/MC-LTO &              26 & -1322.899356 &            94 & -120.916372 &                137 &  -48.017644 &              27 & -355.626869 &             141 &   67.424927 &                        40 &  -77.932424 \\
     GRU-MLP/MC-CONCAT &              97 & -1108.351740 &           131 &  -75.706638 &                155 &  -16.101878 &              82 & -279.838946 &             135 &   67.411968 &                        41 &  -77.920458 \\
    GRU-MLP/MC-LCONCAT &              88 & -1127.773748 &           127 &  -83.039572 &                144 &  -18.539438 &              78 & -281.118874 &             129 &   67.403997 &                        42 &  -77.909627 \\
        GRU-MLP/MC-TEM &             118 & -1052.692163 &           157 &  -19.261144 &                159 &   -6.471514 &             122 & -257.249414 &             131 &   67.405231 &                        51 &  -77.761964 \\
      GRU-MLP/MC-TEMWL &             119 & -1052.692163 &           158 &  -19.261144 &                158 &   -6.471514 &             123 & -257.249414 &             130 &   67.405231 &                        52 &  -77.761964 \\
         GRU-MLP/MC-LE &              66 & -1182.668576 &           135 &  -72.134786 &                150 &  -17.067947 &             107 & -266.498019 &             140 &   67.423803 &                        39 &  -77.943564 \\
       GRU-MLP/MC-LEWL &              70 & -1164.435007 &           141 &  -65.584840 &                151 &  -17.034811 &             110 & -265.105106 &             134 &   67.410634 &                        43 &  -77.891940 \\
          SA-MLP/MC-TO &              67 & -1178.136820 &           143 &  -52.086637 &                148 &  -17.119442 &             138 & -221.565054 &             138 &   67.420884 &                       128 &  -74.367551 \\
         SA-MLP/MC-LTO &              37 & -1264.545915 &            96 & -115.433649 &                131 &  -56.348548 &              44 & -320.432154 &             139 &   67.423104 &                       127 &  -74.413904 \\
      SA-MLP/MC-CONCAT &              96 & -1112.501178 &           134 &  -73.219391 &                153 &  -16.737328 &             126 & -256.686480 &             132 &   67.405846 &                        81 &  -77.002012 \\
     SA-MLP/MC-LCONCAT &              94 & -1114.298374 &           107 & -103.124892 &                146 &  -18.524861 &             132 & -251.212746 &             126 &   67.398963 &                        82 &  -76.943350 \\
         SA-MLP/MC-TEM &             137 & -1002.134208 &           156 &  -21.863156 &                157 &  -11.481387 &             135 & -245.263288 &             128 &   67.399694 &                        87 &  -76.655462 \\
       SA-MLP/MC-TEMWL &             136 & -1002.134208 &           155 &  -21.863156 &                156 &  -11.481387 &             134 & -245.263288 &             127 &   67.399694 &                        88 &  -76.655462 \\
          SA-MLP/MC-LE &              71 & -1161.418759 &           142 &  -64.261195 &                147 &  -17.830659 &             128 & -256.357675 &             144 &   67.429261 &                        84 &  -76.773706 \\
        SA-MLP/MC-LEWL &              89 & -1125.345191 &           140 &  -66.139893 &                143 &  -18.576818 &             133 & -250.872905 &             145 &   67.438483 &                        83 &  -76.777977 \\
           C-MLP/MC-TO &             100 & -1101.079891 &           176 &  131.907270 &                172 &  122.938781 &             147 & -196.072038 &             165 &  117.275609 &                       146 &  -73.677902 \\
          C-MLP/MC-TEM &             149 &  -903.481593 &           175 &  128.872160 &                176 &  123.872780 &             150 & -188.510369 &             168 &  117.280054 &                       145 &  -73.824662 \\
        C-MLP/MC-TEMWL &             148 &  -903.481593 &           174 &  128.872160 &                175 &  123.872780 &             149 & -188.510369 &             167 &  117.280054 &                       144 &  -73.824662 \\
          C-MLP/MC-LTO &              73 & -1157.018548 &           163 &   18.506847 &                161 &   87.128193 &              32 & -328.173201 &             172 &  117.337096 &                       148 &  -73.569628 \\
       C-MLP/MC-CONCAT &             127 & -1031.976406 &           171 &   95.139225 &                170 &  118.209266 &             145 & -204.125686 &             162 &  117.246057 &                       129 &  -74.121562 \\
           C-MLP/MC-LE &              72 & -1160.779155 &           173 &  114.665702 &                166 &  117.136994 &             136 & -238.137240 &             169 &  117.301994 &                       140 &  -73.899480 \\
         C-MLP/MC-LEWL &              95 & -1112.644163 &           172 &   97.366392 &                164 &  111.309461 &             137 & -236.524249 &             166 &  117.278106 &                       135 &  -74.048690 \\
      C-MLP/MC-LCONCAT &             128 & -1026.743124 &           167 &   49.291214 &                171 &  122.513482 &             146 & -201.495324 &             164 &  117.253707 &                       130 &  -74.107125 \\
     GRU-MLP/MC-TO + B &             258 &          NaN &           258 &         NaN &                258 &         NaN &             258 &         NaN &             258 &         NaN &                       258 &         NaN \\
    GRU-MLP/MC-LTO + B &             259 &          NaN &           259 &         NaN &                259 &         NaN &             259 &         NaN &             259 &         NaN &                       259 &         NaN \\
 GRU-MLP/MC-CONCAT + B &             260 &          NaN &           260 &         NaN &                260 &         NaN &             260 &         NaN &             260 &         NaN &                       260 &         NaN \\
GRU-MLP/MC-LCONCAT + B &             203 &          NaN &           203 &         NaN &                203 &         NaN &             203 &         NaN &             203 &         NaN &                       203 &         NaN \\
    GRU-MLP/MC-TEM + B &             104 & -1093.155451 &            61 & -217.470070 &                 89 & -121.894120 &              99 & -271.345092 &              51 &    1.651017 &                        13 &  -78.543757 \\
         GRU-TEMWL + B &             103 & -1093.155451 &            62 & -217.470070 &                 90 & -121.894120 &             100 & -271.345092 &              50 &    1.651017 &                        14 &  -78.543757 \\
     GRU-MLP/MC-LE + B &             261 &          NaN &           261 &         NaN &                261 &         NaN &             261 &         NaN &             261 &         NaN &                       261 &         NaN \\
   GRU-MLP/MC-LEWL + B &             263 &          NaN &           263 &         NaN &                263 &         NaN &             263 &         NaN &             263 &         NaN &                       263 &         NaN \\
      SA-MLP/MC-TO + B &             270 &          NaN &           270 &         NaN &                270 &         NaN &             270 &         NaN &             270 &         NaN &                       270 &         NaN \\
     SA-MLP/MC-LTO + B &             264 &          NaN &           264 &         NaN &                264 &         NaN &             264 &         NaN &             264 &         NaN &                       264 &         NaN \\
  SA-MLP/MC-CONCAT + B &             265 &          NaN &           265 &         NaN &                265 &         NaN &             265 &         NaN &             265 &         NaN &                       265 &         NaN \\
 SA-MLP/MC-LCONCAT + B &             266 &          NaN &           266 &         NaN &                266 &         NaN &             266 &         NaN &             266 &         NaN &                       266 &         NaN \\
     SA-MLP/MC-TEM + B &             134 & -1006.770418 &            59 & -218.448558 &                 85 & -123.244824 &             124 & -256.977153 &              88 &    2.129104 &                        72 &  -77.351543 \\
   SA-MLP/MC-TEMWL + B &             135 & -1006.770418 &            60 & -218.448558 &                 84 & -123.244824 &             125 & -256.977153 &              89 &    2.129104 &                        71 &  -77.351543 \\
      SA-MLP/MC-LE + B &             267 &          NaN &           267 &         NaN &                267 &         NaN &             267 &         NaN &             267 &         NaN &                       267 &         NaN \\
    SA-MLP/MC-LEWL + B &             268 &          NaN &           268 &         NaN &                268 &         NaN &             268 &         NaN &             268 &         NaN &                       268 &         NaN \\
      C-MLP/MC-TEM + B &             140 &  -973.553856 &            66 & -208.184087 &                105 & -107.555406 &             167 & -149.078100 &             107 &    3.007813 &                       166 &  -71.597965 \\
    C-MLP/MC-TEMWL + B &             139 &  -973.553856 &            67 & -208.184087 &                104 & -107.555406 &             168 & -149.078100 &             108 &    3.007813 &                       167 &  -71.597965 \\
          GRU-RMTPP-TO &              69 & -1166.999326 &            81 & -156.866642 &                 40 & -181.709257 &              62 & -299.822949 &               6 &    0.817669 &                        17 &  -78.510569 \\
         GRU-RMTPP-LTO &             269 &          NaN &           269 &         NaN &                269 &         NaN &             269 &         NaN &             269 &         NaN &                       269 &         NaN \\
      GRU-RMTPP-CONCAT &              82 & -1140.401375 &            77 & -162.882818 &                 41 & -172.085359 &              69 & -295.221367 &               7 &    0.890442 &                        22 &  -78.451096 \\
     GRU-RMTPP-LCONCAT &             255 &          NaN &           255 &         NaN &                255 &         NaN &             255 &         NaN &             255 &         NaN &                       255 &         NaN \\
         GRU-RMTPP-TEM &             116 & -1059.707845 &            83 & -156.216215 &                 71 & -138.897717 &              81 & -279.862941 &              25 &    1.331407 &                        23 &  -78.430848 \\
       GRU-RMTPP-TEMWL &             117 & -1059.707845 &            84 & -156.216215 &                 72 & -138.897717 &              80 & -279.862941 &              24 &    1.331407 &                        24 &  -78.430848 \\
          GRU-RMTPP-LE &              74 & -1154.810580 &            82 & -156.728829 &                 52 & -162.847683 &              98 & -272.219208 &               9 &    0.911524 &                        25 &  -78.402461 \\
        GRU-RMTPP-LEWL &              76 & -1152.218289 &            80 & -157.173233 &                 55 & -155.476059 &             131 & -251.346289 &              11 &    0.972064 &                        18 &  -78.494298 \\
           SA-RMTPP-TO &             138 &  -998.903489 &            90 & -146.001055 &                 75 & -135.739724 &             139 & -216.019029 &              48 &    1.647281 &                       126 &  -74.442998 \\
          SA-RMTPP-LTO &             254 &          NaN &           254 &         NaN &                254 &         NaN &             254 &         NaN &             254 &         NaN &                       254 &         NaN \\
       SA-RMTPP-CONCAT &              92 & -1116.698630 &            79 & -157.292618 &                 47 & -167.532285 &             115 & -262.485110 &              52 &    1.656700 &                        73 &  -77.331969 \\
      SA-RMTPP-LCONCAT &             253 &          NaN &           253 &         NaN &                253 &         NaN &             253 &         NaN &             253 &         NaN &                       253 &         NaN \\
          SA-RMTPP-TEM &             130 & -1023.105924 &            86 & -155.640541 &                 46 & -168.005607 &             120 & -258.370162 &              55 &    1.678630 &                        62 &  -77.483234 \\
        SA-RMTPP-TEMWL &             131 & -1023.105924 &            87 & -155.640541 &                 45 & -168.005607 &             121 & -258.370162 &              56 &    1.678630 &                        63 &  -77.483234 \\
           SA-RMTPP-LE &              99 & -1101.683955 &            89 & -151.474396 &                 48 & -166.540240 &             101 & -270.501780 &              49 &    1.649623 &                        79 &  -77.074266 \\
         SA-RMTPP-LEWL &             106 & -1085.821362 &            88 & -155.305169 &                 53 & -162.519638 &             114 & -263.019258 &              53 &    1.656804 &                        78 &  -77.097685 \\
           C-RMTPP-LTO &             252 &          NaN &           252 &         NaN &                252 &         NaN &             252 &         NaN &             252 &         NaN &                       252 &         NaN \\
           C-RMTPP-LTO &             251 &          NaN &           251 &         NaN &                251 &         NaN &             251 &         NaN &             251 &         NaN &                       251 &         NaN \\
            C-RMTPP-TO &             178 &  -216.900584 &           154 &  -36.905774 &                135 &  -50.111279 &             176 &  -82.192398 &             115 &    3.343729 &                       177 &  -48.486196 \\
            C-RMTPP-TO &             177 &  -216.900584 &           153 &  -36.905774 &                134 &  -50.111279 &             177 &  -82.192398 &             114 &    3.343729 &                       176 &  -48.486196 \\
      GRU-RMTPP-TO + B &             250 &          NaN &           250 &         NaN &                250 &         NaN &             250 &         NaN &             250 &         NaN &                       250 &         NaN \\
     GRU-RMTPP-LTO + B &             249 &          NaN &           249 &         NaN &                249 &         NaN &             249 &         NaN &             249 &         NaN &                       249 &         NaN \\
  GRU-RMTPP-CONCAT + B &             248 &          NaN &           248 &         NaN &                248 &         NaN &             248 &         NaN &             248 &         NaN &                       248 &         NaN \\
 GRU-RMTPP-LCONCAT + B &             247 &          NaN &           247 &         NaN &                247 &         NaN &             247 &         NaN &             247 &         NaN &                       247 &         NaN \\
    GRU-RMTPP-TEMP + B &              90 & -1118.021434 &            71 & -202.076615 &                 74 & -136.011553 &              87 & -276.446084 &              27 &    1.342752 &                        19 &  -78.483982 \\
   GRU-RMTPP-TEMWL + B &              91 & -1118.021434 &            70 & -202.076615 &                 73 & -136.011553 &              86 & -276.446084 &              26 &    1.342752 &                        20 &  -78.483982 \\
      GRU-RMTPP-LE + B &             246 &          NaN &           246 &         NaN &                246 &         NaN &             246 &         NaN &             246 &         NaN &                       246 &         NaN \\
    GRU-RMTPP-LEWL + B &             245 &          NaN &           245 &         NaN &                245 &         NaN &             245 &         NaN &             245 &         NaN &                       245 &         NaN \\
       SA-RMTPP-TO + B &             244 &          NaN &           244 &         NaN &                244 &         NaN &             244 &         NaN &             244 &         NaN &                       244 &         NaN \\
      SA-RMTPP-LTO + B &             243 &          NaN &           243 &         NaN &                243 &         NaN &             243 &         NaN &             243 &         NaN &                       243 &         NaN \\
   SA-RMTPP-CONCAT + B &             242 &          NaN &           242 &         NaN &                242 &         NaN &             242 &         NaN &             242 &         NaN &                       242 &         NaN \\
  SA-RMTPP-LCONCAT + B &             241 &          NaN &           241 &         NaN &                241 &         NaN &             241 &         NaN &             241 &         NaN &                       241 &         NaN \\
      SA-RMTPP-TEM + B &             123 & -1038.739954 &            68 & -204.888349 &                 61 & -148.528637 &             118 & -259.527147 &              64 &    1.827163 &                        57 &  -77.546780 \\
    SA-RMTPP-TEMWL + B &             122 & -1038.739954 &            69 & -204.888349 &                 62 & -148.528637 &             119 & -259.527147 &              65 &    1.827163 &                        56 &  -77.546780 \\
       SA-RMTPP-LE + B &             240 &          NaN &           240 &         NaN &                240 &         NaN &             240 &         NaN &             240 &         NaN &                       240 &         NaN \\
     SA-RMTPP-LEWL + B &             239 &          NaN &           239 &         NaN &                239 &         NaN &             239 &         NaN &             239 &         NaN &                       239 &         NaN \\
       C-RMTPP-LTO + B &             204 &          NaN &           204 &         NaN &                204 &         NaN &             204 &         NaN &             204 &         NaN &                       204 &         NaN \\
       C-RMTPP-LTO + B &             262 &          NaN &           262 &         NaN &                262 &         NaN &             262 &         NaN &             262 &         NaN &                       262 &         NaN \\
        C-RMTPP-TO + B &             126 & -1034.900198 &            74 & -189.839964 &                 99 & -115.886014 &             142 & -204.793902 &              97 &    2.795495 &                       142 &  -73.891693 \\
        C-RMTPP-TO + B &             125 & -1034.900198 &            73 & -189.839964 &                 98 & -115.886014 &             143 & -204.793902 &              96 &    2.795495 &                       141 &  -73.891693 \\

\end{tabular}
\label{resultsmark}
\caption{Evaluation of the different neural TPP models on MOOC and LastFM. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}

\newgeometry{left=2cm,bottom=2cm,right=2cm, top=1cm}
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
                models & \multicolumn{12}{c}{NLL Time} \\
                       & \multicolumn{2}{c}{lastfm_filtered} & \multicolumn{2}{c}{mooc_filtered} & \multicolumn{2}{c}{wikipedia_filtered} & \multicolumn{2}{c}{github_filtered} & \multicolumn{2}{c}{mimic2_filtered} & \multicolumn{2}{c}{hawkes_exponential_mutual} \\
                       &               R &          Val &             R &         Val &                  R &         Val &               R &         Val &               R &         Val &                         R &         Val \\
\midrule
          GRU-SA/CM-TO &              20 & -1327.945723 &            28 & -268.006959 &                 26 & -238.452003 &              24 & -358.991875 &             159 &  112.844031 &                       102 &  -75.862460 \\
         GRU-SA/CM-LTO &              34 & -1273.097007 &            27 & -268.067678 &                 31 & -223.004205 &             178 &  787.724825 &             177 & 3358.032593 &                       117 &  -74.841507 \\
      GRU-SA/CM-CONCAT &              79 & -1150.219143 &            45 & -246.336563 &                 44 & -169.795634 &              52 & -309.315896 &              59 &    1.714434 &                       100 &  -75.963360 \\
     GRU-SA/CM-LCONCAT &              52 & -1217.313535 &            46 & -245.811423 &                 67 & -144.080169 &              53 & -308.596498 &              73 &    1.963785 &                       103 &  -75.842985 \\
          GRU-SA/CM-LE &              38 & -1263.263005 &            49 & -240.439779 &                 63 & -146.119989 &              79 & -280.913224 &              45 &    1.603435 &                        98 &  -75.973635 \\
        GRU-SA/CM-LEWL &              51 & -1221.603819 &            56 & -225.859446 &                 51 & -164.619339 &              71 & -294.874990 &              37 &    1.533158 &                        99 &  -75.963742 \\
           SA-SA/CM-TO &              33 & -1274.001331 &            50 & -239.901207 &                 32 & -211.622662 &              54 & -308.283606 &             158 &  107.617252 &                       109 &  -75.531532 \\
          SA-SA/CM-LTO &              29 & -1292.334750 &            29 & -266.876811 &                 25 & -239.520549 &              29 & -340.965269 &             176 & 2405.115115 &                       118 &  -74.829306 \\
       SA-SA/CM-CONCAT &              81 & -1143.067761 &            47 & -245.020132 &                106 & -106.039865 &              49 & -310.691295 &              74 &    1.969942 &                       106 &  -75.675899 \\
      SA-SA/CM-LCONCAT &              59 & -1197.767091 &            48 & -243.435266 &                103 & -109.455544 &              48 & -311.523995 &              71 &    1.941187 &                       105 &  -75.693520 \\
           SA-SA/CM-LE &              50 & -1229.231937 &            44 & -248.464509 &                 80 & -133.461266 &              90 & -275.147934 &              72 &    1.943453 &                       111 &  -75.457521 \\
         SA-SA/CM-LEWL &              60 & -1195.784657 &            53 & -228.989378 &                 57 & -153.317611 &              75 & -292.430286 &              69 &    1.902890 &                       107 &  -75.649462 \\
            C-SA/CM-TO &              32 & -1275.867909 &            52 & -231.051137 &                 33 & -210.357045 &              57 & -304.688408 &             120 &    3.452894 &                       112 &  -75.417196 \\
           C-SA/CM-LTO &              30 & -1284.496069 &            31 & -261.544877 &                 29 & -227.837279 &              30 & -338.161594 &             178 & 4221.429236 &                       125 &  -74.582440 \\
        C-SA/CM-CONCAT &             145 &  -925.239647 &            63 & -217.113125 &                177 &  128.614637 &              96 & -272.410469 &             121 &    3.466299 &                       186 &         NaN \\
       C-SA/CM-LCONCAT &              75 & -1153.982206 &            57 & -225.381282 &                160 &   44.496287 &              95 & -272.902245 &             112 &    3.299987 &                       108 &  -75.537559 \\
            C-SA/CM-LE &              55 & -1210.457308 &            55 & -228.512458 &                 79 & -133.580560 &              83 & -278.747567 &             116 &    3.362581 &                       113 &  -75.414723 \\
          C-SA/CM-LEWL &              68 & -1178.030820 &            51 & -232.273932 &                 76 & -135.408554 &              85 & -276.537900 &             111 &    3.165381 &                       110 &  -75.483248 \\
      GRU-SA/CM-TO + B &             193 &          NaN &           194 &         NaN &                188 &         NaN &             200 &         NaN &             190 &         NaN &                       191 &         NaN \\
     GRU-SA/CM-LTO + B &             194 &          NaN &           195 &         NaN &                189 &         NaN &             199 &         NaN &             191 &         NaN &                       192 &         NaN \\
   GR-SA/CM-CONCAT + B &             195 &          NaN &           196 &         NaN &                190 &         NaN &             198 &         NaN &             192 &         NaN &                       193 &         NaN \\
 GRU-SA/CM-LCONCAT + B &             196 &          NaN &           197 &         NaN &                191 &         NaN &             183 &         NaN &             193 &         NaN &                       194 &         NaN \\
      GRU-SA/CM-LE + B &              42 & -1259.308241 &            40 & -251.388072 &                 42 & -170.293210 &              43 & -320.682665 &              33 &    1.410768 &                        45 &  -77.884016 \\
    GRU-SA/CM-LEWL + B &              41 & -1259.308241 &            41 & -251.388072 &                 43 & -170.293210 &              42 & -320.682665 &              34 &    1.410768 &                        44 &  -77.884016 \\
       SA-SA/CM-TO + B &             199 &          NaN &           201 &         NaN &                196 &         NaN &             196 &         NaN &             202 &         NaN &                       199 &         NaN \\
      SA-SA/CM-LTO + B &             200 &          NaN &           193 &         NaN &                197 &         NaN &             195 &         NaN &             198 &         NaN &                       200 &         NaN \\
   SA-SA/CM-CONCAT + B &             198 &          NaN &           192 &         NaN &                200 &         NaN &             194 &         NaN &             199 &         NaN &                       190 &         NaN \\
  SA-SA/CM-LCONCAT + B &             192 &          NaN &           190 &         NaN &                187 &         NaN &             201 &         NaN &             200 &         NaN &                       189 &         NaN \\
       SA-SA/CM-LE + B &              48 & -1244.434431 &            38 & -251.896412 &                 50 & -165.257397 &              51 & -309.449095 &              58 &    1.697569 &                        49 &  -77.770869 \\
     SA-SA/CM-LEWL + B &              47 & -1244.434431 &            39 & -251.896412 &                 49 & -165.257397 &              50 & -309.449095 &              57 &    1.697569 &                        48 &  -77.770869 \\
        C-SA/CM-TO + B &             187 &          NaN &           182 &         NaN &                198 &         NaN &             185 &         NaN &             187 &         NaN &                       181 &         NaN \\
       C-SA/CM-LTO + B &             201 &          NaN &           181 &         NaN &                195 &         NaN &             197 &         NaN &             179 &         NaN &                       180 &         NaN \\
    C-SA/CM-CONCAT + B &             202 &          NaN &           202 &         NaN &                193 &         NaN &             186 &         NaN &             184 &         NaN &                       179 &         NaN \\
   C-SA/CM-LCONCAT + B &             185 &          NaN &           180 &         NaN &                192 &         NaN &             187 &         NaN &             182 &         NaN &                       178 &         NaN \\
        C-SA/CM-LE + B &              58 & -1201.484926 &            42 & -251.181585 &                 58 & -152.745224 &              59 & -302.618196 &              98 &    2.924250 &                        68 &  -77.454555 \\
      C-SA/CM-LEWL + B &              57 & -1201.484926 &            43 & -251.181585 &                 59 & -152.745224 &              58 & -302.618196 &              99 &    2.924250 &                        69 &  -77.454555 \\
          GRU-SA/MC-TO &             150 &  -871.150856 &           160 &   -3.562893 &                145 &  -18.529812 &             144 & -204.715503 &             154 &   67.533091 &                       149 &  -73.542280 \\
         GRU-SA/MC-LTO &             162 &  -809.598208 &           162 &   -1.501259 &                152 &  -16.846622 &             151 & -180.290490 &             157 &   67.585730 &                       152 &  -72.775196 \\
      GRU-SA/MC-CONCAT &              40 & -1260.605377 &           104 & -105.377412 &                120 &  -71.124683 &              33 & -327.590461 &             146 &   67.438600 &                        50 &  -77.766186 \\
     GRU-SA/MC-LCONCAT &              35 & -1271.644263 &           105 & -104.943667 &                127 &  -58.822390 &              36 & -324.082324 &             148 &   67.467105 &                        53 &  -77.678627 \\
         GRU-SA/MC-TEM &             109 & -1083.455781 &           138 &  -68.605190 &                141 &  -33.095402 &              61 & -300.297649 &             142 &   67.428496 &                        66 &  -77.467841 \\
       GRU-SA/MC-TEMWL &             110 & -1083.455781 &           137 &  -68.605190 &                140 &  -33.095402 &              60 & -300.297649 &             143 &   67.428496 &                        65 &  -77.467841 \\
          GRU-SA/MC-LE &              36 & -1264.568344 &           100 & -109.090750 &                121 &  -68.841741 &              34 & -326.637615 &             153 &   67.514665 &                        54 &  -77.661990 \\
        GRU-SA/MC-LEWL &              46 & -1245.043640 &           112 &  -99.213015 &                132 &  -52.959053 &              41 & -321.113489 &             152 &   67.511149 &                        55 &  -77.586568 \\
           SA-SA/MC-TO &             153 &  -857.316538 &           159 &   -3.882858 &                142 &  -20.388551 &             141 & -208.006355 &             155 &   67.550657 &                       139 &  -73.934007 \\
          SA-SA/MC-LTO &             151 &  -865.590748 &           161 &   -2.150755 &                154 &  -16.610799 &             148 & -195.411525 &             156 &   67.559305 &                       154 &  -72.748847 \\
       SA-SA/MC-CONCAT &              45 & -1245.234007 &           111 &  -99.731594 &                128 &  -58.734352 &              37 & -323.262380 &             147 &   67.446878 &                        64 &  -77.470953 \\
      SA-SA/MC-LCONCAT &              49 & -1243.067875 &           106 & -103.624412 &                122 &  -64.099229 &              35 & -324.520799 &             149 &   67.478619 &                        59 &  -77.497003 \\
          SA-SA/MC-TEM &              86 & -1129.500160 &           151 &  -37.960123 &                139 &  -41.611997 &              64 & -297.793303 &             137 &   67.418114 &                        76 &  -77.134935 \\
        SA-SA/MC-TEMWL &              87 & -1129.500160 &           152 &  -37.960123 &                138 &  -41.611997 &              65 & -297.793303 &             136 &   67.418114 &                        77 &  -77.134935 \\
           SA-SA/MC-LE &              31 & -1278.721520 &           113 &  -97.267268 &                126 &  -60.064925 &              38 & -322.925181 &             151 &   67.490038 &                        70 &  -77.395014 \\
         SA-SA/MC-LEWL &              39 & -1261.258616 &           130 &  -76.510126 &                136 &  -48.353085 &              47 & -316.891507 &             150 &   67.485087 &                        74 &  -77.180381 \\
            C-SA/MC-TO &             152 &  -861.403015 &           177 &  132.076765 &                173 &  122.976422 &             140 & -215.681195 &             170 &  117.320808 &                       150 &  -72.949773 \\
           C-SA/MC-TEM &              83 & -1138.834180 &           170 &   86.108753 &                168 &  118.095880 &              88 & -275.681852 &             160 &  117.230417 &                       134 &  -74.066932 \\
         C-SA/MC-TEMWL &              84 & -1138.834180 &           169 &   86.108753 &                169 &  118.095880 &              89 & -275.681852 &             161 &  117.230417 &                       133 &  -74.066932 \\
           C-SA/MC-LTO &             154 &  -835.133542 &           178 &  132.254979 &                174 &  123.073023 &             164 & -157.089021 &             173 &  117.535839 &                       159 &  -72.193930 \\
        C-SA/MC-CONCAT &              54 & -1213.270712 &           164 &   30.539416 &                162 &   89.176196 &              76 & -289.315075 &             163 &  117.249690 &                       131 &  -74.082060 \\
            C-SA/MC-LE &              43 & -1254.266074 &           168 &   62.799658 &                167 &  117.888597 &              67 & -296.205448 &             174 &  117.570750 &                       143 &  -73.887313 \\
          C-SA/MC-LEWL &              44 & -1246.877020 &           166 &   38.384289 &                165 &  112.760244 &              66 & -297.631751 &             175 &  117.769948 &                       136 &  -74.046530 \\
       C-SA/MC-LCONCAT &              53 & -1216.765984 &           165 &   32.732151 &                163 &   94.606394 &              74 & -293.748607 &             171 &  117.328246 &                       132 &  -74.080805 \\
      GRU-SA/MC-TO + B &             182 &          NaN &           183 &         NaN &                182 &         NaN &             179 &         NaN &             185 &         NaN &                       202 &         NaN \\
     GRU-SA/MC-LTO + B &             181 &          NaN &           184 &         NaN &                183 &         NaN &             180 &         NaN &             180 &         NaN &                       183 &         NaN \\
  GRU-SA/MC-CONCAT + B &             180 &          NaN &           185 &         NaN &                184 &         NaN &             181 &         NaN &             201 &         NaN &                       184 &         NaN \\
 GRU-SA/MC-LCONCAT + B &             186 &          NaN &           186 &         NaN &                202 &         NaN &             192 &         NaN &             186 &         NaN &                       185 &         NaN \\
     GRU-SA/MC-TEM + B &              78 & -1151.631990 &            32 & -260.074951 &                 37 & -188.010243 &              45 & -319.831431 &              41 &    1.561870 &                        26 &  -78.173557 \\
   GRU-SA/MC-TEMWL + B &              77 & -1151.631990 &            33 & -260.074951 &                 36 & -188.010243 &              46 & -319.831431 &              42 &    1.561870 &                        27 &  -78.173557 \\
      GRU-SA/MC-LE + B &             179 &          NaN &           187 &         NaN &                201 &         NaN &             184 &         NaN &             183 &         NaN &                       201 &         NaN \\
    GRU-SA/MC-LEWL + B &             183 &          NaN &           188 &         NaN &                181 &         NaN &             193 &         NaN &             189 &         NaN &                       198 &         NaN \\
       SA-SA/MC-TO + B &             184 &          NaN &           189 &         NaN &                180 &         NaN &             191 &         NaN &             194 &         NaN &                       197 &         NaN \\
      SA-SA/MC-LTO + B &             188 &          NaN &           179 &         NaN &                179 &         NaN &             190 &         NaN &             195 &         NaN &                       196 &         NaN \\
   SA-SA/MC-CONCAT + B &             189 &          NaN &           200 &         NaN &                186 &         NaN &             202 &         NaN &             196 &         NaN &                       195 &         NaN \\
  SA-SA/MC-LCONCAT + B &             190 &          NaN &           199 &         NaN &                185 &         NaN &             189 &         NaN &             197 &         NaN &                       188 &         NaN \\
      SA-SA/MC-TEM + B &              63 & -1191.064389 &            34 & -259.702235 &                 35 & -191.875770 &              39 & -322.644872 &              44 &    1.567217 &                        46 &  -77.818973 \\
    SA-SA/MC-TEMWL + B &              64 & -1191.064389 &            35 & -259.702235 &                 34 & -191.875770 &              40 & -322.644872 &              43 &    1.567217 &                        47 &  -77.818973 \\
       SA-SA/MC-LE + B &             191 &          NaN &           198 &         NaN &                194 &         NaN &             188 &         NaN &             188 &         NaN &                       187 &         NaN \\
     SA-SA/MC-LEWL + B &             197 &          NaN &           191 &         NaN &                199 &         NaN &             182 &         NaN &             181 &         NaN &                       182 &         NaN \\
        C-SA/MC-TO + B &              62 & -1194.697050 &            36 & -259.585209 &                 38 & -182.209495 &              55 & -305.855895 &             101 &    2.938897 &                       124 &  -74.600713 \\
       SA-SA/MC-TO + B &              61 & -1194.697050 &            37 & -259.585209 &                 39 & -182.209495 &              56 & -305.855895 &             100 &    2.938897 &                       123 &  -74.600713 \\
                Hawkes &              65 & -1188.671196 &            58 & -220.820164 &                178 &  338.614547 &              63 & -298.746666 &             125 &    4.256323 &                         7 &  -78.657302 \\
               Poisson &             176 &  -782.721855 &           146 &  -51.743876 &                129 &  -57.322116 &             175 & -142.584864 &             102 &    2.984781 &                       168 &  -71.596478 \\
                   MRC &             271 &          NaN &           271 &         NaN &                271 &         NaN &             271 &         NaN &             271 &         NaN &                       271 &         NaN \\

\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{ccccccccc}
\hline \\
& \multicolumn{8}{c}{\textbf{Wikipedia}} \\ \\
&                      NLL Time &                  NLL Time U. &                    NLL Mark &                   NLL Total &                Time Cal. &             Time Cal. U. &                 Mark Cal. &                  F1-score \\
\hline \\
GRU-CP &                -130.6 (10.28) &              -126.59 (16.49) &             443.74 (140.44) &             313.14 (134.69) &              0.37 (0.01) &              0.32 (0.01) &               0.34 (0.08) &               0.14 (0.08) \\
GRU-CP + B &               -119.28 (14.07) &              -126.42 (16.45) &             480.56 (143.44) &             361.28 (134.16) &              0.35 (0.01) &              0.33 (0.01) &                0.4 (0.05) &               0.13 (0.04) \\
GRU-CP + BFC &               -131.55 (13.95) &           \textbf{nan (nan)} &              534.9 (158.77) &             403.35 (147.56) &              0.36 (0.01) &       \textbf{nan (nan)} &               0.38 (0.07) &               0.16 (0.06) \\
GRU-LNM &               -265.49 (32.65) &              -233.78 (26.81) &              218.49 (25.06) & $\text{-47.0 (29.22)}^{**}$ &              0.09 (0.05) &   $\text{0.03 (0.01)}^*$ &               0.27 (0.05) &               0.43 (0.11) \\
GRU-LNM + B &               -285.22 (29.21) &              -308.62 (26.55) &               277.3 (20.39) &               -7.93 (10.74) &              0.04 (0.01) &               0.1 (0.02) &               0.44 (0.05) &               0.12 (0.08) \\
GRU-LNM + BFC & $\text{-285.49 (26.17)}^{**}$ &                    nan (nan) &               213.42 (25.2) &      \textbf{-72.07 (9.63)} &   $\text{0.03 (0.01)}^*$ &                nan (nan) &               0.22 (0.07) &               0.54 (0.08) \\
GRU-MLP/CM &               -119.86 (12.25) &              -113.49 (19.18) &              262.74 (18.39) &                142.88 (6.8) &                0.2 (0.0) &              0.34 (0.01) &                 0.5 (0.0) &                0.01 (0.0) \\
GRU-MLP/CM + B &               -122.69 (16.76) &               -82.65 (10.92) &              330.45 (43.01) &              207.76 (27.56) &              0.32 (0.01) &              0.35 (0.01) &                 0.5 (0.0) &                0.01 (0.0) \\
GRU-MLP/CM + BFC &               -123.57 (13.83) &                    nan (nan) &               290.04 (36.0) &              166.47 (23.29) &              0.25 (0.01) &                nan (nan) &                 0.5 (0.0) &                0.01 (0.0) \\
GRU-MLP/MC &                 -6.47 (20.35) &              -168.67 (20.25) &              217.08 (16.43) &               210.61 (5.68) &              0.28 (0.01) &              0.25 (0.01) &               0.48 (0.04) &               0.17 (0.03) \\
GRU-MLP/MC + B &               -121.89 (12.23) &              -165.55 (18.26) &   $\text{145.13 (17.34)}^*$ &               23.24 (18.46) &              0.33 (0.01) &              0.26 (0.01) &               0.26 (0.02) &               0.52 (0.04) \\
GRU-MLP/MC + BFC &                -73.07 (23.83) &                    nan (nan) &              188.07 (11.14) &               115.0 (17.24) &               0.3 (0.01) &                nan (nan) &                0.4 (0.04) &               0.31 (0.03) \\
GRU-RMTPP &                -138.9 (18.09) &              -146.36 (18.12) &              263.12 (37.03) &              124.22 (28.16) &               0.3 (0.01) &               0.3 (0.01) &               0.24 (0.06) & $\text{0.57 (0.06)}^{**}$ \\
GRU-RMTPP + B &               -136.01 (22.52) &              -144.27 (17.34) &              264.53 (41.57) &              128.52 (29.98) &              0.32 (0.01) &               0.3 (0.01) &               0.34 (0.08) &               0.46 (0.09) \\
GRU-RMTPP + BFC &               -152.31 (19.46) &                    nan (nan) &              249.19 (40.78) &                96.88 (28.2) &              0.33 (0.01) &                nan (nan) &               0.27 (0.07) &                0.46 (0.1) \\
GRU-SA/CM &               -164.62 (22.57) &               -220.3 (26.43) &              276.43 (26.65) &              111.81 (11.83) &               0.1 (0.01) &               0.08 (0.0) &                 0.5 (0.0) &                 0.0 (0.0) \\
GRU-SA/CM + B &                -170.29 (31.4) &              -224.66 (26.77) &              309.48 (50.99) &              139.19 (41.97) &               0.2 (0.01) & $\text{0.06 (0.0)}^{**}$ &                 0.5 (0.0) &                0.01 (0.0) \\
GRU-SA/CM + BFC &                -147.0 (54.36) &                    nan (nan) &              278.14 (25.97) &              131.14 (32.56) &              0.14 (0.01) &                nan (nan) &                 0.5 (0.0) &                0.01 (0.0) \\
GRU-SA/MC &                 -33.1 (20.13) &              -226.88 (26.37) &              218.69 (15.22) &              185.59 (11.67) &              0.22 (0.02) &              0.07 (0.01) &               0.33 (0.05) &               0.17 (0.02) \\
GRU-SA/MC + B &               -188.01 (21.17) &               -225.18 (25.9) &              150.91 (13.55) &               -37.1 (15.22) &              0.25 (0.01) &              0.08 (0.01) & $\text{0.17 (0.01)}^{**}$ &               0.54 (0.03) \\
GRU-SA/MC + BFC &                -135.6 (17.03) &                    nan (nan) &              175.71 (14.23) &               40.11 (12.82) &              0.22 (0.02) &                nan (nan) &               0.26 (0.04) &                0.4 (0.04) \\
SA-CP &               -134.73 (12.09) &              -123.04 (15.74) &             415.91 (135.01) &             281.18 (127.24) &              0.37 (0.01) &              0.33 (0.01) &               0.43 (0.05) &               0.21 (0.11) \\
SA-CP + B &               -111.69 (15.55) &               -123.15 (15.7) &             591.01 (162.57) &             479.32 (148.01) &              0.35 (0.01) &              0.33 (0.01) &               0.46 (0.03) &               0.14 (0.08) \\
SA-CP + BFC &               -128.54 (12.63) &                    nan (nan) &             453.89 (134.79) &             325.35 (124.46) &              0.35 (0.01) &                nan (nan) &               0.43 (0.06) &               0.16 (0.04) \\
SA-LNM &       \textbf{-288.89 (27.0)} & $\text{-235.18 (26.8)}^{**}$ &              246.11 (18.82) &              -42.78 (24.88) &      \textbf{0.02 (0.0)} &               0.02 (0.0) &               0.33 (0.07) &               0.31 (0.12) \\
SA-LNM + B &               -277.08 (27.38) &    $\text{-302.21 (14.7)}^*$ &              289.16 (14.89) &               12.08 (13.75) & $\text{0.03 (0.0)}^{**}$ &               0.1 (0.01) &                0.4 (0.06) &                0.22 (0.1) \\
SA-LNM + BFC &    $\text{-286.27 (25.62)}^*$ &                    nan (nan) &               227.5 (33.65) &   $\text{-58.78 (14.53)}^*$ &              0.04 (0.01) &                nan (nan) &               0.26 (0.05) &               0.43 (0.08) \\
SA-MLP/CM &                -99.07 (15.68) &               -82.93 (10.82) &              277.28 (28.13) &              178.22 (12.72) &              0.18 (0.01) &              0.35 (0.01) &                 0.5 (0.0) &                 0.0 (0.0) \\
SA-MLP/CM + B &               -116.17 (23.51) &               -83.75 (10.98) &               330.9 (45.83) &              214.73 (23.61) &              0.31 (0.01) &              0.35 (0.01) &                 0.5 (0.0) &                 0.0 (0.0) \\
SA-MLP/CM + BFC &               -104.21 (12.99) &                    nan (nan) &               290.2 (32.22) &              185.99 (21.04) &              0.26 (0.01) &                nan (nan) &                 0.5 (0.0) &                0.01 (0.0) \\
SA-MLP/MC &                 -11.48 (19.9) &              -183.28 (21.15) &              220.69 (12.58) &               209.21 (8.05) &              0.28 (0.01) &              0.22 (0.01) &               0.55 (0.01) &               0.12 (0.03) \\
SA-MLP/MC + B &               -123.24 (19.59) &              -175.89 (21.15) &              149.89 (19.86) &               26.64 (17.49) &               0.35 (0.0) &              0.24 (0.01) &    $\text{0.16 (0.01)}^*$ &               0.49 (0.04) \\
SA-MLP/MC + BFC &                  -88.1 (16.8) &                    nan (nan) &              196.88 (22.67) &              108.78 (14.67) &              0.31 (0.01) &                nan (nan) &                0.4 (0.02) &               0.28 (0.07) \\
SA-RMTPP &               -168.01 (18.84) &               -147.1 (18.32) &              234.26 (37.46) &               66.26 (24.14) &              0.31 (0.01) &              0.29 (0.01) &               0.24 (0.07) &               0.57 (0.07) \\
SA-RMTPP + B &               -148.53 (20.44) &               -146.74 (16.6) &               285.6 (44.04) &              137.07 (36.42) &              0.33 (0.01) &              0.29 (0.01) &               0.29 (0.07) &                0.4 (0.12) \\
SA-RMTPP + BFC &               -154.32 (21.25) &                    nan (nan) &              276.18 (41.33) &              121.86 (29.92) &              0.32 (0.01) &                nan (nan) &               0.36 (0.05) &                0.46 (0.1) \\
SA-SA/CM &               -153.32 (25.01) &              -220.43 (27.34) &              286.24 (32.47) &              132.92 (18.88) &              0.09 (0.01) &              0.08 (0.01) &                 0.5 (0.0) &                 0.0 (0.0) \\
SA-SA/CM + B &               -165.26 (42.01) &                    nan (nan) &              327.52 (50.72) &              162.26 (34.32) &               0.2 (0.01) &                nan (nan) &                 0.5 (0.0) &                0.01 (0.0) \\
SA-SA/CM + BFC &               -148.92 (28.49) &                    nan (nan) &               286.55 (30.7) &              137.63 (19.25) &              0.15 (0.02) &                nan (nan) &                 0.5 (0.0) &                0.01 (0.0) \\
SA-SA/MC &                -41.61 (22.01) &              -225.29 (25.81) &               220.31 (8.94) &               178.7 (13.53) &              0.23 (0.01) &              0.09 (0.01) &               0.44 (0.04) &               0.14 (0.03) \\
SA-SA/MC + B &               -191.88 (17.52) &                    nan (nan) & $\text{149.4 (10.93)}^{**}$ &              -42.47 (16.03) &              0.25 (0.01) &                nan (nan) &               0.18 (0.02) &    $\text{0.58 (0.04)}^*$ \\
SA-SA/MC + BFC &               -135.76 (22.97) &                    nan (nan) &              185.76 (11.12) &                50.0 (17.85) &              0.24 (0.02) &                nan (nan) &                0.3 (0.04) &               0.36 (0.04) \\
Poisson &                -57.32 (16.36) &                    nan (nan) &             534.95 (131.14) &             477.63 (123.65) &              0.34 (0.01) &                nan (nan) &                 0.5 (0.0) &                0.01 (0.0) \\
Hawkes &                338.61 (94.32) &                    nan (nan) &     \textbf{144.69 (12.45)} &                483.3 (82.5) &               0.2 (0.01) &                nan (nan) &      \textbf{0.11 (0.03)} &      \textbf{0.66 (0.02)} \\ \\
\hline \\
& \multicolumn{8}{c}{\textbf{Github}} \\ \\
&                      NLL Time &                    NLL Time U. &                    NLL Mark &                     NLL Total &                Time Cal. &              Time Cal. U. &                 Mark Cal. &                 F1-score \\
\hline \\
GRU-CP &               -273.12 (53.73) &                -463.3 (122.93) &              138.71 (19.91) &               -134.41 (35.45) &               0.2 (0.01) &               0.22 (0.02) &               0.18 (0.01) &              0.42 (0.03) \\
GRU-CP + B &               -270.29 (52.78) &               -455.15 (119.06) &               151.7 (21.25) &               -118.59 (34.75) &               0.2 (0.01) &               0.22 (0.02) &               0.32 (0.03) &              0.42 (0.03) \\
GRU-CP + BFC &               -265.05 (48.53) &             \textbf{nan (nan)} &              141.82 (21.52) &               -123.22 (29.81) &               0.2 (0.01) &        \textbf{nan (nan)} &               0.22 (0.03) &              0.42 (0.03) \\
GRU-LNM &               -374.49 (56.79) &    $\text{-598.33 (154.26)}^*$ &              131.46 (24.14) &               -243.03 (35.32) &   $\text{0.03 (0.01)}^*$ &               0.04 (0.01) &               0.21 (0.05) &               0.5 (0.04) \\
GRU-LNM + B &    $\text{-509.59 (43.49)}^*$ &               -726.89 (133.55) &              161.24 (22.35) &    $\text{-348.35 (30.69)}^*$ &              0.05 (0.01) &                0.1 (0.02) &               0.37 (0.05) &              0.42 (0.03) \\
GRU-LNM + BFC & $\text{-379.13 (59.66)}^{**}$ &                      nan (nan) &     \textbf{120.67 (15.33)} & $\text{-258.46 (44.74)}^{**}$ &      \textbf{0.02 (0.0)} &                 nan (nan) &    $\text{0.17 (0.02)}^*$ &     \textbf{0.56 (0.01)} \\
GRU-MLP/CM &                 -265.6 (47.8) &                -377.64 (106.3) &              158.14 (22.91) &                -107.46 (27.1) &              0.19 (0.02) &               0.29 (0.02) &               0.34 (0.02) &               0.4 (0.03) \\
GRU-MLP/CM + B &               -261.25 (44.92) &                -274.53 (72.29) &              160.33 (24.42) &               -100.92 (25.57) &              0.21 (0.02) &               0.32 (0.03) &                0.4 (0.03) &               0.4 (0.03) \\
GRU-MLP/CM + BFC &               -258.69 (42.19) &                      nan (nan) &              158.52 (25.41) &               -100.16 (22.43) &              0.21 (0.02) &                 nan (nan) &               0.37 (0.04) &               0.4 (0.03) \\
GRU-MLP/MC &               -257.25 (52.66) &               -498.63 (135.83) &              139.71 (19.49) &               -117.54 (34.35) &              0.18 (0.01) &               0.16 (0.01) &                0.2 (0.02) &              0.53 (0.01) \\
GRU-MLP/MC + B &               -271.35 (50.62) &               -491.59 (131.73) &               130.7 (18.32) &               -140.64 (34.28) &              0.19 (0.01) &               0.17 (0.02) &               0.24 (0.02) &              0.49 (0.03) \\
GRU-MLP/MC + BFC &               -269.15 (57.26) &                      nan (nan) &              129.44 (16.55) &               -139.72 (41.45) &              0.17 (0.01) &                 nan (nan) &               0.22 (0.02) & $\text{0.55 (0.0)}^{**}$ \\
GRU-RMTPP &               -279.86 (54.29) &               -489.58 (132.18) &               127.8 (19.96) &                -152.07 (35.8) &              0.18 (0.01) &               0.17 (0.02) &               0.18 (0.02) &              0.49 (0.04) \\
GRU-RMTPP + B &               -276.45 (51.41) &               -487.46 (132.25) &               136.6 (18.94) &               -139.85 (33.21) &              0.18 (0.01) &               0.18 (0.02) &               0.19 (0.02) &              0.48 (0.02) \\
GRU-RMTPP + BFC &               -273.83 (50.72) &                      nan (nan) &              136.74 (21.99) &                -137.1 (31.84) &              0.19 (0.02) &                 nan (nan) & $\text{0.18 (0.02)}^{**}$ &              0.48 (0.03) \\
GRU-SA/CM &               -294.87 (55.43) &               -542.37 (141.78) &              157.01 (21.64) &               -137.86 (35.66) &              0.13 (0.01) &               0.08 (0.01) &               0.41 (0.01) &               0.4 (0.03) \\
GRU-SA/CM + B &               -320.68 (55.92) &               -555.98 (145.16) &               154.45 (21.0) &               -166.24 (36.01) &               0.11 (0.0) & $\text{0.07 (0.01)}^{**}$ &                0.45 (0.0) &               0.4 (0.03) \\
GRU-SA/CM + BFC &               -303.29 (59.26) &                      nan (nan) &               155.7 (21.46) &               -147.59 (39.23) &              0.13 (0.01) &                 nan (nan) &               0.42 (0.01) &               0.4 (0.03) \\
GRU-SA/MC &                -300.3 (55.12) &               -536.71 (139.33) &              136.46 (18.77) &               -163.84 (37.43) &              0.12 (0.01) &               0.09 (0.02) &               0.27 (0.01) &              0.54 (0.02) \\
GRU-SA/MC + B &               -319.83 (52.21) &                -542.16 (143.7) & $\text{125.2 (16.26)}^{**}$ &               -194.63 (36.75) &                0.1 (0.0) &               0.09 (0.01) &               0.23 (0.02) &   $\text{0.56 (0.01)}^*$ \\
GRU-SA/MC + BFC &               -322.09 (57.32) &                      nan (nan) &              132.04 (17.64) &               -190.04 (40.79) &                0.1 (0.0) &                 nan (nan) &               0.22 (0.02) &              0.53 (0.02) \\
SA-CP &               -254.18 (47.64) &                -431.9 (114.64) &              142.12 (20.54) &               -112.05 (28.22) &              0.21 (0.02) &               0.24 (0.02) &                0.2 (0.01) &               0.4 (0.03) \\
SA-CP + B &               -263.15 (53.22) &                -423.1 (111.22) &              152.32 (20.72) &               -110.83 (33.35) &               0.2 (0.01) &               0.25 (0.02) &                0.3 (0.03) &               0.4 (0.03) \\
SA-CP + BFC &                -254.61 (47.4) &                      nan (nan) &              151.07 (22.61) &               -103.54 (26.57) &              0.21 (0.02) &                 nan (nan) &               0.29 (0.02) &               0.4 (0.03) \\
SA-LNM &               -371.99 (57.31) & $\text{-589.71 (152.54)}^{**}$ &              131.43 (20.52) &               -240.55 (37.51) & $\text{0.03 (0.0)}^{**}$ &    $\text{0.06 (0.01)}^*$ &               0.23 (0.02) &              0.51 (0.03) \\
SA-LNM + B &      \textbf{-603.17 (72.96)} &                      nan (nan) &               152.8 (19.96) &      \textbf{-450.37 (60.51)} &              0.06 (0.01) &                 nan (nan) &               0.36 (0.05) &              0.44 (0.03) \\
SA-LNM + BFC &               -373.86 (58.13) &                      nan (nan) &              129.25 (16.48) &                -244.6 (41.93) &              0.04 (0.01) &                 nan (nan) &               0.22 (0.01) &              0.52 (0.01) \\
SA-MLP/CM &               -172.94 (32.92) &                -272.55 (71.93) &              160.58 (20.61) &                -12.36 (12.78) &              0.26 (0.02) &               0.32 (0.03) &               0.47 (0.01) &               0.4 (0.03) \\
SA-MLP/CM + B &                -175.5 (31.64) &                -275.92 (72.72) &               163.4 (22.79) &                 -12.1 (10.98) &              0.28 (0.02) &               0.32 (0.03) &               0.47 (0.01) &               0.4 (0.03) \\
SA-MLP/CM + BFC &                -174.5 (32.88) &                      nan (nan) &              161.32 (21.03) &                -13.19 (12.62) &              0.27 (0.02) &                 nan (nan) &               0.47 (0.01) &               0.4 (0.03) \\
SA-MLP/MC &               -245.26 (49.72) &                -464.65 (122.9) &              142.19 (21.43) &               -103.08 (31.34) &              0.18 (0.01) &               0.19 (0.03) &               0.26 (0.02) &               0.5 (0.04) \\
SA-MLP/MC + B &               -256.98 (46.33) &               -468.24 (126.47) &              138.37 (17.41) &               -118.61 (31.52) &               0.2 (0.01) &                0.2 (0.02) &               0.27 (0.03) &              0.48 (0.04) \\
SA-MLP/MC + BFC &               -246.88 (52.25) &                      nan (nan) &              139.12 (21.22) &               -107.76 (34.49) &              0.18 (0.01) &                 nan (nan) &               0.22 (0.01) &              0.52 (0.02) \\
SA-RMTPP &               -258.37 (44.02) &               -447.72 (118.47) &              138.15 (21.92) &               -120.22 (28.09) &              0.21 (0.03) &               0.22 (0.02) &                0.2 (0.03) &              0.45 (0.03) \\
SA-RMTPP + B &                -259.53 (49.1) &               -449.76 (120.26) &              139.97 (18.33) &               -119.56 (33.65) &              0.18 (0.01) &               0.22 (0.02) &               0.21 (0.03) &              0.47 (0.03) \\
SA-RMTPP + BFC &               -260.01 (46.73) &                      nan (nan) &              137.14 (22.43) &               -122.87 (29.53) &               0.2 (0.02) &                 nan (nan) &               0.23 (0.04) &              0.47 (0.03) \\
SA-SA/CM &               -292.43 (55.48) &               -536.67 (145.01) &              158.45 (21.09) &               -133.98 (35.51) &              0.14 (0.01) &               0.09 (0.01) &               0.39 (0.02) &               0.4 (0.03) \\
SA-SA/CM + B &                -309.45 (58.4) &               -561.32 (269.04) &              154.33 (21.02) &               -155.12 (39.58) &              0.13 (0.01) &               0.08 (0.03) &               0.44 (0.02) &               0.4 (0.03) \\
SA-SA/CM + BFC &               -292.73 (53.48) &                      nan (nan) &              154.84 (21.15) &               -137.89 (33.98) &              0.14 (0.01) &                 nan (nan) &               0.42 (0.01) &               0.4 (0.03) \\
SA-SA/MC &               -297.79 (52.97) &               -533.67 (141.89) &              137.85 (19.01) &               -159.95 (35.05) &              0.11 (0.01) &                0.1 (0.02) &               0.27 (0.01) &              0.52 (0.02) \\
SA-SA/MC + B &               -322.64 (55.78) &                      nan (nan) &              131.79 (19.84) &               -190.85 (37.44) &               0.1 (0.01) &                 nan (nan) &                0.2 (0.02) &              0.52 (0.02) \\
SA-SA/MC + BFC &               -317.08 (53.16) &                      nan (nan) &              132.18 (17.58) &                -184.9 (36.27) &               0.11 (0.0) &                 nan (nan) &               0.27 (0.01) &              0.54 (0.01) \\
Poisson &               -142.58 (26.06) &                      nan (nan) &              168.37 (21.04) &                  25.79 (5.38) &              0.33 (0.02) &                 nan (nan) &               0.49 (0.01) &               0.4 (0.03) \\
Hawkes &                -298.75 (56.8) &                      nan (nan) &   $\text{124.65 (15.73)}^*$ &               -174.09 (41.47) &              0.16 (0.01) &                 nan (nan) &       \textbf{0.05 (0.0)} &              0.53 (0.01) \\ \\
\hline 
\end{tabular}
\label{resultsmark}
\caption{Evaluation of the different neural TPP models on Wikipedia and Github. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%MARKED%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{ccccccccc}
\hline \\
& \multicolumn{8}{c}{\textbf{MIMIC2}} \\ \\
&                  NLL Time &                NLL Time U. &                  NLL Mark &                NLL Total &                 Time Cal. &             Time Cal. U. &                 Mark Cal. &                  F1-score \\
\hline \\
GRU-CP &               1.35 (0.09) &                0.78 (0.05) &               2.76 (0.21) &              4.11 (0.28) &                0.03 (0.0) &              0.07 (0.01) &               0.12 (0.02) &               0.64 (0.05) \\
GRU-CP + B &               1.63 (0.06) &                0.76 (0.04) &               3.96 (0.31) &              5.59 (0.35) &               0.05 (0.01) &              0.06 (0.01) &               0.21 (0.02) &               0.62 (0.04) \\
GRU-CP + BFC &               1.59 (0.05) &         \textbf{nan (nan)} &                3.05 (0.3) &              4.64 (0.33) &               0.03 (0.01) &       \textbf{nan (nan)} &               0.16 (0.01) &               0.65 (0.02) \\
GRU-LNM &               1.36 (0.09) & $\text{-0.27 (0.09)}^{**}$ & $\text{2.12 (0.12)}^{**}$ &   $\text{3.48 (0.19)}^*$ &                0.03 (0.0) &              0.03 (0.01) &               0.13 (0.01) &               0.72 (0.01) \\
GRU-LNM + B &    $\text{1.23 (0.11)}^*$ &    $\text{-0.38 (0.39)}^*$ &                 3.5 (0.1) &               4.73 (0.2) &               0.08 (0.03) &              0.05 (0.01) &                0.2 (0.04) &               0.62 (0.04) \\
GRU-LNM + BFC &               1.55 (0.08) &                  nan (nan) &               2.67 (0.18) &               4.22 (0.2) &               0.03 (0.01) &                nan (nan) & $\text{0.11 (0.02)}^{**}$ &               0.65 (0.05) \\
GRU-MLP/CM &               1.68 (0.04) &                 0.4 (0.17) &               4.49 (0.16) &               6.16 (0.2) &               0.07 (0.01) &               0.03 (0.0) &               0.46 (0.01) &               0.21 (0.02) \\
GRU-MLP/CM + B &               1.55 (0.16) &                 0.3 (0.13) &               3.81 (0.22) &              5.36 (0.36) &               0.05 (0.01) &               0.03 (0.0) &               0.37 (0.03) &               0.36 (0.04) \\
GRU-MLP/CM + BFC &                1.64 (0.2) &                  nan (nan) &                3.97 (0.2) &              5.61 (0.37) &               0.04 (0.01) &                nan (nan) &                0.4 (0.05) &               0.28 (0.05) \\
GRU-MLP/MC &              67.41 (4.12) &                0.52 (0.07) &               7.33 (0.26) &             74.73 (4.34) &                0.48 (0.0) &               0.06 (0.0) &               0.51 (0.01) &               0.06 (0.04) \\
GRU-MLP/MC + B &               1.65 (0.09) &                0.54 (0.07) &               2.84 (0.17) &              4.49 (0.21) &               0.07 (0.01) &               0.04 (0.0) &                0.2 (0.02) &               0.69 (0.03) \\
GRU-MLP/MC + BFC &              31.43 (1.97) &                  nan (nan) &               7.28 (0.26) &             38.72 (2.21) &                0.45 (0.0) &                nan (nan) &                0.53 (0.0) &               0.22 (0.02) \\
GRU-RMTPP &               1.33 (0.09) &                0.73 (0.05) &      \textbf{1.89 (0.12)} &      \textbf{3.22 (0.2)} &               0.04 (0.01) &              0.05 (0.01) &               0.14 (0.01) &    $\text{0.76 (0.02)}^*$ \\
GRU-RMTPP + B &               1.34 (0.14) &                 0.8 (0.19) &               2.43 (0.23) &              3.77 (0.33) &                0.03 (0.0) &              0.05 (0.01) &       \textbf{0.1 (0.01)} & $\text{0.73 (0.03)}^{**}$ \\
GRU-RMTPP + BFC &                1.3 (0.13) &                  nan (nan) &               2.43 (0.15) &              3.73 (0.26) &               0.04 (0.01) &                nan (nan) &     $\text{0.11 (0.0)}^*$ &               0.68 (0.03) \\
GRU-SA/CM &               1.53 (0.14) &                 0.0 (0.18) &                4.61 (0.1) &              6.15 (0.19) &                0.04 (0.0) &               0.03 (0.0) &               0.44 (0.01) &               0.22 (0.02) \\
GRU-SA/CM + B &               1.41 (0.16) &               -0.42 (0.15) &               4.05 (0.19) &              5.46 (0.22) &               0.03 (0.01) &               0.03 (0.0) &               0.38 (0.02) &                0.3 (0.05) \\
GRU-SA/CM + BFC &               1.59 (0.11) &                  nan (nan) &               3.68 (0.07) &              5.27 (0.16) & $\text{0.03 (0.01)}^{**}$ &                nan (nan) &               0.32 (0.02) &               0.34 (0.04) \\
GRU-SA/MC &              67.43 (4.11) &                 0.2 (0.03) &               7.33 (0.26) &             74.76 (4.34) &                0.48 (0.0) &              0.04 (0.01) &                 0.5 (0.0) &               0.02 (0.01) \\
GRU-SA/MC + B &               1.56 (0.18) &               -0.15 (0.03) &               2.56 (0.21) &              4.12 (0.34) &               0.07 (0.01) &    $\text{0.03 (0.0)}^*$ &               0.15 (0.02) &               0.69 (0.03) \\
GRU-SA/MC + BFC &              31.42 (1.98) &                  nan (nan) &               7.31 (0.26) &             38.73 (2.21) &                0.45 (0.0) &                nan (nan) &                0.53 (0.0) &               0.22 (0.02) \\
SA-CP &               2.13 (0.13) &                1.57 (0.04) &               2.73 (0.24) &              4.86 (0.24) &                0.07 (0.0) &              0.11 (0.01) &               0.22 (0.02) &               0.62 (0.05) \\
SA-CP + B &               1.99 (0.15) &                1.57 (0.04) &               3.87 (0.27) &              5.86 (0.35) &               0.07 (0.01) &               0.1 (0.01) &               0.32 (0.03) &               0.55 (0.05) \\
SA-CP + BFC &                2.2 (0.17) &                  nan (nan) &               3.18 (0.21) &              5.38 (0.33) &               0.08 (0.01) &                nan (nan) &               0.32 (0.03) &               0.59 (0.03) \\
SA-LNM & $\text{1.27 (0.28)}^{**}$ &                1.26 (0.03) &                2.33 (0.2) & $\text{3.6 (0.27)}^{**}$ &       \textbf{0.02 (0.0)} &              0.03 (0.01) &               0.25 (0.04) &               0.68 (0.05) \\
SA-LNM + B &      \textbf{1.17 (0.15)} &                0.55 (0.34) &               3.21 (0.27) &              4.37 (0.27) &                0.04 (0.0) &              0.07 (0.02) &                0.2 (0.05) &               0.64 (0.03) \\
SA-LNM + BFC &               1.64 (0.09) &                  nan (nan) &               2.58 (0.08) &              4.22 (0.14) &     $\text{0.02 (0.0)}^*$ &                nan (nan) &               0.14 (0.02) &               0.66 (0.03) \\
SA-MLP/CM &                2.07 (0.1) &                1.55 (0.04) &               4.51 (0.13) &              6.58 (0.18) &                0.1 (0.01) &                0.1 (0.0) &                0.47 (0.0) &               0.22 (0.02) \\
SA-MLP/CM + B &               1.89 (0.16) &                1.56 (0.04) &                3.75 (0.2) &              5.64 (0.15) &               0.08 (0.01) &                0.1 (0.0) &               0.39 (0.03) &               0.32 (0.07) \\
SA-MLP/CM + BFC &               1.84 (0.11) &                  nan (nan) &                4.2 (0.18) &              6.04 (0.25) &                0.05 (0.0) &                nan (nan) &                0.46 (0.0) &               0.22 (0.02) \\
SA-MLP/MC &               67.4 (4.11) &                1.42 (0.04) &               7.33 (0.26) &             74.73 (4.33) &                0.48 (0.0) &              0.05 (0.01) &                0.5 (0.01) &               0.06 (0.04) \\
SA-MLP/MC + B &               2.13 (0.22) &                1.36 (0.04) &               2.55 (0.13) &              4.68 (0.33) &               0.04 (0.01) &               0.05 (0.0) &               0.26 (0.02) &               0.73 (0.02) \\
SA-MLP/MC + BFC &              31.41 (1.98) &                  nan (nan) &                7.3 (0.26) &             38.72 (2.21) &                0.45 (0.0) &                nan (nan) &                0.53 (0.0) &               0.22 (0.02) \\
SA-RMTPP &                1.68 (0.1) &                1.41 (0.04) &    $\text{2.02 (0.13)}^*$ &               3.7 (0.21) &                0.03 (0.0) &               0.06 (0.0) &               0.14 (0.02) &      \textbf{0.77 (0.01)} \\
SA-RMTPP + B &                1.83 (0.1) &                1.39 (0.04) &               2.78 (0.15) &              4.61 (0.23) &                0.03 (0.0) &               0.05 (0.0) &               0.15 (0.02) &               0.67 (0.02) \\
SA-RMTPP + BFC &               1.73 (0.11) &                  nan (nan) &               2.44 (0.21) &              4.17 (0.26) &                0.03 (0.0) &                nan (nan) &               0.13 (0.02) &               0.71 (0.02) \\
SA-SA/CM &                 1.9 (0.1) &                1.23 (0.05) &               4.44 (0.14) &              6.35 (0.22) &               0.05 (0.01) &              0.03 (0.01) &                0.47 (0.0) &               0.22 (0.02) \\
SA-SA/CM + B &                1.7 (0.08) &                  nan (nan) &               4.08 (0.11) &              5.78 (0.17) &               0.05 (0.01) &                nan (nan) &               0.39 (0.02) &               0.25 (0.05) \\
SA-SA/CM + BFC &                1.78 (0.1) &                  nan (nan) &               4.24 (0.11) &              6.02 (0.18) &                0.05 (0.0) &                nan (nan) &               0.42 (0.03) &               0.24 (0.03) \\
SA-SA/MC &              67.42 (4.11) &                0.35 (0.12) &               7.33 (0.26) &             74.75 (4.33) &                0.48 (0.0) & $\text{0.03 (0.0)}^{**}$ &               0.52 (0.01) &               0.13 (0.05) \\
SA-SA/MC + B &               1.57 (0.12) &                  nan (nan) &                2.4 (0.17) &              3.97 (0.24) &               0.04 (0.01) &                nan (nan) &               0.17 (0.02) &                0.7 (0.01) \\
SA-SA/MC + BFC &              31.44 (1.98) &                  nan (nan) &                7.3 (0.26) &             38.74 (2.21) &                0.45 (0.0) &                nan (nan) &                0.53 (0.0) &               0.22 (0.02) \\
Poisson &               2.98 (0.12) &                  nan (nan) &              11.25 (0.46) &             14.24 (0.47) &                0.07 (0.0) &                nan (nan) &                0.47 (0.0) &                0.2 (0.02) \\
Hawkes &               4.26 (0.26) &                  nan (nan) &               8.24 (0.47) &              12.5 (0.71) &                0.05 (0.0) &                nan (nan) &               0.24 (0.04) &                0.63 (0.0) \\ \\
\hline
\end{tabular}
\label{resultsmark}
\caption{Evaluation of the different neural TPP models on MIMIC2. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%SIMULATIONS%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{cccccccc}
\hline \\
& \multicolumn{7}{c}{\textbf{Hawkes Exponential Dependent}} \\ \\
&                     NLL Time &                          NLL Mark &                NLL Window &                  NLL Total &                 Time Cal. &                 Mark Cal. &                        F1-score \\
\hline \\
GRU-CP &               -38.41 (12.52) &                     55.62 (17.22) &               1.18 (0.05) &               17.21 (5.07) &                0.6 (0.18) &               0.79 (0.13) &       $\text{0.72 (0.15)}^{**}$ \\
GRU-CP + B &               -38.45 (12.53) &                      56.2 (17.41) &               1.14 (0.06) &               17.75 (5.25) &               0.58 (0.18) &               0.79 (0.11) &                     0.66 (0.15) \\
GRU-CP + BFC &               -38.45 (12.53) &                     55.73 (17.26) &               1.15 (0.04) &                17.28 (5.1) &               0.59 (0.18) &               0.77 (0.12) &                     0.71 (0.14) \\
GRU-LNM &               -38.69 (12.61) &                     55.63 (17.23) &               1.15 (0.05) &                16.94 (5.0) &               0.58 (0.18) &               0.77 (0.12) &                     0.71 (0.14) \\
GRU-LNM + B &      \textbf{-50.01 (16.19)} &                     56.82 (17.64) & $\text{1.04 (0.02)}^{**}$ &       \textbf{6.81 (2.12)} &               0.54 (0.16) &               0.75 (0.09) &                      0.6 (0.14) \\
GRU-LNM + BFC &               -38.72 (12.61) &                     55.58 (17.22) &               1.13 (0.05) & $\text{16.86 (4.98)}^{**}$ &               0.57 (0.18) &               0.77 (0.12) &                      0.7 (0.14) \\
GRU-MLP/CM &               -37.46 (12.24) &                     56.09 (17.36) &               1.21 (0.04) &               18.63 (5.51) &               0.61 (0.19) &               0.82 (0.13) &                     0.72 (0.16) \\
GRU-MLP/CM + B &                -37.1 (12.07) &                     56.48 (17.53) &               1.06 (0.05) &                19.38 (5.8) &               0.54 (0.16) &                0.76 (0.1) &                     0.59 (0.15) \\
GRU-MLP/CM + BFC &               -37.91 (12.37) &                     56.18 (17.39) &               1.19 (0.06) &                18.27 (5.4) &                0.6 (0.19) &               0.82 (0.12) &                      0.7 (0.16) \\
GRU-MLP/MC &                -38.3 (12.48) &                     56.12 (17.38) &               1.16 (0.05) &               17.82 (5.27) &               0.58 (0.18) &               0.78 (0.12) &                     0.71 (0.14) \\
GRU-MLP/MC + B &               -38.69 (12.61) &                      55.7 (17.25) &               1.16 (0.05) &               17.01 (5.01) &               0.58 (0.18) &               0.78 (0.12) &                     0.71 (0.14) \\
GRU-MLP/MC + BFC &                -38.67 (12.6) &                     55.66 (17.24) &               1.15 (0.04) &               16.98 (5.01) &               0.58 (0.18) &               0.77 (0.12) &                     0.71 (0.14) \\
GRU-RMTPP &               -38.64 (12.59) & $\text{\textbf{55.56 (17.21)}}^*$ &               1.14 (0.04) &               16.91 (4.99) &               0.58 (0.18) &               0.77 (0.12) &                     0.71 (0.14) \\
GRU-RMTPP + B &                -38.67 (12.6) &       $\text{55.57 (17.21)}^{**}$ &               1.15 (0.04) &                16.9 (4.98) &               0.58 (0.18) &               0.77 (0.12) &                     0.71 (0.14) \\
GRU-RMTPP + BFC &                -38.64 (12.6) &                      55.56 (17.2) &               1.17 (0.05) &               16.91 (4.98) &               0.59 (0.19) &               0.79 (0.13) &                     0.72 (0.14) \\
GRU-SA/CM &               -37.35 (12.22) &                       56.3 (17.4) &               1.27 (0.05) &                18.95 (5.6) &                0.64 (0.2) &               0.85 (0.13) &                     0.72 (0.18) \\
GRU-SA/CM + B &               -38.35 (12.51) &                     56.45 (17.48) &               1.18 (0.05) &                18.1 (5.35) &               0.59 (0.19) &               0.81 (0.12) &                     0.66 (0.17) \\
GRU-SA/CM + BFC &               -37.81 (12.36) &                     56.36 (17.43) &               1.25 (0.04) &               18.55 (5.47) &                0.63 (0.2) &               0.84 (0.13) &                      0.7 (0.17) \\
GRU-SA/MC &               -38.14 (12.44) &                     56.34 (17.44) &               1.19 (0.04) &                18.2 (5.38) &                0.6 (0.19) &               0.81 (0.12) &                     0.72 (0.15) \\
GRU-SA/MC + B &                -38.5 (12.55) &                     55.91 (17.31) &               1.17 (0.03) &               17.41 (5.14) &               0.59 (0.19) &                0.8 (0.12) &                     0.71 (0.15) \\
GRU-SA/MC + BFC &               -38.46 (12.55) &                     55.99 (17.33) &                1.2 (0.03) &               17.54 (5.17) &                0.6 (0.19) &               0.81 (0.12) & $\text{\textbf{0.73 (0.15)}}^*$ \\
SA-CP &               -37.78 (12.31) &                     55.89 (17.32) &               1.12 (0.06) &               18.11 (5.37) &               0.57 (0.18) &               0.77 (0.11) &                     0.69 (0.14) \\
SA-CP + B &               -37.72 (12.29) &                     56.32 (17.46) &               1.13 (0.05) &                18.6 (5.53) &               0.58 (0.18) &               0.79 (0.11) &                     0.65 (0.15) \\
SA-CP + BFC &               -37.79 (12.31) &                     55.92 (17.33) &               1.13 (0.06) &               18.13 (5.38) &               0.58 (0.18) &               0.78 (0.11) &                     0.69 (0.14) \\
SA-LNM &               -38.19 (12.43) &                      55.9 (17.33) &               1.11 (0.04) &               17.72 (5.25) &               0.56 (0.18) &               0.76 (0.11) &                     0.68 (0.14) \\
SA-LNM + B &    $\text{-49.36 (16.03)}^*$ &                     56.66 (17.64) &       \textbf{0.9 (0.04)} &      $\text{7.3 (2.84)}^*$ &      \textbf{0.46 (0.14)} &      \textbf{0.67 (0.08)} &                     0.53 (0.12) \\
SA-LNM + BFC &               -38.25 (12.45) &                     55.87 (17.32) &               1.11 (0.05) &               17.62 (5.22) &               0.56 (0.18) &               0.77 (0.11) &                     0.68 (0.14) \\
SA-MLP/CM &               -35.82 (11.68) &                     56.54 (17.53) &                1.1 (0.05) &                20.72 (6.2) &               0.56 (0.17) &                0.79 (0.1) &                      0.6 (0.16) \\
SA-MLP/CM + B &               -36.86 (11.99) &                     56.51 (17.54) &               1.04 (0.04) &               19.65 (5.88) & $\text{0.53 (0.16)}^{**}$ &               0.76 (0.09) &                     0.58 (0.15) \\
SA-MLP/CM + BFC &               -36.36 (11.84) &                     56.51 (17.53) &               1.07 (0.04) &               20.16 (6.03) &               0.55 (0.17) &                0.77 (0.1) &                     0.59 (0.15) \\
SA-MLP/MC &                -37.77 (12.3) &                     56.28 (17.44) &               1.12 (0.04) &                18.51 (5.5) &               0.56 (0.18) &               0.78 (0.11) &                     0.69 (0.14) \\
SA-MLP/MC + B &               -38.13 (12.41) &                     55.87 (17.32) &                1.1 (0.04) &               17.74 (5.26) &               0.56 (0.17) &               0.76 (0.11) &                     0.68 (0.13) \\
SA-MLP/MC + BFC &               -38.16 (12.42) &                      55.9 (17.33) &                1.1 (0.04) &               17.74 (5.26) &               0.56 (0.17) &               0.77 (0.11) &                     0.69 (0.13) \\
SA-RMTPP &               -38.18 (12.43) &                     55.87 (17.31) &               1.13 (0.05) &               17.69 (5.24) &               0.57 (0.18) &               0.77 (0.12) &                     0.69 (0.14) \\
SA-RMTPP + B &               -38.21 (12.44) &                     55.86 (17.31) &               1.12 (0.05) &               17.64 (5.23) &               0.57 (0.18) &               0.77 (0.11) &                     0.69 (0.14) \\
SA-RMTPP + BFC &               -38.23 (12.45) &                     55.89 (17.32) &               1.12 (0.05) &               17.65 (5.23) &               0.57 (0.18) &               0.76 (0.12) &                     0.69 (0.14) \\
SA-SA/CM &               -37.18 (12.17) &                     56.46 (17.45) &               1.29 (0.06) &               19.28 (5.69) &               0.65 (0.21) &               0.87 (0.14) &                     0.71 (0.19) \\
SA-SA/CM + B &               -38.29 (12.49) &                     56.45 (17.48) &               1.19 (0.04) &               18.16 (5.37) &                0.6 (0.19) &               0.82 (0.12) &                     0.66 (0.17) \\
SA-SA/CM + BFC &               -37.77 (12.34) &                     56.46 (17.47) &               1.24 (0.04) &               18.69 (5.52) &                0.62 (0.2) &               0.84 (0.13) &                     0.68 (0.18) \\
SA-SA/MC &               -37.98 (12.39) &                     56.33 (17.44) &               1.18 (0.03) &               18.36 (5.43) &                0.6 (0.19) &               0.81 (0.12) &                     0.72 (0.15) \\
SA-SA/MC + B &                -38.32 (12.5) &                     55.96 (17.33) &               1.18 (0.04) &               17.64 (5.21) &               0.59 (0.19) &               0.81 (0.12) &                     0.72 (0.15) \\
SA-SA/MC + BFC &                -38.31 (12.5) &                     55.97 (17.33) &               1.19 (0.05) &               17.66 (5.21) &                0.6 (0.19) &               0.82 (0.12) &                     0.73 (0.15) \\
Poisson &               -35.33 (11.47) &                      57.2 (17.79) &    $\text{0.94 (0.04)}^*$ &               21.87 (6.62) &    $\text{0.49 (0.14)}^*$ &    $\text{0.71 (0.08)}^*$ &                     0.52 (0.13) \\
Hawkes & $\text{-38.76 (12.62)}^{**}$ &                     55.98 (17.35) &               1.13 (0.05) &               17.22 (5.09) &               0.57 (0.18) & $\text{0.74 (0.13)}^{**}$ &                     0.71 (0.14) \\ \\
\hline \\
& \multicolumn{7}{c}{\textbf{Hawkes Sum of Exponentials Dependent}} \\ \\
&                      NLL Time &                          NLL Mark &                NLL Window &                  NLL Total &                Time Cal. &                Mark Cal. &                  F1-score \\
\hline \\
GRU-CP &                 -41.3 (13.57) &                     57.61 (17.73) &               1.57 (0.05) &               16.31 (4.67) &              0.81 (0.24) &              1.01 (0.18) &                0.9 (0.21) \\
GRU-CP + B &                -41.37 (13.59) &                      57.9 (17.82) &               1.58 (0.05) &               16.54 (4.73) &              0.82 (0.24) &              1.01 (0.18) &               0.87 (0.23) \\
GRU-CP + BFC &                -41.36 (13.58) &                     57.74 (17.77) &               1.56 (0.05) &               16.38 (4.69) &              0.81 (0.24) &               1.0 (0.18) &               0.89 (0.22) \\
GRU-LNM &                -43.34 (14.15) &                     57.43 (17.73) &    $\text{1.38 (0.02)}^*$ &               14.08 (4.02) &     \textbf{0.69 (0.22)} &              0.91 (0.15) &               0.81 (0.18) \\
GRU-LNM + B &     $\text{-59.63 (19.48)}^*$ &                     59.63 (18.43) & $\text{1.38 (0.04)}^{**}$ &     $\text{0.01 (2.07)}^*$ &              0.71 (0.21) &              0.91 (0.15) &               0.77 (0.19) \\
GRU-LNM + BFC &   $\text{-43.4 (14.17)}^{**}$ & $\text{\textbf{57.39 (17.72)}}^*$ &               1.38 (0.02) & $\text{13.99 (3.99)}^{**}$ &   $\text{0.69 (0.22)}^*$ &      \textbf{0.9 (0.15)} &               0.81 (0.18) \\
GRU-MLP/CM &                 -42.16 (13.8) &                     57.76 (17.81) &               1.46 (0.01) &                15.6 (4.48) &              0.74 (0.23) &              0.95 (0.16) &                0.82 (0.2) \\
GRU-MLP/CM + B &                -39.27 (12.96) &                      58.1 (17.85) &               1.67 (0.03) &               18.83 (5.43) &              0.87 (0.25) &              1.07 (0.19) &               0.89 (0.25) \\
GRU-MLP/CM + BFC &                 -41.3 (13.57) &                     57.92 (17.82) &               1.59 (0.04) &               16.62 (4.76) &              0.81 (0.24) &              1.02 (0.18) &               0.88 (0.22) \\
GRU-MLP/MC &                -42.71 (14.03) &                     58.19 (17.89) &               1.63 (0.03) &               15.47 (4.38) &              0.82 (0.26) &              1.02 (0.19) &               0.94 (0.22) \\
GRU-MLP/MC + B &                -43.37 (14.17) &                     57.47 (17.74) &                1.4 (0.02) &                14.1 (4.02) &              0.71 (0.22) &              0.92 (0.15) &               0.82 (0.18) \\
GRU-MLP/MC + BFC &                 -43.4 (14.19) &                     57.62 (17.77) &               1.44 (0.02) &               14.22 (4.04) &              0.72 (0.23) &              0.94 (0.16) &               0.85 (0.19) \\
GRU-RMTPP &                -42.97 (14.04) &                     57.43 (17.72) &                1.4 (0.02) &               14.47 (4.13) &              0.71 (0.22) &              0.91 (0.16) &               0.83 (0.18) \\
GRU-RMTPP + B &                -43.25 (14.13) &       $\text{57.42 (17.72)}^{**}$ &               1.39 (0.02) &               14.17 (4.05) &               0.7 (0.22) & $\text{0.9 (0.16)}^{**}$ &               0.82 (0.18) \\
GRU-RMTPP + BFC &                -43.26 (14.13) &                     57.39 (17.72) &               1.38 (0.02) &               14.13 (4.04) & $\text{0.7 (0.22)}^{**}$ &    $\text{0.9 (0.15)}^*$ &               0.81 (0.18) \\
GRU-SA/CM &                -40.63 (13.38) &                     58.01 (17.83) &               1.66 (0.04) &               17.38 (4.97) &              0.83 (0.26) &              1.06 (0.19) &               0.88 (0.25) \\
GRU-SA/CM + B &                -41.58 (13.65) &                      57.85 (17.8) &               1.57 (0.03) &               16.28 (4.65) &              0.79 (0.25) &              1.01 (0.18) &               0.86 (0.22) \\
GRU-SA/CM + BFC &                -41.09 (13.52) &                     57.94 (17.81) &               1.64 (0.03) &               16.85 (4.81) &              0.82 (0.26) &              1.04 (0.19) &               0.89 (0.24) \\
GRU-SA/MC &                 -42.3 (13.91) &                     58.35 (17.93) &               1.66 (0.04) &               16.06 (4.56) &              0.83 (0.26) &              1.06 (0.19) & $\text{0.95 (0.23)}^{**}$ \\
GRU-SA/MC + B &                -43.02 (14.07) &                     57.57 (17.76) &               1.44 (0.02) &               14.55 (4.15) &              0.72 (0.23) &              0.94 (0.16) &               0.83 (0.19) \\
GRU-SA/MC + BFC &                -42.98 (14.07) &                     57.72 (17.79) &               1.47 (0.04) &                14.74 (4.2) &              0.74 (0.23) &              0.96 (0.16) &                0.85 (0.2) \\
SA-CP &                -39.86 (13.14) &                     57.76 (17.75) &               1.65 (0.05) &                17.9 (5.14) &              0.86 (0.25) &              1.05 (0.19) &               0.94 (0.23) \\
SA-CP + B &                -39.97 (13.17) &                     57.96 (17.81) &               1.66 (0.05) &               17.99 (5.17) &              0.86 (0.25) &              1.05 (0.19) &               0.92 (0.23) \\
SA-CP + BFC &                -39.93 (13.16) &                     57.81 (17.76) &               1.66 (0.05) &               17.88 (5.13) &              0.86 (0.25) &              1.05 (0.19) &               0.94 (0.23) \\
SA-LNM &                -42.54 (13.92) &                     57.64 (17.78) &               1.44 (0.02) &                15.1 (4.32) &              0.72 (0.23) &              0.94 (0.16) &               0.84 (0.19) \\
SA-LNM + B &       \textbf{-67.19 (23.09)} &                     58.78 (18.17) &      \textbf{1.35 (0.06)} &      \textbf{-8.41 (8.37)} &               0.7 (0.21) &               0.9 (0.15) &               0.75 (0.19) \\
SA-LNM + BFC &                -42.54 (13.92) &                     57.62 (17.77) &               1.44 (0.03) &               15.08 (4.31) &              0.72 (0.23) &              0.94 (0.16) &               0.84 (0.19) \\
SA-MLP/CM &                -38.34 (12.68) &                     58.13 (17.84) &               1.73 (0.04) &               19.79 (5.71) &              0.89 (0.27) &                1.1 (0.2) &               0.92 (0.26) \\
SA-MLP/CM + B &                -39.25 (12.96) &                     58.11 (17.85) &               1.69 (0.04) &               18.86 (5.43) &              0.87 (0.26) &              1.08 (0.19) &                0.9 (0.25) \\
SA-MLP/CM + BFC &                -38.84 (12.83) &                     58.12 (17.84) &               1.71 (0.04) &               19.27 (5.56) &              0.88 (0.26) &               1.09 (0.2) &               0.91 (0.25) \\
SA-MLP/MC &                -41.87 (13.79) &                     58.32 (17.91) &               1.69 (0.04) &               16.45 (4.67) &              0.85 (0.27) &               1.07 (0.2) &    $\text{0.96 (0.23)}^*$ \\
SA-MLP/MC + B &                 -42.47 (13.9) &                     57.52 (17.74) &               1.45 (0.03) &                15.06 (4.3) &              0.73 (0.23) &              0.95 (0.16) &               0.85 (0.19) \\
SA-MLP/MC + BFC &                -42.47 (13.91) &                     57.74 (17.79) &               1.48 (0.03) &               15.27 (4.36) &              0.75 (0.23) &              0.96 (0.16) &                0.86 (0.2) \\
SA-RMTPP &                -41.98 (13.76) &                     57.65 (17.76) &                1.5 (0.02) &               15.66 (4.48) &              0.76 (0.23) &              0.97 (0.17) &                0.87 (0.2) \\
SA-RMTPP + B &                 -42.4 (13.88) &                     57.53 (17.73) &               1.47 (0.03) &               15.13 (4.32) &              0.74 (0.23) &              0.95 (0.16) &               0.86 (0.19) \\
SA-RMTPP + BFC &                 -42.48 (13.9) &                     57.56 (17.75) &               1.45 (0.02) &               15.08 (4.31) &              0.73 (0.23) &              0.94 (0.16) &               0.84 (0.19) \\
SA-SA/CM &                -40.51 (13.33) &                     58.03 (17.84) &               1.63 (0.04) &               17.52 (5.03) &              0.82 (0.26) &              1.05 (0.18) &               0.87 (0.24) \\
SA-SA/CM + B &                 -41.5 (13.63) &                     57.87 (17.81) &               1.57 (0.02) &               16.38 (4.68) &              0.79 (0.25) &              1.01 (0.18) &               0.86 (0.23) \\
SA-SA/CM + BFC &                -41.04 (13.48) &                      57.9 (17.82) &               1.55 (0.01) &               16.86 (4.84) &              0.78 (0.24) &               1.0 (0.17) &               0.84 (0.23) \\
SA-SA/MC &                -41.39 (13.64) &                     58.35 (17.91) &               1.72 (0.04) &               16.97 (4.83) &              0.86 (0.27) &               1.09 (0.2) &      \textbf{0.98 (0.24)} \\
SA-SA/MC + B &                -41.94 (13.76) &                      57.7 (17.76) &               1.56 (0.02) &                15.77 (4.5) &              0.78 (0.25) &               1.0 (0.18) &               0.89 (0.21) \\
SA-SA/MC + BFC &                -41.92 (13.77) &                     57.76 (17.77) &               1.58 (0.02) &               15.84 (4.51) &               0.8 (0.25) &              1.02 (0.18) &               0.91 (0.21) \\
Poisson &                -37.02 (12.24) &                     58.84 (18.09) &               1.65 (0.04) &               21.82 (6.38) &              0.87 (0.25) &              1.06 (0.19) &               0.88 (0.25) \\
Hawkes &                -43.23 (14.13) &                      58.02 (17.9) &               1.42 (0.02) &               14.79 (4.23) &              0.72 (0.22) &              0.92 (0.16) &               0.84 (0.18) \\ \\
\hline 
\end{tabular}
\caption{Evaluation of the different neural TPP models on the synthetic datasets. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\label{resultsmark}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ù
\clearpage
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{ccccccccc}
\hline \\
& \multicolumn{2}{c}{\textbf{Taxi}} & \multicolumn{2}{c}{\textbf{Twitter}} & \multicolumn{2}{c}{\textbf{Reddit Subs.}} & \multicolumn{2}{c}{\textbf{PUBG}} \\ \\
                 &                          NLL &                Time Cal. &                         NLL &                Time Cal. &                            NLL &                        Time Cal. &                         NLL &                Time Cal. \\
\hline \\
          GRU-CP &               -136.39 (4.12) &    $\text{0.01 (0.0)}^*$ &                -6.22 (0.46) &               0.13 (0.0) &               -4402.72 (23.78) &                       0.01 (0.0) &               -107.0 (0.22) &               0.02 (0.0) \\
      GRU-CP + B &               -136.78 (3.91) &               0.01 (0.0) &                -6.21 (0.46) &               0.13 (0.0) &                -4403.97 (24.0) &                       0.01 (0.0) &              -106.99 (0.21) &               0.02 (0.0) \\
    GRU-CP + BFC &               -136.65 (4.01) &               0.01 (0.0) &                -6.17 (0.43) &               0.13 (0.0) &               -4403.44 (23.62) &                       0.01 (0.0) &              -106.99 (0.21) &               0.02 (0.0) \\
         GRU-LNM &               -137.02 (3.87) &               0.01 (0.0) & $\text{-12.52 (0.58)}^{**}$ &      \textbf{0.01 (0.0)} & $\text{-4496.27 (37.01)}^{**}$ &                       0.01 (0.0) &    \textbf{-194.39 (18.07)} &      \textbf{0.01 (0.0)} \\
     GRU-LNM + B &   $\text{-235.45 (12.16)}^*$ &              0.08 (0.01) &    $\text{-20.43 (1.38)}^*$ &              0.04 (0.01) &   $\text{-5691.05 (233.79)}^*$ &                      0.07 (0.01) & $\text{-174.0 (4.74)}^{**}$ &              0.06 (0.01) \\
   GRU-LNM + BFC &               -136.88 (3.92) &               0.01 (0.0) &               -12.24 (0.53) &               0.01 (0.0) &                -4439.2 (31.99) &                       0.01 (0.0) &              -146.76 (7.31) &               0.01 (0.0) \\
      GRU-MLP/CM &               -132.57 (5.16) &               0.02 (0.0) &                -3.42 (0.25) &               0.15 (0.0) &               -4268.18 (23.31) &                       0.03 (0.0) &                -98.8 (0.15) &               0.05 (0.0) \\
  GRU-MLP/CM + B &               -126.13 (3.69) &               0.04 (0.0) &                -3.48 (0.25) &               0.15 (0.0) &               -4271.73 (23.53) &                       0.03 (0.0) &                -99.0 (0.15) &               0.05 (0.0) \\
GRU-MLP/CM + BFC &                -125.83 (3.6) &               0.04 (0.0) &                -3.47 (0.25) &               0.15 (0.0) &                -4270.7 (23.52) &                       0.03 (0.0) &               -98.93 (0.16) &               0.05 (0.0) \\
      GRU-MLP/MC &               -136.98 (3.97) &               0.01 (0.0) &               -11.04 (0.54) &               0.02 (0.0) &               -4405.18 (23.94) & $\text{\textbf{0.0 (0.0)}}^{**}$ &              -107.85 (0.19) &               0.01 (0.0) \\
  GRU-MLP/MC + B &               -137.07 (4.02) &               0.01 (0.0) &               -11.19 (0.59) &               0.02 (0.0) &               -4404.68 (23.82) &             $\text{0.0 (0.0)}^*$ &               -107.76 (0.2) &               0.01 (0.0) \\
GRU-MLP/MC + BFC &               -136.87 (4.01) &       \textbf{0.0 (0.0)} &               -10.99 (0.51) &               0.02 (0.0) &               -4405.44 (23.91) &                       0.01 (0.0) &              -107.83 (0.23) &               0.01 (0.0) \\
       GRU-RMTPP &                -136.8 (3.93) &               0.01 (0.0) &                -8.07 (0.51) &               0.09 (0.0) &                -4402.27 (24.1) &                       0.01 (0.0) &              -107.71 (0.23) &               0.01 (0.0) \\
   GRU-RMTPP + B &               -136.19 (4.11) &               0.01 (0.0) &               -10.21 (0.57) &               0.05 (0.0) &               -4403.24 (24.14) &                       0.01 (0.0) &              -107.76 (0.21) &               0.01 (0.0) \\
 GRU-RMTPP + BFC &               -136.53 (4.15) &               0.01 (0.0) &               -10.22 (0.58) &               0.04 (0.0) &               -4401.26 (23.98) &                       0.01 (0.0) &              -107.73 (0.22) &               0.01 (0.0) \\
       GRU-SA/CM &               -135.07 (3.99) &               0.01 (0.0) &                -11.2 (0.49) &               0.01 (0.0) &               -4325.92 (23.95) &                       0.01 (0.0) &              -107.38 (0.21) &               0.01 (0.0) \\
   GRU-SA/CM + B &               -136.09 (4.15) &               0.01 (0.0) &               -11.46 (0.52) &               0.01 (0.0) &               -4337.55 (24.44) &                       0.01 (0.0) &              -107.43 (0.18) &               0.01 (0.0) \\
 GRU-SA/CM + BFC &               -135.35 (4.18) &               0.01 (0.0) &               -11.29 (0.51) &               0.01 (0.0) &                -4336.19 (25.8) &                       0.01 (0.0) &             -133.33 (23.17) &               0.01 (0.0) \\
       GRU-SA/MC &               -137.05 (4.03) &               0.01 (0.0) &               -11.88 (0.57) &               0.01 (0.0) &                -4404.6 (23.63) &                        0.0 (0.0) &              -123.35 (2.43) &               0.01 (0.0) \\
   GRU-SA/MC + B &               -136.97 (4.06) &               0.01 (0.0) &                -12.09 (0.5) &               0.01 (0.0) &               -4404.01 (23.36) &                        0.0 (0.0) &              -118.88 (4.27) &               0.01 (0.0) \\
 GRU-SA/MC + BFC & $\text{-137.09 (4.04)}^{**}$ &               0.01 (0.0) &               -12.15 (0.49) &               0.01 (0.0) &               -4401.33 (23.74) &                       0.01 (0.0) &              -120.79 (3.01) &               0.01 (0.0) \\
           SA-CP &               -130.86 (3.56) &               0.02 (0.0) &                -4.51 (0.38) &               0.15 (0.0) &                 -4320.8 (22.4) &                       0.02 (0.0) &              -104.13 (0.21) &               0.03 (0.0) \\
       SA-CP + B &                -131.2 (3.57) &               0.03 (0.0) &                -4.32 (0.35) &               0.16 (0.0) &                -4322.37 (23.1) &                       0.02 (0.0) &              -104.06 (0.25) &               0.03 (0.0) \\
     SA-CP + BFC &               -132.27 (3.15) &               0.02 (0.0) &                -4.42 (0.36) &               0.15 (0.0) &               -4324.59 (24.66) &                       0.02 (0.0) &              -104.11 (0.26) &               0.03 (0.0) \\
          SA-LNM &               -133.07 (3.84) & $\text{0.01 (0.0)}^{**}$ &                -11.74 (0.6) & $\text{0.01 (0.0)}^{**}$ &               -4405.48 (28.12) &                       0.01 (0.0) &              -137.63 (3.52) &               0.02 (0.0) \\
      SA-LNM + B &     \textbf{-246.92 (12.62)} &               0.09 (0.0) &      \textbf{-21.56 (1.74)} &              0.07 (0.01) &     \textbf{-6110.55 (208.28)} &                      0.06 (0.01) &   $\text{-187.75 (7.55)}^*$ &              0.07 (0.01) \\
    SA-LNM + BFC &                -132.9 (3.75) &               0.01 (0.0) &                -11.7 (0.65) &    $\text{0.01 (0.0)}^*$ &               -4357.62 (26.71) &                       0.01 (0.0) &              -131.33 (2.99) &               0.01 (0.0) \\
       SA-MLP/CM &               -125.59 (3.65) &               0.04 (0.0) &                -3.42 (0.25) &               0.15 (0.0) &               -4263.75 (23.41) &                       0.03 (0.0) &                -98.8 (0.15) &               0.05 (0.0) \\
   SA-MLP/CM + B &               -126.33 (3.62) &               0.04 (0.0) &                -3.49 (0.25) &               0.15 (0.0) &               -4268.13 (22.74) &                       0.03 (0.0) &               -98.99 (0.15) &               0.05 (0.0) \\
 SA-MLP/CM + BFC &               -125.99 (3.65) &               0.04 (0.0) &                -3.46 (0.24) &               0.15 (0.0) &               -4265.26 (22.34) &                       0.03 (0.0) &               -98.92 (0.16) &               0.05 (0.0) \\
       SA-MLP/MC &                -132.91 (3.7) &               0.01 (0.0) &               -10.51 (0.57) &               0.03 (0.0) &               -4336.75 (23.56) &                       0.01 (0.0) &              -106.57 (0.41) &               0.01 (0.0) \\
   SA-MLP/MC + B &                -133.24 (4.0) &               0.01 (0.0) &                -10.7 (0.55) &               0.02 (0.0) &               -4335.22 (23.46) &                       0.01 (0.0) &              -106.27 (0.44) &    $\text{0.01 (0.0)}^*$ \\
 SA-MLP/MC + BFC &               -132.62 (3.68) &               0.01 (0.0) &               -10.66 (0.47) &               0.02 (0.0) &               -4334.97 (23.07) &                       0.01 (0.0) &              -106.15 (0.36) & $\text{0.01 (0.0)}^{**}$ \\
        SA-RMTPP &               -132.44 (3.62) &               0.01 (0.0) &                -7.31 (0.44) &                0.1 (0.0) &               -4327.58 (23.84) &                       0.02 (0.0) &               -105.5 (0.29) &               0.01 (0.0) \\
    SA-RMTPP + B &               -132.89 (3.48) &               0.01 (0.0) &                -9.57 (0.51) &               0.05 (0.0) &                -4327.0 (24.17) &                       0.02 (0.0) &              -105.78 (0.22) &               0.01 (0.0) \\
  SA-RMTPP + BFC &                -132.19 (3.7) &               0.01 (0.0) &                 -9.7 (0.56) &               0.05 (0.0) &               -4327.22 (24.45) &                       0.02 (0.0) &              -106.09 (0.26) &               0.01 (0.0) \\
        SA-SA/CM &               -134.39 (3.97) &               0.01 (0.0) &               -10.81 (0.51) &               0.01 (0.0) &               -4327.87 (25.52) &                       0.01 (0.0) &              -107.27 (0.24) &               0.01 (0.0) \\
    SA-SA/CM + B &               -135.24 (4.13) &               0.01 (0.0) &               -10.86 (0.51) &               0.01 (0.0) &               -4326.64 (23.94) &                       0.01 (0.0) &              -114.97 (6.32) &               0.01 (0.0) \\
  SA-SA/CM + BFC &               -134.56 (4.26) &               0.01 (0.0) &               -10.92 (0.54) &               0.01 (0.0) &               -4326.39 (22.97) &                       0.01 (0.0) &             -118.45 (10.02) &               0.01 (0.0) \\
        SA-SA/MC &               -136.08 (4.11) &               0.01 (0.0) &               -11.48 (0.46) &               0.01 (0.0) &                -4360.57 (30.0) &                        0.0 (0.0) &              -119.94 (2.67) &               0.01 (0.0) \\
    SA-SA/MC + B &               -135.38 (4.34) &               0.01 (0.0) &               -11.98 (0.55) &               0.01 (0.0) &               -4359.53 (25.93) &                       0.01 (0.0) &              -116.46 (3.07) &               0.01 (0.0) \\
  SA-SA/MC + BFC &               -136.27 (4.13) &               0.01 (0.0) &               -11.05 (0.51) &               0.01 (0.0) &               -4364.59 (22.44) &                       0.01 (0.0) &              -117.23 (3.38) &               0.01 (0.0) \\
         Poisson &                -41.71 (1.02) &               0.35 (0.0) &                 5.18 (0.11) &                0.2 (0.0) &                -3706.3 (17.61) &                       0.27 (0.0) &               -93.11 (0.15) &               0.07 (0.0) \\
          Hawkes &               -134.09 (3.93) &               0.01 (0.0) &                -7.61 (0.51) &               0.01 (0.0) &                -4395.2 (23.74) &                        0.0 (0.0) &               -102.69 (0.2) &               0.01 (0.0) \\ \\
\end{tabular}
\begin{tabular}{ccccccccc}
\hline \\
 & \multicolumn{2}{c}{\textbf{Yelp Toronto}} & \multicolumn{2}{c}{\textbf{Yelp Mississauga}} & \multicolumn{2}{c}{\textbf{Reddit Comments.}} & \multicolumn{2}{c}{\textbf{Yelp Airport}} \\ \\
                 &                            NLL &                      Time Cal. &                        NLL &                Time Cal. &                           NLL &                        Time Cal. &                        NLL &                Time Cal. \\
\hline \\
          GRU-CP &               -2798.57 (85.08) &                     0.06 (0.0) &              -56.07 (0.82) &               0.05 (0.0) &               -917.77 (13.08) &                       0.02 (0.0) &               -5.73 (0.18) &               0.02 (0.0) \\
      GRU-CP + B &               -2803.23 (85.58) &                     0.05 (0.0) &              -56.18 (0.76) &               0.05 (0.0) &                -917.48 (13.1) &                       0.02 (0.0) &               -5.76 (0.18) &               0.02 (0.0) \\
    GRU-CP + BFC &               -2800.43 (84.38) &                     0.05 (0.0) &              -56.06 (0.81) &               0.05 (0.0) &               -917.76 (13.08) &                       0.02 (0.0) &               -5.64 (0.17) &               0.02 (0.0) \\
         GRU-LNM & $\text{-2957.96 (92.81)}^{**}$ & $\text{\textbf{0.01 (0.0)}}^*$ & $\text{-59.61 (0.9)}^{**}$ &      \textbf{0.01 (0.0)} &               -926.36 (12.67) & $\text{\textbf{0.0 (0.0)}}^{**}$ &                -6.8 (0.19) &      \textbf{0.01 (0.0)} \\
     GRU-LNM + B &    $\text{-3838.7 (194.65)}^*$ &                     0.08 (0.0) &    \textbf{-120.85 (9.18)} &              0.09 (0.01) &     \textbf{-1263.68 (38.98)} &                      0.06 (0.01) &     \textbf{-32.36 (3.14)} &              0.07 (0.01) \\
   GRU-LNM + BFC &                 -2949.1 (86.9) &       $\text{0.01 (0.0)}^{**}$ &              -59.41 (0.85) &               0.01 (0.0) & $\text{-927.36 (12.25)}^{**}$ &                        0.0 (0.0) &               -6.01 (0.24) &               0.01 (0.0) \\
      GRU-MLP/CM &               -2659.68 (74.25) &                    0.09 (0.01) &              -44.89 (2.28) &              0.09 (0.01) &               -814.67 (31.33) &                      0.09 (0.03) &               -3.86 (0.17) &               0.03 (0.0) \\
  GRU-MLP/CM + B &                -2667.2 (74.98) &                    0.09 (0.01) &              -42.74 (0.64) &                0.1 (0.0) &               -750.01 (12.07) &                       0.14 (0.0) &               -3.78 (0.15) &               0.04 (0.0) \\
GRU-MLP/CM + BFC &                -2661.76 (72.9) &                     0.1 (0.01) &              -42.88 (0.66) &                0.1 (0.0) &               -749.61 (12.02) &                       0.14 (0.0) &               -3.84 (0.14) &               0.04 (0.0) \\
      GRU-MLP/MC &                -2811.3 (86.33) &                     0.05 (0.0) &               -58.1 (0.83) &               0.02 (0.0) &               -922.51 (12.89) &                        0.0 (0.0) &               -6.41 (0.19) &               0.01 (0.0) \\
  GRU-MLP/MC + B &               -2810.11 (86.15) &                     0.05 (0.0) &              -58.04 (0.84) &               0.02 (0.0) &               -922.04 (13.08) &                       0.01 (0.0) &                -6.1 (0.18) &               0.01 (0.0) \\
GRU-MLP/MC + BFC &               -2810.25 (85.82) &                     0.05 (0.0) &              -57.74 (0.77) &               0.02 (0.0) &               -922.46 (12.96) &                       0.01 (0.0) &                -6.4 (0.19) &               0.01 (0.0) \\
       GRU-RMTPP &               -2808.87 (86.74) &                     0.05 (0.0) &              -57.15 (0.84) &               0.03 (0.0) &               -920.83 (13.11) &                       0.01 (0.0) &               -5.98 (0.21) &               0.01 (0.0) \\
   GRU-RMTPP + B &               -2805.92 (85.44) &                     0.05 (0.0) &              -57.43 (0.85) &               0.03 (0.0) &               -920.45 (13.11) &                       0.01 (0.0) &               -6.02 (0.19) &               0.01 (0.0) \\
 GRU-RMTPP + BFC &               -2808.54 (86.16) &                     0.05 (0.0) &              -57.58 (0.86) &               0.03 (0.0) &               -920.91 (12.87) &                       0.01 (0.0) &               -6.05 (0.18) &               0.01 (0.0) \\
       GRU-SA/CM &               -2753.47 (82.19) &                     0.05 (0.0) &              -56.13 (1.05) &               0.01 (0.0) &                -877.89 (13.0) &                       0.01 (0.0) &               -5.94 (0.17) &               0.01 (0.0) \\
   GRU-SA/CM + B &               -2764.26 (79.54) &                     0.04 (0.0) &              -56.29 (0.86) &               0.01 (0.0) &               -878.56 (11.34) &                       0.01 (0.0) &               -5.61 (0.19) &               0.01 (0.0) \\
 GRU-SA/CM + BFC &               -2762.13 (83.35) &                     0.04 (0.0) &              -55.99 (0.92) &               0.01 (0.0) &               -875.91 (12.54) &                       0.01 (0.0) &                -5.7 (0.08) &               0.01 (0.0) \\
       GRU-SA/MC &               -2803.49 (86.66) &                     0.03 (0.0) &               -58.1 (0.83) &               0.02 (0.0) &                -922.28 (13.0) &                       0.01 (0.0) &                -6.77 (0.2) &               0.01 (0.0) \\
   GRU-SA/MC + B &               -2823.58 (90.01) &                     0.03 (0.0) &              -58.77 (0.95) & $\text{0.01 (0.0)}^{**}$ &                -922.4 (12.93) &                        0.0 (0.0) & $\text{-7.09 (0.18)}^{**}$ &               0.01 (0.0) \\
 GRU-SA/MC + BFC &                -2799.78 (87.5) &                     0.03 (0.0) &              -58.43 (0.82) &               0.01 (0.0) &               -922.92 (12.92) &             $\text{0.0 (0.0)}^*$ &               -7.02 (0.21) &               0.01 (0.0) \\
           SA-CP &               -2753.86 (81.24) &                     0.07 (0.0) &              -52.64 (1.07) &               0.06 (0.0) &               -875.97 (12.56) &                       0.06 (0.0) &               -4.77 (0.15) &               0.03 (0.0) \\
       SA-CP + B &               -2757.95 (82.11) &                     0.07 (0.0) &              -52.64 (0.96) &               0.06 (0.0) &               -875.52 (12.84) &                       0.06 (0.0) &                -4.8 (0.17) &               0.03 (0.0) \\
     SA-CP + BFC &               -2757.09 (81.64) &                     0.07 (0.0) &              -53.41 (0.94) &               0.06 (0.0) &                -875.5 (12.88) &                       0.06 (0.0) &               -4.72 (0.19) &               0.03 (0.0) \\
          SA-LNM &               -2925.35 (91.31) &                     0.01 (0.0) &              -57.65 (0.79) &               0.01 (0.0) &               -900.73 (12.41) &                        0.0 (0.0) &               -5.71 (0.16) &               0.01 (0.0) \\
      SA-LNM + B &      \textbf{-3979.6 (200.76)} &                     0.07 (0.0) &  $\text{-109.67 (4.99)}^*$ &              0.08 (0.01) &   $\text{-1225.99 (48.22)}^*$ &                       0.04 (0.0) &   $\text{-28.05 (1.33)}^*$ &              0.08 (0.01) \\
    SA-LNM + BFC &               -2918.12 (90.38) &                     0.01 (0.0) &              -57.42 (0.81) &               0.01 (0.0) &               -899.94 (12.65) &                        0.0 (0.0) &                -5.7 (0.19) &    $\text{0.01 (0.0)}^*$ \\
       SA-MLP/CM &                -2659.22 (73.5) &                     0.1 (0.01) &               -42.34 (0.7) &                0.1 (0.0) &               -747.37 (12.11) &                       0.14 (0.0) &               -3.77 (0.14) &               0.03 (0.0) \\
   SA-MLP/CM + B &               -2666.42 (74.33) &                    0.09 (0.01) &              -42.53 (0.72) &                0.1 (0.0) &               -748.36 (12.06) &                       0.14 (0.0) &               -3.78 (0.16) &               0.04 (0.0) \\
 SA-MLP/CM + BFC &               -2664.26 (73.94) &                     0.1 (0.01) &              -42.43 (0.68) &                0.1 (0.0) &               -748.29 (12.03) &                       0.14 (0.0) &               -3.76 (0.14) &               0.04 (0.0) \\
       SA-MLP/MC &               -2771.19 (85.52) &                     0.06 (0.0) &              -56.24 (0.91) &               0.02 (0.0) &                -896.0 (12.95) &                       0.02 (0.0) &                -5.68 (0.2) &               0.01 (0.0) \\
   SA-MLP/MC + B &               -2772.73 (84.92) &                     0.06 (0.0) &              -56.01 (0.94) &               0.02 (0.0) &               -895.08 (13.06) &                       0.02 (0.0) &                -5.4 (0.17) &               0.01 (0.0) \\
 SA-MLP/MC + BFC &               -2774.25 (84.54) &                     0.06 (0.0) &              -56.11 (0.75) &               0.02 (0.0) &               -895.41 (12.65) &                       0.01 (0.0) &               -5.57 (0.18) & $\text{0.01 (0.0)}^{**}$ \\
        SA-RMTPP &               -2764.26 (84.29) &                     0.06 (0.0) &              -55.01 (0.87) &               0.04 (0.0) &               -887.29 (12.73) &                       0.04 (0.0) &                 -5.3 (0.2) &               0.01 (0.0) \\
    SA-RMTPP + B &               -2765.01 (84.07) &                     0.06 (0.0) &               -55.3 (0.85) &               0.04 (0.0) &                -888.0 (13.15) &                       0.04 (0.0) &                -5.3 (0.17) &               0.01 (0.0) \\
  SA-RMTPP + BFC &               -2764.91 (83.86) &                     0.06 (0.0) &              -55.28 (1.01) &               0.04 (0.0) &               -890.57 (12.91) &                       0.03 (0.0) &               -5.36 (0.17) &               0.01 (0.0) \\
        SA-SA/CM &               -2740.69 (85.18) &                    0.05 (0.01) &              -55.91 (0.92) &               0.02 (0.0) &               -875.99 (14.49) &                       0.01 (0.0) &               -5.33 (0.18) &               0.01 (0.0) \\
    SA-SA/CM + B &               -2753.44 (80.25) &                     0.03 (0.0) &              -55.66 (0.91) &               0.01 (0.0) &               -868.23 (12.43) &                       0.01 (0.0) &               -5.49 (0.15) &               0.01 (0.0) \\
  SA-SA/CM + BFC &                -2752.3 (84.25) &                     0.04 (0.0) &               -55.64 (1.0) &               0.02 (0.0) &               -865.98 (10.76) &                       0.01 (0.0) &               -5.51 (0.19) &               0.01 (0.0) \\
        SA-SA/MC &               -2768.85 (76.57) &                     0.04 (0.0) &               -57.0 (0.81) &               0.01 (0.0) &               -913.99 (12.95) &                        0.0 (0.0) &               -6.15 (0.22) &               0.01 (0.0) \\
    SA-SA/MC + B &               -2772.71 (86.17) &                     0.04 (0.0) &              -57.76 (1.02) &               0.02 (0.0) &               -914.58 (12.76) &                       0.01 (0.0) &               -6.25 (0.26) &               0.01 (0.0) \\
  SA-SA/MC + BFC &               -2781.36 (82.82) &                     0.04 (0.0) &               -57.5 (0.74) &    $\text{0.01 (0.0)}^*$ &                -914.7 (12.84) &                       0.01 (0.0) &               -6.46 (0.16) &               0.01 (0.0) \\
         Poisson &                -673.76 (17.22) &                     0.47 (0.0) &               -25.2 (0.29) &               0.27 (0.0) &                -676.53 (10.2) &                       0.25 (0.0) &                -2.11 (0.1) &               0.12 (0.0) \\
          Hawkes &                -2773.63 (87.1) &                     0.06 (0.0) &               -53.33 (0.8) &               0.05 (0.0) &               -919.51 (12.92) &                       0.01 (0.0) &               -4.62 (0.18) &               0.02 (0.0) \\ \\
\hline
\end{tabular}
\caption{Evaluation of the different neural TPP models on the unmarked datasets. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\label{resultsmark}
\end{table}



\restoregeometry

==> results_tabular_dataset.tex <==
\newgeometry{left=1cm,bottom=2cm,right=1cm, top=0.5cm}


\begin{table}[t]
\tiny
\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
                models & \multicolumn{12}{c}{NLL Time} \\
                       & \multicolumn{2}{c}{lastfm_filtered} & \multicolumn{2}{c}{mooc_filtered} & \multicolumn{2}{c}{wikipedia_filtered} & \multicolumn{2}{c}{github_filtered} & \multicolumn{2}{c}{mimic2_filtered} & \multicolumn{2}{c}{hawkes_exponential_mutual} \\
                       &               R &              Val &             R &            Val &                  R &             Val &               R &             Val &               R &           Val &                         R &           Val \\
\midrule
         GRU-MLP/MC-TO &               7 & -1138.03 (59.22) &            14 &  -66.15 (13.9) &                 14 &  -17.11 (17.96) &               3 & -283.47 (58.31) &              11 &  67.41 (4.11) &                         3 &  -77.98 (0.8) \\
        GRU-MLP/MC-LTO &               1 &  -1322.9 (61.14) &             7 & -120.92 (2.44) &                  8 &  -48.02 (28.18) &               1 & -355.63 (61.39) &              17 &  67.42 (4.11) &                         5 & -77.93 (0.81) \\
     GRU-MLP/MC-CONCAT &              12 & -1108.35 (49.76) &            11 &  -75.71 (4.94) &                 18 &   -16.1 (18.56) &               5 & -279.84 (56.01) &              14 &  67.41 (4.11) &                         6 & -77.92 (0.78) \\
    GRU-MLP/MC-LCONCAT &               8 & -1127.77 (50.38) &            10 &  -83.04 (3.51) &                 10 &  -18.54 (17.81) &               4 &  -281.12 (58.1) &               7 &   67.4 (4.11) &                         7 & -77.91 (0.79) \\
        GRU-MLP/MC-TEM &              15 & -1052.69 (62.83) &            21 &  -19.26 (3.75) &                 21 &   -6.47 (20.35) &              11 & -257.25 (52.66) &              12 &  67.41 (4.12) &                         9 & -77.76 (0.75) \\
      GRU-MLP/MC-TEMWL &              16 & -1052.69 (62.83) &            22 &  -19.26 (3.75) &                 22 &   -6.47 (20.35) &              10 & -257.25 (52.66) &              16 &  67.41 (4.12) &                        10 & -77.76 (0.75) \\
         GRU-MLP/MC-LE &               3 & -1182.67 (35.92) &            13 & -72.13 (12.13) &                 15 &  -17.07 (12.71) &               8 &  -266.5 (34.75) &              20 &  67.42 (2.91) &                         4 & -77.94 (0.56) \\
       GRU-MLP/MC-LEWL &               5 & -1164.44 (52.43) &            16 & -65.58 (16.21) &                 16 &  -17.03 (18.01) &               9 & -265.11 (51.92) &              13 &  67.41 (4.11) &                         8 & -77.89 (0.78) \\
          SA-MLP/MC-TO &               4 & -1178.14 (43.54) &            18 & -52.09 (11.81) &                 13 &  -17.12 (17.96) &              20 & -221.57 (36.55) &              19 &  67.42 (4.11) &                        20 & -74.37 (0.72) \\
         SA-MLP/MC-LTO &               2 & -1264.55 (59.31) &             8 & -115.43 (3.23) &                  7 &  -56.35 (24.67) &               2 & -320.43 (59.49) &              18 &  67.42 (4.11) &                        19 & -74.41 (0.71) \\
      SA-MLP/MC-CONCAT &              11 &  -1112.5 (50.01) &            12 &  -73.22 (5.16) &                 17 &  -16.74 (18.42) &              14 & -256.69 (48.39) &              15 &  67.41 (4.11) &                        13 &  -77.0 (0.73) \\
     SA-MLP/MC-LCONCAT &              10 &  -1114.3 (50.96) &             9 & -103.12 (1.46) &                 11 &  -18.52 (18.77) &              16 & -251.21 (45.72) &              10 &   67.4 (4.11) &                        14 & -76.94 (0.72) \\
         SA-MLP/MC-TEM &              19 & -1002.13 (46.68) &            19 &  -21.86 (5.96) &                 19 &   -11.48 (19.9) &              18 & -245.26 (49.72) &               9 &   67.4 (4.11) &                        17 & -76.66 (0.69) \\
       SA-MLP/MC-TEMWL &              20 & -1002.13 (46.68) &            20 &  -21.86 (5.96) &                 20 &   -11.48 (19.9) &              19 & -245.26 (49.72) &               8 &   67.4 (4.11) &                        18 & -76.66 (0.69) \\
          SA-MLP/MC-LE &               6 & -1161.42 (44.61) &            17 &  -64.26 (12.5) &                 12 &  -17.83 (12.37) &              15 & -256.36 (33.29) &              21 &  67.43 (2.91) &                        16 &  -76.77 (0.5) \\
        SA-MLP/MC-LEWL &               9 &  -1125.35 (54.3) &            15 & -66.14 (11.98) &                  9 &  -18.58 (17.01) &              17 & -250.87 (45.03) &              22 &  67.44 (4.12) &                        15 &  -76.78 (0.7) \\
           C-MLP/MC-TO &              23 &  -903.48 (37.15) &            24 &  128.87 (0.88) &                 24 &  123.87 (19.07) &              22 & -188.51 (43.29) &              24 & 117.28 (5.02) &                        22 & -73.82 (0.71) \\
           C-MLP/MC-TO &              24 &  -903.48 (37.15) &            23 &  128.87 (0.88) &                 23 &  123.87 (19.07) &              21 & -188.51 (43.29) &              23 & 117.28 (5.02) &                        21 & -73.82 (0.71) \\
     GRU-MLP/MC-TO + B &              27 &        nan (nan) &            32 &      nan (nan) &                 32 &       nan (nan) &              27 &       nan (nan) &              29 &     nan (nan) &                        27 &     nan (nan) \\
    GRU-MLP/MC-LTO + B &              26 &        nan (nan) &            26 &      nan (nan) &                 26 &       nan (nan) &              26 &       nan (nan) &              34 &     nan (nan) &                        26 &     nan (nan) \\
 GRU-MLP/MC-CONCAT + B &              36 &        nan (nan) &            25 &      nan (nan) &                 25 &       nan (nan) &              36 &       nan (nan) &              33 &     nan (nan) &                        36 &     nan (nan) \\
GRU-MLP/MC-LCONCAT + B &              25 &        nan (nan) &            35 &      nan (nan) &                 35 &       nan (nan) &              25 &       nan (nan) &              32 &     nan (nan) &                        25 &     nan (nan) \\
    GRU-MLP/MC-TEM + B &              14 &  -1093.16 (59.2) &             4 & -217.47 (4.61) &                  4 & -121.89 (12.23) &               7 & -271.35 (50.62) &               2 &   1.65 (0.09) &                         1 & -78.54 (0.76) \\
         GRU-TEMWL + B &              13 &  -1093.16 (59.2) &             3 & -217.47 (4.61) &                  3 & -121.89 (12.23) &               6 & -271.35 (50.62) &               1 &   1.65 (0.09) &                         2 & -78.54 (0.76) \\
     GRU-MLP/MC-LE + B &              28 &        nan (nan) &            36 &      nan (nan) &                 36 &       nan (nan) &              28 &       nan (nan) &              31 &     nan (nan) &                        28 &     nan (nan) \\
   GRU-MLP/MC-LEWL + B &              29 &        nan (nan) &            27 &      nan (nan) &                 27 &       nan (nan) &              29 &       nan (nan) &              30 &     nan (nan) &                        29 &     nan (nan) \\
      SA-MLP/MC-TO + B &              30 &        nan (nan) &            28 &      nan (nan) &                 28 &       nan (nan) &              30 &       nan (nan) &              36 &     nan (nan) &                        30 &     nan (nan) \\
     SA-MLP/MC-LTO + B &              31 &        nan (nan) &            29 &      nan (nan) &                 29 &       nan (nan) &              31 &       nan (nan) &              35 &     nan (nan) &                        31 &     nan (nan) \\
  SA-MLP/MC-CONCAT + B &              32 &        nan (nan) &            30 &      nan (nan) &                 30 &       nan (nan) &              32 &       nan (nan) &              28 &     nan (nan) &                        32 &     nan (nan) \\
 SA-MLP/MC-LCONCAT + B &              33 &        nan (nan) &            31 &      nan (nan) &                 31 &       nan (nan) &              33 &       nan (nan) &              27 &     nan (nan) &                        33 &     nan (nan) \\
     SA-MLP/MC-TEM + B &              18 & -1006.77 (53.09) &             2 & -218.45 (3.98) &                  2 & -123.24 (19.59) &              13 & -256.98 (46.33) &               4 &   2.13 (0.22) &                        11 & -77.35 (0.75) \\
   SA-MLP/MC-TEMWL + B &              17 & -1006.77 (53.09) &             1 & -218.45 (3.98) &                  1 & -123.24 (19.59) &              12 & -256.98 (46.33) &               3 &   2.13 (0.22) &                        12 & -77.35 (0.75) \\
      SA-MLP/MC-LE + B &              34 &        nan (nan) &            33 &      nan (nan) &                 33 &       nan (nan) &              34 &       nan (nan) &              26 &     nan (nan) &                        34 &     nan (nan) \\
    SA-MLP/MC-LEWL + B &              35 &        nan (nan) &            34 &      nan (nan) &                 34 &       nan (nan) &              35 &       nan (nan) &              25 &     nan (nan) &                        35 &     nan (nan) \\
       C-MLP/MC-TO + B &              22 &  -973.55 (37.06) &             6 & -208.18 (3.43) &                  6 & -107.56 (13.84) &              23 & -149.08 (28.22) &               6 &   3.01 (0.13) &                        23 &  -71.6 (0.71) \\
    C-MLP/MC-TEMWL + B &              21 &  -973.55 (37.06) &             5 & -208.18 (3.43) &                  5 & -107.56 (13.84) &              24 & -149.08 (28.22) &               5 &   3.01 (0.13) &                        24 &  -71.6 (0.71) \\
\bottomrule
\end{tabular}



\label{resultsmark}
%\caption{Evaluation of the different neural TPP models on MOOC and LastFM. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}


\begin{table}[t]
\tiny
\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
                models & \multicolumn{12}{c}{NLL Time} \\
                       & \multicolumn{2}{c}{lastfm_filtered} & \multicolumn{2}{c}{mooc_filtered} & \multicolumn{2}{c}{wikipedia_filtered} & \multicolumn{2}{c}{github_filtered} & \multicolumn{2}{c}{mimic2_filtered} & \multicolumn{2}{c}{hawkes_exponential_mutual} \\
                       &               R &       Val &             R &       Val &                  R &       Val &               R &       Val &               R &       Val &                         R &       Val \\
\midrule
         GRU-MLP/MC-TO &               7 & -0.513393 &            14 &  0.212795 &                 14 &  0.236025 &               3 & -0.713008 &              14 &  0.362139 &                         3 & -0.747663 \\
        GRU-MLP/MC-LTO &               1 & -2.337395 &             7 & -0.366330 &                  8 & -0.247770 &               1 & -2.301003 &              20 &  0.362663 &                         5 & -0.725976 \\
     GRU-MLP/MC-CONCAT &              12 & -0.220542 &            11 &  0.111704 &                 18 &  0.251849 &               5 & -0.633157 &              16 &  0.362276 &                         6 & -0.720028 \\
    GRU-MLP/MC-LCONCAT &               8 & -0.412171 &            10 &  0.034168 &                 10 &  0.213691 &               4 & -0.661325 &              10 &  0.362038 &                         7 & -0.714645 \\
        GRU-MLP/MC-TEM &              15 &  0.328628 &            21 &  0.708543 &                 21 &  0.402605 &              11 & -0.136035 &              11 &  0.362075 &                         9 & -0.641251 \\
      GRU-MLP/MC-TEMWL &              16 &  0.328628 &            22 &  0.708543 &                 22 &  0.402605 &              10 & -0.136035 &              12 &  0.362075 &                        10 & -0.641251 \\
         GRU-MLP/MC-LE &               3 & -0.953796 &            13 &  0.149472 &                 15 &  0.236726 &               8 & -0.339567 &              19 &  0.362630 &                         4 & -0.731512 \\
       GRU-MLP/MC-LEWL &               5 & -0.773893 &            16 &  0.218729 &                 16 &  0.237244 &               9 & -0.308914 &              15 &  0.362236 &                         8 & -0.705854 \\
          SA-MLP/MC-TO &               4 & -0.909083 &            18 &  0.361455 &                 13 &  0.235920 &              20 &  0.649261 &              17 &  0.362543 &                        20 &  1.045881 \\
         SA-MLP/MC-LTO &               2 & -1.761646 &             8 & -0.308358 &                  7 & -0.378184 &               2 & -1.526482 &              18 &  0.362609 &                        19 &  1.022842 \\
      SA-MLP/MC-CONCAT &              11 & -0.261483 &            12 &  0.138004 &                 17 &  0.241901 &              14 & -0.123647 &              13 &  0.362094 &                        13 & -0.263531 \\
     SA-MLP/MC-LCONCAT &              10 & -0.279215 &             9 & -0.178208 &                 11 &  0.213919 &              16 & -0.003188 &               7 &  0.361888 &                        14 & -0.234374 \\
         SA-MLP/MC-TEM &              19 &  0.827462 &            19 &  0.681030 &                 19 &  0.324179 &              18 &  0.127740 &               9 &  0.361910 &                        17 & -0.091284 \\
       SA-MLP/MC-TEMWL &              20 &  0.827462 &            20 &  0.681030 &                 20 &  0.324179 &              19 &  0.127740 &               8 &  0.361910 &                        18 & -0.091284 \\
          SA-MLP/MC-LE &               6 & -0.744133 &            17 &  0.232725 &                 12 &  0.224786 &              15 & -0.116411 &              21 &  0.362793 &                        16 & -0.150055 \\
        SA-MLP/MC-LEWL &               9 & -0.388210 &            15 &  0.212860 &                  9 &  0.213105 &              17 &  0.004291 &              22 &  0.363068 &                        15 & -0.152178 \\
           C-MLP/MC-TO &              23 &  1.800827 &            24 &  2.274861 &                 24 &  2.443054 &              22 &  1.376687 &              24 &  1.851530 &                        22 &  1.315714 \\
           C-MLP/MC-TO &              24 &  1.800827 &            23 &  2.274861 &                 23 &  2.443054 &              21 &  1.376687 &              23 &  1.851530 &                        21 &  1.315714 \\
     GRU-MLP/MC-TO + B &              27 &       NaN &            32 &       NaN &                 32 &       NaN &              27 &       NaN &              32 &       NaN &                        27 &       NaN \\
    GRU-MLP/MC-LTO + B &              26 &       NaN &            26 &       NaN &                 26 &       NaN &              26 &       NaN &              26 &       NaN &                        26 &       NaN \\
 GRU-MLP/MC-CONCAT + B &              36 &       NaN &            25 &       NaN &                 25 &       NaN &              36 &       NaN &              25 &       NaN &                        36 &       NaN \\
GRU-MLP/MC-LCONCAT + B &              25 &       NaN &            35 &       NaN &                 35 &       NaN &              25 &       NaN &              35 &       NaN &                        25 &       NaN \\
    GRU-MLP/MC-TEM + B &              14 & -0.070607 &             4 & -1.387261 &                  4 & -1.404254 &               7 & -0.446235 &               2 & -1.601600 &                         1 & -1.029828 \\
         GRU-TEMWL + B &              13 & -0.070607 &             3 & -1.387261 &                  3 & -1.404254 &               6 & -0.446235 &               1 & -1.601600 &                         2 & -1.029828 \\
     GRU-MLP/MC-LE + B &              28 &       NaN &            36 &       NaN &                 36 &       NaN &              28 &       NaN &              36 &       NaN &                        28 &       NaN \\
   GRU-MLP/MC-LEWL + B &              29 &       NaN &            27 &       NaN &                 27 &       NaN &              29 &       NaN &              27 &       NaN &                        29 &       NaN \\
      SA-MLP/MC-TO + B &              30 &       NaN &            28 &       NaN &                 28 &       NaN &              30 &       NaN &              28 &       NaN &                        30 &       NaN \\
     SA-MLP/MC-LTO + B &              31 &       NaN &            29 &       NaN &                 29 &       NaN &              31 &       NaN &              29 &       NaN &                        31 &       NaN \\
  SA-MLP/MC-CONCAT + B &              32 &       NaN &            30 &       NaN &                 30 &       NaN &              32 &       NaN &              30 &       NaN &                        32 &       NaN \\
 SA-MLP/MC-LCONCAT + B &              33 &       NaN &            31 &       NaN &                 31 &       NaN &              33 &       NaN &              31 &       NaN &                        33 &       NaN \\
     SA-MLP/MC-TEM + B &              18 &  0.781719 &             2 & -1.397607 &                  2 & -1.425398 &              13 & -0.130044 &               4 & -1.587323 &                        11 & -0.437259 \\
   SA-MLP/MC-TEMWL + B &              17 &  0.781719 &             1 & -1.397607 &                  1 & -1.425398 &              12 & -0.130044 &               3 & -1.587323 &                        12 & -0.437259 \\
      SA-MLP/MC-LE + B &              34 &       NaN &            33 &       NaN &                 33 &       NaN &              34 &       NaN &              33 &       NaN &                        34 &       NaN \\
    SA-MLP/MC-LEWL + B &              35 &       NaN &            34 &       NaN &                 34 &       NaN &              35 &       NaN &              34 &       NaN &                        35 &       NaN \\
       C-MLP/MC-TO + B &              22 &  1.109453 &             6 & -1.289074 &                  6 & -1.179792 &              23 &  2.244463 &               6 & -1.561081 &                        23 &  2.422455 \\
    C-MLP/MC-TEMWL + B &              21 &  1.109453 &             5 & -1.289074 &                  5 & -1.179792 &              24 &  2.244463 &               5 & -1.561081 &                        24 &  2.422455 \\
\bottomrule
\end{tabular}




\label{resultsmark}
%\caption{Evaluation of the different neural TPP models on MOOC and LastFM. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
\begin{table}[t]
\tiny
\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccc|cc|cc|cc|cc|cc|cc|cc}
\hline \\
 & \multicolumn{16}{c}{Time Calibration} \\ \\
                   & \multicolumn{2}{c}{LastFM} & \multicolumn{2}{c}{MOOC} & \multicolumn{2}{c}{Wiki.} & \multicolumn{2}{c}{Github} & \multicolumn{2}{c}{MIMIC2} & \multicolumn{2}{c}{Hawkes Exp.} & \multicolumn{2}{c}{Hawkes Sum. Exp.} & \multicolumn{2}{c}{Taxi} \\ \\
                   &               R &         Val &             R &         Val &                  R &         Val &               R &         Val &               R &         Val &                         R &         Val &                             R &         Val &    R &         Val \\ \\
\hline \\
        GRU-CP-TEM &              40 & 0.28 (0.01) &            48 &  0.39 (0.0) &                 52 & 0.37 (0.01) &              37 &  0.2 (0.01) &               9 &  0.03 (0.0) &                        36 &  0.02 (0.0) &                            46 &  0.06 (0.0) &    1 &  0.01 (0.0) \\
    GRU-CP-TEM + B &              38 & 0.28 (0.01) &            46 &  0.39 (0.0) &                 49 & 0.35 (0.01) &              34 &  0.2 (0.01) &              22 & 0.05 (0.01) &                        39 &  0.02 (0.0) &                            39 &  0.05 (0.0) &   26 &  0.01 (0.0) \\
         GRU-CP-TO &              37 &  0.27 (0.0) &            44 &  0.37 (0.0) &                 43 &  0.34 (0.0) &              29 & 0.18 (0.01) &              37 & 0.09 (0.01) &                        40 &  0.02 (0.0) &                            43 &  0.06 (0.0) &   27 &  0.01 (0.0) \\
         SA-CP-TEM &              42 &  0.3 (0.01) &            47 &  0.39 (0.0) &                 51 & 0.37 (0.01) &              40 & 0.21 (0.02) &              29 &  0.07 (0.0) &                        42 &  0.03 (0.0) &                            44 &  0.06 (0.0) &   32 &  0.02 (0.0) \\
     SA-CP-TEM + B &              41 &   0.3 (0.0) &            51 &   0.4 (0.0) &                 48 & 0.35 (0.01) &              35 &  0.2 (0.01) &              28 & 0.07 (0.01) &                        43 &  0.03 (0.0) &                            45 &  0.06 (0.0) &   39 &  0.03 (0.0) \\
          SA-CP-TO &              51 & 0.35 (0.01) &            49 &   0.4 (0.0) &                 46 & 0.35 (0.01) &              50 &  0.3 (0.02) &              25 &  0.06 (0.0) &                        51 &  0.04 (0.0) &                            51 &  0.08 (0.0) &   40 &  0.04 (0.0) \\
         C-CP-TEMP &              50 & 0.35 (0.01) &            52 &   0.4 (0.0) &                 50 & 0.36 (0.01) &              51 & 0.31 (0.02) &              26 &  0.07 (0.0) &                        50 &  0.04 (0.0) &                            52 &  0.08 (0.0) &   48 &  0.05 (0.0) \\
       GRU-LNM-TEM &               5 &  0.03 (0.0) &             2 &   0.0 (0.0) &                 11 & 0.09 (0.05) &               4 & 0.03 (0.01) &              11 &  0.03 (0.0) &                         2 &   0.0 (0.0) &                             3 &   0.0 (0.0) &   25 &  0.01 (0.0) \\
   GRU-LNM-TEM + B &               8 & 0.05 (0.01) &             3 &   0.0 (0.0) &                  5 & 0.04 (0.01) &               8 & 0.05 (0.01) &              35 & 0.08 (0.03) &                        48 & 0.03 (0.01) &                            41 & 0.05 (0.01) &   50 & 0.08 (0.01) \\
        GRU-LNM-TO &               1 &  0.01 (0.0) &             4 &   0.0 (0.0) &                  8 & 0.08 (0.05) &               1 & 0.02 (0.01) &               1 &  0.02 (0.0) &                         3 &   0.0 (0.0) &                             4 &   0.0 (0.0) &   28 &  0.01 (0.0) \\
        GRU-LNM-K1 &              11 & 0.06 (0.01) &            10 &  0.04 (0.0) &                 22 & 0.21 (0.06) &               5 &  0.04 (0.0) &              13 & 0.04 (0.01) &                        49 &  0.03 (0.0) &                            34 &  0.02 (0.0) &   44 &  0.04 (0.0) \\
        SA-LNM-TEM &               6 &  0.03 (0.0) &             5 &   0.0 (0.0) &                  1 &  0.02 (0.0) &               3 &  0.03 (0.0) &               5 &  0.02 (0.0) &                         4 &   0.0 (0.0) &                            17 &  0.01 (0.0) &   29 &  0.01 (0.0) \\
    SA-LNM-TEM + B &               9 & 0.05 (0.01) &             1 &   0.0 (0.0) &                  3 &  0.03 (0.0) &              10 & 0.06 (0.01) &              15 &  0.04 (0.0) &                        45 & 0.03 (0.01) &                            37 &  0.04 (0.0) &   52 &  0.09 (0.0) \\
         SA-LNM-TO &               4 &  0.02 (0.0) &             7 &  0.01 (0.0) &                  4 & 0.04 (0.01) &               9 & 0.05 (0.01) &               4 &  0.02 (0.0) &                        32 &  0.01 (0.0) &                            24 &  0.01 (0.0) &   31 &  0.01 (0.0) \\
         SA-LNM-K1 &              10 & 0.06 (0.01) &             8 &  0.04 (0.0) &                 21 & 0.21 (0.06) &               6 & 0.04 (0.01) &               3 &  0.02 (0.0) &                        46 &  0.03 (0.0) &                            32 &  0.02 (0.0) &   38 &  0.03 (0.0) \\
        C-LNM-TEMP &               3 &  0.02 (0.0) &             6 &  0.01 (0.0) &                  2 & 0.03 (0.01) &               7 & 0.05 (0.01) &               2 &  0.02 (0.0) &                         7 &   0.0 (0.0) &                             5 &   0.0 (0.0) &   30 &  0.01 (0.0) \\
     GRU-MLP/CM-LE &              26 & 0.23 (0.01) &            14 &  0.05 (0.0) &                 18 &   0.2 (0.0) &              33 & 0.19 (0.02) &              27 & 0.07 (0.01) &                        30 &  0.01 (0.0) &                            33 &  0.02 (0.0) &   33 &  0.02 (0.0) \\
 GRU-MLP/CM-LE + B &              44 &  0.32 (0.0) &            45 &  0.38 (0.0) &                 39 & 0.32 (0.01) &              38 & 0.21 (0.02) &              23 & 0.05 (0.01) &                        47 &  0.03 (0.0) &                            48 &  0.06 (0.0) &   41 &  0.04 (0.0) \\
     GRU-MLP/CM-TO &              25 & 0.22 (0.01) &            21 & 0.15 (0.02) &                 16 &  0.19 (0.0) &              31 & 0.19 (0.01) &              24 &  0.06 (0.0) &                        31 &  0.01 (0.0) &                            36 &  0.04 (0.0) &   51 & 0.09 (0.01) \\
      SA-MLP/CM-LE &              47 & 0.32 (0.01) &            22 & 0.17 (0.02) &                 13 & 0.18 (0.01) &              47 & 0.26 (0.02) &              38 &  0.1 (0.01) &                        38 &  0.02 (0.0) &                            42 &  0.05 (0.0) &   46 &  0.04 (0.0) \\
  SA-MLP/CM-LE + B &              48 & 0.33 (0.01) &            34 & 0.31 (0.04) &                 38 & 0.31 (0.01) &              49 & 0.28 (0.02) &              36 & 0.08 (0.01) &                        37 &  0.02 (0.0) &                            47 &  0.06 (0.0) &   47 &  0.04 (0.0) \\
      SA-MLP/CM-TO &              46 & 0.32 (0.01) &            24 &  0.21 (0.0) &                 14 &  0.19 (0.0) &              46 & 0.26 (0.02) &              40 & 0.11 (0.01) &                        44 &  0.03 (0.0) &                            49 &  0.07 (0.0) &   49 &  0.07 (0.0) \\
       C-MLP/CM-LE &              49 & 0.33 (0.01) &            15 &  0.09 (0.0) &                 15 &  0.19 (0.0) &              48 & 0.27 (0.02) &              39 & 0.11 (0.01) &                        35 &  0.01 (0.0) &                            31 & 0.02 (0.01) &   42 &  0.04 (0.0) \\
    GRU-MLP/MC-TEM &              28 &  0.24 (0.0) &            38 & 0.32 (0.01) &                 31 & 0.28 (0.01) &              30 & 0.18 (0.01) &              49 &  0.48 (0.0) &                        33 &  0.01 (0.0) &                            10 &  0.01 (0.0) &   22 &  0.01 (0.0) \\
GRU-MLP/MC-TEM + B &              31 & 0.25 (0.01) &            29 & 0.24 (0.01) &                 42 & 0.33 (0.01) &              32 & 0.19 (0.01) &              32 & 0.07 (0.01) &                        34 &  0.01 (0.0) &                             9 &  0.01 (0.0) &   21 &  0.01 (0.0) \\
     GRU-MLP/MC-TO &              23 &  0.21 (0.0) &            25 & 0.22 (0.04) &                 34 & 0.29 (0.01) &              20 & 0.14 (0.01) &              46 &  0.48 (0.0) &                        29 &  0.01 (0.0) &                             8 &  0.01 (0.0) &    2 &  0.01 (0.0) \\
     SA-MLP/MC-TEM &              30 & 0.25 (0.01) &            35 & 0.32 (0.01) &                 30 & 0.28 (0.01) &              28 & 0.18 (0.01) &              53 &  0.48 (0.0) &                        28 &  0.01 (0.0) &                             6 &  0.01 (0.0) &   23 &  0.01 (0.0) \\
 SA-MLP/MC-TEM + B &              33 & 0.26 (0.01) &            27 &  0.24 (0.0) &                 47 &  0.35 (0.0) &              36 &  0.2 (0.01) &              18 & 0.04 (0.01) &                        27 &  0.01 (0.0) &                            14 &  0.01 (0.0) &    3 &  0.01 (0.0) \\
      SA-MLP/MC-TO &              14 & 0.13 (0.02) &            30 & 0.26 (0.03) &                 33 & 0.29 (0.01) &              41 & 0.21 (0.03) &              44 &  0.48 (0.0) &                        17 &  0.01 (0.0) &                            25 &  0.01 (0.0) &   37 &  0.03 (0.0) \\
     C-MLP/MC-TEMP &              39 & 0.28 (0.01) &            41 &  0.35 (0.0) &                 29 & 0.28 (0.01) &              42 & 0.23 (0.02) &              42 &  0.48 (0.0) &                         8 &  0.01 (0.0) &                             7 &  0.01 (0.0) &   36 &  0.03 (0.0) \\
     GRU-RMTPP-TEM &              32 & 0.26 (0.01) &            37 &  0.32 (0.0) &                 35 &  0.3 (0.01) &              27 & 0.18 (0.01) &              12 & 0.04 (0.01) &                         9 &  0.01 (0.0) &                            29 &  0.02 (0.0) &    4 &  0.01 (0.0) \\
 GRU-RMTPP-TEM + B &              29 &  0.25 (0.0) &            31 & 0.27 (0.01) &                 40 & 0.32 (0.01) &              25 & 0.18 (0.01) &               6 &  0.03 (0.0) &                        10 &  0.01 (0.0) &                            11 &  0.01 (0.0) &    5 &  0.01 (0.0) \\
      GRU-RMTPP-TO &              27 &  0.23 (0.0) &            36 &  0.32 (0.0) &                 37 & 0.31 (0.01) &              24 & 0.17 (0.01) &              34 & 0.08 (0.01) &                        11 &  0.01 (0.0) &                            28 &  0.02 (0.0) &    6 & 0.01 (0.01) \\
      SA-RMTPP-TEM &              34 & 0.27 (0.01) &            39 &  0.32 (0.0) &                 36 & 0.31 (0.01) &              39 & 0.21 (0.03) &               7 &  0.03 (0.0) &                        12 &  0.01 (0.0) &                            27 &  0.02 (0.0) &    7 &  0.01 (0.0) \\
  SA-RMTPP-TEM + B &              35 & 0.27 (0.01) &            32 & 0.27 (0.01) &                 41 & 0.33 (0.01) &              26 & 0.18 (0.01) &               8 &  0.03 (0.0) &                        13 &  0.01 (0.0) &                            26 &  0.02 (0.0) &    8 &  0.01 (0.0) \\
       SA-RMTPP-TO &              36 & 0.27 (0.01) &            40 &  0.33 (0.0) &                 44 & 0.34 (0.01) &              43 & 0.24 (0.03) &              14 &  0.04 (0.0) &                        14 &  0.01 (0.0) &                            35 &  0.03 (0.0) &   35 & 0.03 (0.01) \\
      C-RMTPP-TEMP &              53 &  0.48 (0.0) &            53 &  0.42 (0.0) &                 53 & 0.41 (0.01) &              53 &  0.4 (0.01) &              41 &  0.13 (0.0) &                        53 &  0.23 (0.0) &                            53 &  0.26 (0.0) &   34 & 0.03 (0.01) \\
      GRU-SA/CM-LE &              15 & 0.15 (0.01) &            13 &  0.05 (0.0) &                 12 &  0.1 (0.01) &              19 & 0.13 (0.01) &              16 &  0.04 (0.0) &                        15 &  0.01 (0.0) &                            12 &  0.01 (0.0) &    9 &  0.01 (0.0) \\
  GRU-SA/CM-LE + B &              12 &  0.12 (0.0) &            18 & 0.14 (0.01) &                 19 &  0.2 (0.01) &              14 &  0.11 (0.0) &              10 & 0.03 (0.01) &                         6 &   0.0 (0.0) &                            13 &  0.01 (0.0) &   10 &  0.01 (0.0) \\
      GRU-SA/CM-TO &               2 &  0.02 (0.0) &            16 &   0.1 (0.0) &                  7 & 0.05 (0.01) &               2 &  0.03 (0.0) &              52 &  0.48 (0.0) &                        26 &  0.01 (0.0) &                            15 &  0.01 (0.0) &   43 & 0.04 (0.01) \\
       SA-SA/CM-LE &              17 & 0.16 (0.01) &            11 &  0.05 (0.0) &                 10 & 0.09 (0.01) &              21 & 0.14 (0.01) &              19 & 0.05 (0.01) &                        16 &  0.01 (0.0) &                            16 &  0.01 (0.0) &   11 &  0.01 (0.0) \\
   SA-SA/CM-LE + B &              13 & 0.13 (0.01) &            19 &  0.14 (0.0) &                 17 &  0.2 (0.01) &              17 & 0.13 (0.01) &              20 & 0.05 (0.01) &                         5 &   0.0 (0.0) &                            18 &  0.01 (0.0) &   12 &  0.01 (0.0) \\
       SA-SA/CM-TO &               7 &  0.05 (0.0) &            12 &  0.05 (0.0) &                  6 &  0.04 (0.0) &              11 & 0.09 (0.01) &              43 &  0.48 (0.0) &                        18 &  0.01 (0.0) &                            19 &  0.01 (0.0) &   45 & 0.04 (0.01) \\
        C-SA/CM-LE &              21 &  0.18 (0.0) &             9 &  0.04 (0.0) &                  9 &  0.09 (0.0) &              22 & 0.15 (0.01) &              33 & 0.07 (0.01) &                        19 &  0.01 (0.0) &                            20 &  0.01 (0.0) &   13 &  0.01 (0.0) \\
     GRU-SA/MC-TEM &              18 & 0.18 (0.02) &            23 &  0.2 (0.02) &                 23 & 0.22 (0.02) &              16 & 0.12 (0.01) &              45 &  0.48 (0.0) &                        20 &  0.01 (0.0) &                             2 &   0.0 (0.0) &   14 &  0.01 (0.0) \\
 GRU-SA/MC-TEM + B &              22 & 0.19 (0.01) &            17 & 0.14 (0.01) &                 25 & 0.25 (0.01) &              12 &   0.1 (0.0) &              31 & 0.07 (0.01) &                        21 &  0.01 (0.0) &                             1 &   0.0 (0.0) &   15 &  0.01 (0.0) \\
      GRU-SA/MC-TO &              43 & 0.31 (0.01) &            43 &  0.36 (0.0) &                 32 & 0.29 (0.01) &              45 & 0.25 (0.02) &              47 &  0.48 (0.0) &                        41 &  0.02 (0.0) &                            38 & 0.04 (0.01) &   16 &  0.01 (0.0) \\
      SA-SA/MC-TEM &              16 & 0.16 (0.01) &            33 & 0.28 (0.02) &                 24 & 0.23 (0.01) &              15 & 0.11 (0.01) &              48 &  0.48 (0.0) &                        22 &  0.01 (0.0) &                            21 &  0.01 (0.0) &   17 &  0.01 (0.0) \\
  SA-SA/MC-TEM + B &              19 & 0.18 (0.01) &            20 &  0.15 (0.0) &                 26 & 0.25 (0.01) &              13 &  0.1 (0.01) &              17 & 0.04 (0.01) &                        23 &  0.01 (0.0) &                            22 &  0.01 (0.0) &   18 &  0.01 (0.0) \\
       SA-SA/MC-TO &              45 & 0.32 (0.01) &            42 & 0.36 (0.01) &                 27 & 0.28 (0.01) &              44 & 0.24 (0.02) &              50 &  0.48 (0.0) &                        24 &  0.01 (0.0) &                            40 & 0.05 (0.01) &   19 &  0.01 (0.0) \\
      C-SA/MC-TEMP &              20 & 0.18 (0.01) &            28 & 0.24 (0.03) &                 28 & 0.28 (0.01) &              18 & 0.13 (0.01) &              51 &  0.48 (0.0) &                        25 &  0.01 (0.0) &                            23 &  0.01 (0.0) &   20 &  0.01 (0.0) \\
           Poisson &              52 & 0.35 (0.01) &            50 &   0.4 (0.0) &                 45 & 0.34 (0.01) &              52 & 0.33 (0.02) &              30 &  0.07 (0.0) &                        52 &  0.04 (0.0) &                            50 &  0.08 (0.0) &   53 &  0.35 (0.0) \\
            Hawkes &              24 &  0.21 (0.0) &            26 &  0.23 (0.0) &                 20 &  0.2 (0.01) &              23 & 0.16 (0.01) &              21 &  0.05 (0.0) &                         1 &   0.0 (0.0) &                            30 &  0.02 (0.0) &   24 &  0.01 (0.0) \\ \\
\end{tabular}
\begin{tabular}{ccc|cc|cc|cc|cc|cc|cc}
\hline \\
& \multicolumn{14}{c}{Time Calibration} \\ \\
                   & \multicolumn{2}{c}{Twitter} & \multicolumn{2}{c}{Reddit Subs.} & \multicolumn{2}{c}{PUBG} & \multicolumn{2}{c}{Yelp T.} & \multicolumn{2}{c}{Yelp M.} & \multicolumn{2}{c}{Reddit Coms.} & \multicolumn{2}{c}{Yelp A.} \\ \\
                   &         R &         Val &                           R &         Val &    R &         Val &            R &         Val &                R &         Val &                          R &         Val &            R &         Val \\ \\
\hline \\
        GRU-CP-TEM &        43 &  0.13 (0.0) &                          21 &  0.01 (0.0) &   35 &  0.02 (0.0) &           27 &  0.06 (0.0) &               33 &  0.05 (0.0) &                         24 &  0.02 (0.0) &           33 &  0.02 (0.0) \\
    GRU-CP-TEM + B &        41 &  0.13 (0.0) &                          28 &  0.01 (0.0) &   31 &  0.02 (0.0) &           23 &  0.05 (0.0) &               35 &  0.05 (0.0) &                         26 &  0.02 (0.0) &           35 &  0.02 (0.0) \\
         GRU-CP-TO &        42 &  0.13 (0.0) &                           7 &   0.0 (0.0) &   32 &  0.02 (0.0) &           22 &  0.05 (0.0) &               36 &  0.05 (0.0) &                         27 &  0.02 (0.0) &           36 &  0.02 (0.0) \\
         SA-CP-TEM &        45 &  0.15 (0.0) &                          35 &  0.02 (0.0) &   42 &  0.03 (0.0) &           31 &  0.07 (0.0) &               40 &  0.06 (0.0) &                         39 &  0.06 (0.0) &           38 &  0.03 (0.0) \\
     SA-CP-TEM + B &        50 &  0.16 (0.0) &                          36 &  0.02 (0.0) &   41 &  0.03 (0.0) &           32 &  0.07 (0.0) &               38 &  0.06 (0.0) &                         40 &  0.06 (0.0) &           39 &  0.03 (0.0) \\
          SA-CP-TO &        51 &  0.17 (0.0) &                          48 &  0.05 (0.0) &   49 &  0.06 (0.0) &           47 &  0.1 (0.01) &               52 &  0.12 (0.0) &                         51 &  0.17 (0.0) &           47 &  0.04 (0.0) \\
         C-CP-TEMP &        52 &   0.2 (0.0) &                          50 &  0.06 (0.0) &   51 &  0.07 (0.0) &           51 & 0.11 (0.01) &               51 &  0.12 (0.0) &                         52 &  0.18 (0.0) &           46 &  0.04 (0.0) \\
       GRU-LNM-TEM &        10 &  0.01 (0.0) &                          23 &  0.01 (0.0) &   26 &  0.01 (0.0) &            3 &  0.01 (0.0) &                6 &  0.01 (0.0) &                          3 &   0.0 (0.0) &           23 &  0.01 (0.0) \\
   GRU-LNM-TEM + B &        29 & 0.04 (0.01) &                          52 & 0.07 (0.01) &   50 & 0.06 (0.01) &           36 &  0.08 (0.0) &               46 & 0.09 (0.01) &                         38 & 0.06 (0.01) &           51 & 0.07 (0.01) \\
        GRU-LNM-TO &         9 &  0.01 (0.0) &                          24 &  0.01 (0.0) &   27 &  0.01 (0.0) &            2 &  0.01 (0.0) &                4 &  0.01 (0.0) &                          2 &   0.0 (0.0) &           21 &  0.01 (0.0) \\
        GRU-LNM-K1 &         7 &  0.01 (0.0) &                          40 &  0.03 (0.0) &   34 &  0.02 (0.0) &           33 &  0.07 (0.0) &               32 &  0.04 (0.0) &                         33 &  0.03 (0.0) &           50 &  0.04 (0.0) \\
        SA-LNM-TEM &         6 &  0.01 (0.0) &                          25 &  0.01 (0.0) &   33 &  0.02 (0.0) &            1 &  0.01 (0.0) &                3 &  0.01 (0.0) &                          1 &   0.0 (0.0) &           20 &  0.01 (0.0) \\
    SA-LNM-TEM + B &        34 & 0.07 (0.01) &                          51 & 0.06 (0.01) &   53 & 0.07 (0.01) &           34 &  0.07 (0.0) &               44 & 0.08 (0.01) &                         35 &  0.04 (0.0) &           52 & 0.08 (0.01) \\
         SA-LNM-TO &        21 &  0.02 (0.0) &                          27 &  0.01 (0.0) &   30 &  0.01 (0.0) &            4 &  0.02 (0.0) &                2 &  0.01 (0.0) &                         14 &  0.01 (0.0) &           18 &  0.01 (0.0) \\
         SA-LNM-K1 &         4 &  0.01 (0.0) &                          31 &  0.02 (0.0) &   36 &  0.02 (0.0) &           35 &  0.07 (0.0) &               23 &  0.03 (0.0) &                         28 &  0.02 (0.0) &           45 &  0.04 (0.0) \\
        C-LNM-TEMP &        25 &  0.02 (0.0) &                          26 &  0.01 (0.0) &   29 &  0.01 (0.0) &            5 &  0.02 (0.0) &                1 &  0.01 (0.0) &                         12 &  0.01 (0.0) &           16 &  0.01 (0.0) \\
     GRU-MLP/CM-LE &        49 &  0.15 (0.0) &                          37 &  0.03 (0.0) &   44 &  0.05 (0.0) &           42 & 0.09 (0.01) &               45 & 0.09 (0.01) &                         44 & 0.09 (0.03) &           41 &  0.03 (0.0) \\
 GRU-MLP/CM-LE + B &        44 &  0.15 (0.0) &                          38 &  0.03 (0.0) &   45 &  0.05 (0.0) &           43 & 0.09 (0.01) &               47 &   0.1 (0.0) &                         49 &  0.14 (0.0) &           48 &  0.04 (0.0) \\
     GRU-MLP/CM-TO &        46 &  0.15 (0.0) &                          43 &  0.04 (0.0) &   46 &  0.05 (0.0) &           52 & 0.18 (0.01) &               50 &   0.1 (0.0) &                         43 & 0.07 (0.03) &           42 &  0.03 (0.0) \\
      SA-MLP/CM-LE &        47 &  0.15 (0.0) &                          41 &  0.03 (0.0) &   47 &  0.05 (0.0) &           46 &  0.1 (0.01) &               48 &   0.1 (0.0) &                         48 &  0.14 (0.0) &           43 &  0.03 (0.0) \\
  SA-MLP/CM-LE + B &        48 &  0.15 (0.0) &                          39 &  0.03 (0.0) &   48 &  0.05 (0.0) &           44 & 0.09 (0.01) &               49 &   0.1 (0.0) &                         47 &  0.14 (0.0) &           49 &  0.04 (0.0) \\
      SA-MLP/CM-TO &        18 &  0.02 (0.0) &                          46 &  0.05 (0.0) &   25 &  0.01 (0.0) &           45 &  0.1 (0.01) &               16 &  0.02 (0.0) &                         50 &  0.15 (0.0) &           40 &  0.03 (0.0) \\
       C-MLP/CM-LE &        30 & 0.05 (0.03) &                          42 & 0.03 (0.01) &   28 &  0.01 (0.0) &           40 & 0.09 (0.01) &               34 & 0.05 (0.02) &                         34 &  0.03 (0.0) &            9 &  0.01 (0.0) \\
    GRU-MLP/MC-TEM &        17 &  0.02 (0.0) &                           6 &   0.0 (0.0) &   23 &  0.01 (0.0) &           15 &  0.05 (0.0) &               15 &  0.02 (0.0) &                          5 &   0.0 (0.0) &            8 &  0.01 (0.0) \\
GRU-MLP/MC-TEM + B &        20 &  0.02 (0.0) &                           3 &   0.0 (0.0) &   11 &  0.01 (0.0) &           18 &  0.05 (0.0) &               13 &  0.02 (0.0) &                         15 &  0.01 (0.0) &            7 &  0.01 (0.0) \\
     GRU-MLP/MC-TO &        22 &  0.02 (0.0) &                          19 &  0.01 (0.0) &    2 &  0.01 (0.0) &           20 &  0.05 (0.0) &               17 &  0.02 (0.0) &                          8 &  0.01 (0.0) &            6 &  0.01 (0.0) \\
     SA-MLP/MC-TEM &        28 &  0.03 (0.0) &                          22 &  0.01 (0.0) &    1 &  0.01 (0.0) &           28 &  0.06 (0.0) &               18 &  0.02 (0.0) &                         25 &  0.02 (0.0) &            1 &  0.01 (0.0) \\
 SA-MLP/MC-TEM + B &        26 &  0.02 (0.0) &                          18 &  0.01 (0.0) &    3 &  0.01 (0.0) &           30 &  0.06 (0.0) &               12 &  0.02 (0.0) &                         23 &  0.02 (0.0) &            4 &  0.01 (0.0) \\
      SA-MLP/MC-TO &        27 &  0.03 (0.0) &                          29 &  0.02 (0.0) &    4 &  0.01 (0.0) &           41 & 0.09 (0.01) &               14 &  0.02 (0.0) &                         30 &  0.03 (0.0) &            3 &  0.01 (0.0) \\
     C-MLP/MC-TEMP &        19 &  0.02 (0.0) &                          30 &  0.02 (0.0) &    5 &  0.01 (0.0) &           38 & 0.09 (0.01) &               25 &  0.03 (0.0) &                         31 &  0.03 (0.0) &            2 &  0.01 (0.0) \\
     GRU-RMTPP-TEM &        36 &  0.09 (0.0) &                          17 &  0.01 (0.0) &    6 &  0.01 (0.0) &           19 &  0.05 (0.0) &               26 &  0.03 (0.0) &                          9 &  0.01 (0.0) &           29 &  0.01 (0.0) \\
 GRU-RMTPP-TEM + B &        31 &  0.05 (0.0) &                          16 &  0.01 (0.0) &    7 &  0.01 (0.0) &           14 &  0.05 (0.0) &               27 &  0.03 (0.0) &                         10 &  0.01 (0.0) &           30 &  0.01 (0.0) \\
      GRU-RMTPP-TO &        37 &  0.09 (0.0) &                          15 &  0.01 (0.0) &    8 &  0.01 (0.0) &           16 &  0.05 (0.0) &               24 &  0.03 (0.0) &                         11 &  0.01 (0.0) &            5 &  0.01 (0.0) \\
      SA-RMTPP-TEM &        38 &   0.1 (0.0) &                          33 &  0.02 (0.0) &    9 &  0.01 (0.0) &           26 &  0.06 (0.0) &               31 &  0.04 (0.0) &                         36 &  0.04 (0.0) &           10 &  0.01 (0.0) \\
  SA-RMTPP-TEM + B &        32 &  0.05 (0.0) &                          34 &  0.02 (0.0) &   10 &  0.01 (0.0) &           25 &  0.06 (0.0) &               30 &  0.04 (0.0) &                         37 &  0.04 (0.0) &           11 &  0.01 (0.0) \\
       SA-RMTPP-TO &        39 &   0.1 (0.0) &                          47 & 0.05 (0.01) &   37 &  0.03 (0.0) &           50 &  0.1 (0.01) &               29 &  0.04 (0.0) &                         41 &  0.07 (0.0) &           12 &  0.01 (0.0) \\
      C-RMTPP-TEMP &        40 &  0.12 (0.0) &                          49 &  0.05 (0.0) &   38 &  0.03 (0.0) &           49 &  0.1 (0.01) &               28 &  0.04 (0.0) &                         42 &  0.07 (0.0) &           13 &  0.01 (0.0) \\
      GRU-SA/CM-LE &        16 &  0.01 (0.0) &                          14 &  0.01 (0.0) &   12 &  0.01 (0.0) &           17 &  0.05 (0.0) &                5 &  0.01 (0.0) &                         13 &  0.01 (0.0) &           14 &  0.01 (0.0) \\
  GRU-SA/CM-LE + B &         8 &  0.01 (0.0) &                          13 &  0.01 (0.0) &   22 &  0.01 (0.0) &           13 &  0.04 (0.0) &               11 &  0.01 (0.0) &                         21 &  0.01 (0.0) &           15 &  0.01 (0.0) \\
      GRU-SA/CM-TO &         2 &  0.01 (0.0) &                           2 &   0.0 (0.0) &   13 &  0.01 (0.0) &            6 &  0.02 (0.0) &               43 & 0.07 (0.03) &                         16 &  0.01 (0.0) &           44 & 0.03 (0.01) \\
       SA-SA/CM-LE &         3 &  0.01 (0.0) &                          20 &  0.01 (0.0) &   14 &  0.01 (0.0) &           24 & 0.05 (0.01) &               19 &  0.02 (0.0) &                         18 &  0.01 (0.0) &           17 &  0.01 (0.0) \\
   SA-SA/CM-LE + B &         5 &  0.01 (0.0) &                          11 &  0.01 (0.0) &   15 &  0.01 (0.0) &            7 &  0.03 (0.0) &                7 &  0.01 (0.0) &                         20 &  0.01 (0.0) &           19 &  0.01 (0.0) \\
       SA-SA/CM-TO &        15 &  0.01 (0.0) &                          10 &  0.01 (0.0) &   16 &  0.01 (0.0) &           21 &  0.05 (0.0) &               42 & 0.06 (0.02) &                         32 &  0.03 (0.0) &           31 & 0.02 (0.01) \\
        C-SA/CM-LE &        23 &  0.02 (0.0) &                          32 &  0.02 (0.0) &   17 &  0.01 (0.0) &           37 & 0.09 (0.01) &               20 &  0.02 (0.0) &                         29 & 0.03 (0.01) &           22 &  0.01 (0.0) \\
     GRU-SA/MC-TEM &        11 &  0.01 (0.0) &                           4 &   0.0 (0.0) &   18 &  0.01 (0.0) &            8 &  0.03 (0.0) &               21 &  0.02 (0.0) &                          7 &  0.01 (0.0) &           24 &  0.01 (0.0) \\
 GRU-SA/MC-TEM + B &        12 &  0.01 (0.0) &                           5 &   0.0 (0.0) &   19 &  0.01 (0.0) &            9 &  0.03 (0.0) &                8 &  0.01 (0.0) &                          4 &   0.0 (0.0) &           25 &  0.01 (0.0) \\
      GRU-SA/MC-TO &        35 & 0.08 (0.02) &                          45 &  0.05 (0.0) &   43 & 0.03 (0.01) &           39 & 0.09 (0.01) &               39 & 0.06 (0.01) &                         46 & 0.12 (0.01) &           32 &  0.02 (0.0) \\
      SA-SA/MC-TEM &        13 &  0.01 (0.0) &                           8 &   0.0 (0.0) &   20 &  0.01 (0.0) &           10 &  0.04 (0.0) &                9 &  0.01 (0.0) &                          6 &   0.0 (0.0) &           26 &  0.01 (0.0) \\
  SA-SA/MC-TEM + B &        14 &  0.01 (0.0) &                           9 &  0.01 (0.0) &   21 &  0.01 (0.0) &           11 &  0.04 (0.0) &               22 &  0.02 (0.0) &                         19 &  0.01 (0.0) &           27 &  0.01 (0.0) \\
       SA-SA/MC-TO &        33 & 0.06 (0.02) &                          44 &  0.05 (0.0) &   40 & 0.03 (0.01) &           48 &  0.1 (0.01) &               41 & 0.06 (0.02) &                         45 & 0.12 (0.01) &           37 & 0.03 (0.01) \\
      C-SA/MC-TEMP &        24 &  0.02 (0.0) &                          12 &  0.01 (0.0) &   39 & 0.03 (0.01) &           12 & 0.04 (0.01) &               10 &  0.01 (0.0) &                         17 &  0.01 (0.0) &           28 &  0.01 (0.0) \\
           Poisson &        53 &   0.2 (0.0) &                          53 &  0.27 (0.0) &   52 &  0.07 (0.0) &           53 &  0.47 (0.0) &               53 &  0.27 (0.0) &                         53 &  0.25 (0.0) &           53 &  0.12 (0.0) \\
            Hawkes &         1 &  0.01 (0.0) &                           1 &   0.0 (0.0) &   24 &  0.01 (0.0) &           29 &  0.06 (0.0) &               37 &  0.05 (0.0) &                         22 &  0.01 (0.0) &           34 &  0.02 (0.0) \\ \\
\hline \\
\end{tabular}

\label{resultsmark}
%\caption{Evaluation of the different neural TPP models on MOOC and LastFM. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\tiny
\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccc|cc|cc|cc|cc|cc|cc}
\hline \\
& \multicolumn{14}{c}{NLL Mark} \\ \\
                   & \multicolumn{2}{c}{LastFM} & \multicolumn{2}{c}{MOOC} & \multicolumn{2}{c}{Wiki.} & \multicolumn{2}{c}{Github} & \multicolumn{2}{c}{MIMIC2} & \multicolumn{2}{c}{Hawkes Exp.} & \multicolumn{2}{c}{Hawkes Sum. Exp.} \\ \\
                   &               R &            Val &             R &            Val &                  R &             Val &               R &            Val &               R &          Val &                         R &           Val &                             R &           Val \\ \\
\hline \\
        GRU-CP-TEM &              17 & 818.67 (21.56) &            11 &   96.55 (1.44) &                 50 & 443.74 (140.44) &              15 & 138.71 (19.91) &              12 &  2.76 (0.21) &                         4 & 110.06 (0.53) &                             8 &  113.65 (0.9) \\
    GRU-CP-TEM + B &              23 & 853.67 (24.72) &            19 &  118.26 (2.51) &                 51 & 480.56 (143.44) &              22 &  151.7 (21.25) &              20 &  3.96 (0.31) &                        18 & 111.26 (0.57) &                            18 &  114.23 (0.9) \\
         GRU-CP-TO &              34 & 870.76 (29.88) &            28 &  152.98 (1.71) &                 37 &   289.66 (41.0) &              29 &  154.62 (21.3) &              28 &   4.4 (0.16) &                        26 & 111.66 (0.55) &                            19 &  114.24 (0.9) \\
         SA-CP-TEM &              22 & 850.92 (28.09) &            12 &   97.51 (0.99) &                 49 & 415.91 (135.01) &              19 & 142.12 (20.54) &              11 &  2.73 (0.24) &                        12 & 110.66 (0.56) &                            13 &  113.87 (0.9) \\
     SA-CP-TEM + B &              26 &  865.9 (28.31) &            18 &  117.77 (3.18) &                 53 & 591.01 (162.57) &              23 & 152.32 (20.72) &              19 &  3.87 (0.27) &                        23 &  111.52 (0.6) &                            22 & 114.26 (0.89) \\
          SA-CP-TO &              29 &  869.97 (30.6) &            43 &  184.53 (2.35) &                 31 &  277.79 (23.05) &              45 & 162.74 (21.32) &              25 &   4.3 (0.13) &                        39 &  112.0 (0.53) &                            28 &  114.53 (0.9) \\
         C-CP-TEMP &              46 & 873.89 (30.33) &            49 &  188.13 (2.37) &                 33 &  283.06 (20.12) &              47 & 163.29 (21.28) &              36 &  6.63 (0.16) &                        51 & 113.46 (0.54) &                            46 &  116.0 (0.91) \\
       GRU-LNM-TEM &               2 & 689.53 (15.13) &             3 &   88.17 (1.27) &                  7 &  218.49 (25.06) &               7 & 131.46 (24.14) &               4 &  2.12 (0.12) &                         5 & 110.12 (0.54) &                             3 &  113.47 (0.9) \\
   GRU-LNM-TEM + B &              50 &  874.9 (30.05) &             2 &   88.11 (1.09) &                 30 &   277.3 (20.39) &              41 & 161.24 (22.35) &              16 &    3.5 (0.1) &                        45 &  112.6 (0.63) &                            52 & 117.89 (1.36) \\
        GRU-LNM-TO &              43 & 873.29 (31.11) &            25 &  149.51 (2.59) &                 44 &  315.21 (31.94) &              25 & 153.98 (21.55) &              27 &  4.33 (0.14) &                        28 & 111.68 (0.55) &                            21 &  114.25 (0.9) \\
        GRU-LNM-K1 &               4 & 708.17 (20.48) &             1 &   87.78 (1.51) &                 20 &  261.32 (14.94) &               1 & 123.28 (18.16) &               5 &  2.17 (0.17) &                         3 & 110.04 (0.54) &                             5 &  113.53 (0.9) \\
        SA-LNM-TEM &               8 & 773.35 (32.98) &             9 &   93.71 (1.67) &                 12 &  246.11 (18.82) &               6 & 131.43 (20.52) &               6 &   2.33 (0.2) &                        13 &  110.7 (0.51) &                            12 & 113.85 (0.92) \\
    SA-LNM-TEM + B &              45 & 873.88 (29.62) &             6 &   92.02 (1.36) &                 36 &  289.16 (14.89) &              24 &  152.8 (19.96) &              15 &  3.21 (0.27) &                        43 & 112.42 (0.58) &                            49 & 116.21 (0.82) \\
         SA-LNM-TO &              37 & 871.04 (29.87) &            44 &  184.53 (2.35) &                 38 &  303.24 (22.88) &              32 & 157.72 (21.14) &              24 &  4.28 (0.13) &                        35 & 111.98 (0.54) &                            33 &  114.54 (0.9) \\
         SA-LNM-K1 &               9 & 780.68 (23.85) &             7 &   92.92 (1.33) &                 23 &  264.32 (16.04) &              13 &  138.34 (21.6) &               3 &  2.04 (0.06) &                         9 & 110.61 (0.56) &                            14 &  113.87 (0.9) \\
        C-LNM-TEMP &              48 & 874.12 (29.76) &            47 &  188.12 (2.37) &                 39 &  306.08 (23.59) &              37 & 159.41 (21.21) &              35 &  6.62 (0.16) &                        50 & 113.45 (0.54) &                            47 &  116.0 (0.91) \\
     GRU-MLP/CM-LE &              25 & 864.56 (29.49) &            20 &  128.17 (6.99) &                 21 &  262.74 (18.39) &              35 & 158.14 (22.91) &              30 &  4.49 (0.16) &                        16 & 110.96 (0.64) &                            15 & 114.06 (0.91) \\
 GRU-MLP/CM-LE + B &              33 &  870.6 (29.91) &            23 &  148.46 (5.88) &                 47 &  330.45 (43.01) &              39 & 160.33 (24.42) &              18 &  3.81 (0.22) &                        33 &  111.9 (0.57) &                            31 &  114.53 (0.9) \\
     GRU-MLP/CM-TO &              39 & 871.23 (30.22) &            34 &  161.34 (2.82) &                 40 &  306.94 (40.27) &              42 & 161.37 (22.74) &              32 &  4.59 (0.17) &                        27 & 111.68 (0.55) &                            23 &  114.27 (0.9) \\
      SA-MLP/CM-LE &              36 & 871.02 (30.02) &            27 &  152.09 (2.54) &                 29 &  277.28 (28.13) &              40 & 160.58 (20.61) &              31 &  4.51 (0.13) &                        37 & 111.98 (0.54) &                            30 &  114.53 (0.9) \\
  SA-MLP/CM-LE + B &              35 & 870.94 (29.97) &            33 &  159.87 (7.03) &                 48 &   330.9 (45.83) &              49 &  163.4 (22.79) &              17 &   3.75 (0.2) &                        34 & 111.97 (0.54) &                            29 &  114.53 (0.9) \\
      SA-MLP/CM-TO &              32 & 870.39 (30.23) &            45 &  184.53 (2.35) &                 24 &  264.36 (21.07) &              44 & 161.57 (20.86) &              34 &  4.62 (0.16) &                        38 & 111.99 (0.54) &                            34 & 114.54 (0.91) \\
       C-MLP/CM-LE &              47 & 874.07 (30.06) &            22 &  143.83 (2.31) &                 26 &  266.35 (18.68) &              43 & 161.54 (19.84) &              37 &   7.0 (0.18) &                        48 & 112.88 (0.52) &                            44 & 115.76 (0.94) \\
    GRU-MLP/MC-TEM &               6 & 768.24 (33.55) &            29 &   155.94 (5.5) &                  6 &  217.08 (16.43) &              16 & 139.71 (19.49) &              47 &  7.33 (0.26) &                        17 & 111.08 (0.58) &                            36 & 114.74 (0.88) \\
GRU-MLP/MC-TEM + B &               7 & 769.23 (31.98) &            13 &   98.27 (3.09) &                  2 &  145.13 (17.34) &               5 &  130.7 (18.32) &              14 &  2.84 (0.17) &                         6 & 110.25 (0.56) &                             4 & 113.53 (0.93) \\
     GRU-MLP/MC-TO &              52 & 876.07 (31.35) &            37 &  167.16 (7.48) &                 15 &  256.13 (18.29) &              46 & 162.79 (21.89) &              46 &  7.33 (0.26) &                        44 & 112.56 (0.55) &                            43 & 115.44 (0.91) \\
     SA-MLP/MC-TEM &              14 & 808.01 (28.29) &            30 &  158.58 (5.88) &                 10 &  220.69 (12.58) &              20 & 142.19 (21.43) &              44 &  7.33 (0.26) &                        20 & 111.43 (0.54) &                            37 & 114.94 (0.91) \\
 SA-MLP/MC-TEM + B &              12 & 793.71 (26.11) &            16 &   103.3 (4.38) &                  4 &  149.89 (19.86) &              14 & 138.37 (17.41) &               9 &  2.55 (0.13) &                        10 & 110.63 (0.56) &                             6 & 113.59 (0.88) \\
      SA-MLP/MC-TO &              42 & 872.92 (30.75) &            52 &   193.3 (4.87) &                 16 &  256.14 (18.29) &              50 & 163.56 (21.83) &              45 &  7.33 (0.26) &                        42 & 112.33 (0.55) &                            42 &  115.4 (0.88) \\
     C-MLP/MC-TEMP &              10 & 781.82 (28.59) &            46 &  186.74 (2.63) &                 14 &  253.73 (16.66) &              18 & 141.53 (19.51) &              51 & 11.09 (0.26) &                        46 & 112.64 (0.54) &                            50 & 116.43 (0.92) \\
     GRU-RMTPP-TEM &               3 & 707.88 (21.42) &             4 &   88.46 (1.89) &                 22 &  263.12 (37.03) &               4 &  127.8 (19.96) &               1 &  1.89 (0.12) &                         1 & 109.98 (0.55) &                             2 &  113.46 (0.9) \\
 GRU-RMTPP-TEM + B &               5 & 750.69 (32.06) &             5 &   88.58 (1.71) &                 25 &  264.53 (41.57) &              10 &  136.6 (18.94) &               8 &  2.43 (0.23) &                         2 & 109.99 (0.55) &                             1 & 113.45 (0.87) \\
      GRU-RMTPP-TO &              51 & 875.49 (31.26) &            24 &   149.24 (2.1) &                 42 &  310.93 (26.65) &              26 & 154.03 (21.77) &              26 &  4.32 (0.14) &                        25 & 111.66 (0.55) &                            20 &  114.25 (0.9) \\
      SA-RMTPP-TEM &              11 & 787.54 (23.83) &            10 &   94.23 (2.34) &                 11 &  234.26 (37.46) &              12 & 138.15 (21.92) &               2 &  2.02 (0.13) &                         8 & 110.61 (0.55) &                            10 &  113.8 (0.91) \\
  SA-RMTPP-TEM + B &              18 &  826.77 (30.2) &             8 &   93.06 (0.86) &                 34 &   285.6 (44.04) &              17 & 139.97 (18.33) &              13 &  2.78 (0.15) &                         7 &  110.6 (0.56) &                             7 &  113.6 (0.87) \\
       SA-RMTPP-TO &              38 &  871.14 (30.1) &            42 &  184.53 (2.35) &                 45 &  320.97 (40.84) &              34 & 158.12 (21.54) &              23 &  4.28 (0.13) &                        36 & 111.98 (0.54) &                            27 & 114.53 (0.91) \\
      C-RMTPP-TEMP &              49 & 874.64 (28.16) &            53 &  195.92 (2.51) &                 19 &   260.05 (18.3) &              53 & 216.79 (26.09) &              50 & 11.09 (0.26) &                        53 & 116.31 (0.55) &                            53 & 119.06 (0.86) \\
      GRU-SA/CM-LE &              21 &   849.9 (26.6) &            39 &   167.74 (2.5) &                 28 &  276.43 (26.65) &              30 & 157.01 (21.64) &              33 &   4.61 (0.1) &                        19 & 111.33 (0.35) &                            24 & 114.37 (0.91) \\
  GRU-SA/CM-LE + B &              27 & 866.33 (29.31) &            40 &   176.3 (2.28) &                 41 &  309.48 (50.99) &              28 &  154.45 (21.0) &              21 &  4.05 (0.19) &                        29 & 111.72 (0.54) &                            16 & 114.14 (0.88) \\
      GRU-SA/CM-TO &              40 & 872.31 (30.45) &            32 &  159.42 (2.12) &                 43 &  311.78 (47.45) &              38 & 159.59 (22.81) &              48 &  7.41 (0.29) &                        32 & 111.87 (0.54) &                            32 &  114.54 (0.9) \\
       SA-SA/CM-LE &              24 & 863.77 (28.84) &            38 &  167.42 (1.46) &                 35 &  286.24 (32.47) &              36 & 158.45 (21.09) &              29 &  4.44 (0.14) &                        24 & 111.63 (0.57) &                            25 & 114.43 (0.89) \\
   SA-SA/CM-LE + B &              28 &  867.9 (28.66) &            41 &  177.16 (2.71) &                 46 &  327.52 (50.72) &              27 & 154.33 (21.02) &              22 &  4.08 (0.11) &                        30 & 111.72 (0.55) &                            17 & 114.18 (0.87) \\
       SA-SA/CM-TO &              41 & 872.36 (30.23) &            36 &  163.99 (2.29) &                 27 &  276.17 (21.96) &              33 & 157.81 (21.98) &              39 &  7.32 (0.28) &                        31 & 111.86 (0.54) &                            26 & 114.51 (0.91) \\
        C-SA/CM-LE &              53 & 877.82 (30.44) &            31 &  159.14 (5.02) &                 32 &  278.41 (23.18) &              31 & 157.17 (21.16) &              38 &  7.15 (0.17) &                        49 & 112.98 (0.56) &                            45 & 115.78 (0.92) \\
     GRU-SA/MC-TEM &              13 & 806.55 (17.88) &            21 &  142.04 (5.47) &                  8 &  218.69 (15.22) &               9 & 136.46 (18.77) &              42 &  7.33 (0.26) &                        22 & 111.49 (0.55) &                            39 & 115.04 (0.87) \\
 GRU-SA/MC-TEM + B &              15 & 812.16 (26.32) &            15 &  101.24 (1.54) &                  5 &  150.91 (13.55) &               3 &  125.2 (16.26) &              10 &  2.56 (0.21) &                        11 & 110.65 (0.59) &                             9 &  113.7 (0.86) \\
      GRU-SA/MC-TO &              30 & 869.98 (29.93) &            51 &  190.08 (2.59) &                 17 &  256.56 (18.52) &              51 & 163.72 (22.15) &              43 &  7.33 (0.26) &                        40 & 112.22 (0.51) &                            41 & 115.26 (0.87) \\
      SA-SA/MC-TEM &              20 & 835.17 (29.13) &            35 &  163.39 (6.32) &                  9 &   220.31 (8.94) &              11 & 137.85 (19.01) &              40 &  7.33 (0.26) &                        21 & 111.48 (0.56) &                            38 & 114.99 (0.89) \\
  SA-SA/MC-TEM + B &              16 & 816.79 (31.72) &            14 &     98.6 (2.1) &                  3 &   149.4 (10.93) &               8 & 131.79 (19.84) &               7 &   2.4 (0.17) &                        14 & 110.75 (0.51) &                            11 & 113.85 (0.83) \\
       SA-SA/MC-TO &              31 & 870.31 (29.76) &            50 &  189.34 (3.53) &                 18 &   257.9 (18.24) &              48 & 163.34 (23.04) &              41 &  7.33 (0.26) &                        41 & 112.31 (0.56) &                            40 &  115.1 (0.89) \\
      C-SA/MC-TEMP &              19 & 828.98 (33.29) &            26 & 150.83 (11.47) &                 13 &  253.09 (15.97) &              21 & 149.39 (22.34) &              52 & 11.09 (0.26) &                        47 & 112.67 (0.55) &                            51 & 116.48 (0.89) \\
           Poisson &              44 & 873.82 (30.24) &            48 &  188.13 (2.37) &                 52 & 534.95 (131.14) &              52 & 168.37 (21.04) &              53 & 11.25 (0.46) &                        52 & 113.46 (0.54) &                            48 & 116.03 (0.91) \\
            Hawkes &               1 & 514.09 (16.24) &            17 &  114.99 (1.54) &                  1 &  144.69 (12.45) &               2 & 124.65 (15.73) &              49 &  8.24 (0.47) &                        15 & 110.83 (0.54) &                            35 & 114.61 (0.88) \\ \\
\hline 
\end{tabular}

\label{resultsmark}
\caption{Evaluation of the different neural TPP models on MOOC and LastFM. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\tiny
\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccc|cc|cc|cc|cc|cc|cc}
\hline \\
 & \multicolumn{14}{c}{F1-score} \\ \\
                   & \multicolumn{2}{c}{LastFM} & \multicolumn{2}{c}{MOOC} & \multicolumn{2}{c}{Wiki.} & \multicolumn{2}{c}{Github} & \multicolumn{2}{c}{MIMIC2} & \multicolumn{2}{c}{Hawkes Exp.} & \multicolumn{2}{c}{Hawkes Sum. Exp.} \\ \\
                   &               R &         Val &             R &         Val &                  R &         Val &               R &         Val &               R &         Val &                         R &         Val &                             R &         Val \\ \\
\hline \\
        GRU-CP-TEM &              20 &  0.03 (0.0) &            15 & 0.29 (0.01) &                 19 & 0.14 (0.08) &              22 & 0.42 (0.03) &              13 & 0.64 (0.05) &                         9 &  0.27 (0.0) &                            15 &  0.24 (0.0) \\
    GRU-CP-TEM + B &              23 &  0.01 (0.0) &            18 &  0.25 (0.0) &                 21 & 0.13 (0.04) &              23 & 0.42 (0.03) &              16 & 0.62 (0.04) &                        23 & 0.19 (0.01) &                            26 & 0.17 (0.01) \\
         GRU-CP-TO &              32 &   0.0 (0.0) &            29 &  0.06 (0.0) &                 24 &  0.02 (0.0) &              32 &  0.4 (0.03) &              27 & 0.22 (0.02) &                        35 & 0.13 (0.01) &                            27 & 0.17 (0.01) \\
         SA-CP-TEM &              26 &  0.01 (0.0) &            16 &  0.29 (0.0) &                 13 & 0.21 (0.11) &              30 &  0.4 (0.03) &              17 & 0.62 (0.05) &                        20 &  0.25 (0.0) &                            17 &  0.23 (0.0) \\
     SA-CP-TEM + B &              35 &   0.0 (0.0) &            19 & 0.24 (0.01) &                 18 & 0.14 (0.08) &              27 &  0.4 (0.03) &              19 & 0.55 (0.05) &                        26 & 0.17 (0.02) &                            22 & 0.18 (0.01) \\
          SA-CP-TO &              31 &   0.0 (0.0) &            47 &  0.01 (0.0) &                 41 &   0.0 (0.0) &              26 &  0.4 (0.03) &              28 & 0.22 (0.02) &                        43 &  0.11 (0.0) &                            43 &  0.11 (0.0) \\
         C-CP-TEMP &              30 &   0.0 (0.0) &            46 &  0.01 (0.0) &                 42 &   0.0 (0.0) &              24 &  0.4 (0.03) &              41 &  0.2 (0.02) &                        44 &  0.11 (0.0) &                            44 &  0.11 (0.0) \\
       GRU-LNM-TEM &               3 &  0.2 (0.01) &             1 &   0.4 (0.0) &                  9 & 0.43 (0.11) &              10 &  0.5 (0.04) &               6 & 0.72 (0.01) &                         3 &  0.27 (0.0) &                             5 &  0.24 (0.0) \\
   GRU-LNM-TEM + B &              33 &   0.0 (0.0) &             2 &   0.4 (0.0) &                 23 & 0.12 (0.08) &              21 & 0.42 (0.03) &              18 & 0.62 (0.04) &                        27 &  0.17 (0.0) &                            30 & 0.16 (0.01) \\
        GRU-LNM-TO &              24 &  0.01 (0.0) &            27 &  0.08 (0.0) &                 28 &  0.01 (0.0) &              28 &  0.4 (0.03) &              29 & 0.22 (0.02) &                        31 & 0.15 (0.01) &                            29 &  0.17 (0.0) \\
        GRU-LNM-K1 &               5 & 0.17 (0.02) &             3 &   0.4 (0.0) &                 15 & 0.17 (0.11) &               2 & 0.54 (0.02) &               7 & 0.71 (0.02) &                         4 &  0.27 (0.0) &                             6 &  0.24 (0.0) \\
        SA-LNM-TEM &              16 & 0.08 (0.02) &            11 & 0.35 (0.01) &                 11 & 0.31 (0.12) &               9 & 0.51 (0.03) &              11 & 0.68 (0.05) &                        21 &  0.25 (0.0) &                             7 &  0.24 (0.0) \\
    SA-LNM-TEM + B &              36 &   0.0 (0.0) &             9 &  0.36 (0.0) &                 12 &  0.22 (0.1) &              20 & 0.44 (0.03) &              14 & 0.64 (0.03) &                        28 & 0.17 (0.02) &                            32 & 0.15 (0.01) \\
         SA-LNM-TO &              37 &   0.0 (0.0) &            43 &  0.01 (0.0) &                 46 &   0.0 (0.0) &              33 &  0.4 (0.03) &              30 & 0.22 (0.02) &                        50 &  0.11 (0.0) &                            47 &  0.11 (0.0) \\
         SA-LNM-K1 &              17 & 0.07 (0.01) &            10 & 0.36 (0.01) &                 14 &  0.19 (0.1) &              17 & 0.47 (0.04) &               2 & 0.76 (0.02) &                        14 &  0.26 (0.0) &                             8 &  0.24 (0.0) \\
        C-LNM-TEMP &              39 &   0.0 (0.0) &            48 &  0.01 (0.0) &                 48 &   0.0 (0.0) &              34 &  0.4 (0.03) &              39 &  0.2 (0.02) &                        46 &  0.11 (0.0) &                            49 &  0.11 (0.0) \\
     GRU-MLP/CM-LE &              29 &  0.01 (0.0) &            24 & 0.14 (0.03) &                 31 &  0.01 (0.0) &              35 &  0.4 (0.03) &              35 & 0.21 (0.02) &                        22 & 0.22 (0.01) &                            24 & 0.18 (0.01) \\
 GRU-MLP/CM-LE + B &              40 &   0.0 (0.0) &            34 & 0.05 (0.02) &                 26 &  0.01 (0.0) &              25 &  0.4 (0.03) &              20 & 0.36 (0.04) &                        37 & 0.12 (0.01) &                            50 &  0.11 (0.0) \\
     GRU-MLP/CM-TO &              41 &   0.0 (0.0) &            33 & 0.05 (0.01) &                 51 &   0.0 (0.0) &              37 &  0.4 (0.03) &              32 & 0.22 (0.02) &                        34 & 0.14 (0.01) &                            25 &  0.17 (0.0) \\
      SA-MLP/CM-LE &              42 &   0.0 (0.0) &            32 & 0.05 (0.01) &                 52 &   0.0 (0.0) &              38 &  0.4 (0.03) &              31 & 0.22 (0.02) &                        51 &  0.11 (0.0) &                            52 &  0.11 (0.0) \\
  SA-MLP/CM-LE + B &              43 &   0.0 (0.0) &            35 & 0.05 (0.01) &                 36 &   0.0 (0.0) &              52 &  0.4 (0.03) &              21 & 0.32 (0.07) &                        49 &  0.11 (0.0) &                            46 &  0.11 (0.0) \\
      SA-MLP/CM-TO &              53 &   0.0 (0.0) &            49 &  0.01 (0.0) &                 35 &   0.0 (0.0) &              50 &  0.4 (0.03) &              26 & 0.22 (0.02) &                        52 &  0.11 (0.0) &                            45 &  0.11 (0.0) \\
       C-MLP/CM-LE &              45 &   0.0 (0.0) &            31 &  0.06 (0.0) &                 50 &   0.0 (0.0) &              49 &  0.4 (0.03) &              36 &  0.2 (0.02) &                        24 & 0.19 (0.02) &                            35 & 0.13 (0.01) \\
    GRU-MLP/MC-TEM &               6 & 0.14 (0.02) &            21 & 0.17 (0.02) &                 17 & 0.17 (0.03) &               6 & 0.53 (0.01) &              47 & 0.06 (0.04) &                         5 &  0.27 (0.0) &                             2 &  0.25 (0.0) \\
GRU-MLP/MC-TEM + B &               8 & 0.13 (0.02) &             6 & 0.38 (0.01) &                  6 & 0.52 (0.04) &              13 & 0.49 (0.03) &              10 & 0.69 (0.03) &                         6 &  0.27 (0.0) &                             9 &  0.24 (0.0) \\
     GRU-MLP/MC-TO &              25 &  0.01 (0.0) &            30 & 0.06 (0.01) &                 34 &  0.01 (0.0) &              47 &  0.4 (0.03) &              51 &   0.0 (0.0) &                        25 & 0.18 (0.01) &                            23 & 0.18 (0.01) \\
     SA-MLP/MC-TEM &               9 & 0.12 (0.01) &            23 & 0.14 (0.02) &                 22 & 0.12 (0.03) &              11 &  0.5 (0.04) &              46 & 0.06 (0.04) &                        12 &  0.26 (0.0) &                            14 &  0.24 (0.0) \\
 SA-MLP/MC-TEM + B &               7 & 0.14 (0.03) &             7 & 0.37 (0.01) &                  7 & 0.49 (0.04) &              16 & 0.48 (0.04) &               4 & 0.73 (0.02) &                         7 &  0.27 (0.0) &                            10 &  0.24 (0.0) \\
      SA-MLP/MC-TO &              27 &  0.01 (0.0) &            45 &  0.01 (0.0) &                 39 &   0.0 (0.0) &              45 &  0.4 (0.03) &              45 & 0.06 (0.06) &                        38 & 0.12 (0.01) &                            33 & 0.15 (0.01) \\
     C-MLP/MC-TEMP &               2 & 0.23 (0.01) &            36 &  0.04 (0.0) &                 25 & 0.02 (0.01) &               5 & 0.53 (0.02) &              50 &   0.0 (0.0) &                        16 & 0.26 (0.01) &                            11 &  0.24 (0.0) \\
     GRU-RMTPP-TEM &               4 & 0.18 (0.02) &             4 & 0.39 (0.01) &                  3 & 0.57 (0.06) &              14 & 0.49 (0.04) &               3 & 0.76 (0.02) &                         8 &  0.27 (0.0) &                             3 &  0.25 (0.0) \\
 GRU-RMTPP-TEM + B &              12 & 0.11 (0.01) &             5 &  0.39 (0.0) &                  8 & 0.46 (0.09) &              15 & 0.48 (0.02) &               5 & 0.73 (0.03) &                         2 &  0.27 (0.0) &                            12 &  0.24 (0.0) \\
      GRU-RMTPP-TO &              21 &  0.01 (0.0) &            26 &  0.08 (0.0) &                 30 &  0.01 (0.0) &              43 &  0.4 (0.03) &              24 & 0.24 (0.03) &                        30 & 0.15 (0.01) &                            28 &  0.17 (0.0) \\
      SA-RMTPP-TEM &              13 &  0.1 (0.01) &            12 & 0.35 (0.01) &                  4 & 0.57 (0.07) &              19 & 0.45 (0.03) &               1 & 0.77 (0.01) &                        18 &  0.26 (0.0) &                            13 &  0.24 (0.0) \\
  SA-RMTPP-TEM + B &              19 & 0.04 (0.01) &             8 & 0.36 (0.01) &                 10 &  0.4 (0.12) &              18 & 0.47 (0.03) &              12 & 0.67 (0.02) &                        13 &  0.26 (0.0) &                             4 &  0.24 (0.0) \\
       SA-RMTPP-TO &              48 &   0.0 (0.0) &            50 &  0.01 (0.0) &                 53 &   0.0 (0.0) &              42 &  0.4 (0.03) &              33 & 0.22 (0.02) &                        42 &  0.11 (0.0) &                            40 &  0.11 (0.0) \\
      C-RMTPP-TEMP &              49 &   0.0 (0.0) &            52 &   0.0 (0.0) &                 37 &   0.0 (0.0) &              53 &  0.01 (0.0) &              37 &  0.2 (0.02) &                        53 &  0.04 (0.0) &                            53 &  0.04 (0.0) \\
      GRU-SA/CM-LE &              28 &  0.01 (0.0) &            37 &  0.04 (0.0) &                 38 &   0.0 (0.0) &              41 &  0.4 (0.03) &              25 & 0.22 (0.02) &                        29 & 0.16 (0.03) &                            51 &  0.11 (0.0) \\
  GRU-SA/CM-LE + B &              22 &  0.01 (0.0) &            42 &  0.03 (0.0) &                 32 &  0.01 (0.0) &              40 &  0.4 (0.03) &              22 &  0.3 (0.05) &                        32 & 0.14 (0.01) &                            31 & 0.16 (0.01) \\
      GRU-SA/CM-TO &              50 &   0.0 (0.0) &            41 &  0.03 (0.0) &                 47 &   0.0 (0.0) &              39 &  0.4 (0.03) &              52 &   0.0 (0.0) &                        41 &  0.11 (0.0) &                            41 &  0.11 (0.0) \\
       SA-SA/CM-LE &              51 &   0.0 (0.0) &            38 &  0.04 (0.0) &                 49 &   0.0 (0.0) &              51 &  0.4 (0.03) &              34 & 0.22 (0.02) &                        39 & 0.12 (0.01) &                            42 &  0.11 (0.0) \\
   SA-SA/CM-LE + B &              52 &   0.0 (0.0) &            40 &  0.03 (0.0) &                 29 &  0.01 (0.0) &              36 &  0.4 (0.03) &              23 & 0.25 (0.05) &                        33 & 0.14 (0.01) &                            34 & 0.15 (0.01) \\
       SA-SA/CM-TO &              44 &   0.0 (0.0) &            39 &  0.03 (0.0) &                 45 &   0.0 (0.0) &              44 &  0.4 (0.03) &              49 &   0.0 (0.0) &                        40 & 0.12 (0.01) &                            39 &  0.11 (0.0) \\
        C-SA/CM-LE &              38 &   0.0 (0.0) &            28 & 0.07 (0.01) &                 44 &   0.0 (0.0) &              48 &  0.4 (0.03) &              38 &  0.2 (0.02) &                        36 & 0.13 (0.02) &                            38 & 0.12 (0.01) \\
     GRU-SA/MC-TEM &              11 & 0.12 (0.03) &            20 & 0.18 (0.03) &                 16 & 0.17 (0.02) &               3 & 0.54 (0.02) &              48 & 0.02 (0.01) &                        17 & 0.26 (0.01) &                            19 & 0.23 (0.01) \\
 GRU-SA/MC-TEM + B &              15 & 0.08 (0.02) &            14 & 0.32 (0.01) &                  5 & 0.54 (0.03) &               1 & 0.56 (0.01) &               9 & 0.69 (0.03) &                        19 &  0.26 (0.0) &                            21 & 0.22 (0.01) \\
      GRU-SA/MC-TO &              47 &   0.0 (0.0) &            51 &   0.0 (0.0) &                 43 &   0.0 (0.0) &              31 &  0.4 (0.03) &              44 & 0.07 (0.06) &                        45 &  0.11 (0.0) &                            37 & 0.12 (0.01) \\
      SA-SA/MC-TEM &              18 & 0.06 (0.02) &            25 & 0.09 (0.02) &                 20 & 0.14 (0.03) &               8 & 0.52 (0.02) &              42 & 0.13 (0.05) &                        10 &  0.27 (0.0) &                            20 &  0.23 (0.0) \\
  SA-SA/MC-TEM + B &              14 &  0.1 (0.04) &            13 & 0.34 (0.01) &                  2 & 0.58 (0.04) &               7 & 0.52 (0.02) &               8 &  0.7 (0.01) &                        15 &  0.26 (0.0) &                            18 &  0.23 (0.0) \\
       SA-SA/MC-TO &              34 &   0.0 (0.0) &            53 &   0.0 (0.0) &                 40 &   0.0 (0.0) &              29 &  0.4 (0.03) &              53 &   0.0 (0.0) &                        48 &  0.11 (0.0) &                            36 & 0.12 (0.01) \\
      C-SA/MC-TEMP &              10 & 0.12 (0.03) &            22 & 0.16 (0.04) &                 27 & 0.01 (0.01) &              12 &  0.5 (0.04) &              43 & 0.07 (0.04) &                        11 &  0.27 (0.0) &                            16 &  0.24 (0.0) \\
           Poisson &              46 &   0.0 (0.0) &            44 &  0.01 (0.0) &                 33 &  0.01 (0.0) &              46 &  0.4 (0.03) &              40 &  0.2 (0.02) &                        47 &  0.11 (0.0) &                            48 &  0.11 (0.0) \\
            Hawkes &               1 &   0.3 (0.0) &            17 &  0.26 (0.0) &                  1 & 0.66 (0.02) &               4 & 0.53 (0.01) &              15 &  0.63 (0.0) &                         1 &  0.28 (0.0) &                             1 &  0.26 (0.0) \\ \\
\hline
\end{tabular}
\label{resultsmark}
\caption{Evaluation of the different neural TPP models on MOOC and LastFM. For each metric, best score is indicated in \textbf{bold}, second and third best results are indicated by the suffixes '*' and '**', respectively. Mean and standard error are computed over five runs on different random splits of the datasets.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\small
%\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccccc}
\hline \\
&  Time Cal. &  NLL Time &  NLL Mark &  F1-score \\ \\
\hline \\
        GRU-CP-TEM &      32.33 &     22.27 &     16.71 &     16.14 \\
    GRU-CP-TEM + B &      34.13 &     23.20 &     24.43 &     21.43 \\
         GRU-CP-TO &      33.47 &     19.27 &     28.71 &     29.43 \\
         SA-CP-TEM &      39.80 &     34.13 &     19.71 &     19.86 \\
     SA-CP-TEM + B &      40.40 &     34.13 &     26.29 &     23.71 \\
          SA-CP-TO &      47.20 &     46.67 &     34.29 &     37.00 \\
         C-CP-TEMP &      48.80 &     48.47 &     44.00 &     38.71 \\
       GRU-LNM-TEM &      10.47 &      4.47 &      4.43 &      5.29 \\
   GRU-LNM-TEM + B &      33.33 &      2.07 &     33.71 &     22.00 \\
        GRU-LNM-TO &       9.27 &      4.20 &     30.43 &     28.00 \\
        GRU-LNM-K1 &      27.80 &     20.40 &      5.57 &      6.00 \\
        SA-LNM-TEM &      10.60 &     10.47 &      9.43 &     12.29 \\
    SA-LNM-TEM + B &      31.67 &      2.07 &     31.14 &     21.57 \\
         SA-LNM-TO &      15.40 &     20.07 &     34.71 &     40.86 \\
         SA-LNM-K1 &      24.40 &     24.67 &     11.14 &     11.71 \\
        C-LNM-TEMP &      11.73 &     22.73 &     43.29 &     43.29 \\
     GRU-MLP/CM-LE &      34.40 &     33.80 &     23.14 &     28.57 \\
 GRU-MLP/CM-LE + B &      42.60 &     38.87 &     32.00 &     33.14 \\
     GRU-MLP/CM-TO &      37.13 &     36.13 &     33.86 &     36.14 \\
      SA-MLP/CM-LE &      40.87 &     43.60 &     32.86 &     42.57 \\
  SA-MLP/CM-LE + B &      44.00 &     41.13 &     35.00 &     40.29 \\
      SA-MLP/CM-TO &      36.80 &     44.40 &     35.86 &     44.29 \\
       C-MLP/CM-LE &      32.73 &     42.93 &     38.14 &     38.57 \\
    GRU-MLP/MC-TEM &      22.00 &     21.27 &     22.43 &     14.86 \\
GRU-MLP/MC-TEM + B &      21.13 &     15.13 &      7.29 &      8.29 \\
     GRU-MLP/MC-TO &      18.73 &     19.53 &     40.43 &     33.57 \\
     SA-MLP/MC-TEM &      23.73 &     29.73 &     25.00 &     19.57 \\
 SA-MLP/MC-TEM + B &      21.40 &     25.53 &     10.14 &      8.29 \\
      SA-MLP/MC-TO &      25.93 &     38.20 &     41.29 &     38.86 \\
     C-MLP/MC-TEMP &      26.27 &     43.07 &     33.57 &     20.71 \\
     GRU-RMTPP-TEM &      21.80 &     17.20 &      5.29 &      5.57 \\
 GRU-RMTPP-TEM + B &      19.47 &     16.20 &      8.00 &      8.43 \\
      GRU-RMTPP-TO &      21.27 &     14.60 &     30.57 &     28.86 \\
      SA-RMTPP-TEM &      25.60 &     27.00 &      9.14 &     11.43 \\
  SA-RMTPP-TEM + B &      24.53 &     26.00 &     14.86 &     12.00 \\
       SA-RMTPP-TO &      34.40 &     38.40 &     35.00 &     44.00 \\
      C-RMTPP-TEMP &      43.47 &     45.93 &     47.14 &     47.71 \\
      GRU-SA/CM-LE &      13.47 &     21.93 &     27.71 &     35.57 \\
  GRU-SA/CM-LE + B &      13.67 &     17.67 &     28.86 &     31.57 \\
      GRU-SA/CM-TO &      19.27 &     23.60 &     37.86 &     44.43 \\
       SA-SA/CM-LE &      15.73 &     24.80 &     30.14 &     43.43 \\
   SA-SA/CM-LE + B &      13.67 &     20.80 &     30.14 &     35.29 \\
       SA-SA/CM-TO &      21.87 &     29.13 &     33.29 &     42.86 \\
        C-SA/CM-LE &      21.73 &     30.00 &     39.86 &     38.57 \\
     GRU-SA/MC-TEM &      16.93 &     18.80 &     22.00 &     19.14 \\
 GRU-SA/MC-TEM + B &      15.07 &     10.00 &      9.71 &     12.00 \\
      GRU-SA/MC-TO &      38.93 &     44.20 &     39.00 &     42.57 \\
      SA-SA/MC-TEM &      19.20 &     23.40 &     24.86 &     20.43 \\
  SA-SA/MC-TEM + B &      18.73 &     14.67 &     10.43 &     11.00 \\
       SA-SA/MC-TO &      38.60 &     44.93 &     38.43 &     41.86 \\
      C-SA/MC-TEMP &      23.67 &     34.60 &     32.71 &     20.14 \\
           Poisson &      50.27 &     49.93 &     49.86 &     43.43 \\
            Hawkes &      21.13 &     24.60 &     17.14 &      5.71 \\ \\
\hline 
\end{tabular}
\label{resultsmark}
\caption{Average model's rank on the evaluation metrics.}
\end{table}





\restoregeometry






==> results_tabular_ranked.tex <==
\newgeometry{left=2cm,bottom=0cm,right=2cm, top=0.5cm}
\begin{landscape}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{cccccccccccc}
\hline \\
               0 &          NLL Time &                2 &       NLL Mark &                3 &        NLL Total &                4 &   Time Cal. &                6 &   Mark Cal. &                7 &    F1-score \\
\hline \\
     GRU-LNM + B & -1740.43 (176.37) &           Hawkes & 514.09 (16.24) &      GRU-LNM + B & -865.53 (158.29) &    GRU-LNM + BFC &  0.03 (0.0) &           Hawkes &  0.03 (0.0) &           Hawkes &   0.3 (0.0) \\
      SA-LNM + B &  -1527.56 (26.36) &  GRU-RMTPP + BFC & 696.66 (23.55) &           Hawkes &  -674.58 (39.99) &     SA-LNM + BFC & 0.04 (0.01) &          GRU-LNM & 0.22 (0.02) &  GRU-RMTPP + BFC & 0.19 (0.03) \\
   GRU-LNM + BFC &  -1325.08 (40.08) &          GRU-LNM & 698.85 (13.07) &       SA-LNM + B &  -653.68 (19.34) &          GRU-LNM & 0.04 (0.01) &       GRU-LNM-K1 & 0.25 (0.02) &          GRU-LNM & 0.18 (0.01) \\
    SA-LNM + BFC &  -1321.58 (56.78) &        GRU-RMTPP & 707.88 (21.42) &          GRU-LNM &  -619.78 (30.07) &           SA-LNM & 0.04 (0.01) & GRU-MLP/MC + BFC & 0.25 (0.02) &        GRU-RMTPP & 0.18 (0.02) \\
         GRU-LNM &  -1318.62 (40.13) &       GRU-LNM-K1 & 708.17 (20.48) &       GRU-LNM-K1 &  -601.45 (38.87) &       SA-LNM + B & 0.05 (0.01) &        SA-MLP/MC & 0.27 (0.03) &       GRU-LNM-K1 & 0.17 (0.02) \\
          SA-LNM &  -1312.68 (40.11) &    GRU-LNM + BFC & 729.82 (18.02) &    GRU-LNM + BFC &  -595.26 (24.37) &      GRU-LNM + B & 0.05 (0.01) &       GRU-MLP/MC & 0.27 (0.02) & GRU-MLP/MC + BFC & 0.17 (0.02) \\
      GRU-LNM-K1 &  -1309.62 (55.07) & GRU-MLP/MC + BFC & 748.04 (18.35) &     SA-LNM + BFC &   -548.4 (31.61) &       GRU-LNM-K1 & 0.06 (0.01) &  GRU-RMTPP + BFC & 0.27 (0.03) &    SA-MLP/MC + B & 0.14 (0.03) \\
   GRU-SA/CM + B &  -1259.31 (55.19) &    GRU-RMTPP + B & 750.69 (32.06) &           SA-LNM &  -535.76 (26.57) &    GRU-SA/CM + B &  0.12 (0.0) &    GRU-LNM + BFC & 0.28 (0.03) &   SA-SA/MC + BFC & 0.14 (0.02) \\
    SA-SA/CM + B &  -1244.43 (60.21) &       GRU-MLP/MC & 768.24 (33.55) &    GRU-SA/CM + B &  -392.98 (27.03) &     SA-SA/CM + B & 0.13 (0.01) &   SA-SA/MC + BFC &  0.3 (0.04) &    GRU-LNM + BFC & 0.14 (0.01) \\
 GRU-SA/CM + BFC &  -1234.37 (54.45) &   GRU-MLP/MC + B & 769.23 (31.98) &  GRU-SA/CM + BFC &   -378.0 (26.34) &  GRU-SA/CM + BFC & 0.13 (0.01) &        GRU-RMTPP &  0.3 (0.01) &       GRU-MLP/MC & 0.14 (0.02) \\
       GRU-SA/CM &   -1221.6 (58.26) &     SA-LNM + BFC & 773.18 (26.78) &     SA-SA/CM + B &  -376.53 (32.26) &   SA-SA/CM + BFC & 0.15 (0.01) &  SA-MLP/MC + BFC &  0.3 (0.03) &   GRU-MLP/MC + B & 0.13 (0.02) \\
  SA-SA/CM + BFC &  -1214.79 (55.86) &           SA-LNM & 776.92 (21.09) &     SA-SA/MC + B &   -374.27 (24.4) &        GRU-SA/CM & 0.15 (0.01) &    GRU-RMTPP + B & 0.31 (0.02) &        GRU-SA/MC & 0.12 (0.03) \\
        SA-SA/CM &  -1195.78 (52.64) &   SA-SA/MC + BFC &  778.0 (32.53) &        GRU-SA/CM &   -371.7 (31.88) &         SA-SA/CM & 0.16 (0.01) &   GRU-MLP/MC + B & 0.31 (0.01) &        SA-MLP/MC & 0.12 (0.01) \\
    SA-SA/MC + B &  -1191.06 (54.39) &         SA-RMTPP & 787.54 (23.83) &    GRU-RMTPP + B &  -367.34 (25.96) &         SA-SA/MC & 0.16 (0.01) &  GRU-SA/MC + BFC & 0.33 (0.02) &  SA-MLP/MC + BFC & 0.12 (0.02) \\
          Hawkes &  -1188.67 (55.46) &    SA-MLP/MC + B & 793.71 (26.11) &        GRU-RMTPP &  -351.83 (39.36) &     SA-SA/MC + B & 0.18 (0.01) &    SA-MLP/MC + B & 0.33 (0.01) &    GRU-RMTPP + B & 0.11 (0.01) \\
   GRU-SA/MC + B &  -1151.63 (44.04) &  SA-MLP/MC + BFC & 794.56 (25.69) &   SA-SA/CM + BFC &  -351.82 (26.74) &        GRU-SA/MC & 0.18 (0.02) &           SA-LNM & 0.33 (0.03) &  GRU-SA/MC + BFC & 0.11 (0.03) \\
 GRU-SA/MC + BFC &  -1134.99 (54.28) &  GRU-SA/MC + BFC & 800.88 (27.56) &    GRU-SA/MC + B &  -339.47 (17.91) &    GRU-SA/MC + B & 0.19 (0.01) &         SA-RMTPP & 0.35 (0.03) &         SA-RMTPP &  0.1 (0.01) \\
        SA-SA/MC &   -1129.5 (43.03) &        GRU-SA/MC & 806.55 (17.88) &   SA-SA/MC + BFC &  -338.76 (33.73) &  GRU-SA/MC + BFC & 0.19 (0.02) &        GRU-SA/MC & 0.36 (0.02) &     SA-SA/MC + B &  0.1 (0.04) \\
   GRU-RMTPP + B &  -1118.02 (52.48) &        SA-MLP/MC & 808.01 (28.29) &  GRU-RMTPP + BFC &   -336.8 (32.13) &   SA-SA/MC + BFC &  0.2 (0.01) &         SA-SA/MC & 0.36 (0.03) &    GRU-SA/MC + B & 0.08 (0.02) \\
  SA-SA/MC + BFC &  -1116.77 (62.51) &   SA-RMTPP + BFC & 811.27 (32.47) &  GRU-SA/MC + BFC &   -334.12 (29.4) &           Hawkes &  0.21 (0.0) &     SA-LNM + BFC & 0.37 (0.03) &     SA-LNM + BFC & 0.08 (0.01) \\
      GRU-MLP/CM &   -1096.25 (52.1) &    GRU-SA/MC + B & 812.16 (26.32) &         SA-SA/CM &  -332.02 (24.57) &       GRU-MLP/CM & 0.23 (0.01) &    GRU-SA/MC + B & 0.38 (0.04) &           SA-LNM & 0.08 (0.01) \\
  GRU-MLP/MC + B &   -1093.16 (59.2) &     SA-SA/MC + B & 816.79 (31.72) &   GRU-MLP/MC + B &  -323.92 (28.57) &       GRU-MLP/MC &  0.24 (0.0) &   SA-RMTPP + BFC & 0.41 (0.03) &   SA-RMTPP + BFC & 0.06 (0.02) \\
       GRU-SA/MC &   -1083.46 (65.8) &           GRU-CP & 818.67 (21.56) & GRU-MLP/MC + BFC &   -303.37 (40.7) &    GRU-RMTPP + B &  0.25 (0.0) &     SA-SA/MC + B & 0.42 (0.02) &         SA-SA/MC & 0.06 (0.02) \\
          GRU-CP &   -1060.32 (44.6) &     SA-RMTPP + B &  826.77 (30.2) &         SA-SA/MC &   -294.33 (22.0) & GRU-MLP/MC + BFC & 0.25 (0.01) &     SA-RMTPP + B & 0.43 (0.03) &     SA-RMTPP + B & 0.04 (0.01) \\
       GRU-RMTPP &  -1059.71 (55.94) &     GRU-CP + BFC & 828.27 (17.72) &       GRU-MLP/MC &  -284.46 (35.48) &   GRU-MLP/MC + B & 0.25 (0.01) &           GRU-CP & 0.45 (0.01) &     GRU-CP + BFC &  0.03 (0.0) \\
      GRU-MLP/MC &  -1052.69 (62.83) &         SA-SA/MC & 835.17 (29.13) &        GRU-SA/MC &    -276.9 (51.1) &        SA-MLP/MC & 0.25 (0.01) &     GRU-CP + BFC & 0.46 (0.01) &           GRU-CP &  0.03 (0.0) \\
GRU-MLP/MC + BFC &  -1051.41 (55.12) &        GRU-SA/CM &   849.9 (26.6) &           GRU-CP &   -241.65 (23.1) &  GRU-RMTPP + BFC & 0.26 (0.01) &            SA-CP & 0.48 (0.01) &            SA-CP &  0.01 (0.0) \\
    SA-RMTPP + B &  -1038.74 (50.37) &            SA-CP & 850.92 (28.09) &         SA-RMTPP &  -235.57 (25.33) &        GRU-RMTPP & 0.26 (0.01) &       GRU-CP + B &  0.49 (0.0) &       GRU-MLP/CM &  0.01 (0.0) \\
 GRU-RMTPP + BFC &  -1033.46 (41.75) &       GRU-CP + B & 853.67 (24.72) &       GRU-MLP/CM &   -231.7 (34.19) &    SA-MLP/MC + B & 0.26 (0.01) &        GRU-SA/CM &  0.49 (0.0) &    GRU-SA/CM + B &  0.01 (0.0) \\
    GRU-CP + BFC &  -1027.21 (30.36) &      SA-CP + BFC & 854.45 (31.36) &    SA-MLP/MC + B &  -213.06 (27.79) &  SA-MLP/MC + BFC & 0.26 (0.01) &      SA-CP + BFC & 0.49 (0.01) &        GRU-SA/CM &  0.01 (0.0) \\
        SA-RMTPP &  -1023.11 (46.43) &  GRU-SA/CM + BFC & 856.37 (29.88) &     SA-RMTPP + B &  -211.97 (21.84) &     SA-RMTPP + B & 0.27 (0.01) &       SA-LNM + B &   0.5 (0.0) &      SA-CP + BFC &  0.01 (0.0) \\
      GRU-CP + B &  -1022.67 (43.59) & GRU-MLP/CM + BFC & 857.23 (22.96) &  SA-MLP/MC + BFC &  -209.99 (32.99) &         SA-RMTPP & 0.27 (0.01) &          Poisson &   0.5 (0.0) &       GRU-CP + B &  0.01 (0.0) \\
  SA-RMTPP + BFC &  -1007.29 (61.17) &   SA-SA/CM + BFC & 862.96 (29.36) &     GRU-CP + BFC &  -198.95 (16.76) &   SA-RMTPP + BFC & 0.28 (0.01) &      GRU-LNM + B &   0.5 (0.0) &   SA-SA/CM + BFC &  0.01 (0.0) \\
   SA-MLP/MC + B &  -1006.77 (53.09) &         SA-SA/CM & 863.77 (28.84) &   SA-RMTPP + BFC &  -196.02 (34.62) &           GRU-CP & 0.28 (0.01) &   SA-SA/CM + BFC &   0.5 (0.0) &  GRU-SA/CM + BFC &  0.01 (0.0) \\
GRU-MLP/CM + BFC &  -1004.56 (54.39) &       GRU-MLP/CM & 864.56 (29.49) &        SA-MLP/MC &  -194.12 (19.82) & GRU-MLP/CM + BFC & 0.28 (0.01) &     SA-SA/CM + B &   0.5 (0.0) & GRU-MLP/CM + BFC &  0.01 (0.0) \\
 SA-MLP/MC + BFC &  -1004.55 (54.12) &        SA-CP + B &  865.9 (28.31) &       GRU-CP + B &   -169.0 (26.12) &     GRU-CP + BFC &  0.28 (0.0) &         SA-SA/CM &   0.5 (0.0) &          Poisson &   0.0 (0.0) \\
       SA-MLP/MC &  -1002.13 (46.68) &    GRU-SA/CM + B & 866.33 (29.31) & GRU-MLP/CM + BFC &   -147.32 (35.5) &       GRU-CP + B & 0.28 (0.01) &   GRU-MLP/CM + B &   0.5 (0.0) &      GRU-LNM + B &   0.0 (0.0) \\
       SA-CP + B &   -962.07 (42.44) &     SA-SA/CM + B &  867.9 (28.66) &            SA-CP &   -97.68 (27.17) &            SA-CP &  0.3 (0.01) & GRU-MLP/CM + BFC &   0.5 (0.0) &     SA-SA/CM + B &   0.0 (0.0) \\
           SA-CP &    -948.6 (52.53) &   GRU-MLP/CM + B &  870.6 (29.91) &        SA-CP + B &   -96.17 (16.82) &        SA-CP + B &   0.3 (0.0) &    GRU-SA/CM + B &   0.5 (0.0) &         SA-SA/CM &   0.0 (0.0) \\
     SA-CP + BFC &    -921.17 (56.8) &  SA-MLP/CM + BFC & 870.93 (30.09) &      SA-CP + BFC &   -66.72 (25.78) &      SA-CP + BFC & 0.31 (0.01) &  GRU-SA/CM + BFC &   0.5 (0.0) &   GRU-MLP/CM + B &   0.0 (0.0) \\
  GRU-MLP/CM + B &   -912.22 (80.24) &    SA-MLP/CM + B & 870.94 (29.97) &   GRU-MLP/CM + B &   -41.62 (51.03) &        SA-MLP/CM & 0.32 (0.01) &  SA-MLP/CM + BFC &   0.5 (0.0) &  SA-MLP/CM + BFC &   0.0 (0.0) \\
   SA-MLP/CM + B &   -826.12 (34.58) &        SA-MLP/CM & 871.02 (30.02) &    SA-MLP/CM + B &     44.82 (5.82) &   GRU-MLP/CM + B &  0.32 (0.0) &    SA-MLP/CM + B &   0.5 (0.0) &    SA-MLP/CM + B &   0.0 (0.0) \\
 SA-MLP/CM + BFC &   -821.94 (34.65) &          Poisson & 873.82 (30.24) &  SA-MLP/CM + BFC &     48.99 (5.84) &    SA-MLP/CM + B & 0.33 (0.01) &        SA-MLP/CM &   0.5 (0.0) &        SA-MLP/CM &   0.0 (0.0) \\
       SA-MLP/CM &    -818.12 (34.6) &       SA-LNM + B & 873.88 (29.62) &        SA-MLP/CM &     52.91 (5.73) &  SA-MLP/CM + BFC & 0.33 (0.01) &       GRU-MLP/CM &   0.5 (0.0) &       SA-LNM + B &   0.0 (0.0) \\
         Poisson &   -782.72 (33.38) &      GRU-LNM + B &  874.9 (30.05) &          Poisson &      91.1 (4.68) &          Poisson & 0.35 (0.01) &        SA-CP + B &   0.5 (0.0) &        SA-CP + B &   0.0 (0.0) \\ \\
\hline
\end{tabular}
\label{resultsmark}
\caption{LastFM}
\end{table}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{cccccccccccc}
\hline \\
               0 &        NLL Time &                2 &      NLL Mark &                3 &      NLL Total &                4 &   Time Cal. &                6 &   Mark Cal. &                7 &    F1-score \\
\hline \\
     GRU-LNM + B &  -305.89 (3.52) &    GRU-LNM + BFC &  87.15 (0.98) &    GRU-LNM + BFC & -218.21 (2.38) &     SA-LNM + BFC &   0.0 (0.0) &    GRU-RMTPP + B & 0.06 (0.01) &       GRU-LNM-K1 &   0.4 (0.0) \\
   GRU-LNM + BFC &   -305.36 (3.0) &       GRU-LNM-K1 &  87.78 (1.51) &      GRU-LNM + B & -217.77 (2.52) &       SA-LNM + B &   0.0 (0.0) &  GRU-RMTPP + BFC & 0.07 (0.01) &          GRU-LNM &   0.4 (0.0) \\
      SA-LNM + B &  -303.99 (3.79) &          GRU-LNM &  87.98 (0.99) &       SA-LNM + B & -211.97 (2.59) &      GRU-LNM + B &   0.0 (0.0) &   GRU-MLP/MC + B & 0.08 (0.02) &      GRU-LNM + B &   0.4 (0.0) \\
    SA-LNM + BFC &  -303.47 (3.53) &      GRU-LNM + B &  88.11 (1.09) &     SA-LNM + BFC &  -211.0 (2.06) &    GRU-LNM + BFC &   0.0 (0.0) &     SA-RMTPP + B & 0.09 (0.02) &  GRU-RMTPP + BFC &   0.4 (0.0) \\
         GRU-LNM &  -294.55 (4.89) &  GRU-RMTPP + BFC &  88.27 (0.87) &          GRU-LNM & -206.58 (4.49) &          GRU-LNM & 0.02 (0.01) &    GRU-LNM + BFC & 0.09 (0.01) &    GRU-LNM + BFC &  0.4 (0.01) \\
          SA-LNM &  -292.56 (4.85) &        GRU-RMTPP &  88.46 (1.89) &           SA-LNM & -199.38 (4.21) &           SA-LNM & 0.02 (0.01) &       GRU-LNM-K1 &  0.1 (0.01) &        GRU-RMTPP & 0.39 (0.01) \\
      GRU-LNM-K1 &  -281.56 (3.63) &    GRU-RMTPP + B &  88.58 (1.71) &       GRU-LNM-K1 & -193.78 (2.47) &       GRU-LNM-K1 &  0.04 (0.0) &          GRU-LNM &  0.1 (0.01) &    GRU-RMTPP + B &  0.39 (0.0) \\
   GRU-SA/MC + B &  -260.07 (3.92) &       SA-LNM + B &  92.02 (1.36) &     SA-SA/MC + B & -161.11 (1.41) &       GRU-MLP/CM &  0.05 (0.0) &   SA-RMTPP + BFC & 0.11 (0.01) &   GRU-MLP/MC + B & 0.38 (0.01) \\
    SA-SA/MC + B &   -259.7 (3.24) &     SA-LNM + BFC &  92.47 (1.53) &    GRU-SA/MC + B & -158.83 (2.48) &         SA-SA/CM &  0.05 (0.0) &        GRU-RMTPP & 0.11 (0.02) &    SA-MLP/MC + B & 0.37 (0.01) \\
    SA-SA/CM + B &   -251.9 (3.94) &     SA-RMTPP + B &  93.06 (0.86) &   GRU-MLP/MC + B &  -119.2 (6.15) &        GRU-SA/CM &  0.05 (0.0) &         SA-RMTPP & 0.12 (0.02) &     SA-RMTPP + B & 0.36 (0.01) \\
   GRU-SA/CM + B &  -251.39 (1.23) &           SA-LNM &  93.17 (1.41) &    SA-MLP/MC + B & -115.15 (6.89) &   SA-SA/CM + BFC &   0.1 (0.0) &      GRU-LNM + B & 0.13 (0.01) &     SA-LNM + BFC & 0.36 (0.01) \\
 GRU-SA/CM + BFC &  -238.61 (3.19) &   SA-RMTPP + BFC &  93.98 (0.88) &    GRU-RMTPP + B &  -113.5 (8.68) &  GRU-SA/CM + BFC &  0.1 (0.01) &    SA-MLP/MC + B & 0.13 (0.02) &       SA-LNM + B &  0.36 (0.0) \\
  SA-SA/CM + BFC &  -236.87 (3.75) &         SA-RMTPP &  94.23 (2.34) &     SA-RMTPP + B & -111.83 (5.44) &    GRU-SA/MC + B & 0.14 (0.01) &       SA-LNM + B & 0.14 (0.02) &         SA-RMTPP & 0.35 (0.01) \\
        SA-SA/CM &  -228.99 (2.83) &           GRU-CP &  96.55 (1.44) &   SA-RMTPP + BFC &  -111.6 (2.93) &    GRU-SA/CM + B & 0.14 (0.01) &     SA-LNM + BFC & 0.15 (0.02) &           SA-LNM & 0.35 (0.01) \\
      GRU-MLP/CM &  -228.56 (4.47) &            SA-CP &  97.51 (0.99) &  GRU-RMTPP + BFC &  -111.4 (6.24) &     SA-SA/CM + B &  0.14 (0.0) &           SA-LNM & 0.16 (0.01) &   SA-RMTPP + BFC &  0.35 (0.0) \\
       GRU-SA/CM &  -225.86 (1.84) &   GRU-MLP/MC + B &  98.27 (3.09) &           Hawkes & -105.83 (2.27) &     SA-SA/MC + B &  0.15 (0.0) &           GRU-CP & 0.16 (0.02) &     SA-SA/MC + B & 0.34 (0.01) \\
          Hawkes &  -220.82 (3.57) &     SA-SA/MC + B &    98.6 (2.1) &       GRU-MLP/CM & -100.39 (3.13) &  GRU-SA/MC + BFC & 0.15 (0.01) & GRU-MLP/MC + BFC & 0.18 (0.02) &    GRU-SA/MC + B & 0.32 (0.01) \\
   SA-MLP/MC + B &  -218.45 (3.98) &    GRU-SA/MC + B & 101.24 (1.54) &  GRU-SA/CM + BFC &  -78.95 (2.49) &   SA-SA/MC + BFC & 0.16 (0.01) &           Hawkes & 0.19 (0.01) & GRU-MLP/MC + BFC &  0.3 (0.01) \\
  GRU-MLP/MC + B &  -217.47 (4.61) &    SA-MLP/MC + B &  103.3 (4.38) &    GRU-SA/CM + B &  -75.09 (1.73) &        SA-MLP/CM & 0.17 (0.02) &       GRU-MLP/MC & 0.19 (0.03) &            SA-CP &  0.29 (0.0) \\
  SA-RMTPP + BFC &  -205.59 (3.38) &     GRU-CP + BFC & 104.36 (1.25) &     SA-SA/CM + B &  -74.74 (1.29) &        GRU-SA/MC &  0.2 (0.02) &  SA-MLP/MC + BFC &  0.2 (0.01) &           GRU-CP & 0.29 (0.01) \\
    SA-RMTPP + B &  -204.89 (5.41) &      SA-CP + BFC & 105.03 (1.66) &   SA-SA/CM + BFC &  -73.19 (1.64) &           Hawkes &  0.23 (0.0) &            SA-CP & 0.21 (0.03) &     GRU-CP + BFC & 0.28 (0.01) \\
   GRU-RMTPP + B &   -202.08 (9.0) &           Hawkes & 114.99 (1.54) &        GRU-RMTPP &  -67.75 (1.38) &   GRU-MLP/MC + B & 0.24 (0.01) &        SA-MLP/MC & 0.23 (0.01) &      SA-CP + BFC & 0.28 (0.01) \\
 GRU-RMTPP + BFC &  -199.67 (5.97) &  GRU-SA/MC + BFC & 117.45 (1.67) &         SA-SA/CM &  -61.57 (1.45) &    SA-MLP/MC + B &  0.24 (0.0) &     GRU-CP + BFC & 0.23 (0.01) &           Hawkes &  0.26 (0.0) \\
 GRU-SA/MC + BFC &  -174.93 (5.31) &        SA-CP + B & 117.77 (3.18) &         SA-RMTPP &  -61.41 (1.42) & GRU-MLP/CM + BFC & 0.26 (0.03) &     SA-SA/MC + B & 0.24 (0.03) &  GRU-SA/MC + BFC & 0.26 (0.01) \\
  SA-SA/MC + BFC &  -168.88 (6.22) &       GRU-CP + B & 118.26 (2.51) &        GRU-SA/CM &  -58.12 (1.91) & GRU-MLP/MC + BFC & 0.26 (0.01) &      SA-CP + BFC & 0.24 (0.01) &   SA-SA/MC + BFC & 0.26 (0.01) \\
       GRU-RMTPP &  -156.22 (2.53) &   SA-SA/MC + BFC & 118.84 (2.73) &  GRU-SA/MC + BFC &  -57.49 (4.62) &   SA-RMTPP + BFC &  0.27 (0.0) &    GRU-SA/MC + B & 0.25 (0.01) &       GRU-CP + B &  0.25 (0.0) \\
        SA-RMTPP &  -155.64 (2.76) & GRU-MLP/CM + BFC & 124.38 (3.44) &   SA-SA/MC + BFC &  -50.03 (7.33) &     SA-RMTPP + B & 0.27 (0.01) &       GRU-CP + B & 0.26 (0.02) &  SA-MLP/MC + BFC & 0.25 (0.02) \\
   SA-MLP/CM + B & -142.27 (28.98) & GRU-MLP/MC + BFC & 125.23 (3.54) & GRU-MLP/MC + BFC &   -8.27 (3.42) &    GRU-RMTPP + B & 0.27 (0.01) &  GRU-SA/MC + BFC & 0.28 (0.02) &        SA-CP + B & 0.24 (0.01) \\
GRU-MLP/MC + BFC &  -133.51 (5.01) &       GRU-MLP/CM & 128.17 (6.99) &           GRU-CP &   -4.74 (0.36) &  GRU-RMTPP + BFC & 0.27 (0.01) &   SA-SA/MC + BFC & 0.29 (0.02) &        GRU-SA/MC & 0.18 (0.03) \\
 SA-MLP/MC + BFC &  -127.37 (4.46) &  SA-MLP/MC + BFC & 129.61 (4.61) &            SA-CP &    1.27 (0.33) &  SA-MLP/MC + BFC & 0.28 (0.01) &        SA-CP + B & 0.31 (0.02) &       GRU-MLP/MC & 0.17 (0.02) \\
       SA-MLP/CM & -115.45 (23.25) &  SA-MLP/CM + BFC & 141.71 (2.09) &  SA-MLP/MC + BFC &    2.24 (6.17) &         SA-SA/MC & 0.28 (0.02) &        GRU-SA/MC & 0.34 (0.04) &        SA-MLP/MC & 0.14 (0.02) \\
GRU-MLP/CM + BFC & -113.04 (20.57) &        GRU-SA/MC & 142.04 (5.47) &     GRU-CP + BFC &    6.75 (1.28) &  SA-MLP/CM + BFC &   0.3 (0.0) & GRU-MLP/CM + BFC & 0.41 (0.03) &       GRU-MLP/CM & 0.14 (0.03) \\
          GRU-CP &  -101.29 (1.46) &   GRU-MLP/CM + B & 148.46 (5.88) &      SA-CP + BFC &      9.0 (0.6) &    SA-MLP/CM + B & 0.31 (0.04) &         SA-SA/MC & 0.42 (0.03) & GRU-MLP/CM + BFC & 0.13 (0.02) \\
    GRU-CP + BFC &    -97.6 (0.93) &        SA-MLP/CM & 152.09 (2.54) & GRU-MLP/CM + BFC &   11.35 (21.4) &       GRU-MLP/MC & 0.32 (0.01) &       GRU-MLP/CM & 0.44 (0.04) &         SA-SA/MC & 0.09 (0.02) \\
           SA-CP &   -96.24 (1.12) &       GRU-MLP/MC &  155.94 (5.5) &    SA-MLP/CM + B &   17.6 (25.29) &        SA-MLP/MC & 0.32 (0.01) &   SA-SA/CM + BFC & 0.45 (0.01) &  SA-MLP/CM + BFC & 0.07 (0.01) \\
     SA-CP + BFC &   -96.02 (1.51) &        SA-MLP/MC & 158.58 (5.88) &       GRU-CP + B &   23.94 (1.58) &         SA-RMTPP &  0.32 (0.0) &        GRU-SA/CM &  0.46 (0.0) &   GRU-MLP/CM + B & 0.05 (0.02) \\
      GRU-CP + B &   -94.32 (1.49) &  GRU-SA/CM + BFC & 159.67 (2.75) &        SA-CP + B &   25.39 (2.29) &        GRU-RMTPP &  0.32 (0.0) &  GRU-SA/CM + BFC & 0.46 (0.01) &        SA-MLP/CM & 0.05 (0.01) \\
       SA-CP + B &   -92.38 (1.17) &    SA-MLP/CM + B & 159.87 (7.03) &        SA-MLP/CM &  36.64 (21.89) &   GRU-MLP/CM + B &  0.38 (0.0) &    GRU-SA/CM + B & 0.46 (0.01) &   SA-SA/CM + BFC &  0.05 (0.0) \\
  GRU-MLP/CM + B &   -91.99 (1.18) &         SA-SA/MC & 163.39 (6.32) &   GRU-MLP/CM + B &   56.47 (5.31) &           GRU-CP &  0.39 (0.0) &   GRU-MLP/CM + B & 0.47 (0.01) &    SA-MLP/CM + B & 0.05 (0.01) \\
 SA-MLP/CM + BFC &   -81.62 (0.67) &   SA-SA/CM + BFC & 163.68 (3.06) &  SA-MLP/CM + BFC &   60.09 (1.64) &            SA-CP &  0.39 (0.0) &     SA-SA/CM + B &  0.47 (0.0) &        GRU-SA/CM &  0.04 (0.0) \\
       GRU-SA/MC &   -68.61 (9.45) &         SA-SA/CM & 167.42 (1.46) &        GRU-SA/MC &  73.44 (12.27) &     GRU-CP + BFC &  0.39 (0.0) &    SA-MLP/CM + B & 0.48 (0.01) &  GRU-SA/CM + BFC &  0.04 (0.0) \\
         Poisson &   -51.74 (1.01) &        GRU-SA/CM &  167.74 (2.5) &         SA-SA/MC & 125.43 (14.98) &       GRU-CP + B &  0.39 (0.0) &        SA-MLP/CM &  0.48 (0.0) &         SA-SA/CM &  0.04 (0.0) \\
        SA-SA/MC &   -37.96 (8.85) &    GRU-SA/CM + B &  176.3 (2.28) &          Poisson &  136.39 (1.39) &      SA-CP + BFC &  0.39 (0.0) &         SA-SA/CM & 0.48 (0.01) &     SA-SA/CM + B &  0.03 (0.0) \\
       SA-MLP/MC &   -21.86 (5.96) &     SA-SA/CM + B & 177.16 (2.71) &       GRU-MLP/MC &  136.68 (8.21) &          Poisson &   0.4 (0.0) &  SA-MLP/CM + BFC &  0.48 (0.0) &    GRU-SA/CM + B &  0.03 (0.0) \\
      GRU-MLP/MC &   -19.26 (3.75) &          Poisson & 188.13 (2.37) &        SA-MLP/MC & 136.72 (11.32) &        SA-CP + B &   0.4 (0.0) &          Poisson &   0.5 (0.0) &          Poisson &  0.01 (0.0) \\ \\
\hline 
\end{tabular}
\label{resultsmark}
\caption{MOOC}
\end{table}



\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccccccccccc}
\hline \\
                 0 &        NLL Time &                2 &        NLL Mark &                3 &       NLL Total &                4 &   Time Cal. &                6 &   Mark Cal. &                7 &    F1-score \\
\hline \\
      SA-LNM + BFC & -286.27 (25.62) &           Hawkes &  144.69 (12.45) &    GRU-LNM + BFC &    -66.1 (9.55) &       SA-LNM + B &  0.03 (0.0) &           Hawkes & 0.11 (0.03) &           Hawkes & 0.66 (0.02) \\
       GRU-LNM + B & -285.22 (29.21) &   GRU-MLP/MC + B &  145.13 (17.34) &     SA-LNM + BFC &  -58.78 (14.53) &      GRU-LNM + B & 0.04 (0.01) &    SA-MLP/MC + B & 0.16 (0.01) &     SA-SA/MC + B & 0.58 (0.04) \\
     GRU-LNM + BFC & -281.63 (17.43) &     SA-SA/MC + B &   149.4 (10.93) &     SA-SA/MC + B &  -42.47 (16.03) &    GRU-LNM + BFC & 0.04 (0.01) &    GRU-SA/MC + B & 0.17 (0.01) &        GRU-RMTPP & 0.57 (0.06) \\
        SA-LNM + B & -277.08 (27.38) &    SA-MLP/MC + B &  149.89 (19.86) &    GRU-SA/MC + B &   -37.1 (15.22) &     SA-LNM + BFC & 0.04 (0.01) &     SA-SA/MC + B & 0.18 (0.02) &         SA-RMTPP & 0.57 (0.07) \\
            SA-LNM & -266.68 (23.24) &    GRU-SA/MC + B &  150.91 (13.55) &          GRU-LNM &  -13.74 (21.04) &         SA-SA/CM & 0.09 (0.01) &    GRU-LNM + BFC & 0.23 (0.04) &    GRU-SA/MC + B & 0.54 (0.03) \\
           GRU-LNM & -253.64 (24.06) &  GRU-SA/MC + BFC &  175.71 (14.23) &      GRU-LNM + B &   -7.93 (10.74) &        GRU-SA/CM &  0.1 (0.01) &        GRU-RMTPP & 0.24 (0.06) &    GRU-LNM + BFC & 0.53 (0.05) \\
        GRU-LNM-K1 & -241.79 (34.54) &   SA-SA/MC + BFC &  185.76 (11.12) &           SA-LNM &   -6.37 (18.79) &  GRU-SA/CM + BFC & 0.11 (0.01) &         SA-RMTPP & 0.24 (0.07) &   GRU-MLP/MC + B & 0.52 (0.04) \\
      SA-SA/MC + B & -191.88 (17.52) &  SA-MLP/MC + BFC &  196.88 (22.67) &       SA-LNM + B &   12.08 (13.75) &           SA-LNM & 0.12 (0.04) &   GRU-MLP/MC + B & 0.26 (0.02) &    SA-MLP/MC + B & 0.49 (0.04) \\
     GRU-SA/MC + B & -188.01 (21.17) & GRU-MLP/MC + BFC &  209.92 (11.35) &       GRU-LNM-K1 &   19.53 (21.76) &   SA-SA/CM + BFC & 0.15 (0.02) &     SA-LNM + BFC & 0.26 (0.05) &    GRU-RMTPP + B & 0.46 (0.09) \\
     GRU-SA/CM + B &  -170.29 (31.4) &    GRU-LNM + BFC &  215.53 (19.62) &   GRU-MLP/MC + B &   23.24 (18.46) &          GRU-LNM & 0.15 (0.04) &  GRU-SA/MC + BFC & 0.26 (0.04) &   SA-RMTPP + BFC &  0.46 (0.1) \\
          SA-RMTPP & -168.01 (18.84) &       GRU-MLP/MC &  217.08 (16.43) &    SA-MLP/MC + B &   26.64 (17.49) &        SA-MLP/CM & 0.18 (0.01) &     SA-RMTPP + B & 0.29 (0.07) &  GRU-RMTPP + BFC & 0.44 (0.06) \\
      SA-SA/CM + B & -165.26 (42.01) &        GRU-SA/MC &  218.69 (15.22) &  GRU-SA/MC + BFC &   40.11 (12.82) &     SA-SA/CM + B &  0.2 (0.01) &  GRU-RMTPP + BFC &  0.3 (0.05) &     SA-LNM + BFC & 0.43 (0.08) \\
         GRU-SA/CM & -164.62 (22.57) &         SA-SA/MC &   220.31 (8.94) &   SA-SA/MC + BFC &    50.0 (17.85) &       GRU-MLP/CM &   0.2 (0.0) &   SA-SA/MC + BFC &  0.3 (0.04) &     SA-RMTPP + B &  0.4 (0.12) \\
    SA-RMTPP + BFC & -154.32 (21.25) &        SA-MLP/MC &  220.69 (12.58) &         SA-RMTPP &   66.26 (24.14) &           Hawkes &  0.2 (0.01) &        GRU-SA/MC & 0.33 (0.05) &  GRU-SA/MC + BFC &  0.4 (0.04) \\
          SA-SA/CM & -153.32 (25.01) &     SA-LNM + BFC &   227.5 (33.65) &  GRU-RMTPP + BFC &   96.21 (17.01) &    GRU-SA/CM + B &  0.2 (0.01) &          GRU-LNM & 0.34 (0.05) &   SA-SA/MC + BFC & 0.36 (0.04) \\
   GRU-RMTPP + BFC & -150.97 (15.06) &         SA-RMTPP &  234.26 (37.46) &  SA-MLP/MC + BFC &  108.78 (14.67) &       GRU-LNM-K1 & 0.21 (0.06) &    GRU-RMTPP + B & 0.34 (0.08) &          GRU-LNM &  0.3 (0.09) \\
    SA-SA/CM + BFC & -148.92 (28.49) &          GRU-LNM &  239.91 (16.08) &        GRU-SA/CM &  111.81 (11.83) & GRU-MLP/CM + BFC & 0.21 (0.01) &           SA-LNM & 0.34 (0.05) &  SA-MLP/MC + BFC & 0.28 (0.07) \\
      SA-RMTPP + B & -148.53 (20.44) &  GRU-RMTPP + BFC &  247.19 (27.25) &   SA-RMTPP + BFC &  121.86 (29.92) &        GRU-SA/MC & 0.22 (0.02) &           GRU-CP & 0.34 (0.08) &           SA-LNM & 0.26 (0.08) \\
   GRU-SA/CM + BFC & -139.02 (34.07) &           SA-LNM &  260.31 (14.31) &        GRU-RMTPP &  124.22 (28.16) &  GRU-SA/MC + BFC & 0.22 (0.02) &   SA-RMTPP + BFC & 0.36 (0.05) &       SA-LNM + B &  0.22 (0.1) \\
         GRU-RMTPP &  -138.9 (18.09) &       GRU-LNM-K1 &  261.32 (14.94) &  GRU-SA/CM + BFC &  128.25 (19.95) &         SA-SA/MC & 0.23 (0.01) &       SA-LNM + B &  0.4 (0.06) &            SA-CP & 0.21 (0.11) \\
     GRU-RMTPP + B & -136.01 (22.52) &       GRU-MLP/CM &  262.74 (18.39) &    GRU-RMTPP + B &  128.52 (29.98) &   SA-SA/MC + BFC & 0.24 (0.02) &  SA-MLP/MC + BFC &  0.4 (0.02) & GRU-MLP/MC + BFC & 0.21 (0.04) \\
    SA-SA/MC + BFC & -135.76 (22.97) &        GRU-RMTPP &  263.12 (37.03) &         SA-SA/CM &  132.92 (18.88) &    GRU-SA/MC + B & 0.25 (0.01) &       GRU-LNM-K1 &  0.4 (0.06) &       GRU-MLP/MC & 0.17 (0.03) \\
   GRU-SA/MC + BFC &  -135.6 (17.03) &    GRU-RMTPP + B &  264.53 (41.57) &     SA-RMTPP + B &  137.07 (36.42) &     SA-SA/MC + B & 0.25 (0.01) &       GRU-CP + B &  0.4 (0.05) &        GRU-SA/MC & 0.17 (0.02) \\
             SA-CP & -134.73 (12.09) &  GRU-SA/CM + BFC &  267.27 (17.11) &   SA-SA/CM + BFC &  137.63 (19.25) &  SA-MLP/CM + BFC & 0.26 (0.01) &     GRU-CP + BFC & 0.41 (0.04) &       GRU-LNM-K1 & 0.17 (0.11) \\
            GRU-CP &  -130.6 (10.28) &   SA-RMTPP + BFC &  276.18 (41.33) &    GRU-SA/CM + B &  139.19 (41.97) &       GRU-MLP/MC & 0.28 (0.01) &      SA-CP + BFC & 0.43 (0.06) &      SA-CP + BFC & 0.16 (0.04) \\
       SA-CP + BFC & -128.54 (12.63) &        GRU-SA/CM &  276.43 (26.65) &       GRU-MLP/CM &    142.88 (6.8) &        SA-MLP/MC & 0.28 (0.01) &            SA-CP & 0.43 (0.05) &     GRU-CP + BFC & 0.14 (0.04) \\
      GRU-CP + BFC &  -123.26 (9.04) &        SA-MLP/CM &  277.28 (28.13) &     SA-SA/CM + B &  162.26 (34.32) & GRU-MLP/MC + BFC & 0.29 (0.01) &         SA-SA/MC & 0.44 (0.04) &        SA-CP + B & 0.14 (0.08) \\
     SA-MLP/MC + B & -123.24 (19.59) &      GRU-LNM + B &   277.3 (20.39) & GRU-MLP/CM + BFC &   170.0 (15.75) &        GRU-RMTPP &  0.3 (0.01) &      GRU-LNM + B & 0.44 (0.05) &           GRU-CP & 0.14 (0.08) \\
    GRU-MLP/CM + B & -122.69 (16.76) &     SA-RMTPP + B &   285.6 (44.04) & GRU-MLP/MC + BFC &   171.8 (20.44) &         SA-RMTPP & 0.31 (0.01) & GRU-MLP/MC + BFC & 0.45 (0.03) &         SA-SA/MC & 0.14 (0.03) \\
    GRU-MLP/MC + B & -121.89 (12.23) &         SA-SA/CM &  286.24 (32.47) &        SA-MLP/CM &  178.22 (12.72) &    SA-MLP/CM + B & 0.31 (0.01) &        SA-CP + B & 0.46 (0.03) &       GRU-CP + B & 0.13 (0.04) \\
  GRU-MLP/CM + BFC &   -120.5 (9.89) &   SA-SA/CM + BFC &   286.55 (30.7) &         SA-SA/MC &   178.7 (13.53) &  SA-MLP/MC + BFC & 0.31 (0.01) &       GRU-MLP/MC & 0.48 (0.04) &      GRU-LNM + B & 0.12 (0.08) \\
        GRU-MLP/CM & -119.86 (12.25) &       SA-LNM + B &  289.16 (14.89) &        GRU-SA/MC &  185.59 (11.67) &   SA-RMTPP + BFC & 0.32 (0.01) &          Poisson &   0.5 (0.0) &        SA-MLP/MC & 0.12 (0.03) \\
        GRU-CP + B & -119.28 (14.07) &  SA-MLP/CM + BFC &   290.2 (32.22) &  SA-MLP/CM + BFC &  185.99 (21.04) &    GRU-RMTPP + B & 0.32 (0.01) &   SA-SA/CM + BFC &   0.5 (0.0) &   GRU-MLP/CM + B &  0.01 (0.0) \\
     SA-MLP/CM + B & -116.17 (23.51) & GRU-MLP/CM + BFC &   290.5 (23.68) &   GRU-MLP/CM + B &  207.76 (27.56) &   GRU-MLP/CM + B & 0.32 (0.01) &     SA-SA/CM + B &   0.5 (0.0) &          Poisson &  0.01 (0.0) \\
         SA-CP + B & -111.69 (15.55) &    GRU-SA/CM + B &  309.48 (50.99) &        SA-MLP/MC &   209.21 (8.05) &  GRU-RMTPP + BFC &  0.33 (0.0) &         SA-SA/CM &   0.5 (0.0) &   SA-SA/CM + BFC &  0.01 (0.0) \\
   SA-MLP/CM + BFC & -104.21 (12.99) &     SA-SA/CM + B &  327.52 (50.72) &       GRU-MLP/MC &   210.61 (5.68) &     SA-RMTPP + B & 0.33 (0.01) &  GRU-SA/CM + BFC &   0.5 (0.0) &       GRU-MLP/CM &  0.01 (0.0) \\
         SA-MLP/CM &  -99.07 (15.68) &   GRU-MLP/CM + B &  330.45 (43.01) &    SA-MLP/CM + B &  214.73 (23.61) &   GRU-MLP/MC + B & 0.33 (0.01) & GRU-MLP/CM + BFC &   0.5 (0.0) &  GRU-SA/CM + BFC &  0.01 (0.0) \\
   SA-MLP/MC + BFC &    -88.1 (16.8) &    SA-MLP/CM + B &   330.9 (45.83) &            SA-CP & 281.18 (127.24) &          Poisson & 0.34 (0.01) &  SA-MLP/CM + BFC &   0.5 (0.0) &    GRU-SA/CM + B &  0.01 (0.0) \\
           Poisson &  -57.32 (16.36) &            SA-CP & 415.91 (135.01) &           GRU-CP & 313.14 (134.69) &        SA-CP + B & 0.35 (0.01) &    SA-MLP/CM + B &   0.5 (0.0) &     SA-SA/CM + B &  0.01 (0.0) \\
          SA-SA/MC &  -41.61 (22.01) &           GRU-CP & 443.74 (140.44) &      SA-CP + BFC & 325.35 (124.46) &      SA-CP + BFC & 0.35 (0.01) &        SA-MLP/CM &   0.5 (0.0) &  SA-MLP/CM + BFC &  0.01 (0.0) \\
  GRU-MLP/MC + BFC &  -38.12 (18.83) &      SA-CP + BFC & 453.89 (134.79) &     GRU-CP + BFC &   352.0 (97.28) &     GRU-CP + BFC & 0.35 (0.01) &        GRU-SA/CM &   0.5 (0.0) & GRU-MLP/CM + BFC &  0.01 (0.0) \\
         GRU-SA/MC &   -33.1 (20.13) &     GRU-CP + BFC & 475.27 (103.94) &       GRU-CP + B & 361.28 (134.16) &       GRU-CP + B & 0.35 (0.01) &    GRU-SA/CM + B &   0.5 (0.0) &         SA-SA/CM &   0.0 (0.0) \\
         SA-MLP/MC &   -11.48 (19.9) &       GRU-CP + B & 480.56 (143.44) &          Poisson & 477.63 (123.65) &    SA-MLP/MC + B &  0.35 (0.0) &       GRU-MLP/CM &   0.5 (0.0) &    SA-MLP/CM + B &   0.0 (0.0) \\
        GRU-MLP/MC &   -6.47 (20.35) &          Poisson & 534.95 (131.14) &        SA-CP + B & 479.32 (148.01) &            SA-CP & 0.37 (0.01) &   GRU-MLP/CM + B &   0.5 (0.0) &        SA-MLP/CM &   0.0 (0.0) \\
            Hawkes &  338.61 (94.32) &        SA-CP + B & 591.01 (162.57) &           Hawkes &    483.3 (82.5) &           GRU-CP & 0.37 (0.01) &        SA-MLP/MC & 0.55 (0.01) &        GRU-SA/CM &   0.0 (0.0) \\ \\
\hline
\end{tabular}
\label{resultsmark}
\caption{Wikipedia}
\end{table}



\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccccccccccc}
\hline \\
               0 &        NLL Time &                2 &       NLL Mark &                3 &       NLL Total &                4 &   Time Cal. &                6 &   Mark Cal. &                7 &    F1-score \\
\hline \\
      SA-LNM + B & -603.17 (72.96) &    GRU-LNM + BFC & 120.33 (10.87) &       SA-LNM + B & -450.37 (60.51) &    GRU-LNM + BFC &  0.02 (0.0) &           Hawkes &  0.05 (0.0) &    GRU-SA/MC + B & 0.56 (0.01) \\
     GRU-LNM + B & -509.59 (43.49) &       GRU-LNM-K1 & 123.28 (18.16) &      GRU-LNM + B & -348.35 (30.69) &          GRU-LNM &  0.03 (0.0) &    GRU-LNM + BFC & 0.16 (0.01) &    GRU-LNM + BFC & 0.55 (0.01) \\
   GRU-LNM + BFC &  -379.3 (42.51) &           Hawkes & 124.65 (15.73) &    GRU-LNM + BFC & -258.97 (31.87) &       GRU-LNM-K1 &  0.04 (0.0) &       GRU-LNM-K1 & 0.17 (0.02) &       GRU-LNM-K1 & 0.54 (0.02) \\
    SA-LNM + BFC & -373.86 (58.13) &    GRU-SA/MC + B &  125.2 (16.26) &       GRU-LNM-K1 & -246.34 (39.92) &     SA-LNM + BFC & 0.04 (0.01) &  GRU-RMTPP + BFC & 0.17 (0.01) & GRU-MLP/MC + BFC & 0.54 (0.01) \\
         GRU-LNM & -372.05 (40.32) &          GRU-LNM & 127.37 (15.16) &          GRU-LNM & -244.68 (26.66) &           SA-LNM &  0.04 (0.0) &        GRU-RMTPP & 0.18 (0.02) &        GRU-SA/MC & 0.54 (0.02) \\
      GRU-LNM-K1 & -369.62 (57.24) &        GRU-RMTPP &  127.8 (19.96) &     SA-LNM + BFC &  -244.6 (41.93) &      GRU-LNM + B & 0.05 (0.01) &           GRU-CP & 0.18 (0.01) &   SA-SA/MC + BFC & 0.54 (0.01) \\
          SA-LNM & -369.44 (40.51) &     SA-LNM + BFC & 129.25 (16.48) &           SA-LNM & -235.35 (25.87) &       SA-LNM + B & 0.06 (0.01) &          GRU-LNM & 0.19 (0.03) &  GRU-SA/MC + BFC & 0.53 (0.02) \\
 GRU-SA/MC + BFC & -333.77 (48.94) &   GRU-MLP/MC + B &  130.7 (18.32) &  GRU-SA/MC + BFC & -197.97 (34.75) &     SA-SA/MC + B &  0.1 (0.01) &    GRU-RMTPP + B & 0.19 (0.02) &           Hawkes & 0.53 (0.01) \\
    SA-SA/MC + B & -322.64 (55.78) &     SA-SA/MC + B & 131.79 (19.84) &    GRU-SA/MC + B & -194.63 (36.75) &  GRU-SA/MC + BFC &   0.1 (0.0) &     SA-SA/MC + B &  0.2 (0.02) &       GRU-MLP/MC & 0.53 (0.01) \\
   GRU-SA/CM + B & -320.68 (55.92) &   SA-SA/MC + BFC & 132.18 (17.58) &     SA-SA/MC + B & -190.85 (37.44) &    GRU-SA/MC + B &   0.1 (0.0) &       GRU-MLP/MC &  0.2 (0.02) &         SA-SA/MC & 0.52 (0.02) \\
   GRU-SA/MC + B & -319.83 (52.21) &  GRU-RMTPP + BFC & 133.19 (15.22) &   SA-SA/MC + BFC &  -184.9 (36.27) &   SA-SA/MC + BFC &  0.11 (0.0) &         SA-RMTPP &  0.2 (0.03) &     SA-SA/MC + B & 0.52 (0.02) \\
  SA-SA/MC + BFC & -317.08 (53.16) & GRU-MLP/MC + BFC & 133.22 (11.87) &           Hawkes & -174.09 (41.47) &         SA-SA/MC & 0.11 (0.01) &            SA-CP &  0.2 (0.01) &  SA-MLP/MC + BFC & 0.52 (0.02) \\
    SA-SA/CM + B &  -309.45 (58.4) &           SA-LNM & 134.09 (15.56) &    GRU-SA/CM + B & -166.24 (36.01) &    GRU-SA/CM + B &  0.11 (0.0) &     SA-RMTPP + B & 0.21 (0.03) &     SA-LNM + BFC & 0.52 (0.01) \\
       GRU-SA/MC &  -300.3 (55.12) &  GRU-SA/MC + BFC &   135.8 (15.1) &        GRU-SA/MC & -163.84 (37.43) &        GRU-SA/MC & 0.12 (0.01) &     GRU-CP + BFC & 0.21 (0.02) &          GRU-LNM & 0.52 (0.02) \\
          Hawkes &  -298.75 (56.8) &        GRU-SA/MC & 136.46 (18.77) &         SA-SA/MC & -159.95 (35.05) &     SA-SA/CM + B & 0.13 (0.01) &  SA-MLP/MC + BFC & 0.22 (0.01) &        SA-MLP/MC &  0.5 (0.04) \\
 GRU-SA/CM + BFC & -298.68 (40.34) &    GRU-RMTPP + B &  136.6 (18.94) &     SA-SA/CM + B & -155.12 (39.58) &  GRU-SA/CM + BFC & 0.13 (0.01) & GRU-MLP/MC + BFC & 0.22 (0.02) &        GRU-RMTPP & 0.49 (0.04) \\
        SA-SA/MC & -297.79 (52.97) &   SA-RMTPP + BFC & 137.14 (22.43) &        GRU-RMTPP &  -152.07 (35.8) &        GRU-SA/CM & 0.13 (0.01) &     SA-LNM + BFC & 0.22 (0.01) &           SA-LNM & 0.49 (0.02) \\
       GRU-SA/CM & -294.87 (55.43) &         SA-SA/MC & 137.85 (19.01) &  GRU-RMTPP + BFC &  -144.2 (23.59) &         SA-SA/CM & 0.14 (0.01) &  GRU-SA/MC + BFC & 0.22 (0.01) &   GRU-MLP/MC + B & 0.49 (0.03) \\
  SA-SA/CM + BFC & -292.73 (53.48) &         SA-RMTPP & 138.15 (21.92) &  GRU-SA/CM + BFC & -143.49 (26.35) &   SA-SA/CM + BFC & 0.14 (0.01) &   SA-RMTPP + BFC & 0.23 (0.04) &  GRU-RMTPP + BFC & 0.48 (0.03) \\
        SA-SA/CM & -292.43 (55.48) &    SA-MLP/MC + B & 138.37 (17.41) &   GRU-MLP/MC + B & -140.64 (34.28) &           Hawkes & 0.16 (0.01) &    GRU-SA/MC + B & 0.23 (0.02) &    GRU-RMTPP + B & 0.48 (0.02) \\
       GRU-RMTPP & -279.86 (54.29) &           GRU-CP & 138.71 (19.91) &    GRU-RMTPP + B & -139.85 (33.21) & GRU-MLP/MC + BFC &  0.17 (0.0) &   GRU-MLP/MC + B & 0.24 (0.02) &    SA-MLP/MC + B & 0.48 (0.04) \\
 GRU-RMTPP + BFC & -277.39 (37.21) &  SA-MLP/MC + BFC & 139.12 (21.22) &   SA-SA/CM + BFC & -137.89 (33.98) &  GRU-RMTPP + BFC & 0.18 (0.01) &           SA-LNM & 0.25 (0.02) &     SA-RMTPP + B & 0.47 (0.03) \\
   GRU-RMTPP + B & -276.45 (51.41) &       GRU-MLP/MC & 139.71 (19.49) &        GRU-SA/CM & -137.86 (35.66) &    GRU-RMTPP + B & 0.18 (0.01) &        SA-MLP/MC & 0.26 (0.02) &   SA-RMTPP + BFC & 0.47 (0.03) \\
          GRU-CP & -273.12 (53.73) &     SA-RMTPP + B & 139.97 (18.33) &           GRU-CP & -134.41 (35.45) &        GRU-RMTPP & 0.18 (0.01) &        GRU-SA/MC & 0.27 (0.01) &         SA-RMTPP & 0.45 (0.03) \\
  GRU-MLP/MC + B & -271.35 (50.62) &            SA-CP & 142.12 (20.54) &         SA-SA/CM & -133.98 (35.51) &       GRU-MLP/MC & 0.18 (0.01) &    SA-MLP/MC + B & 0.27 (0.03) &       SA-LNM + B & 0.44 (0.03) \\
      GRU-CP + B & -270.29 (52.78) &        SA-MLP/MC & 142.19 (21.43) & GRU-MLP/MC + BFC & -131.32 (28.14) &     SA-RMTPP + B & 0.18 (0.01) &         SA-SA/MC & 0.27 (0.01) &      GRU-LNM + B & 0.42 (0.03) \\
    GRU-CP + BFC &  -268.33 (35.5) &     GRU-CP + BFC & 143.41 (15.44) &     GRU-CP + BFC & -124.91 (21.56) &  SA-MLP/MC + BFC & 0.18 (0.01) &   SA-SA/MC + BFC & 0.27 (0.01) &       GRU-CP + B & 0.42 (0.03) \\
      GRU-MLP/CM &   -265.6 (47.8) &      SA-CP + BFC & 151.07 (22.61) &   SA-RMTPP + BFC & -122.87 (29.53) &        SA-MLP/MC & 0.18 (0.01) &      SA-CP + BFC & 0.29 (0.02) &           GRU-CP & 0.42 (0.03) \\
GRU-MLP/MC + BFC &  -264.55 (39.2) &       GRU-CP + B &  151.7 (21.25) &         SA-RMTPP & -120.22 (28.09) &   GRU-MLP/MC + B & 0.19 (0.01) &        SA-CP + B &  0.3 (0.03) &     GRU-CP + BFC & 0.41 (0.02) \\
       SA-CP + B & -263.15 (53.22) &        SA-CP + B & 152.32 (20.72) &     SA-RMTPP + B & -119.56 (33.65) &       GRU-MLP/CM & 0.19 (0.02) &       GRU-CP + B & 0.32 (0.03) &    GRU-SA/CM + B &  0.4 (0.03) \\
GRU-MLP/CM + BFC & -261.91 (32.01) &       SA-LNM + B &  152.8 (19.96) &    SA-MLP/MC + B & -118.61 (31.52) &   SA-RMTPP + BFC &  0.2 (0.02) &       GRU-MLP/CM & 0.34 (0.02) &   GRU-MLP/CM + B &  0.4 (0.03) \\
  GRU-MLP/CM + B & -261.25 (44.92) &     SA-SA/CM + B & 154.33 (21.02) &       GRU-CP + B & -118.59 (34.75) &           GRU-CP &  0.2 (0.01) &       SA-LNM + B & 0.36 (0.05) &          Poisson &  0.4 (0.03) \\
  SA-RMTPP + BFC & -260.01 (46.73) &    GRU-SA/CM + B &  154.45 (21.0) &       GRU-MLP/MC & -117.54 (34.35) & GRU-MLP/CM + BFC &  0.2 (0.01) &      GRU-LNM + B & 0.37 (0.05) &   SA-SA/CM + BFC &  0.4 (0.03) \\
    SA-RMTPP + B &  -259.53 (49.1) &   SA-SA/CM + BFC & 154.84 (21.15) &            SA-CP & -112.05 (28.22) &     GRU-CP + BFC &  0.2 (0.01) & GRU-MLP/CM + BFC & 0.37 (0.02) &     SA-SA/CM + B &  0.4 (0.03) \\
        SA-RMTPP & -258.37 (44.02) &  GRU-SA/CM + BFC & 155.19 (15.08) &        SA-CP + B & -110.83 (33.35) &       GRU-CP + B &  0.2 (0.01) &         SA-SA/CM & 0.39 (0.02) &         SA-SA/CM &  0.4 (0.03) \\
      GRU-MLP/MC & -257.25 (52.66) & GRU-MLP/CM + BFC & 156.95 (16.95) &  SA-MLP/MC + BFC & -107.76 (34.49) &    SA-MLP/MC + B &  0.2 (0.01) &   GRU-MLP/CM + B &  0.4 (0.03) &       GRU-MLP/CM &  0.4 (0.03) \\
   SA-MLP/MC + B & -256.98 (46.33) &        GRU-SA/CM & 157.01 (21.64) &       GRU-MLP/CM &  -107.46 (27.1) &        SA-CP + B &  0.2 (0.01) &        GRU-SA/CM & 0.41 (0.01) & GRU-MLP/CM + BFC &  0.4 (0.02) \\
     SA-CP + BFC &  -254.61 (47.4) &       GRU-MLP/CM & 158.14 (22.91) & GRU-MLP/CM + BFC & -104.96 (17.88) &         SA-RMTPP & 0.21 (0.03) &  GRU-SA/CM + BFC & 0.42 (0.01) &        GRU-SA/CM &  0.4 (0.03) \\
           SA-CP & -254.18 (47.64) &         SA-SA/CM & 158.45 (21.09) &      SA-CP + BFC & -103.54 (26.57) &      SA-CP + BFC & 0.21 (0.02) &   SA-SA/CM + BFC & 0.42 (0.01) &  SA-MLP/CM + BFC &  0.4 (0.03) \\
 SA-MLP/MC + BFC & -246.88 (52.25) &   GRU-MLP/CM + B & 160.33 (24.42) &        SA-MLP/MC & -103.08 (31.34) &            SA-CP & 0.21 (0.02) &     SA-SA/CM + B & 0.44 (0.02) &    SA-MLP/CM + B &  0.4 (0.03) \\
       SA-MLP/MC & -245.26 (49.72) &        SA-MLP/CM & 160.58 (20.61) &   GRU-MLP/CM + B & -100.92 (25.57) &   GRU-MLP/CM + B & 0.21 (0.02) &    GRU-SA/CM + B &  0.45 (0.0) &        SA-MLP/CM &  0.4 (0.03) \\
   SA-MLP/CM + B &  -175.5 (31.64) &      GRU-LNM + B & 161.24 (22.35) &  SA-MLP/CM + BFC &  -13.19 (12.62) &        SA-MLP/CM & 0.26 (0.02) &    SA-MLP/CM + B & 0.47 (0.01) &      SA-CP + BFC &  0.4 (0.03) \\
 SA-MLP/CM + BFC &  -174.5 (32.88) &  SA-MLP/CM + BFC & 161.32 (21.03) &        SA-MLP/CM &  -12.36 (12.78) &  SA-MLP/CM + BFC & 0.27 (0.02) &        SA-MLP/CM & 0.47 (0.01) &            SA-CP &  0.4 (0.03) \\
       SA-MLP/CM & -172.94 (32.92) &    SA-MLP/CM + B &  163.4 (22.79) &    SA-MLP/CM + B &   -12.1 (10.98) &    SA-MLP/CM + B & 0.28 (0.02) &  SA-MLP/CM + BFC & 0.47 (0.01) &  GRU-SA/CM + BFC &  0.4 (0.02) \\
         Poisson & -142.58 (26.06) &          Poisson & 168.37 (21.04) &          Poisson &    25.79 (5.38) &          Poisson & 0.33 (0.02) &          Poisson & 0.49 (0.01) &        SA-CP + B &  0.4 (0.03) \\
\hline \\
\end{tabular}
\label{resultsmark}
\caption{Github}
\end{table}



\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering
\begin{tabular}{cccccccccccc}
\hline \\
               0 &     NLL Time &                2 &     NLL Mark &                3 &    NLL Total &                4 &   Time Cal. &                6 &   Mark Cal. &                7 &    F1-score \\
\hline \\
      SA-LNM + B &  1.17 (0.15) &        GRU-RMTPP &  1.89 (0.12) &        GRU-RMTPP &   3.22 (0.2) &     SA-LNM + BFC &  0.02 (0.0) &    GRU-RMTPP + B &  0.1 (0.01) &         SA-RMTPP & 0.77 (0.01) \\
     GRU-LNM + B &  1.23 (0.11) &         SA-RMTPP &  2.02 (0.13) &          GRU-LNM &  3.57 (0.22) &           SA-LNM &  0.02 (0.0) &           GRU-CP & 0.12 (0.02) &        GRU-RMTPP & 0.76 (0.02) \\
       GRU-RMTPP &  1.33 (0.09) &          GRU-LNM &  2.14 (0.11) &       GRU-LNM-K1 &  3.66 (0.38) &           GRU-CP &  0.03 (0.0) &   SA-RMTPP + BFC & 0.13 (0.02) &    GRU-RMTPP + B & 0.73 (0.03) \\
   GRU-RMTPP + B &  1.34 (0.14) &       GRU-LNM-K1 &  2.17 (0.17) &           SA-LNM &  3.66 (0.15) &   SA-RMTPP + BFC &  0.03 (0.0) &  GRU-RMTPP + BFC & 0.13 (0.01) &    SA-MLP/MC + B & 0.73 (0.02) \\
          GRU-CP &  1.35 (0.09) &           SA-LNM &   2.2 (0.12) &         SA-RMTPP &   3.7 (0.21) &          GRU-LNM &  0.03 (0.0) &          GRU-LNM & 0.14 (0.01) &       GRU-LNM-K1 & 0.71 (0.02) \\
   GRU-SA/CM + B &  1.41 (0.16) &     SA-SA/MC + B &   2.4 (0.17) &    GRU-RMTPP + B &  3.77 (0.33) &     SA-RMTPP + B &  0.03 (0.0) &         SA-RMTPP & 0.14 (0.02) &          GRU-LNM & 0.71 (0.01) \\
         GRU-LNM &  1.43 (0.12) &    GRU-RMTPP + B &  2.43 (0.23) &     SA-SA/MC + B &  3.97 (0.24) &    GRU-LNM + BFC &  0.03 (0.0) &     SA-LNM + BFC & 0.14 (0.02) &   SA-RMTPP + BFC & 0.71 (0.02) \\
          SA-LNM &  1.47 (0.16) &   SA-RMTPP + BFC &  2.44 (0.21) &  GRU-RMTPP + BFC &  4.05 (0.23) &         SA-RMTPP &  0.03 (0.0) &        GRU-RMTPP & 0.14 (0.01) &           SA-LNM & 0.71 (0.03) \\
 GRU-RMTPP + BFC &  1.47 (0.13) &    SA-MLP/MC + B &  2.55 (0.13) &           GRU-CP &  4.11 (0.28) &  GRU-SA/CM + BFC & 0.03 (0.01) &     SA-RMTPP + B & 0.15 (0.02) &     SA-SA/MC + B &  0.7 (0.01) \\
      GRU-LNM-K1 &  1.49 (0.21) &    GRU-SA/MC + B &  2.56 (0.21) &    GRU-SA/MC + B &  4.12 (0.34) &    GRU-SA/CM + B & 0.03 (0.01) &    GRU-SA/MC + B & 0.15 (0.02) &   GRU-MLP/MC + B & 0.69 (0.03) \\
       GRU-SA/CM &  1.53 (0.14) &  GRU-RMTPP + BFC &  2.57 (0.12) &   SA-RMTPP + BFC &  4.17 (0.26) &    GRU-RMTPP + B &  0.03 (0.0) &       GRU-LNM-K1 & 0.15 (0.02) &    GRU-SA/MC + B & 0.69 (0.03) \\
  GRU-MLP/CM + B &  1.55 (0.16) &     SA-LNM + BFC &  2.58 (0.08) &     SA-LNM + BFC &  4.22 (0.14) &     SA-SA/MC + B & 0.04 (0.01) &    GRU-LNM + BFC & 0.16 (0.03) &  GRU-RMTPP + BFC & 0.68 (0.02) \\
   GRU-SA/MC + B &  1.56 (0.18) &            SA-CP &  2.73 (0.24) &       SA-LNM + B &  4.37 (0.27) &    SA-MLP/MC + B & 0.04 (0.01) &     SA-SA/MC + B & 0.17 (0.02) &     SA-RMTPP + B & 0.67 (0.02) \\
   GRU-LNM + BFC &  1.56 (0.06) &           GRU-CP &  2.76 (0.21) &   GRU-MLP/MC + B &  4.49 (0.21) &       SA-LNM + B &  0.04 (0.0) &      GRU-LNM + B &  0.2 (0.04) &     SA-LNM + BFC & 0.66 (0.03) \\
    SA-SA/MC + B &  1.57 (0.12) &     SA-RMTPP + B &  2.78 (0.15) &    GRU-LNM + BFC &  4.59 (0.22) &        GRU-SA/CM &  0.04 (0.0) &   GRU-MLP/MC + B &  0.2 (0.02) &       SA-LNM + B & 0.64 (0.03) \\
 GRU-SA/CM + BFC &  1.59 (0.11) &   GRU-MLP/MC + B &  2.84 (0.17) &     SA-RMTPP + B &  4.61 (0.23) &       GRU-LNM-K1 & 0.04 (0.01) &       SA-LNM + B &  0.2 (0.05) &           GRU-CP & 0.64 (0.05) \\
      GRU-CP + B &  1.63 (0.06) &    GRU-LNM + BFC &   3.03 (0.2) &    SA-MLP/MC + B &  4.68 (0.33) &        GRU-RMTPP & 0.04 (0.01) &     GRU-CP + BFC &  0.2 (0.02) &           Hawkes &  0.63 (0.0) \\
    SA-LNM + BFC &  1.64 (0.09) &      SA-CP + BFC &  3.18 (0.21) &      GRU-LNM + B &   4.73 (0.2) &     GRU-CP + BFC & 0.04 (0.01) &       GRU-CP + B & 0.21 (0.02) &       GRU-CP + B & 0.62 (0.04) \\
    GRU-CP + BFC &  1.65 (0.05) &       SA-LNM + B &  3.21 (0.27) &            SA-CP &  4.86 (0.24) & GRU-MLP/CM + BFC &  0.04 (0.0) &           SA-LNM & 0.21 (0.03) &      GRU-LNM + B & 0.62 (0.04) \\
  GRU-MLP/MC + B &  1.65 (0.09) &     GRU-CP + BFC &   3.3 (0.22) &     GRU-CP + BFC &  4.95 (0.26) &  GRU-RMTPP + BFC &  0.04 (0.0) &            SA-CP & 0.22 (0.02) &            SA-CP & 0.62 (0.05) \\
      GRU-MLP/CM &  1.68 (0.04) &      GRU-LNM + B &    3.5 (0.1) &  GRU-SA/CM + BFC &  5.27 (0.16) &       GRU-CP + B & 0.05 (0.01) &           Hawkes & 0.24 (0.04) &     GRU-CP + BFC & 0.61 (0.02) \\
        SA-RMTPP &   1.68 (0.1) &  GRU-SA/CM + BFC &  3.68 (0.07) &   GRU-MLP/CM + B &  5.36 (0.36) &   SA-SA/CM + BFC &  0.05 (0.0) &    SA-MLP/MC + B & 0.26 (0.02) &      SA-CP + BFC & 0.59 (0.03) \\
    SA-SA/CM + B &   1.7 (0.08) &    SA-MLP/CM + B &   3.75 (0.2) &      SA-CP + BFC &  5.38 (0.33) &     SA-SA/CM + B & 0.05 (0.01) &        SA-CP + B & 0.32 (0.03) &    GRU-LNM + BFC & 0.59 (0.05) \\
  SA-RMTPP + BFC &  1.73 (0.11) &   GRU-MLP/CM + B &  3.81 (0.22) &    GRU-SA/CM + B &  5.46 (0.22) &         SA-SA/CM & 0.05 (0.01) &  GRU-SA/CM + BFC & 0.32 (0.02) &        SA-CP + B & 0.55 (0.05) \\
  SA-SA/CM + BFC &   1.78 (0.1) &        SA-CP + B &  3.87 (0.27) &       GRU-CP + B &  5.59 (0.35) &           Hawkes &  0.05 (0.0) &      SA-CP + BFC & 0.32 (0.03) &   GRU-MLP/CM + B & 0.36 (0.04) \\
GRU-MLP/CM + BFC &  1.78 (0.12) &       GRU-CP + B &  3.96 (0.31) &    SA-MLP/CM + B &  5.64 (0.15) &   GRU-MLP/CM + B & 0.05 (0.01) &   GRU-MLP/CM + B & 0.37 (0.03) &  GRU-SA/CM + BFC & 0.34 (0.04) \\
    SA-RMTPP + B &   1.83 (0.1) &    GRU-SA/CM + B &  4.05 (0.19) &     SA-SA/CM + B &  5.78 (0.17) &  SA-MLP/CM + BFC &  0.05 (0.0) &    GRU-SA/CM + B & 0.38 (0.02) &    SA-MLP/CM + B & 0.32 (0.07) \\
 SA-MLP/CM + BFC &  1.84 (0.11) &     SA-SA/CM + B &  4.08 (0.11) &        SA-CP + B &  5.86 (0.35) &          Poisson &  0.07 (0.0) &    SA-MLP/CM + B & 0.39 (0.03) &    GRU-SA/CM + B &  0.3 (0.05) \\
   SA-MLP/CM + B &  1.89 (0.16) & GRU-MLP/CM + BFC &  4.13 (0.13) & GRU-MLP/CM + BFC &   5.9 (0.23) &       GRU-MLP/CM & 0.07 (0.01) &     SA-SA/CM + B & 0.39 (0.02) & GRU-MLP/CM + BFC & 0.25 (0.03) \\
        SA-SA/CM &    1.9 (0.1) &  SA-MLP/CM + BFC &   4.2 (0.18) &   SA-SA/CM + BFC &  6.02 (0.18) &        SA-CP + B & 0.07 (0.01) &   SA-SA/CM + BFC & 0.42 (0.03) &     SA-SA/CM + B & 0.25 (0.05) \\
       SA-CP + B &  1.99 (0.15) &   SA-SA/CM + BFC &  4.24 (0.11) &  SA-MLP/CM + BFC &  6.04 (0.25) &   GRU-MLP/MC + B & 0.07 (0.01) & GRU-MLP/CM + BFC & 0.43 (0.03) &   SA-SA/CM + BFC & 0.24 (0.03) \\
       SA-MLP/CM &   2.07 (0.1) &         SA-SA/CM &  4.44 (0.14) &        GRU-SA/CM &  6.15 (0.19) &            SA-CP &  0.07 (0.0) &        GRU-SA/CM & 0.44 (0.01) &        SA-MLP/CM & 0.22 (0.02) \\
   SA-MLP/MC + B &  2.13 (0.22) &       GRU-MLP/CM &  4.49 (0.16) &       GRU-MLP/CM &   6.16 (0.2) &    GRU-SA/MC + B & 0.07 (0.01) &       GRU-MLP/CM & 0.46 (0.01) &   SA-SA/MC + BFC & 0.22 (0.02) \\
           SA-CP &  2.13 (0.13) &        SA-MLP/CM &  4.51 (0.13) &         SA-SA/CM &  6.35 (0.22) &      GRU-LNM + B & 0.08 (0.03) &  SA-MLP/CM + BFC &  0.46 (0.0) &        GRU-SA/CM & 0.22 (0.02) \\
     SA-CP + BFC &   2.2 (0.17) &        GRU-SA/CM &   4.61 (0.1) &        SA-MLP/CM &  6.58 (0.18) &      SA-CP + BFC & 0.08 (0.01) &         SA-SA/CM &  0.47 (0.0) &         SA-SA/CM & 0.22 (0.02) \\
         Poisson &  2.98 (0.12) &  SA-MLP/MC + BFC &   7.3 (0.26) &           Hawkes &  12.5 (0.71) &    SA-MLP/CM + B & 0.08 (0.01) &          Poisson &  0.47 (0.0) &  GRU-SA/MC + BFC & 0.22 (0.02) \\
          Hawkes &  4.26 (0.26) &   SA-SA/MC + BFC &   7.3 (0.26) &          Poisson & 14.24 (0.47) &        SA-MLP/CM &  0.1 (0.01) &        SA-MLP/CM &  0.47 (0.0) &  SA-MLP/MC + BFC & 0.22 (0.02) \\
 SA-MLP/MC + BFC & 31.41 (1.98) & GRU-MLP/MC + BFC &  7.31 (0.18) &  SA-MLP/MC + BFC & 38.72 (2.21) &  SA-MLP/MC + BFC &  0.45 (0.0) &        SA-MLP/MC &  0.5 (0.01) &  SA-MLP/CM + BFC & 0.22 (0.02) \\
 GRU-SA/MC + BFC & 31.42 (1.98) &  GRU-SA/MC + BFC &  7.31 (0.26) &  GRU-SA/MC + BFC & 38.73 (2.21) &  GRU-SA/MC + BFC &  0.45 (0.0) &        GRU-SA/MC &   0.5 (0.0) &       GRU-MLP/CM & 0.21 (0.02) \\
  SA-SA/MC + BFC & 31.44 (1.98) &        SA-MLP/MC &  7.33 (0.26) &   SA-SA/MC + BFC & 38.74 (2.21) &   SA-SA/MC + BFC &  0.45 (0.0) &       GRU-MLP/MC & 0.51 (0.01) &          Poisson &  0.2 (0.02) \\
GRU-MLP/MC + BFC & 49.41 (6.12) &       GRU-MLP/MC &  7.33 (0.26) & GRU-MLP/MC + BFC & 56.72 (6.19) & GRU-MLP/MC + BFC &  0.46 (0.0) & GRU-MLP/MC + BFC &  0.51 (0.0) &         SA-SA/MC & 0.13 (0.05) \\
       SA-MLP/MC &  67.4 (4.11) &        GRU-SA/MC &  7.33 (0.26) &        SA-MLP/MC & 74.73 (4.33) &       GRU-MLP/MC &  0.48 (0.0) &         SA-SA/MC & 0.52 (0.01) & GRU-MLP/MC + BFC & 0.11 (0.04) \\
      GRU-MLP/MC & 67.41 (4.12) &         SA-SA/MC &  7.33 (0.26) &       GRU-MLP/MC & 74.73 (4.34) &         SA-SA/MC &  0.48 (0.0) &  GRU-SA/MC + BFC &  0.53 (0.0) &       GRU-MLP/MC & 0.06 (0.04) \\
        SA-SA/MC & 67.42 (4.11) &           Hawkes &  8.24 (0.47) &         SA-SA/MC & 74.75 (4.33) &        GRU-SA/MC &  0.48 (0.0) &   SA-SA/MC + BFC &  0.53 (0.0) &        SA-MLP/MC & 0.06 (0.04) \\
       GRU-SA/MC & 67.43 (4.11) &          Poisson & 11.25 (0.46) &        GRU-SA/MC & 74.76 (4.34) &        SA-MLP/MC &  0.48 (0.0) &  SA-MLP/MC + BFC &  0.53 (0.0) &        GRU-SA/MC & 0.02 (0.01) \\
\hline \\
\end{tabular}



\caption{MIMIC2}
\end{table}


\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccccccccccccc}
\toprule
                        0 &       NLL Time &                1 &      NLL Mark &                2 &  NLL Window &                3 &    NLL Total &                4 &   Time Cal. &                5 &   Mark Cal. &                6 &    F1-score \\
\midrule
              GRU-LNM + B & -50.01 (16.19) &  GRU-RMTPP + BFC &  55.56 (17.2) &       SA-LNM + B &  0.9 (0.04) &      GRU-LNM + B &  6.81 (2.12) &       SA-LNM + B & 0.46 (0.14) &       SA-LNM + B & 0.67 (0.08) &   SA-SA/MC + BFC & 0.73 (0.15) \\
               SA-LNM + B & -49.36 (16.03) &        GRU-RMTPP & 55.56 (17.21) &          Poisson & 0.94 (0.04) &       SA-LNM + B &   7.3 (2.84) &          Poisson & 0.49 (0.14) &          Poisson & 0.71 (0.08) &  GRU-SA/MC + BFC & 0.73 (0.15) \\
                   Hawkes & -38.76 (12.62) &    GRU-RMTPP + B & 55.57 (17.21) &      GRU-LNM + B & 1.04 (0.02) &    GRU-LNM + BFC & 16.86 (4.98) &    SA-MLP/CM + B & 0.53 (0.16) &           Hawkes & 0.74 (0.13) &           GRU-CP & 0.72 (0.15) \\
            GRU-LNM + BFC & -38.72 (12.61) &    GRU-LNM + BFC & 55.58 (17.22) &    SA-MLP/CM + B & 1.04 (0.04) &    GRU-RMTPP + B &  16.9 (4.98) &      GRU-LNM + B & 0.54 (0.16) &      GRU-LNM + B & 0.75 (0.09) &     SA-SA/MC + B & 0.72 (0.15) \\
                  GRU-LNM & -38.69 (12.61) &           GRU-CP & 55.62 (17.22) &   GRU-MLP/CM + B & 1.06 (0.05) &  GRU-RMTPP + BFC & 16.91 (4.98) &   GRU-MLP/CM + B & 0.54 (0.16) &   SA-RMTPP + BFC & 0.76 (0.12) &         SA-SA/MC & 0.72 (0.15) \\
           GRU-MLP/MC + B & -38.69 (12.61) &          GRU-LNM & 55.63 (17.23) &  SA-MLP/CM + BFC & 1.07 (0.04) &        GRU-RMTPP & 16.91 (4.99) &  SA-MLP/CM + BFC & 0.55 (0.17) &    SA-MLP/MC + B & 0.76 (0.11) &        GRU-SA/MC & 0.72 (0.15) \\
         GRU-MLP/MC + BFC &  -38.67 (12.6) & GRU-MLP/MC + BFC & 55.66 (17.24) &  SA-MLP/MC + BFC &  1.1 (0.04) &          GRU-LNM &  16.94 (5.0) &  SA-MLP/MC + BFC & 0.56 (0.17) &   GRU-MLP/CM + B &  0.76 (0.1) &        GRU-SA/CM & 0.72 (0.18) \\
            GRU-RMTPP + B &  -38.67 (12.6) &   GRU-MLP/MC + B &  55.7 (17.25) &    SA-MLP/MC + B &  1.1 (0.04) & GRU-MLP/MC + BFC & 16.98 (5.01) &    SA-MLP/MC + B & 0.56 (0.17) &    SA-MLP/CM + B & 0.76 (0.09) &       GRU-MLP/CM & 0.72 (0.16) \\
          GRU-RMTPP + BFC &  -38.64 (12.6) &     GRU-CP + BFC & 55.73 (17.26) &        SA-MLP/CM &  1.1 (0.05) &   GRU-MLP/MC + B & 17.01 (5.01) &        SA-MLP/MC & 0.56 (0.18) &           SA-LNM & 0.76 (0.11) &  GRU-RMTPP + BFC & 0.72 (0.14) \\
                GRU-RMTPP & -38.64 (12.59) &     SA-RMTPP + B & 55.86 (17.31) &           SA-LNM & 1.11 (0.04) &           GRU-CP & 17.21 (5.07) &        SA-MLP/CM & 0.56 (0.17) &     SA-RMTPP + B & 0.77 (0.11) &        GRU-RMTPP & 0.71 (0.14) \\
            GRU-SA/MC + B &  -38.5 (12.55) &         SA-RMTPP & 55.87 (17.31) &     SA-LNM + BFC & 1.11 (0.05) &           Hawkes & 17.22 (5.09) &     SA-LNM + BFC & 0.56 (0.18) &         SA-RMTPP & 0.77 (0.12) &    GRU-RMTPP + B & 0.71 (0.14) \\
          GRU-SA/MC + BFC & -38.46 (12.55) &    SA-MLP/MC + B & 55.87 (17.32) &            SA-CP & 1.12 (0.06) &     GRU-CP + BFC &  17.28 (5.1) &           SA-LNM & 0.56 (0.18) &  SA-MLP/MC + BFC & 0.77 (0.11) &       GRU-MLP/MC & 0.71 (0.14) \\
               GRU-CP + B & -38.45 (12.53) &     SA-LNM + BFC & 55.87 (17.32) &     SA-RMTPP + B & 1.12 (0.05) &    GRU-SA/MC + B & 17.41 (5.14) &            SA-CP & 0.57 (0.18) &  SA-MLP/CM + BFC &  0.77 (0.1) & GRU-MLP/MC + BFC & 0.71 (0.14) \\
             GRU-CP + BFC & -38.45 (12.53) &   SA-RMTPP + BFC & 55.89 (17.32) &   SA-RMTPP + BFC & 1.12 (0.05) &  GRU-SA/MC + BFC & 17.54 (5.17) &   SA-RMTPP + BFC & 0.57 (0.18) &     SA-LNM + BFC & 0.77 (0.11) &   GRU-MLP/MC + B & 0.71 (0.14) \\
                   GRU-CP & -38.41 (12.52) &            SA-CP & 55.89 (17.32) &        SA-MLP/MC & 1.12 (0.04) &     SA-LNM + BFC & 17.62 (5.22) &     SA-RMTPP + B & 0.57 (0.18) &            SA-CP & 0.77 (0.11) &          GRU-LNM & 0.71 (0.14) \\
            GRU-SA/CM + B & -38.35 (12.51) &  SA-MLP/MC + BFC &  55.9 (17.33) &         SA-RMTPP & 1.13 (0.05) &     SA-SA/MC + B & 17.64 (5.21) &         SA-RMTPP & 0.57 (0.18) & GRU-MLP/MC + BFC & 0.77 (0.12) &     GRU-CP + BFC & 0.71 (0.14) \\
             SA-SA/MC + B &  -38.32 (12.5) &           SA-LNM &  55.9 (17.33) &      SA-CP + BFC & 1.13 (0.06) &     SA-RMTPP + B & 17.64 (5.23) &           Hawkes & 0.57 (0.18) &     GRU-CP + BFC & 0.77 (0.12) &    GRU-SA/MC + B & 0.71 (0.15) \\
           SA-SA/MC + BFC &  -38.31 (12.5) &    GRU-SA/MC + B & 55.91 (17.31) &        SA-CP + B & 1.13 (0.05) &   SA-RMTPP + BFC & 17.65 (5.23) &    GRU-LNM + BFC & 0.57 (0.18) &          GRU-LNM & 0.77 (0.12) &           Hawkes & 0.71 (0.14) \\
               GRU-MLP/MC &  -38.3 (12.48) &      SA-CP + BFC & 55.92 (17.33) &           Hawkes & 1.13 (0.05) &   SA-SA/MC + BFC & 17.66 (5.21) &        GRU-RMTPP & 0.58 (0.18) &    GRU-LNM + BFC & 0.77 (0.12) &         SA-SA/CM & 0.71 (0.19) \\
             SA-SA/CM + B & -38.29 (12.49) &     SA-SA/MC + B & 55.96 (17.33) &    GRU-LNM + BFC & 1.13 (0.05) &         SA-RMTPP & 17.69 (5.24) &          GRU-LNM & 0.58 (0.18) &    GRU-RMTPP + B & 0.77 (0.12) &    GRU-LNM + BFC &  0.7 (0.14) \\
             SA-LNM + BFC & -38.25 (12.45) &   SA-SA/MC + BFC & 55.97 (17.33) &       GRU-CP + B & 1.14 (0.06) &           SA-LNM & 17.72 (5.25) &       GRU-MLP/MC & 0.58 (0.18) &        GRU-RMTPP & 0.77 (0.12) & GRU-MLP/CM + BFC &  0.7 (0.16) \\
           SA-RMTPP + BFC & -38.23 (12.45) &           Hawkes & 55.98 (17.35) &        GRU-RMTPP & 1.14 (0.04) &    SA-MLP/MC + B & 17.74 (5.26) &   GRU-MLP/MC + B & 0.58 (0.18) &        SA-MLP/MC & 0.78 (0.11) &  GRU-SA/CM + BFC &  0.7 (0.17) \\
             SA-RMTPP + B & -38.21 (12.44) &  GRU-SA/MC + BFC & 55.99 (17.33) &     GRU-CP + BFC & 1.15 (0.04) &  SA-MLP/MC + BFC & 17.74 (5.26) & GRU-MLP/MC + BFC & 0.58 (0.18) &       GRU-MLP/MC & 0.78 (0.12) &  SA-MLP/MC + BFC & 0.69 (0.13) \\
                   SA-LNM & -38.19 (12.43) &       GRU-MLP/CM & 56.09 (17.36) &    GRU-RMTPP + B & 1.15 (0.04) &       GRU-CP + B & 17.75 (5.25) &    GRU-RMTPP + B & 0.58 (0.18) &      SA-CP + BFC & 0.78 (0.11) &        SA-MLP/MC & 0.69 (0.14) \\
                 SA-RMTPP & -38.18 (12.43) &       GRU-MLP/MC & 56.12 (17.38) & GRU-MLP/MC + BFC & 1.15 (0.04) &       GRU-MLP/MC & 17.82 (5.27) &       GRU-CP + B & 0.58 (0.18) &   GRU-MLP/MC + B & 0.78 (0.12) &   SA-RMTPP + BFC & 0.69 (0.14) \\
          SA-MLP/MC + BFC & -38.16 (12.42) & GRU-MLP/CM + BFC & 56.18 (17.39) &          GRU-LNM & 1.15 (0.05) &    GRU-SA/CM + B &  18.1 (5.35) &      SA-CP + BFC & 0.58 (0.18) &  GRU-RMTPP + BFC & 0.79 (0.13) &     SA-RMTPP + B & 0.69 (0.14) \\
                GRU-SA/MC & -38.14 (12.44) &       GRU-CP + B &  56.2 (17.41) &   GRU-MLP/MC + B & 1.16 (0.05) &            SA-CP & 18.11 (5.37) &        SA-CP + B & 0.58 (0.18) &        SA-MLP/CM &  0.79 (0.1) &         SA-RMTPP & 0.69 (0.14) \\
            SA-MLP/MC + B & -38.13 (12.41) &        SA-MLP/MC & 56.28 (17.44) &       GRU-MLP/MC & 1.16 (0.05) &      SA-CP + BFC & 18.13 (5.38) &     GRU-CP + BFC & 0.59 (0.18) &           GRU-CP & 0.79 (0.13) &            SA-CP & 0.69 (0.14) \\
                 SA-SA/MC & -37.98 (12.39) &        GRU-SA/CM &   56.3 (17.4) &    GRU-SA/MC + B & 1.17 (0.03) &     SA-SA/CM + B & 18.16 (5.37) &     SA-SA/MC + B & 0.59 (0.19) &        SA-CP + B & 0.79 (0.11) &      SA-CP + BFC & 0.69 (0.14) \\
         GRU-MLP/CM + BFC & -37.91 (12.37) &        SA-CP + B & 56.32 (17.46) &  GRU-RMTPP + BFC & 1.17 (0.05) &        GRU-SA/MC &  18.2 (5.38) &    GRU-SA/CM + B & 0.59 (0.19) &       GRU-CP + B & 0.79 (0.11) &    SA-MLP/MC + B & 0.68 (0.13) \\
          GRU-SA/CM + BFC & -37.81 (12.36) &         SA-SA/MC & 56.33 (17.44) &     SA-SA/MC + B & 1.18 (0.04) & GRU-MLP/CM + BFC &  18.27 (5.4) &    GRU-SA/MC + B & 0.59 (0.19) &    GRU-SA/MC + B &  0.8 (0.12) &           SA-LNM & 0.68 (0.14) \\
              SA-CP + BFC & -37.79 (12.31) &        GRU-SA/MC & 56.34 (17.44) &         SA-SA/MC & 1.18 (0.03) &         SA-SA/MC & 18.36 (5.43) &  GRU-RMTPP + BFC & 0.59 (0.19) &  GRU-SA/MC + BFC & 0.81 (0.12) &     SA-LNM + BFC & 0.68 (0.14) \\
                    SA-CP & -37.78 (12.31) &  GRU-SA/CM + BFC & 56.36 (17.43) &           GRU-CP & 1.18 (0.05) &        SA-MLP/MC &  18.51 (5.5) &         SA-SA/MC &  0.6 (0.19) &     SA-SA/MC + B & 0.81 (0.12) &   SA-SA/CM + BFC & 0.68 (0.18) \\
           SA-SA/CM + BFC & -37.77 (12.34) &     SA-SA/CM + B & 56.45 (17.48) &    GRU-SA/CM + B & 1.18 (0.05) &  GRU-SA/CM + BFC & 18.55 (5.47) &     SA-SA/CM + B &  0.6 (0.19) &        GRU-SA/MC & 0.81 (0.12) &    GRU-SA/CM + B & 0.66 (0.17) \\
                SA-MLP/MC &  -37.77 (12.3) &    GRU-SA/CM + B & 56.45 (17.48) & GRU-MLP/CM + BFC & 1.19 (0.06) &        SA-CP + B &  18.6 (5.53) &   SA-SA/MC + BFC &  0.6 (0.19) &    GRU-SA/CM + B & 0.81 (0.12) &     SA-SA/CM + B & 0.66 (0.17) \\
                SA-CP + B & -37.72 (12.29) &         SA-SA/CM & 56.46 (17.45) &     SA-SA/CM + B & 1.19 (0.04) &       GRU-MLP/CM & 18.63 (5.51) & GRU-MLP/CM + BFC &  0.6 (0.19) &         SA-SA/MC & 0.81 (0.12) &       GRU-CP + B & 0.66 (0.15) \\
               GRU-MLP/CM & -37.46 (12.24) &   SA-SA/CM + BFC & 56.46 (17.47) &   SA-SA/MC + BFC & 1.19 (0.05) &   SA-SA/CM + BFC & 18.69 (5.52) &           GRU-CP &  0.6 (0.18) &   SA-SA/MC + BFC & 0.82 (0.12) &        SA-CP + B & 0.65 (0.15) \\
                GRU-SA/CM & -37.35 (12.22) &   GRU-MLP/CM + B & 56.48 (17.53) &        GRU-SA/MC & 1.19 (0.04) &        GRU-SA/CM &  18.95 (5.6) &  GRU-SA/MC + BFC &  0.6 (0.19) & GRU-MLP/CM + BFC & 0.82 (0.12) &        SA-MLP/CM &  0.6 (0.16) \\
                 SA-SA/CM & -37.18 (12.17) &    SA-MLP/CM + B & 56.51 (17.54) &  GRU-SA/MC + BFC &  1.2 (0.03) &         SA-SA/CM & 19.28 (5.69) &        GRU-SA/MC &  0.6 (0.19) &       GRU-MLP/CM & 0.82 (0.13) &      GRU-LNM + B &  0.6 (0.14) \\
           GRU-MLP/CM + B &  -37.1 (12.07) &  SA-MLP/CM + BFC & 56.51 (17.53) &       GRU-MLP/CM & 1.21 (0.04) &   GRU-MLP/CM + B &  19.38 (5.8) &       GRU-MLP/CM & 0.61 (0.19) &     SA-SA/CM + B & 0.82 (0.12) &  SA-MLP/CM + BFC & 0.59 (0.15) \\
            SA-MLP/CM + B & -36.86 (11.99) &        SA-MLP/CM & 56.54 (17.53) &   SA-SA/CM + BFC & 1.24 (0.04) &    SA-MLP/CM + B & 19.65 (5.88) &   SA-SA/CM + BFC &  0.62 (0.2) &   SA-SA/CM + BFC & 0.84 (0.13) &   GRU-MLP/CM + B & 0.59 (0.15) \\
          SA-MLP/CM + BFC & -36.36 (11.84) &       SA-LNM + B & 56.66 (17.64) &  GRU-SA/CM + BFC & 1.25 (0.04) &  SA-MLP/CM + BFC & 20.16 (6.03) &  GRU-SA/CM + BFC &  0.63 (0.2) &  GRU-SA/CM + BFC & 0.84 (0.13) &    SA-MLP/CM + B & 0.58 (0.15) \\
                SA-MLP/CM & -35.82 (11.68) &      GRU-LNM + B & 56.82 (17.64) &        GRU-SA/CM & 1.27 (0.05) &        SA-MLP/CM &  20.72 (6.2) &        GRU-SA/CM &  0.64 (0.2) &        GRU-SA/CM & 0.85 (0.13) &       SA-LNM + B & 0.53 (0.12) \\
                  Poisson & -35.33 (11.47) &          Poisson &  57.2 (17.79) &         SA-SA/CM & 1.29 (0.06) &          Poisson & 21.87 (6.62) &         SA-SA/CM & 0.65 (0.21) &         SA-SA/CM & 0.87 (0.14) &          Poisson & 0.52 (0.13) \\
\bottomrule
\end{tabular}

\label{resultsmark}
\caption{Hawkes Exponential Dependent}
\end{table}


\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccccccccccccc}
\toprule
               0 &       NLL Time &                1 &      NLL Mark &                2 &  NLL Window &                3 &    NLL Total &                4 &   Time Cal. &                5 &   Mark Cal. &                6 &    F1-score \\
\midrule
      SA-LNM + B & -67.19 (23.09) &  GRU-RMTPP + BFC & 57.39 (17.72) &       SA-LNM + B & 1.35 (0.06) &       SA-LNM + B & -8.41 (8.37) &          GRU-LNM & 0.69 (0.22) &    GRU-LNM + BFC &  0.9 (0.15) &         SA-SA/MC & 0.98 (0.24) \\
     GRU-LNM + B & -59.63 (19.48) &    GRU-LNM + BFC & 57.39 (17.72) &          GRU-LNM & 1.38 (0.02) &      GRU-LNM + B &  0.01 (2.07) &    GRU-LNM + BFC & 0.69 (0.22) &  GRU-RMTPP + BFC &  0.9 (0.15) &        SA-MLP/MC & 0.96 (0.23) \\
   GRU-LNM + BFC &  -43.4 (14.17) &    GRU-RMTPP + B & 57.42 (17.72) &      GRU-LNM + B & 1.38 (0.04) &    GRU-LNM + BFC & 13.99 (3.99) &  GRU-RMTPP + BFC &  0.7 (0.22) &    GRU-RMTPP + B &  0.9 (0.16) &        GRU-SA/MC & 0.95 (0.23) \\
GRU-MLP/MC + BFC &  -43.4 (14.19) &          GRU-LNM & 57.43 (17.73) &    GRU-LNM + BFC & 1.38 (0.02) &          GRU-LNM & 14.08 (4.02) &    GRU-RMTPP + B &  0.7 (0.22) &       SA-LNM + B &  0.9 (0.15) &            SA-CP & 0.94 (0.23) \\
  GRU-MLP/MC + B & -43.37 (14.17) &        GRU-RMTPP & 57.43 (17.72) &  GRU-RMTPP + BFC & 1.38 (0.02) &   GRU-MLP/MC + B &  14.1 (4.02) &       SA-LNM + B &  0.7 (0.21) &          GRU-LNM & 0.91 (0.15) &       GRU-MLP/MC & 0.94 (0.22) \\
         GRU-LNM & -43.34 (14.15) &   GRU-MLP/MC + B & 57.47 (17.74) &    GRU-RMTPP + B & 1.39 (0.02) &  GRU-RMTPP + BFC & 14.13 (4.04) &        GRU-RMTPP & 0.71 (0.22) &      GRU-LNM + B & 0.91 (0.15) &      SA-CP + BFC & 0.94 (0.23) \\
 GRU-RMTPP + BFC & -43.26 (14.13) &    SA-MLP/MC + B & 57.52 (17.74) &        GRU-RMTPP &  1.4 (0.02) &    GRU-RMTPP + B & 14.17 (4.05) &      GRU-LNM + B & 0.71 (0.21) &        GRU-RMTPP & 0.91 (0.16) &        SA-CP + B & 0.92 (0.23) \\
   GRU-RMTPP + B & -43.25 (14.13) &     SA-RMTPP + B & 57.53 (17.73) &   GRU-MLP/MC + B &  1.4 (0.02) & GRU-MLP/MC + BFC & 14.22 (4.04) &   GRU-MLP/MC + B & 0.71 (0.22) &           Hawkes & 0.92 (0.16) &        SA-MLP/CM & 0.92 (0.26) \\
          Hawkes & -43.23 (14.13) &   SA-RMTPP + BFC & 57.56 (17.75) &           Hawkes & 1.42 (0.02) &        GRU-RMTPP & 14.47 (4.13) &     SA-LNM + BFC & 0.72 (0.23) &   GRU-MLP/MC + B & 0.92 (0.15) &   SA-SA/MC + BFC & 0.91 (0.21) \\
   GRU-SA/MC + B & -43.02 (14.07) &    GRU-SA/MC + B & 57.57 (17.76) &     SA-LNM + BFC & 1.44 (0.03) &    GRU-SA/MC + B & 14.55 (4.15) &    GRU-SA/MC + B & 0.72 (0.23) &     SA-LNM + BFC & 0.94 (0.16) &  SA-MLP/CM + BFC & 0.91 (0.25) \\
 GRU-SA/MC + BFC & -42.98 (14.07) &           GRU-CP & 57.61 (17.73) &    GRU-SA/MC + B & 1.44 (0.02) &  GRU-SA/MC + BFC &  14.74 (4.2) & GRU-MLP/MC + BFC & 0.72 (0.23) &    GRU-SA/MC + B & 0.94 (0.16) &    SA-MLP/CM + B &  0.9 (0.25) \\
       GRU-RMTPP & -42.97 (14.04) & GRU-MLP/MC + BFC & 57.62 (17.77) & GRU-MLP/MC + BFC & 1.44 (0.02) &           Hawkes & 14.79 (4.23) &           Hawkes & 0.72 (0.22) & GRU-MLP/MC + BFC & 0.94 (0.16) &           GRU-CP &  0.9 (0.21) \\
      GRU-MLP/MC & -42.71 (14.03) &     SA-LNM + BFC & 57.62 (17.77) &           SA-LNM & 1.44 (0.02) &    SA-MLP/MC + B &  15.06 (4.3) &           SA-LNM & 0.72 (0.23) &   SA-RMTPP + BFC & 0.94 (0.16) &     GRU-CP + BFC & 0.89 (0.22) \\
    SA-LNM + BFC & -42.54 (13.92) &           SA-LNM & 57.64 (17.78) &    SA-MLP/MC + B & 1.45 (0.03) &   SA-RMTPP + BFC & 15.08 (4.31) &    SA-MLP/MC + B & 0.73 (0.23) &           SA-LNM & 0.94 (0.16) &   GRU-MLP/CM + B & 0.89 (0.25) \\
          SA-LNM & -42.54 (13.92) &         SA-RMTPP & 57.65 (17.76) &   SA-RMTPP + BFC & 1.45 (0.02) &     SA-LNM + BFC & 15.08 (4.31) &   SA-RMTPP + BFC & 0.73 (0.23) &       GRU-MLP/CM & 0.95 (0.16) &     SA-SA/MC + B & 0.89 (0.21) \\
  SA-RMTPP + BFC &  -42.48 (13.9) &     SA-SA/MC + B &  57.7 (17.76) &       GRU-MLP/CM & 1.46 (0.01) &           SA-LNM &  15.1 (4.32) &       GRU-MLP/CM & 0.74 (0.23) &     SA-RMTPP + B & 0.95 (0.16) &  GRU-SA/CM + BFC & 0.89 (0.24) \\
   SA-MLP/MC + B &  -42.47 (13.9) &  GRU-SA/MC + BFC & 57.72 (17.79) &     SA-RMTPP + B & 1.47 (0.03) &     SA-RMTPP + B & 15.13 (4.32) &     SA-RMTPP + B & 0.74 (0.23) &    SA-MLP/MC + B & 0.95 (0.16) &        GRU-SA/CM & 0.88 (0.25) \\
 SA-MLP/MC + BFC & -42.47 (13.91) &     GRU-CP + BFC & 57.74 (17.77) &  GRU-SA/MC + BFC & 1.47 (0.04) &  SA-MLP/MC + BFC & 15.27 (4.36) &  GRU-SA/MC + BFC & 0.74 (0.23) &  SA-MLP/MC + BFC & 0.96 (0.16) & GRU-MLP/CM + BFC & 0.88 (0.22) \\
    SA-RMTPP + B &  -42.4 (13.88) &  SA-MLP/MC + BFC & 57.74 (17.79) &  SA-MLP/MC + BFC & 1.48 (0.03) &       GRU-MLP/MC & 15.47 (4.38) &  SA-MLP/MC + BFC & 0.75 (0.23) &  GRU-SA/MC + BFC & 0.96 (0.16) &          Poisson & 0.88 (0.25) \\
       GRU-SA/MC &  -42.3 (13.91) &   SA-SA/MC + BFC & 57.76 (17.77) &         SA-RMTPP &  1.5 (0.02) &       GRU-MLP/CM &  15.6 (4.48) &         SA-RMTPP & 0.76 (0.23) &         SA-RMTPP & 0.97 (0.17) &         SA-RMTPP &  0.87 (0.2) \\
      GRU-MLP/CM &  -42.16 (13.8) &            SA-CP & 57.76 (17.75) &   SA-SA/CM + BFC & 1.55 (0.01) &         SA-RMTPP & 15.66 (4.48) &   SA-SA/CM + BFC & 0.78 (0.24) &   SA-SA/CM + BFC &  1.0 (0.17) &       GRU-CP + B & 0.87 (0.23) \\
        SA-RMTPP & -41.98 (13.76) &       GRU-MLP/CM & 57.76 (17.81) &     GRU-CP + BFC & 1.56 (0.05) &     SA-SA/MC + B &  15.77 (4.5) &     SA-SA/MC + B & 0.78 (0.25) &     GRU-CP + BFC &  1.0 (0.18) &         SA-SA/CM & 0.87 (0.24) \\
    SA-SA/MC + B & -41.94 (13.76) &      SA-CP + BFC & 57.81 (17.76) &     SA-SA/MC + B & 1.56 (0.02) &   SA-SA/MC + BFC & 15.84 (4.51) &     SA-SA/CM + B & 0.79 (0.25) &     SA-SA/MC + B &  1.0 (0.18) &    GRU-SA/CM + B & 0.86 (0.22) \\
  SA-SA/MC + BFC & -41.92 (13.77) &    GRU-SA/CM + B &  57.85 (17.8) &     SA-SA/CM + B & 1.57 (0.02) &        GRU-SA/MC & 16.06 (4.56) &    GRU-SA/CM + B & 0.79 (0.25) &     SA-SA/CM + B & 1.01 (0.18) &     SA-RMTPP + B & 0.86 (0.19) \\
       SA-MLP/MC & -41.87 (13.79) &     SA-SA/CM + B & 57.87 (17.81) &           GRU-CP & 1.57 (0.05) &    GRU-SA/CM + B & 16.28 (4.65) &   SA-SA/MC + BFC &  0.8 (0.25) &           GRU-CP & 1.01 (0.18) &     SA-SA/CM + B & 0.86 (0.23) \\
   GRU-SA/CM + B & -41.58 (13.65) &       GRU-CP + B &  57.9 (17.82) &    GRU-SA/CM + B & 1.57 (0.03) &           GRU-CP & 16.31 (4.67) &           GRU-CP & 0.81 (0.24) &       GRU-CP + B & 1.01 (0.18) &  SA-MLP/MC + BFC &  0.86 (0.2) \\
    SA-SA/CM + B &  -41.5 (13.63) &   SA-SA/CM + BFC &  57.9 (17.82) &   SA-SA/MC + BFC & 1.58 (0.02) &     GRU-CP + BFC & 16.38 (4.69) &     GRU-CP + BFC & 0.81 (0.24) &    GRU-SA/CM + B & 1.01 (0.18) & GRU-MLP/MC + BFC & 0.85 (0.19) \\
        SA-SA/MC & -41.39 (13.64) & GRU-MLP/CM + BFC & 57.92 (17.82) &       GRU-CP + B & 1.58 (0.05) &     SA-SA/CM + B & 16.38 (4.68) & GRU-MLP/CM + BFC & 0.81 (0.24) &   SA-SA/MC + BFC & 1.02 (0.18) &    SA-MLP/MC + B & 0.85 (0.19) \\
      GRU-CP + B & -41.37 (13.59) &  GRU-SA/CM + BFC & 57.94 (17.81) & GRU-MLP/CM + BFC & 1.59 (0.04) &        SA-MLP/MC & 16.45 (4.67) &       GRU-CP + B & 0.82 (0.24) & GRU-MLP/CM + BFC & 1.02 (0.18) &  GRU-SA/MC + BFC &  0.85 (0.2) \\
    GRU-CP + BFC & -41.36 (13.58) &        SA-CP + B & 57.96 (17.81) &         SA-SA/CM & 1.63 (0.04) &       GRU-CP + B & 16.54 (4.73) &  GRU-SA/CM + BFC & 0.82 (0.26) &       GRU-MLP/MC & 1.02 (0.19) &   SA-SA/CM + BFC & 0.84 (0.23) \\
          GRU-CP &  -41.3 (13.57) &        GRU-SA/CM & 58.01 (17.83) &       GRU-MLP/MC & 1.63 (0.03) & GRU-MLP/CM + BFC & 16.62 (4.76) &         SA-SA/CM & 0.82 (0.26) &  GRU-SA/CM + BFC & 1.04 (0.19) &           SA-LNM & 0.84 (0.19) \\
GRU-MLP/CM + BFC &  -41.3 (13.57) &           Hawkes &  58.02 (17.9) &  GRU-SA/CM + BFC & 1.64 (0.03) &  GRU-SA/CM + BFC & 16.85 (4.81) &       GRU-MLP/MC & 0.82 (0.26) &        SA-CP + B & 1.05 (0.19) &     SA-LNM + BFC & 0.84 (0.19) \\
 GRU-SA/CM + BFC & -41.09 (13.52) &         SA-SA/CM & 58.03 (17.84) &            SA-CP & 1.65 (0.05) &   SA-SA/CM + BFC & 16.86 (4.84) &        GRU-SA/CM & 0.83 (0.26) &         SA-SA/CM & 1.05 (0.18) &   SA-RMTPP + BFC & 0.84 (0.19) \\
  SA-SA/CM + BFC & -41.04 (13.48) &   GRU-MLP/CM + B &  58.1 (17.85) &          Poisson & 1.65 (0.04) &         SA-SA/MC & 16.97 (4.83) &        GRU-SA/MC & 0.83 (0.26) &      SA-CP + BFC & 1.05 (0.19) &           Hawkes & 0.84 (0.18) \\
       GRU-SA/CM & -40.63 (13.38) &    SA-MLP/CM + B & 58.11 (17.85) &        SA-CP + B & 1.66 (0.05) &        GRU-SA/CM & 17.38 (4.97) &        SA-MLP/MC & 0.85 (0.27) &            SA-CP & 1.05 (0.19) &        GRU-RMTPP & 0.83 (0.18) \\
        SA-SA/CM & -40.51 (13.33) &  SA-MLP/CM + BFC & 58.12 (17.84) &        GRU-SA/MC & 1.66 (0.04) &         SA-SA/CM & 17.52 (5.03) &         SA-SA/MC & 0.86 (0.27) &          Poisson & 1.06 (0.19) &    GRU-SA/MC + B & 0.83 (0.19) \\
       SA-CP + B & -39.97 (13.17) &        SA-MLP/CM & 58.13 (17.84) &      SA-CP + BFC & 1.66 (0.05) &      SA-CP + BFC & 17.88 (5.13) &        SA-CP + B & 0.86 (0.25) &        GRU-SA/MC & 1.06 (0.19) &    GRU-RMTPP + B & 0.82 (0.18) \\
     SA-CP + BFC & -39.93 (13.16) &       GRU-MLP/MC & 58.19 (17.89) &        GRU-SA/CM & 1.66 (0.04) &            SA-CP &  17.9 (5.14) &      SA-CP + BFC & 0.86 (0.25) &        GRU-SA/CM & 1.06 (0.19) &   GRU-MLP/MC + B & 0.82 (0.18) \\
           SA-CP & -39.86 (13.14) &        SA-MLP/MC & 58.32 (17.91) &   GRU-MLP/CM + B & 1.67 (0.03) &        SA-CP + B & 17.99 (5.17) &            SA-CP & 0.86 (0.25) &        SA-MLP/MC &  1.07 (0.2) &       GRU-MLP/CM &  0.82 (0.2) \\
  GRU-MLP/CM + B & -39.27 (12.96) &         SA-SA/MC & 58.35 (17.91) &        SA-MLP/MC & 1.69 (0.04) &   GRU-MLP/CM + B & 18.83 (5.43) &          Poisson & 0.87 (0.25) &   GRU-MLP/CM + B & 1.07 (0.19) &  GRU-RMTPP + BFC & 0.81 (0.18) \\
   SA-MLP/CM + B & -39.25 (12.96) &        GRU-SA/MC & 58.35 (17.93) &    SA-MLP/CM + B & 1.69 (0.04) &    SA-MLP/CM + B & 18.86 (5.43) &   GRU-MLP/CM + B & 0.87 (0.25) &    SA-MLP/CM + B & 1.08 (0.19) &    GRU-LNM + BFC & 0.81 (0.18) \\
 SA-MLP/CM + BFC & -38.84 (12.83) &       SA-LNM + B & 58.78 (18.17) &  SA-MLP/CM + BFC & 1.71 (0.04) &  SA-MLP/CM + BFC & 19.27 (5.56) &    SA-MLP/CM + B & 0.87 (0.26) &  SA-MLP/CM + BFC &  1.09 (0.2) &          GRU-LNM & 0.81 (0.18) \\
       SA-MLP/CM & -38.34 (12.68) &          Poisson & 58.84 (18.09) &         SA-SA/MC & 1.72 (0.04) &        SA-MLP/CM & 19.79 (5.71) &  SA-MLP/CM + BFC & 0.88 (0.26) &         SA-SA/MC &  1.09 (0.2) &      GRU-LNM + B & 0.77 (0.19) \\
         Poisson & -37.02 (12.24) &      GRU-LNM + B & 59.63 (18.43) &        SA-MLP/CM & 1.73 (0.04) &          Poisson & 21.82 (6.38) &        SA-MLP/CM & 0.89 (0.27) &        SA-MLP/CM &   1.1 (0.2) &       SA-LNM + B & 0.75 (0.19) \\
\bottomrule
\end{tabular}

\label{resultsmark}
\caption{Hawkes Sum Exponential Dependent}
\end{table}


\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccc|cccc|cccc}
\toprule
            \multicolumn{4}{c}{\textbf{taxi}} & \multicolumn{4}{c}{\textbf{twitter}} & \multicolumn{4}{c}{\textbf{Reddit politics submissions}} \\
               0 &             NLL &                1 &   Time Cal. &                2 &           NLL &                3 &   Time Cal. &                           4 &               NLL &                5 &   Time Cal. \\
\midrule
      SA-LNM + B & -246.92 (12.62) & GRU-MLP/MC + BFC &   0.0 (0.0) &       SA-LNM + B & -21.56 (1.74) &           Hawkes &  0.01 (0.0) &                  SA-LNM + B & -6110.55 (208.28) &           Hawkes &   0.0 (0.0) \\
     GRU-LNM + B & -235.45 (12.16) &           GRU-CP &  0.01 (0.0) &      GRU-LNM + B & -20.43 (1.38) &     SA-LNM + BFC &  0.01 (0.0) &                 GRU-LNM + B & -5691.05 (233.79) &   GRU-MLP/MC + B &   0.0 (0.0) \\
 GRU-SA/MC + BFC &  -137.09 (4.04) &           SA-LNM &  0.01 (0.0) &          GRU-LNM & -12.52 (0.58) &           SA-LNM &  0.01 (0.0) &                     GRU-LNM &  -4496.27 (37.01) &       GRU-MLP/MC &   0.0 (0.0) \\
  GRU-MLP/MC + B &  -137.07 (4.02) &     SA-LNM + BFC &  0.01 (0.0) &    GRU-LNM + BFC & -12.24 (0.53) &         SA-SA/CM &  0.01 (0.0) &               GRU-LNM + BFC &   -4439.2 (31.99) &    GRU-SA/MC + B &   0.0 (0.0) \\
       GRU-SA/MC &  -137.05 (4.03) &        SA-MLP/MC &  0.01 (0.0) &  GRU-SA/MC + BFC & -12.15 (0.49) &  GRU-SA/MC + BFC &  0.01 (0.0) &                      SA-LNM &  -4405.48 (28.12) &        GRU-SA/MC &   0.0 (0.0) \\
         GRU-LNM &  -137.02 (3.87) &    SA-MLP/MC + B &  0.01 (0.0) &    GRU-SA/MC + B &  -12.09 (0.5) &    GRU-SA/MC + B &  0.01 (0.0) &            GRU-MLP/MC + BFC &  -4405.44 (23.91) &         SA-SA/MC &   0.0 (0.0) \\
      GRU-MLP/MC &  -136.98 (3.97) &  SA-MLP/MC + BFC &  0.01 (0.0) &     SA-SA/MC + B & -11.98 (0.55) &        GRU-SA/MC &  0.01 (0.0) &                  GRU-MLP/MC &  -4405.18 (23.94) &     SA-SA/CM + B &  0.01 (0.0) \\
   GRU-SA/MC + B &  -136.97 (4.06) &         SA-RMTPP &  0.01 (0.0) &        GRU-SA/MC & -11.88 (0.57) &  GRU-SA/CM + BFC &  0.01 (0.0) &              GRU-MLP/MC + B &  -4404.68 (23.82) &         SA-SA/CM &  0.01 (0.0) \\
   GRU-LNM + BFC &  -136.88 (3.92) &     SA-RMTPP + B &  0.01 (0.0) &           SA-LNM &  -11.74 (0.6) &    GRU-SA/CM + B &  0.01 (0.0) &                   GRU-SA/MC &   -4404.6 (23.63) &  SA-MLP/MC + BFC &  0.01 (0.0) \\
GRU-MLP/MC + BFC &  -136.87 (4.01) &   SA-RMTPP + BFC &  0.01 (0.0) &     SA-LNM + BFC &  -11.7 (0.65) &        GRU-SA/CM &  0.01 (0.0) &               GRU-SA/MC + B &  -4404.01 (23.36) &     SA-SA/MC + B &  0.01 (0.0) \\
       GRU-RMTPP &   -136.8 (3.93) &         SA-SA/CM &  0.01 (0.0) &         SA-SA/MC & -11.48 (0.46) &   SA-SA/MC + BFC &  0.01 (0.0) &                  GRU-CP + B &   -4403.97 (24.0) &   SA-SA/MC + BFC &  0.01 (0.0) \\
      GRU-CP + B &  -136.78 (3.91) &     SA-SA/CM + B &  0.01 (0.0) &    GRU-SA/CM + B & -11.46 (0.52) &     SA-SA/MC + B &  0.01 (0.0) &                GRU-CP + BFC &  -4403.44 (23.62) &        SA-MLP/MC &  0.01 (0.0) \\
    GRU-CP + BFC &  -136.65 (4.01) &   SA-SA/CM + BFC &  0.01 (0.0) &  GRU-SA/CM + BFC & -11.29 (0.51) &     SA-SA/CM + B &  0.01 (0.0) &               GRU-RMTPP + B &  -4403.24 (24.14) &     SA-LNM + BFC &  0.01 (0.0) \\
 GRU-RMTPP + BFC &  -136.53 (4.15) &         SA-SA/MC &  0.01 (0.0) &        GRU-SA/CM &  -11.2 (0.49) &   SA-SA/CM + BFC &  0.01 (0.0) &                      GRU-CP &  -4402.72 (23.78) &           SA-LNM &  0.01 (0.0) \\
          GRU-CP &  -136.39 (4.12) &     SA-SA/MC + B &  0.01 (0.0) &   GRU-MLP/MC + B & -11.19 (0.59) &         SA-SA/MC &  0.01 (0.0) &                   GRU-RMTPP &   -4402.27 (24.1) &  GRU-SA/MC + BFC &  0.01 (0.0) \\
  SA-SA/MC + BFC &  -136.27 (4.13) &   SA-SA/MC + BFC &  0.01 (0.0) &   SA-SA/MC + BFC & -11.05 (0.51) &    GRU-LNM + BFC &  0.01 (0.0) &             GRU-SA/MC + BFC &  -4401.33 (23.74) &   SA-SA/CM + BFC &  0.01 (0.0) \\
   GRU-RMTPP + B &  -136.19 (4.11) &  GRU-SA/MC + BFC &  0.01 (0.0) &       GRU-MLP/MC & -11.04 (0.54) &          GRU-LNM &  0.01 (0.0) &             GRU-RMTPP + BFC &  -4401.26 (23.98) &    SA-MLP/MC + B &  0.01 (0.0) \\
   GRU-SA/CM + B &  -136.09 (4.15) &    GRU-SA/MC + B &  0.01 (0.0) & GRU-MLP/MC + BFC & -10.99 (0.51) &   GRU-MLP/MC + B &  0.02 (0.0) &                      Hawkes &   -4395.2 (23.74) &           GRU-CP &  0.01 (0.0) \\
        SA-SA/MC &  -136.08 (4.11) &           Hawkes &  0.01 (0.0) &   SA-SA/CM + BFC & -10.92 (0.54) & GRU-MLP/MC + BFC &  0.02 (0.0) &              SA-SA/MC + BFC &  -4364.59 (22.44) &    GRU-SA/CM + B &  0.01 (0.0) \\
    SA-SA/MC + B &  -135.38 (4.34) &  GRU-SA/CM + BFC &  0.01 (0.0) &     SA-SA/CM + B & -10.86 (0.51) &  SA-MLP/MC + BFC &  0.02 (0.0) &                    SA-SA/MC &   -4360.57 (30.0) &       GRU-CP + B &  0.01 (0.0) \\
 GRU-SA/CM + BFC &  -135.35 (4.18) &       GRU-CP + B &  0.01 (0.0) &         SA-SA/CM & -10.81 (0.51) &    SA-MLP/MC + B &  0.02 (0.0) &                SA-SA/MC + B &  -4359.53 (25.93) &     GRU-CP + BFC &  0.01 (0.0) \\
    SA-SA/CM + B &  -135.24 (4.13) &     GRU-CP + BFC &  0.01 (0.0) &    SA-MLP/MC + B &  -10.7 (0.55) &       GRU-MLP/MC &  0.02 (0.0) &                SA-LNM + BFC &  -4357.62 (26.71) &          GRU-LNM &  0.01 (0.0) \\
       GRU-SA/CM &  -135.07 (3.99) &          GRU-LNM &  0.01 (0.0) &  SA-MLP/MC + BFC & -10.66 (0.47) &        SA-MLP/MC &  0.03 (0.0) &               GRU-SA/CM + B &  -4337.55 (24.44) &    GRU-LNM + BFC &  0.01 (0.0) \\
  SA-SA/CM + BFC &  -134.56 (4.26) &    GRU-LNM + BFC &  0.01 (0.0) &        SA-MLP/MC & -10.51 (0.57) &  GRU-RMTPP + BFC &  0.04 (0.0) &                   SA-MLP/MC &  -4336.75 (23.56) &  GRU-SA/CM + BFC &  0.01 (0.0) \\
        SA-SA/CM &  -134.39 (3.97) &       GRU-MLP/MC &  0.01 (0.0) &  GRU-RMTPP + BFC & -10.22 (0.58) &      GRU-LNM + B & 0.04 (0.01) &             GRU-SA/CM + BFC &   -4336.19 (25.8) &        GRU-RMTPP &  0.01 (0.0) \\
          Hawkes &  -134.09 (3.93) &   GRU-MLP/MC + B &  0.01 (0.0) &    GRU-RMTPP + B & -10.21 (0.57) &     SA-RMTPP + B &  0.05 (0.0) &               SA-MLP/MC + B &  -4335.22 (23.46) & GRU-MLP/MC + BFC &  0.01 (0.0) \\
   SA-MLP/MC + B &   -133.24 (4.0) &        GRU-SA/MC &  0.01 (0.0) &   SA-RMTPP + BFC &   -9.7 (0.56) &    GRU-RMTPP + B &  0.05 (0.0) &             SA-MLP/MC + BFC &  -4334.97 (23.07) &    GRU-RMTPP + B &  0.01 (0.0) \\
          SA-LNM &  -133.07 (3.84) &    GRU-RMTPP + B &  0.01 (0.0) &     SA-RMTPP + B &  -9.57 (0.51) &   SA-RMTPP + BFC &  0.05 (0.0) &                    SA-SA/CM &  -4327.87 (25.52) &        GRU-SA/CM &  0.01 (0.0) \\
       SA-MLP/MC &   -132.91 (3.7) &        GRU-RMTPP &  0.01 (0.0) &        GRU-RMTPP &  -8.07 (0.51) &       SA-LNM + B & 0.07 (0.01) &                    SA-RMTPP &  -4327.58 (23.84) &  GRU-RMTPP + BFC &  0.01 (0.0) \\
    SA-LNM + BFC &   -132.9 (3.75) &  GRU-RMTPP + BFC &  0.01 (0.0) &           Hawkes &  -7.61 (0.51) &        GRU-RMTPP &  0.09 (0.0) &              SA-RMTPP + BFC &  -4327.22 (24.45) &        SA-CP + B &  0.02 (0.0) \\
    SA-RMTPP + B &  -132.89 (3.48) &        GRU-SA/CM &  0.01 (0.0) &         SA-RMTPP &  -7.31 (0.44) &         SA-RMTPP &   0.1 (0.0) &                SA-RMTPP + B &   -4327.0 (24.17) &   SA-RMTPP + BFC &  0.02 (0.0) \\
 SA-MLP/MC + BFC &  -132.62 (3.68) &    GRU-SA/CM + B &  0.01 (0.0) &           GRU-CP &  -6.22 (0.46) &           GRU-CP &  0.13 (0.0) &                SA-SA/CM + B &  -4326.64 (23.94) &         SA-RMTPP &  0.02 (0.0) \\
      GRU-MLP/CM &  -132.57 (5.16) &       GRU-MLP/CM &  0.02 (0.0) &       GRU-CP + B &  -6.21 (0.46) &     GRU-CP + BFC &  0.13 (0.0) &              SA-SA/CM + BFC &  -4326.39 (22.97) &     SA-RMTPP + B &  0.02 (0.0) \\
        SA-RMTPP &  -132.44 (3.62) &      SA-CP + BFC &  0.02 (0.0) &     GRU-CP + BFC &  -6.17 (0.43) &       GRU-CP + B &  0.13 (0.0) &                   GRU-SA/CM &  -4325.92 (23.95) &      SA-CP + BFC &  0.02 (0.0) \\
     SA-CP + BFC &  -132.27 (3.15) &            SA-CP &  0.02 (0.0) &            SA-CP &  -4.51 (0.38) &    SA-MLP/CM + B &  0.15 (0.0) &                 SA-CP + BFC &  -4324.59 (24.66) &            SA-CP &  0.02 (0.0) \\
  SA-RMTPP + BFC &   -132.19 (3.7) &        SA-CP + B &  0.03 (0.0) &      SA-CP + BFC &  -4.42 (0.36) &        SA-MLP/CM &  0.15 (0.0) &                   SA-CP + B &   -4322.37 (23.1) & GRU-MLP/CM + BFC &  0.03 (0.0) \\
       SA-CP + B &   -131.2 (3.57) &  SA-MLP/CM + BFC &  0.04 (0.0) &        SA-CP + B &  -4.32 (0.35) &      SA-CP + BFC &  0.15 (0.0) &                       SA-CP &    -4320.8 (22.4) &       GRU-MLP/CM &  0.03 (0.0) \\
           SA-CP &  -130.86 (3.56) &        SA-MLP/CM &  0.04 (0.0) &    SA-MLP/CM + B &  -3.49 (0.25) & GRU-MLP/CM + BFC &  0.15 (0.0) &              GRU-MLP/CM + B &  -4271.73 (23.53) &  SA-MLP/CM + BFC &  0.03 (0.0) \\
   SA-MLP/CM + B &  -126.33 (3.62) & GRU-MLP/CM + BFC &  0.04 (0.0) &   GRU-MLP/CM + B &  -3.48 (0.25) &   GRU-MLP/CM + B &  0.15 (0.0) &            GRU-MLP/CM + BFC &   -4270.7 (23.52) &    SA-MLP/CM + B &  0.03 (0.0) \\
  GRU-MLP/CM + B &  -126.13 (3.69) &   GRU-MLP/CM + B &  0.04 (0.0) & GRU-MLP/CM + BFC &  -3.47 (0.25) &       GRU-MLP/CM &  0.15 (0.0) &                  GRU-MLP/CM &  -4268.18 (23.31) &        SA-MLP/CM &  0.03 (0.0) \\
 SA-MLP/CM + BFC &  -125.99 (3.65) &    SA-MLP/CM + B &  0.04 (0.0) &  SA-MLP/CM + BFC &  -3.46 (0.24) &  SA-MLP/CM + BFC &  0.15 (0.0) &               SA-MLP/CM + B &  -4268.13 (22.74) &   GRU-MLP/CM + B &  0.03 (0.0) \\
GRU-MLP/CM + BFC &   -125.83 (3.6) &      GRU-LNM + B & 0.08 (0.01) &        SA-MLP/CM &  -3.42 (0.25) &            SA-CP &  0.15 (0.0) &             SA-MLP/CM + BFC &  -4265.26 (22.34) &       SA-LNM + B & 0.06 (0.01) \\
       SA-MLP/CM &  -125.59 (3.65) &       SA-LNM + B &  0.09 (0.0) &       GRU-MLP/CM &  -3.42 (0.25) &        SA-CP + B &  0.16 (0.0) &                   SA-MLP/CM &  -4263.75 (23.41) &      GRU-LNM + B & 0.07 (0.01) \\
         Poisson &   -41.71 (1.02) &          Poisson &  0.35 (0.0) &          Poisson &   5.18 (0.11) &          Poisson &   0.2 (0.0) &                     Poisson &   -3706.3 (17.61) &          Poisson &  0.27 (0.0) \\
\bottomrule
\end{tabular}

\label{resultsmark}
\caption{Taxi/Twitter/Reddit Subs.}
\end{table}


\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccc|cccc|cccc}
\toprule
            \multicolumn{4}{c}{\textbf{pubg}} & \multicolumn{4}{c}{\textbf{yelp toronto}} & \multicolumn{4}{c}{\textbf{yelp mississauga}} \\
               0 &             NLL &                1 &   Time Cal. &                2 &              NLL &                3 &   Time Cal. &                4 &            NLL &                5 &   Time Cal. \\
\midrule
         GRU-LNM & -194.39 (18.07) &           Hawkes &  0.01 (0.0) &       SA-LNM + B & -3979.6 (200.76) &           SA-LNM &  0.01 (0.0) &      GRU-LNM + B & -120.85 (9.18) &           SA-LNM &  0.01 (0.0) \\
      SA-LNM + B &  -187.75 (7.55) &    SA-MLP/MC + B &  0.01 (0.0) &      GRU-LNM + B & -3838.7 (194.65) &          GRU-LNM &  0.01 (0.0) &       SA-LNM + B & -109.67 (4.99) &   SA-SA/MC + BFC &  0.01 (0.0) \\
     GRU-LNM + B &   -174.0 (4.74) &  SA-MLP/MC + BFC &  0.01 (0.0) &          GRU-LNM & -2957.96 (92.81) &    GRU-LNM + BFC &  0.01 (0.0) &          GRU-LNM &   -59.61 (0.9) &    GRU-SA/MC + B &  0.01 (0.0) \\
   GRU-LNM + BFC &  -146.76 (7.31) &         SA-RMTPP &  0.01 (0.0) &    GRU-LNM + BFC &   -2949.1 (86.9) &     SA-LNM + BFC &  0.01 (0.0) &    GRU-LNM + BFC &  -59.41 (0.85) &          GRU-LNM &  0.01 (0.0) \\
          SA-LNM &  -137.63 (3.52) &     SA-RMTPP + B &  0.01 (0.0) &           SA-LNM & -2925.35 (91.31) &     SA-SA/CM + B &  0.03 (0.0) &    GRU-SA/MC + B &  -58.77 (0.95) &         SA-SA/MC &  0.01 (0.0) \\
 GRU-SA/CM + BFC & -133.33 (23.17) &   SA-RMTPP + BFC &  0.01 (0.0) &     SA-LNM + BFC & -2918.12 (90.38) &  GRU-SA/MC + BFC &  0.03 (0.0) &  GRU-SA/MC + BFC &  -58.43 (0.82) &    GRU-LNM + BFC &  0.01 (0.0) \\
    SA-LNM + BFC &  -131.33 (2.99) &  GRU-SA/MC + BFC &  0.01 (0.0) &    GRU-SA/MC + B & -2823.58 (90.01) &    GRU-SA/MC + B &  0.03 (0.0) &        GRU-SA/MC &   -58.1 (0.83) &     SA-SA/CM + B &  0.01 (0.0) \\
       GRU-SA/MC &  -123.35 (2.43) &    GRU-SA/MC + B &  0.01 (0.0) &       GRU-MLP/MC &  -2811.3 (86.33) &        GRU-SA/MC &  0.03 (0.0) &       GRU-MLP/MC &   -58.1 (0.83) &  GRU-SA/CM + BFC &  0.01 (0.0) \\
 GRU-SA/MC + BFC &  -120.79 (3.01) &        GRU-SA/MC &  0.01 (0.0) & GRU-MLP/MC + BFC & -2810.25 (85.82) &   SA-SA/MC + BFC &  0.04 (0.0) &   GRU-MLP/MC + B &  -58.04 (0.84) &    GRU-SA/CM + B &  0.01 (0.0) \\
        SA-SA/MC &  -119.94 (2.67) &  GRU-SA/CM + BFC &  0.01 (0.0) &   GRU-MLP/MC + B & -2810.11 (86.15) &     SA-SA/MC + B &  0.04 (0.0) &     SA-SA/MC + B &  -57.76 (1.02) &  GRU-SA/MC + BFC &  0.01 (0.0) \\
   GRU-SA/MC + B &  -118.88 (4.27) &    GRU-SA/CM + B &  0.01 (0.0) &        GRU-RMTPP & -2808.87 (86.74) &         SA-SA/MC &  0.04 (0.0) & GRU-MLP/MC + BFC &  -57.74 (0.77) &        GRU-SA/CM &  0.01 (0.0) \\
  SA-SA/CM + BFC & -118.45 (10.02) &        GRU-SA/CM &  0.01 (0.0) &  GRU-RMTPP + BFC & -2808.54 (86.16) &   SA-SA/CM + BFC &  0.04 (0.0) &           SA-LNM &  -57.65 (0.79) &     SA-LNM + BFC &  0.01 (0.0) \\
  SA-SA/MC + BFC &  -117.23 (3.38) &  GRU-RMTPP + BFC &  0.01 (0.0) &    GRU-RMTPP + B & -2805.92 (85.44) &  GRU-SA/CM + BFC &  0.04 (0.0) &  GRU-RMTPP + BFC &  -57.58 (0.86) &        GRU-SA/MC &  0.02 (0.0) \\
    SA-SA/MC + B &  -116.46 (3.07) &    GRU-RMTPP + B &  0.01 (0.0) &        GRU-SA/MC & -2803.49 (86.66) &    GRU-SA/CM + B &  0.04 (0.0) &   SA-SA/MC + BFC &   -57.5 (0.74) &    SA-MLP/MC + B &  0.02 (0.0) \\
    SA-SA/CM + B &  -114.97 (6.32) &        GRU-RMTPP &  0.01 (0.0) &       GRU-CP + B & -2803.23 (85.58) &         SA-SA/CM & 0.05 (0.01) &    GRU-RMTPP + B &  -57.43 (0.85) &        SA-MLP/MC &  0.02 (0.0) \\
      GRU-MLP/MC &  -107.85 (0.19) & GRU-MLP/MC + BFC &  0.01 (0.0) &     GRU-CP + BFC & -2800.43 (84.38) &  GRU-RMTPP + BFC &  0.05 (0.0) &     SA-LNM + BFC &  -57.42 (0.81) & GRU-MLP/MC + BFC &  0.02 (0.0) \\
GRU-MLP/MC + BFC &  -107.83 (0.23) &   GRU-MLP/MC + B &  0.01 (0.0) &  GRU-SA/MC + BFC &  -2799.78 (87.5) &    GRU-RMTPP + B &  0.05 (0.0) &        GRU-RMTPP &  -57.15 (0.84) &       GRU-MLP/MC &  0.02 (0.0) \\
   GRU-RMTPP + B &  -107.76 (0.21) &       GRU-MLP/MC &  0.01 (0.0) &           GRU-CP & -2798.57 (85.08) & GRU-MLP/MC + BFC &  0.05 (0.0) &         SA-SA/MC &   -57.0 (0.81) &         SA-SA/CM &  0.02 (0.0) \\
  GRU-MLP/MC + B &   -107.76 (0.2) &         SA-SA/CM &  0.01 (0.0) &   SA-SA/MC + BFC & -2781.36 (82.82) &   GRU-MLP/MC + B &  0.05 (0.0) &    GRU-SA/CM + B &  -56.29 (0.86) &   SA-SA/CM + BFC &  0.02 (0.0) \\
 GRU-RMTPP + BFC &  -107.73 (0.22) &     SA-SA/CM + B &  0.01 (0.0) &  SA-MLP/MC + BFC & -2774.25 (84.54) &       GRU-MLP/MC &  0.05 (0.0) &        SA-MLP/MC &  -56.24 (0.91) &     SA-SA/MC + B &  0.02 (0.0) \\
       GRU-RMTPP &  -107.71 (0.23) &   SA-SA/CM + BFC &  0.01 (0.0) &           Hawkes &  -2773.63 (87.1) &     GRU-CP + BFC &  0.05 (0.0) &       GRU-CP + B &  -56.18 (0.76) &  SA-MLP/MC + BFC &  0.02 (0.0) \\
   GRU-SA/CM + B &  -107.43 (0.18) &    GRU-LNM + BFC &  0.01 (0.0) &    SA-MLP/MC + B & -2772.73 (84.92) &       GRU-CP + B &  0.05 (0.0) &        GRU-SA/CM &  -56.13 (1.05) &   GRU-MLP/MC + B &  0.02 (0.0) \\
       GRU-SA/CM &  -107.38 (0.21) &         SA-SA/MC &  0.01 (0.0) &     SA-SA/MC + B & -2772.71 (86.17) &        GRU-SA/CM &  0.05 (0.0) &  SA-MLP/MC + BFC &  -56.11 (0.75) &  GRU-RMTPP + BFC &  0.03 (0.0) \\
        SA-SA/CM &  -107.27 (0.24) &          GRU-LNM &  0.01 (0.0) &        SA-MLP/MC & -2771.19 (85.52) &        GRU-RMTPP &  0.05 (0.0) &           GRU-CP &  -56.07 (0.82) &    GRU-RMTPP + B &  0.03 (0.0) \\
          GRU-CP &   -107.0 (0.22) &     SA-SA/MC + B &  0.01 (0.0) &         SA-SA/MC & -2768.85 (76.57) &         SA-RMTPP &  0.06 (0.0) &     GRU-CP + BFC &  -56.06 (0.81) &        GRU-RMTPP &  0.03 (0.0) \\
    GRU-CP + BFC &  -106.99 (0.21) &   SA-SA/MC + BFC &  0.01 (0.0) &     SA-RMTPP + B & -2765.01 (84.07) &           GRU-CP &  0.06 (0.0) &    SA-MLP/MC + B &  -56.01 (0.94) &         SA-RMTPP &  0.04 (0.0) \\
      GRU-CP + B &  -106.99 (0.21) &     SA-LNM + BFC &  0.01 (0.0) &   SA-RMTPP + BFC & -2764.91 (83.86) &   SA-RMTPP + BFC &  0.06 (0.0) &  GRU-SA/CM + BFC &  -55.99 (0.92) &   SA-RMTPP + BFC &  0.04 (0.0) \\
       SA-MLP/MC &  -106.57 (0.41) &        SA-MLP/MC &  0.01 (0.0) &    GRU-SA/CM + B & -2764.26 (79.54) &  SA-MLP/MC + BFC &  0.06 (0.0) &         SA-SA/CM &  -55.91 (0.92) &     SA-RMTPP + B &  0.04 (0.0) \\
   SA-MLP/MC + B &  -106.27 (0.44) &           GRU-CP &  0.02 (0.0) &         SA-RMTPP & -2764.26 (84.29) &     SA-RMTPP + B &  0.06 (0.0) &     SA-SA/CM + B &  -55.66 (0.91) &           GRU-CP &  0.05 (0.0) \\
 SA-MLP/MC + BFC &  -106.15 (0.36) &           SA-LNM &  0.02 (0.0) &  GRU-SA/CM + BFC & -2762.13 (83.35) &    SA-MLP/MC + B &  0.06 (0.0) &   SA-SA/CM + BFC &   -55.64 (1.0) &           Hawkes &  0.05 (0.0) \\
  SA-RMTPP + BFC &  -106.09 (0.26) &     GRU-CP + BFC &  0.02 (0.0) &        SA-CP + B & -2757.95 (82.11) &           Hawkes &  0.06 (0.0) &     SA-RMTPP + B &   -55.3 (0.85) &     GRU-CP + BFC &  0.05 (0.0) \\
    SA-RMTPP + B &  -105.78 (0.22) &       GRU-CP + B &  0.02 (0.0) &      SA-CP + BFC & -2757.09 (81.64) &        SA-MLP/MC &  0.06 (0.0) &   SA-RMTPP + BFC &  -55.28 (1.01) &       GRU-CP + B &  0.05 (0.0) \\
        SA-RMTPP &   -105.5 (0.29) &      SA-CP + BFC &  0.03 (0.0) &            SA-CP & -2753.86 (81.24) &       SA-LNM + B &  0.07 (0.0) &         SA-RMTPP &  -55.01 (0.87) &      SA-CP + BFC &  0.06 (0.0) \\
           SA-CP &  -104.13 (0.21) &        SA-CP + B &  0.03 (0.0) &        GRU-SA/CM & -2753.47 (82.19) &      SA-CP + BFC &  0.07 (0.0) &      SA-CP + BFC &  -53.41 (0.94) &        SA-CP + B &  0.06 (0.0) \\
     SA-CP + BFC &  -104.11 (0.26) &            SA-CP &  0.03 (0.0) &     SA-SA/CM + B & -2753.44 (80.25) &        SA-CP + B &  0.07 (0.0) &           Hawkes &   -53.33 (0.8) &            SA-CP &  0.06 (0.0) \\
       SA-CP + B &  -104.06 (0.25) &  SA-MLP/CM + BFC &  0.05 (0.0) &   SA-SA/CM + BFC &  -2752.3 (84.25) &            SA-CP &  0.07 (0.0) &        SA-CP + B &  -52.64 (0.96) &       SA-LNM + B & 0.08 (0.01) \\
          Hawkes &   -102.69 (0.2) &        SA-MLP/CM &  0.05 (0.0) &         SA-SA/CM & -2740.69 (85.18) &      GRU-LNM + B &  0.08 (0.0) &            SA-CP &  -52.64 (1.07) &       GRU-MLP/CM & 0.09 (0.01) \\
  GRU-MLP/CM + B &    -99.0 (0.15) & GRU-MLP/CM + BFC &  0.05 (0.0) &   GRU-MLP/CM + B &  -2667.2 (74.98) &    SA-MLP/CM + B & 0.09 (0.01) &       GRU-MLP/CM &  -44.89 (2.28) &      GRU-LNM + B & 0.09 (0.01) \\
   SA-MLP/CM + B &   -98.99 (0.15) &   GRU-MLP/CM + B &  0.05 (0.0) &    SA-MLP/CM + B & -2666.42 (74.33) &   GRU-MLP/CM + B & 0.09 (0.01) & GRU-MLP/CM + BFC &  -42.88 (0.66) &    SA-MLP/CM + B &   0.1 (0.0) \\
GRU-MLP/CM + BFC &   -98.93 (0.16) &       GRU-MLP/CM &  0.05 (0.0) &  SA-MLP/CM + BFC & -2664.26 (73.94) &       GRU-MLP/CM & 0.09 (0.01) &   GRU-MLP/CM + B &  -42.74 (0.64) &        SA-MLP/CM &   0.1 (0.0) \\
 SA-MLP/CM + BFC &   -98.92 (0.16) &    SA-MLP/CM + B &  0.05 (0.0) & GRU-MLP/CM + BFC &  -2661.76 (72.9) &  SA-MLP/CM + BFC &  0.1 (0.01) &    SA-MLP/CM + B &  -42.53 (0.72) & GRU-MLP/CM + BFC &   0.1 (0.0) \\
       SA-MLP/CM &    -98.8 (0.15) &      GRU-LNM + B & 0.06 (0.01) &       GRU-MLP/CM & -2659.68 (74.25) &        SA-MLP/CM &  0.1 (0.01) &  SA-MLP/CM + BFC &  -42.43 (0.68) &   GRU-MLP/CM + B &   0.1 (0.0) \\
      GRU-MLP/CM &    -98.8 (0.15) &       SA-LNM + B & 0.07 (0.01) &        SA-MLP/CM &  -2659.22 (73.5) & GRU-MLP/CM + BFC &  0.1 (0.01) &        SA-MLP/CM &   -42.34 (0.7) &  SA-MLP/CM + BFC &   0.1 (0.0) \\
         Poisson &   -93.11 (0.15) &          Poisson &  0.07 (0.0) &          Poisson &  -673.76 (17.22) &          Poisson &  0.47 (0.0) &          Poisson &   -25.2 (0.29) &          Poisson &  0.27 (0.0) \\
\bottomrule
\end{tabular}


\label{resultsmark}
\caption{PUBG/Yelp Toronto/Yelp Mississauga}
\end{table}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\tiny
\setlength\tabcolsep{1pt}
\centering


\begin{tabular}{cccc|cccc}
\toprule
\multicolumn{4}{c}{\textbf{reddit askscience comments}} & \multicolumn{4}{c}{\textbf{yelp airport}} \\
                         0 &              NLL &                1 &   Time Cal. &                2 &           NLL &                3 &   Time Cal. \\
\midrule
               GRU-LNM + B & -1263.68 (38.98) &     SA-LNM + BFC &   0.0 (0.0) &      GRU-LNM + B & -32.36 (3.14) &  GRU-RMTPP + BFC &  0.01 (0.0) \\
                SA-LNM + B & -1225.99 (48.22) &  GRU-SA/MC + BFC &   0.0 (0.0) &       SA-LNM + B & -28.05 (1.33) &     SA-LNM + BFC &  0.01 (0.0) \\
             GRU-LNM + BFC &  -927.36 (12.25) &          GRU-LNM &   0.0 (0.0) &    GRU-SA/MC + B &  -7.09 (0.18) &  SA-MLP/MC + BFC &  0.01 (0.0) \\
                   GRU-LNM &  -926.36 (12.67) &         SA-SA/MC &   0.0 (0.0) &  GRU-SA/MC + BFC &  -7.02 (0.21) &           SA-LNM &  0.01 (0.0) \\
           GRU-SA/MC + BFC &  -922.92 (12.92) &    GRU-LNM + BFC &   0.0 (0.0) &          GRU-LNM &   -6.8 (0.19) &         SA-RMTPP &  0.01 (0.0) \\
                GRU-MLP/MC &  -922.51 (12.89) &    GRU-SA/MC + B &   0.0 (0.0) &        GRU-SA/MC &   -6.77 (0.2) &     SA-RMTPP + B &  0.01 (0.0) \\
          GRU-MLP/MC + BFC &  -922.46 (12.96) &       GRU-MLP/MC &   0.0 (0.0) &   SA-SA/MC + BFC &  -6.46 (0.16) &   SA-RMTPP + BFC &  0.01 (0.0) \\
             GRU-SA/MC + B &   -922.4 (12.93) &           SA-LNM &   0.0 (0.0) &       GRU-MLP/MC &  -6.41 (0.19) &  GRU-SA/MC + BFC &  0.01 (0.0) \\
                 GRU-SA/MC &   -922.28 (13.0) &  SA-MLP/MC + BFC &  0.01 (0.0) & GRU-MLP/MC + BFC &   -6.4 (0.19) &    GRU-SA/MC + B &  0.01 (0.0) \\
            GRU-MLP/MC + B &  -922.04 (13.08) &        GRU-SA/MC &  0.01 (0.0) &     SA-SA/MC + B &  -6.25 (0.26) &        GRU-SA/MC &  0.01 (0.0) \\
           GRU-RMTPP + BFC &  -920.91 (12.87) &  GRU-SA/CM + BFC &  0.01 (0.0) &         SA-SA/MC &  -6.15 (0.22) &  GRU-SA/CM + BFC &  0.01 (0.0) \\
                 GRU-RMTPP &  -920.83 (13.11) &    GRU-SA/CM + B &  0.01 (0.0) &   GRU-MLP/MC + B &   -6.1 (0.18) &    GRU-SA/CM + B &  0.01 (0.0) \\
             GRU-RMTPP + B &  -920.45 (13.11) &        GRU-SA/CM &  0.01 (0.0) &  GRU-RMTPP + BFC &  -6.05 (0.18) &        GRU-SA/CM &  0.01 (0.0) \\
                    Hawkes &  -919.51 (12.92) &  GRU-RMTPP + BFC &  0.01 (0.0) &    GRU-RMTPP + B &  -6.02 (0.19) &    SA-MLP/MC + B &  0.01 (0.0) \\
                    GRU-CP &  -917.77 (13.08) &           Hawkes &  0.01 (0.0) &    GRU-LNM + BFC &  -6.01 (0.24) &        SA-MLP/MC &  0.01 (0.0) \\
              GRU-CP + BFC &  -917.76 (13.08) & GRU-MLP/MC + BFC &  0.01 (0.0) &        GRU-RMTPP &  -5.98 (0.21) &        GRU-RMTPP &  0.01 (0.0) \\
                GRU-CP + B &   -917.48 (13.1) &   GRU-MLP/MC + B &  0.01 (0.0) &        GRU-SA/CM &  -5.94 (0.17) & GRU-MLP/MC + BFC &  0.01 (0.0) \\
            SA-SA/MC + BFC &   -914.7 (12.84) &         SA-SA/CM &  0.01 (0.0) &       GRU-CP + B &  -5.76 (0.18) &   GRU-MLP/MC + B &  0.01 (0.0) \\
              SA-SA/MC + B &  -914.58 (12.76) &     SA-SA/CM + B &  0.01 (0.0) &           GRU-CP &  -5.73 (0.18) &       GRU-MLP/MC &  0.01 (0.0) \\
                  SA-SA/MC &  -913.99 (12.95) &   SA-SA/CM + BFC &  0.01 (0.0) &           SA-LNM &  -5.71 (0.16) &         SA-SA/CM &  0.01 (0.0) \\
                    SA-LNM &  -900.73 (12.41) &     SA-SA/MC + B &  0.01 (0.0) &     SA-LNM + BFC &   -5.7 (0.19) &     SA-SA/CM + B &  0.01 (0.0) \\
              SA-LNM + BFC &  -899.94 (12.65) &   SA-SA/MC + BFC &  0.01 (0.0) &  GRU-SA/CM + BFC &   -5.7 (0.08) &   SA-SA/CM + BFC &  0.01 (0.0) \\
                 SA-MLP/MC &   -896.0 (12.95) &    GRU-RMTPP + B &  0.01 (0.0) &        SA-MLP/MC &   -5.68 (0.2) &    GRU-LNM + BFC &  0.01 (0.0) \\
           SA-MLP/MC + BFC &  -895.41 (12.65) &        GRU-RMTPP &  0.01 (0.0) &     GRU-CP + BFC &  -5.64 (0.17) &         SA-SA/MC &  0.01 (0.0) \\
             SA-MLP/MC + B &  -895.08 (13.06) &    SA-MLP/MC + B &  0.02 (0.0) &    GRU-SA/CM + B &  -5.61 (0.19) &          GRU-LNM &  0.01 (0.0) \\
            SA-RMTPP + BFC &  -890.57 (12.91) &        SA-MLP/MC &  0.02 (0.0) &  SA-MLP/MC + BFC &  -5.57 (0.18) &     SA-SA/MC + B &  0.01 (0.0) \\
              SA-RMTPP + B &   -888.0 (13.15) &           GRU-CP &  0.02 (0.0) &   SA-SA/CM + BFC &  -5.51 (0.19) &   SA-SA/MC + BFC &  0.01 (0.0) \\
                  SA-RMTPP &  -887.29 (12.73) &       GRU-CP + B &  0.02 (0.0) &     SA-SA/CM + B &  -5.49 (0.15) &    GRU-RMTPP + B &  0.01 (0.0) \\
             GRU-SA/CM + B &  -878.56 (11.34) &     GRU-CP + BFC &  0.02 (0.0) &    SA-MLP/MC + B &   -5.4 (0.17) &           GRU-CP &  0.02 (0.0) \\
                 GRU-SA/CM &   -877.89 (13.0) &   SA-RMTPP + BFC &  0.03 (0.0) &   SA-RMTPP + BFC &  -5.36 (0.17) &           Hawkes &  0.02 (0.0) \\
                  SA-SA/CM &  -875.99 (14.49) &       SA-LNM + B &  0.04 (0.0) &         SA-SA/CM &  -5.33 (0.18) &     GRU-CP + BFC &  0.02 (0.0) \\
                     SA-CP &  -875.97 (12.56) &     SA-RMTPP + B &  0.04 (0.0) &     SA-RMTPP + B &   -5.3 (0.17) &       GRU-CP + B &  0.02 (0.0) \\
           GRU-SA/CM + BFC &  -875.91 (12.54) &         SA-RMTPP &  0.04 (0.0) &         SA-RMTPP &    -5.3 (0.2) &        SA-MLP/CM &  0.03 (0.0) \\
                 SA-CP + B &  -875.52 (12.84) &      GRU-LNM + B & 0.06 (0.01) &        SA-CP + B &   -4.8 (0.17) &      SA-CP + BFC &  0.03 (0.0) \\
               SA-CP + BFC &   -875.5 (12.88) &            SA-CP &  0.06 (0.0) &            SA-CP &  -4.77 (0.15) &        SA-CP + B &  0.03 (0.0) \\
              SA-SA/CM + B &  -868.23 (12.43) &        SA-CP + B &  0.06 (0.0) &      SA-CP + BFC &  -4.72 (0.19) &       GRU-MLP/CM &  0.03 (0.0) \\
            SA-SA/CM + BFC &  -865.98 (10.76) &      SA-CP + BFC &  0.06 (0.0) &           Hawkes &  -4.62 (0.18) &            SA-CP &  0.03 (0.0) \\
                GRU-MLP/CM &  -814.67 (31.33) &       GRU-MLP/CM & 0.09 (0.03) &       GRU-MLP/CM &  -3.86 (0.17) &    SA-MLP/CM + B &  0.04 (0.0) \\
            GRU-MLP/CM + B &  -750.01 (12.07) & GRU-MLP/CM + BFC &  0.14 (0.0) & GRU-MLP/CM + BFC &  -3.84 (0.14) & GRU-MLP/CM + BFC &  0.04 (0.0) \\
          GRU-MLP/CM + BFC &  -749.61 (12.02) &   GRU-MLP/CM + B &  0.14 (0.0) &    SA-MLP/CM + B &  -3.78 (0.16) &   GRU-MLP/CM + B &  0.04 (0.0) \\
             SA-MLP/CM + B &  -748.36 (12.06) &  SA-MLP/CM + BFC &  0.14 (0.0) &   GRU-MLP/CM + B &  -3.78 (0.15) &  SA-MLP/CM + BFC &  0.04 (0.0) \\
           SA-MLP/CM + BFC &  -748.29 (12.03) &    SA-MLP/CM + B &  0.14 (0.0) &        SA-MLP/CM &  -3.77 (0.14) &      GRU-LNM + B & 0.07 (0.01) \\
                 SA-MLP/CM &  -747.37 (12.11) &        SA-MLP/CM &  0.14 (0.0) &  SA-MLP/CM + BFC &  -3.76 (0.14) &       SA-LNM + B & 0.08 (0.01) \\
                   Poisson &   -676.53 (10.2) &          Poisson &  0.25 (0.0) &          Poisson &   -2.11 (0.1) &          Poisson &  0.12 (0.0) \\
\bottomrule
\end{tabular}

\label{resultsmark}
\caption{Yelp Airport/Reddit Comments}
\end{table}



\end{landscape}
\restoregeometry

==> stat_tests.tex <==
\newgeometry{left=2cm,bottom=0cm,right=2cm, top=0.5cm}
\begin{table}[t]
\tiny
\setlength\tabcolsep{1.5pt}
\centering
\begin{tabular}{cccccccc}
\hline \\
                                 Comp. &        Z &            p &       Adj. p &                                 Comp. &        Z &            p &   Adj. p \\ \\
\hline \\
                 GRU-LNM-TO vs Poisson & 8.098149 & 6.661338e-16 & 9.179324e-13 &             SA-LNM-TEM vs SA-RMTPP-TO & 5.012577 & 5.370594e-07 & 0.000677 \\
               C-CP-TEMP vs GRU-LNM-TO & 7.979928 & 1.554312e-15 & 2.140288e-12 &           C-RMTPP-TEMP vs SA-SA/CM-LE & 5.000755 & 5.710634e-07 & 0.000719 \\
                GRU-LNM-TEM vs Poisson & 7.944461 & 1.998401e-15 & 2.749800e-12 &       C-CP-TEMP vs GRU-MLP/MC-TEM + B & 4.988933 & 6.071384e-07 & 0.000764 \\
              C-CP-TEMP vs GRU-LNM-TEM & 7.826240 & 5.107026e-15 & 7.022161e-12 &              GRU-CP-TEM vs GRU-LNM-TO & 4.977110 & 6.454050e-07 & 0.000811 \\
                 SA-LNM-TEM vs Poisson & 7.672553 & 1.687539e-14 & 2.318679e-11 &             C-CP-TEMP vs C-SA/MC-TEMP & 4.977110 & 6.454050e-07 & 0.000811 \\
                SA-CP-TO vs GRU-LNM-TO & 7.660731 & 1.842970e-14 & 2.530398e-11 &             SA-LNM-TO vs GRU-SA/MC-TO & 4.971199 & 6.653998e-07 & 0.000835 \\
               C-CP-TEMP vs SA-LNM-TEM & 7.554332 & 4.218847e-14 & 5.788259e-11 &        GRU-LNM-TEM vs GRU-LNM-TEM + B & 4.941644 & 7.746654e-07 & 0.000971 \\
               SA-CP-TO vs GRU-LNM-TEM & 7.507043 & 6.039613e-14 & 8.280310e-11 &            C-LNM-TEMP vs SA-MLP/CM-TO & 4.941644 & 7.746654e-07 & 0.000971 \\
                SA-CP-TO vs SA-LNM-TEM & 7.235134 & 4.649614e-13 & 6.369971e-10 &          GRU-RMTPP-TEM + B vs Poisson & 4.941644 & 7.746654e-07 & 0.000971 \\
                 C-LNM-TEMP vs Poisson & 7.223312 & 5.073719e-13 & 6.945922e-10 &       GRU-SA/CM-LE + B vs SA-SA/MC-TO & 4.935733 & 7.985028e-07 & 0.000999 \\
               C-CP-TEMP vs C-LNM-TEMP & 7.105091 & 1.202372e-12 & 1.644844e-09 &         SA-CP-TEM vs GRU-SA/CM-LE + B & 4.929822 & 8.230459e-07 & 0.001029 \\
        GRU-LNM-TO vs SA-MLP/CM-LE + B & 6.951404 & 3.616663e-12 & 4.943978e-09 &     SA-CP-TEM + B vs GRU-SA/CM-LE + B & 4.929822 & 8.230459e-07 & 0.001029 \\
            GRU-LNM-TO vs C-RMTPP-TEMP & 6.904115 & 5.051737e-12 & 6.900672e-09 &             SA-LNM-TO vs SA-MLP/CM-LE & 4.929822 & 8.230459e-07 & 0.001029 \\
       GRU-LNM-TEM vs SA-MLP/CM-LE + B & 6.797716 & 1.062905e-11 & 1.450866e-08 &           C-LNM-TEMP vs GRU-MLP/CM-TO & 4.929822 & 8.230459e-07 & 0.001029 \\
                  SA-LNM-TO vs Poisson & 6.797716 & 1.062905e-11 & 1.450866e-08 &         GRU-CP-TEM + B vs GRU-LNM-TEM & 4.918000 & 8.743298e-07 & 0.001089 \\
                SA-CP-TO vs C-LNM-TEMP & 6.785894 & 1.153699e-11 & 1.572492e-08 & GRU-MLP/CM-LE + B vs SA-SA/MC-TEM + B & 4.894356 & 9.862835e-07 & 0.001228 \\
       GRU-LNM-TO vs GRU-MLP/CM-LE + B & 6.762250 & 1.358647e-11 & 1.850477e-08 &        SA-SA/CM-LE + B vs SA-SA/MC-TO & 4.864800 & 1.145724e-06 & 0.001425 \\
           GRU-LNM-TEM vs C-RMTPP-TEMP & 6.750428 & 1.474110e-11 & 2.006263e-08 &          SA-CP-TEM vs SA-SA/CM-LE + B & 4.858889 & 1.180461e-06 & 0.001467 \\
                C-CP-TEMP vs SA-LNM-TO & 6.679495 & 2.397660e-11 & 3.260817e-08 &      SA-CP-TEM + B vs SA-SA/CM-LE + B & 4.858889 & 1.180461e-06 & 0.001467 \\
           GRU-SA/CM-LE + B vs Poisson & 6.632207 & 3.307044e-11 & 4.494272e-08 &          GRU-LNM-TO vs SA-LNM-TEM + B & 4.858889 & 1.180461e-06 & 0.001467 \\
      GRU-LNM-TEM vs GRU-MLP/CM-LE + B & 6.608562 & 3.880696e-11 & 5.269985e-08 &      GRU-MLP/CM-LE + B vs SA-SA/CM-LE & 4.858889 & 1.180461e-06 & 0.001467 \\
            SA-SA/CM-LE + B vs Poisson & 6.561274 & 5.334999e-11 & 7.239594e-08 &           GRU-LNM-TO vs C-MLP/MC-TEMP & 4.847067 & 1.253000e-06 & 0.001552 \\
        SA-LNM-TEM vs SA-MLP/CM-LE + B & 6.525807 & 6.763612e-11 & 9.171458e-08 &             GRU-CP-TEM vs GRU-LNM-TEM & 4.823423 & 1.411153e-06 & 0.001747 \\
         C-CP-TEMP vs GRU-SA/CM-LE + B & 6.513985 & 7.318257e-11 & 9.916238e-08 &        C-CP-TEMP vs GRU-RMTPP-TEM + B & 4.823423 & 1.411153e-06 & 0.001747 \\
            SA-LNM-TEM vs C-RMTPP-TEMP & 6.478519 & 9.262724e-11 & 1.254173e-07 &             GRU-LNM-TO vs C-MLP/CM-LE & 4.823423 & 1.411153e-06 & 0.001747 \\
          GRU-SA/MC-TEM + B vs Poisson & 6.454875 & 1.083085e-10 & 1.465414e-07 &      GRU-SA/CM-LE + B vs GRU-SA/MC-TO & 4.805690 & 1.542189e-06 & 0.001905 \\
          C-CP-TEMP vs SA-SA/CM-LE + B & 6.443053 & 1.170941e-10 & 1.583112e-07 &                    SA-CP-TO vs Hawkes & 4.787957 & 1.684881e-06 & 0.002079 \\
             GRU-LNM-TO vs SA-SA/MC-TO & 6.401675 & 1.536813e-10 & 2.076234e-07 &          SA-MLP/MC-TEM + B vs Poisson & 4.787957 & 1.684881e-06 & 0.002079 \\
               SA-CP-TEM vs GRU-LNM-TO & 6.395764 & 1.597464e-10 & 2.156577e-07 &           SA-LNM-TEM vs GRU-MLP/CM-LE & 4.776134 & 1.786969e-06 & 0.002202 \\
           SA-CP-TEM + B vs GRU-LNM-TO & 6.395764 & 1.597464e-10 & 2.156577e-07 &     SA-MLP/CM-LE + B vs GRU-SA/MC-TEM & 4.770223 & 1.840217e-06 & 0.002265 \\
                 SA-CP-TO vs SA-LNM-TO & 6.360298 & 2.013629e-10 & 2.714372e-07 &               GRU-CP-TO vs GRU-LNM-TO & 4.764312 & 1.894988e-06 & 0.002331 \\
               GRU-SA/CM-LE vs Poisson & 6.360298 & 2.013629e-10 & 2.714372e-07 &      SA-MLP/CM-LE vs GRU-SA/CM-LE + B & 4.764312 & 1.894988e-06 & 0.002331 \\
        C-CP-TEMP vs GRU-SA/MC-TEM + B & 6.336654 & 2.348091e-10 & 3.160530e-07 &      GRU-SA/MC-TEM + B vs SA-SA/MC-TO & 4.758401 & 1.951323e-06 & 0.002396 \\
       SA-LNM-TEM vs GRU-MLP/CM-LE + B & 6.336654 & 2.348091e-10 & 3.160530e-07 &        SA-CP-TEM vs GRU-SA/MC-TEM + B & 4.752490 & 2.009265e-06 & 0.002465 \\
            GRU-LNM-TO vs GRU-SA/MC-TO & 6.271632 & 3.572831e-10 & 4.801885e-07 &    SA-CP-TEM + B vs GRU-SA/MC-TEM + B & 4.752490 & 2.009265e-06 & 0.002465 \\
            GRU-LNM-TEM vs SA-SA/MC-TO & 6.247988 & 4.157741e-10 & 5.583846e-07 &              SA-CP-TO vs GRU-SA/CM-TO & 4.740668 & 2.130146e-06 & 0.002609 \\
              SA-CP-TEM vs GRU-LNM-TEM & 6.242077 & 4.317990e-10 & 5.794743e-07 &       SA-SA/CM-LE + B vs GRU-SA/MC-TO & 4.734757 & 2.193176e-06 & 0.002684 \\
          SA-CP-TEM + B vs GRU-LNM-TEM & 6.242077 & 4.317990e-10 & 5.794743e-07 &                SA-CP-TO vs C-SA/CM-LE & 4.728846 & 2.257996e-06 & 0.002762 \\
             C-CP-TEMP vs GRU-SA/CM-LE & 6.242077 & 4.317990e-10 & 5.794743e-07 &         C-RMTPP-TEMP vs GRU-SA/MC-TEM & 4.722935 & 2.324652e-06 & 0.002841 \\
            GRU-LNM-TO vs SA-MLP/CM-LE & 6.230255 & 4.656777e-10 & 6.235425e-07 &         GRU-LNM-TEM vs SA-LNM-TEM + B & 4.705202 & 2.536150e-06 & 0.003097 \\
           SA-SA/MC-TEM + B vs Poisson & 6.230255 & 4.656777e-10 & 6.235425e-07 &          GRU-LNM-TEM vs C-MLP/MC-TEMP & 4.693380 & 2.687281e-06 & 0.003278 \\
          SA-CP-TO vs GRU-SA/CM-LE + B & 6.194788 & 5.836343e-10 & 7.803190e-07 &       SA-MLP/CM-LE vs SA-SA/CM-LE + B & 4.693380 & 2.687281e-06 & 0.003278 \\
                SA-SA/CM-LE vs Poisson & 6.194788 & 5.836343e-10 & 7.803190e-07 &        SA-CP-TO vs GRU-MLP/MC-TEM + B & 4.669735 & 3.015879e-06 & 0.003673 \\
           SA-CP-TO vs SA-SA/CM-LE + B & 6.123856 & 9.133769e-10 & 1.219358e-06 &        C-CP-TEMP vs SA-MLP/MC-TEM + B & 4.669735 & 3.015879e-06 & 0.003673 \\
           GRU-LNM-TEM vs GRU-SA/MC-TO & 6.117945 & 9.479004e-10 & 1.264499e-06 &            GRU-LNM-TEM vs C-MLP/CM-LE & 4.669735 & 3.015879e-06 & 0.003673 \\
         C-CP-TEMP vs SA-SA/MC-TEM + B & 6.112033 & 9.836953e-10 & 1.311266e-06 &         GRU-LNM-TEM + B vs SA-LNM-TEM & 4.669735 & 3.015879e-06 & 0.003673 \\
              C-CP-TEMP vs SA-SA/CM-LE & 6.076567 & 1.227826e-09 & 1.635465e-06 &           GRU-SA/CM-LE vs SA-SA/MC-TO & 4.663824 & 3.103863e-06 & 0.003768 \\
           GRU-LNM-TEM vs SA-MLP/CM-LE & 6.076567 & 1.227826e-09 & 1.635465e-06 &             SA-CP-TEM vs GRU-SA/CM-LE & 4.657913 & 3.194306e-06 & 0.003875 \\
        C-LNM-TEMP vs SA-MLP/CM-LE + B & 6.076567 & 1.227826e-09 & 1.635465e-06 &         SA-CP-TEM + B vs GRU-SA/CM-LE & 4.657913 & 3.194306e-06 & 0.003875 \\
            C-LNM-TEMP vs C-RMTPP-TEMP & 6.029279 & 1.646931e-09 & 2.188771e-06 &              SA-CP-TO vs C-SA/MC-TEMP & 4.657913 & 3.194306e-06 & 0.003875 \\
         SA-CP-TO vs GRU-SA/MC-TEM + B & 6.017457 & 1.771788e-09 & 2.352935e-06 &          GRU-CP-TEM + B vs SA-LNM-TEM & 4.646091 & 3.382835e-06 & 0.004093 \\
             SA-LNM-TEM vs SA-SA/MC-TO & 5.976079 & 2.285720e-09 & 3.033150e-06 &     GRU-SA/MC-TEM + B vs GRU-SA/MC-TO & 4.628358 & 3.685764e-06 & 0.004456 \\
               SA-CP-TEM vs SA-LNM-TEM & 5.970168 & 2.370093e-09 & 3.142743e-06 &              GRU-CP-TO vs GRU-LNM-TEM & 4.610625 & 4.014604e-06 & 0.004850 \\
           SA-CP-TEM + B vs SA-LNM-TEM & 5.970168 & 2.370093e-09 & 3.142743e-06 &              SA-MLP/MC-TEM vs Poisson & 4.604714 & 4.130335e-06 & 0.004985 \\
              SA-CP-TO vs GRU-SA/CM-LE & 5.922880 & 3.163524e-09 & 4.188506e-06 &            GRU-LNM-TO vs SA-RMTPP-TEM & 4.598803 & 4.249259e-06 & 0.005125 \\
              GRU-SA/MC-TEM vs Poisson & 5.916969 & 3.279293e-09 & 4.338505e-06 &      SA-MLP/CM-LE + B vs SA-SA/MC-TEM & 4.592892 & 4.371460e-06 & 0.005268 \\
       C-LNM-TEMP vs GRU-MLP/CM-LE + B & 5.887413 & 3.922869e-09 & 5.186032e-06 &     SA-MLP/CM-LE vs GRU-SA/MC-TEM + B & 4.586981 & 4.497024e-06 & 0.005414 \\
            SA-LNM-TEM vs GRU-SA/MC-TO & 5.846036 & 5.034255e-09 & 6.650251e-06 &    GRU-MLP/CM-LE + B vs GRU-SA/MC-TEM & 4.581070 & 4.626039e-06 & 0.005565 \\
            GRU-LNM-TO vs SA-MLP/CM-TO & 5.816481 & 6.009951e-09 & 7.933136e-06 &             C-LNM-TEMP vs SA-RMTPP-TO & 4.563336 & 5.034704e-06 & 0.006052 \\
           GRU-LNM-TO vs GRU-MLP/CM-TO & 5.804658 & 6.449733e-09 & 8.507198e-06 &              GRU-CP-TEM vs SA-LNM-TEM & 4.551514 & 5.326118e-06 & 0.006397 \\
            SA-LNM-TEM vs SA-MLP/CM-LE & 5.804658 & 6.449733e-09 & 8.507198e-06 &          C-RMTPP-TEMP vs SA-SA/MC-TEM & 4.545603 & 5.477814e-06 & 0.006573 \\
            C-CP-TEMP vs GRU-SA/MC-TEM & 5.798747 & 6.681207e-09 & 8.799150e-06 &          GRU-SA/CM-LE vs GRU-SA/MC-TO & 4.533781 & 5.793707e-06 & 0.006947 \\
          SA-CP-TO vs SA-SA/MC-TEM + B & 5.792836 & 6.920753e-09 & 9.107711e-06 &       SA-SA/MC-TEM + B vs SA-SA/MC-TO & 4.533781 & 5.793707e-06 & 0.006947 \\
               SA-CP-TO vs SA-SA/CM-LE & 5.757370 & 8.543450e-09 & 1.123464e-05 &         SA-CP-TEM vs SA-SA/MC-TEM + B & 4.527870 & 5.958120e-06 & 0.007132 \\
               SA-SA/MC-TEM vs Poisson & 5.739637 & 9.487979e-09 & 1.246720e-05 &     SA-CP-TEM + B vs SA-SA/MC-TEM + B & 4.527870 & 5.958120e-06 & 0.007132 \\
           GRU-LNM-TEM vs SA-MLP/CM-TO & 5.662793 & 1.489287e-08 & 1.955434e-05 &                SA-SA/CM-TO vs Poisson & 4.527870 & 5.958120e-06 & 0.007132 \\
          GRU-LNM-TEM vs GRU-MLP/CM-TO & 5.650971 & 1.595440e-08 & 2.093218e-05 &             SA-LNM-TO vs SA-MLP/CM-TO & 4.516048 & 6.300441e-06 & 0.007523 \\
         SA-LNM-TO vs SA-MLP/CM-LE + B & 5.650971 & 1.595440e-08 & 2.093218e-05 &         SA-CP-TO vs GRU-RMTPP-TEM + B & 4.504226 & 6.661534e-06 & 0.007947 \\
             C-CP-TEMP vs SA-SA/MC-TEM & 5.621416 & 1.893989e-08 & 2.481126e-05 &            SA-LNM-TO vs GRU-MLP/CM-TO & 4.504226 & 6.661534e-06 & 0.007947 \\
             SA-LNM-TO vs C-RMTPP-TEMP & 5.603683 & 2.098449e-08 & 2.746870e-05 &            SA-SA/CM-LE vs SA-SA/MC-TO & 4.498315 & 6.849424e-06 & 0.008158 \\
              GRU-MLP/MC-TO vs Poisson & 5.597771 & 2.171247e-08 & 2.839991e-05 &              SA-CP-TEM vs SA-SA/CM-LE & 4.492404 & 7.042376e-06 & 0.008380 \\
             C-LNM-TEMP vs SA-SA/MC-TO & 5.526839 & 3.260523e-08 & 4.261504e-05 &          SA-CP-TEM + B vs SA-SA/CM-LE & 4.492404 & 7.042376e-06 & 0.008380 \\
               SA-CP-TEM vs C-LNM-TEMP & 5.520928 & 3.372145e-08 & 4.404021e-05 &          SA-MLP/CM-LE vs GRU-SA/CM-LE & 4.492404 & 7.042376e-06 & 0.008380 \\
           SA-CP-TEM + B vs C-LNM-TEMP & 5.520928 & 3.372145e-08 & 4.404021e-05 &            C-CP-TEMP vs SA-MLP/MC-TEM & 4.486493 & 7.240521e-06 & 0.008594 \\
             GRU-MLP/MC-TEM vs Poisson & 5.503195 & 3.729705e-08 & 4.863535e-05 &              GRU-RMTPP-TEM vs Poisson & 4.468759 & 7.867453e-06 & 0.009331 \\
  SA-MLP/CM-LE + B vs GRU-SA/CM-LE + B & 5.485461 & 4.123917e-08 & 5.373463e-05 &     SA-MLP/CM-LE + B vs GRU-MLP/MC-TO & 4.451026 & 8.546087e-06 & 0.010127 \\
             SA-CP-TO vs GRU-SA/MC-TEM & 5.479550 & 4.264082e-08 & 5.551834e-05 &           GRU-LNM-TEM vs SA-RMTPP-TEM & 4.445115 & 8.784476e-06 & 0.010401 \\
            C-CP-TEMP vs GRU-MLP/MC-TO & 5.479550 & 4.264082e-08 & 5.551834e-05 &          SA-LNM-TEM vs SA-LNM-TEM + B & 4.433293 & 9.280455e-06 & 0.010979 \\
        SA-LNM-TO vs GRU-MLP/CM-LE + B & 5.461817 & 4.712854e-08 & 6.126710e-05 &           SA-LNM-TEM vs C-MLP/MC-TEMP & 4.421471 & 9.803121e-06 & 0.011587 \\
             GRU-LNM-TO vs SA-RMTPP-TO & 5.438173 & 5.382972e-08 & 6.992481e-05 &              C-CP-TEMP vs SA-SA/CM-TO & 4.409649 & 1.035383e-05 & 0.012228 \\
      C-RMTPP-TEMP vs GRU-SA/CM-LE + B & 5.438173 & 5.382972e-08 & 6.992481e-05 &     GRU-MLP/CM-LE + B vs SA-SA/MC-TEM & 4.403738 & 1.064015e-05 & 0.012555 \\
   SA-MLP/CM-LE + B vs SA-SA/CM-LE + B & 5.414529 & 6.145035e-08 & 7.970111e-05 &         GRU-MLP/MC-TO vs C-RMTPP-TEMP & 4.403738 & 1.064015e-05 & 0.012555 \\
            C-LNM-TEMP vs GRU-SA/MC-TO & 5.396796 & 6.784163e-08 & 8.792275e-05 &      GRU-SA/MC-TO vs SA-SA/MC-TEM + B & 4.403738 & 1.064015e-05 & 0.012555 \\
            SA-LNM-TEM vs SA-MLP/CM-TO & 5.390884 & 7.011175e-08 & 9.079471e-05 &             SA-LNM-TEM vs C-MLP/CM-LE & 4.397827 & 1.093402e-05 & 0.012869 \\
           C-CP-TEMP vs GRU-MLP/MC-TEM & 5.384973 & 7.245536e-08 & 9.375724e-05 &           SA-SA/CM-LE vs GRU-SA/MC-TO & 4.368272 & 1.252337e-05 & 0.014727 \\
           SA-LNM-TEM vs GRU-MLP/CM-TO & 5.379062 & 7.487478e-08 & 9.681309e-05 &      SA-MLP/CM-LE vs SA-SA/MC-TEM + B & 4.362360 & 1.286667e-05 & 0.015118 \\
       C-RMTPP-TEMP vs SA-SA/CM-LE + B & 5.367240 & 7.995054e-08 & 1.032961e-04 &    SA-MLP/CM-LE + B vs GRU-MLP/MC-TEM & 4.356449 & 1.321892e-05 & 0.015519 \\
            C-LNM-TEMP vs SA-MLP/CM-LE & 5.355418 & 8.535880e-08 & 1.101982e-04 &         SA-CP-TO vs SA-MLP/MC-TEM + B & 4.350538 & 1.358037e-05 & 0.015930 \\
 SA-MLP/CM-LE + B vs GRU-SA/MC-TEM + B & 5.308130 & 1.107559e-07 & 1.428750e-04 &            C-CP-TEMP vs GRU-RMTPP-TEM & 4.350538 & 1.358037e-05 & 0.015930 \\
              SA-CP-TO vs SA-SA/MC-TEM & 5.302219 & 1.144037e-07 & 1.474664e-04 &      SA-MLP/CM-TO vs GRU-SA/CM-LE + B & 4.350538 & 1.358037e-05 & 0.015930 \\
 GRU-MLP/CM-LE + B vs GRU-SA/CM-LE + B & 5.296308 & 1.181678e-07 & 1.522001e-04 &               GRU-CP-TO vs SA-LNM-TEM & 4.338716 & 1.433174e-05 & 0.016768 \\
            GRU-LNM-TEM vs SA-RMTPP-TO & 5.284485 & 1.260586e-07 & 1.622374e-04 &                  SA-LNM-K1 vs Poisson & 4.338716 & 1.433174e-05 & 0.016768 \\
     C-RMTPP-TEMP vs GRU-SA/MC-TEM + B & 5.260841 & 1.433978e-07 & 1.844096e-04 &     GRU-MLP/CM-TO vs GRU-SA/CM-LE + B & 4.338716 & 1.433174e-05 & 0.016768 \\
  GRU-MLP/CM-LE + B vs SA-SA/CM-LE + B & 5.225375 & 1.738026e-07 & 2.233364e-04 &        GRU-LNM-TO vs SA-RMTPP-TEM + B & 4.326894 & 1.512266e-05 & 0.017648 \\
                     Poisson vs Hawkes & 5.225375 & 1.738026e-07 & 2.233364e-04 &           C-LNM-TEMP vs GRU-MLP/CM-LE & 4.326894 & 1.512266e-05 & 0.017648 \\
      SA-MLP/CM-LE + B vs GRU-SA/CM-LE & 5.213553 & 1.852578e-07 & 2.376858e-04 &           SA-MLP/CM-LE vs SA-SA/CM-LE & 4.326894 & 1.512266e-05 & 0.017648 \\
           GRU-LNM-TO vs GRU-MLP/CM-LE & 5.201731 & 1.974413e-07 & 2.531197e-04 &        GRU-MLP/MC-TEM vs C-RMTPP-TEMP & 4.309161 & 1.638751e-05 & 0.019075 \\
               GRU-SA/CM-TO vs Poisson & 5.178086 & 2.241734e-07 & 2.871662e-04 &       SA-MLP/CM-TO vs SA-SA/CM-LE + B & 4.279606 & 1.872248e-05 & 0.021774 \\
          C-RMTPP-TEMP vs GRU-SA/CM-LE & 5.166264 & 2.388191e-07 & 3.056884e-04 &      GRU-MLP/CM-TO vs SA-SA/CM-LE + B & 4.267784 & 1.974248e-05 & 0.022941 \\
                 C-SA/CM-LE vs Poisson & 5.166264 & 2.388191e-07 & 3.056884e-04 &    GRU-MLP/CM-LE + B vs GRU-MLP/MC-TO & 4.261872 & 2.027211e-05 & 0.023536 \\
             SA-CP-TO vs GRU-MLP/MC-TO & 5.160353 & 2.464844e-07 & 3.150070e-04 &               GRU-RMTPP-TO vs Poisson & 4.232317 & 2.312959e-05 & 0.026830 \\
GRU-MLP/CM-LE + B vs GRU-SA/MC-TEM + B & 5.118976 & 3.071994e-07 & 3.922936e-04 &                C-CP-TEMP vs SA-LNM-K1 & 4.220495 & 2.437664e-05 & 0.028253 \\
                   C-CP-TEMP vs Hawkes & 5.107154 & 3.270477e-07 & 4.173129e-04 &         GRU-LNM-TEM + B vs C-LNM-TEMP & 4.220495 & 2.437664e-05 & 0.028253 \\
         GRU-MLP/MC-TEM + B vs Poisson & 5.107154 & 3.270477e-07 & 4.173129e-04 &          GRU-SA/MC-TEM vs SA-SA/MC-TO & 4.220495 & 2.437664e-05 & 0.028253 \\
              SA-LNM-TO vs SA-SA/MC-TO & 5.101243 & 3.374306e-07 & 4.298866e-04 &            SA-CP-TEM vs GRU-SA/MC-TEM & 4.214584 & 2.502390e-05 & 0.028928 \\
                SA-CP-TEM vs SA-LNM-TO & 5.095332 & 3.481314e-07 & 4.431713e-04 &        SA-CP-TEM + B vs GRU-SA/MC-TEM & 4.214584 & 2.502390e-05 & 0.028928 \\
            SA-CP-TEM + B vs SA-LNM-TO & 5.095332 & 3.481314e-07 & 4.431713e-04 &          GRU-CP-TEM + B vs C-LNM-TEMP & 4.196851 & 2.706521e-05 & 0.031233 \\
         GRU-LNM-TEM + B vs GRU-LNM-TO & 5.095332 & 3.481314e-07 & 4.431713e-04 &       GRU-LNM-TEM vs SA-RMTPP-TEM + B & 4.173207 & 3.003424e-05 & 0.034629 \\
               C-SA/MC-TEMP vs Poisson & 5.095332 & 3.481314e-07 & 4.431713e-04 &            SA-LNM-TEM vs SA-RMTPP-TEM & 4.173207 & 3.003424e-05 & 0.034629 \\
  SA-MLP/CM-LE + B vs SA-SA/MC-TEM + B & 5.083509 & 3.705241e-07 & 4.701951e-04 &     SA-MLP/CM-TO vs GRU-SA/MC-TEM + B & 4.173207 & 3.003424e-05 & 0.034629 \\
          GRU-CP-TEM + B vs GRU-LNM-TO & 5.071687 & 3.943038e-07 & 4.999772e-04 &             SA-CP-TO vs SA-MLP/MC-TEM & 4.167296 & 3.082348e-05 & 0.035447 \\
            SA-CP-TO vs GRU-MLP/MC-TEM & 5.065776 & 4.067394e-07 & 5.153388e-04 &   GRU-MLP/CM-LE + B vs GRU-MLP/MC-TEM & 4.167296 & 3.082348e-05 & 0.035447 \\
             C-CP-TEMP vs GRU-SA/CM-TO & 5.059865 & 4.195529e-07 & 5.311540e-04 &    GRU-MLP/CM-TO vs GRU-SA/MC-TEM + B & 4.161384 & 3.163240e-05 & 0.036314 \\
               C-CP-TEMP vs C-SA/CM-LE & 5.048043 & 4.463584e-07 & 5.646434e-04 &              SA-LNM-TO vs SA-RMTPP-TO & 4.137740 & 3.507431e-05 & 0.040230 \\
          GRU-LNM-TEM vs GRU-MLP/CM-LE & 5.048043 & 4.463584e-07 & 5.646434e-04 &             C-CP-TEMP vs GRU-RMTPP-TO & 4.114096 & 3.886996e-05 & 0.044545 \\
       SA-MLP/CM-LE + B vs SA-SA/CM-LE & 5.048043 & 4.463584e-07 & 5.646434e-04 &              GRU-CP-TEM vs C-LNM-TEMP & 4.102274 & 4.091095e-05 & 0.046843 \\
      C-RMTPP-TEMP vs SA-SA/MC-TEM + B & 5.036221 & 4.748123e-07 & 5.992132e-04 &               SA-CP-TO vs SA-SA/CM-TO & 4.090452 & 4.305337e-05 & 0.049253 \\
     GRU-MLP/CM-LE + B vs GRU-SA/CM-LE & 5.024399 & 5.050118e-07 & 6.368198e-04 &         GRU-SA/MC-TEM vs GRU-SA/MC-TO & 4.090452 & 4.305337e-05 & 0.049253 \\ \\
\hline \\
\end{tabular}
\caption{Pairwise comparisons of all models on the time NLL using Schaffer's correction.}
\end{table}

\begin{comment}
\clearpage
\begin{table}[t]
\tiny
\setlength\tabcolsep{1.5pt}
\centering
\begin{tabular}{cccccccc}
\hline \\
                             Comp. &        Z &            p &   Adj. p &                             Comp. &        Z &        p &   Adj. p \\ \\
\hline \\
            GRU-LNM-TEM vs Poisson & 5.503246 & 3.728620e-08 & 0.000051 &          GRU-LNM-K1 vs C-LNM-TEMP & 4.568732 & 0.000005 & 0.006649 \\
          GRU-RMTPP-TEM vs Poisson & 5.399411 & 6.686005e-08 & 0.000092 & C-RMTPP-TEMP vs GRU-SA/MC-TEM + B & 4.551427 & 0.000005 & 0.007215 \\
             GRU-LNM-K1 vs Poisson & 5.364799 & 8.103925e-08 & 0.000112 & SA-MLP/MC-TEM + B vs C-RMTPP-TEMP & 4.499509 & 0.000007 & 0.009215 \\
       GRU-LNM-TEM vs C-RMTPP-TEMP & 5.191741 & 2.083363e-07 & 0.000286 &   C-CP-TEMP vs GRU-MLP/MC-TEM + B & 4.447592 & 0.000009 & 0.011741 \\
     GRU-MLP/MC-TEM + B vs Poisson & 5.157130 & 2.507641e-07 & 0.000345 &  C-RMTPP-TEMP vs SA-SA/MC-TEM + B & 4.447592 & 0.000009 & 0.011741 \\
     GRU-RMTPP-TEM vs C-RMTPP-TEMP & 5.087906 & 3.620378e-07 & 0.000497 &         SA-LNM-K1 vs C-RMTPP-TEMP & 4.412980 & 0.000010 & 0.013764 \\
      GRU-RMTPP-TEM + B vs Poisson & 5.070601 & 3.965620e-07 & 0.000544 &       GRU-LNM-TEM vs SA-MLP/MC-TO & 4.395674 & 0.000011 & 0.014897 \\
        GRU-LNM-K1 vs C-RMTPP-TEMP & 5.053295 & 4.342526e-07 & 0.000595 &      GRU-LNM-TEM vs GRU-MLP/MC-TO & 4.378369 & 0.000012 & 0.016118 \\
             SA-LNM-TEM vs Poisson & 4.914848 & 8.885117e-07 & 0.001217 &    C-CP-TEMP vs GRU-RMTPP-TEM + B & 4.361063 & 0.000013 & 0.017435 \\
           SA-RMTPP-TEM vs Poisson & 4.914848 & 8.885117e-07 & 0.001217 &  C-LNM-TEMP vs GRU-MLP/MC-TEM + B & 4.361063 & 0.000013 & 0.017435 \\
      GRU-SA/MC-TEM + B vs Poisson & 4.862931 & 1.156602e-06 & 0.001582 &         GRU-LNM-TEM vs C-SA/CM-LE & 4.291839 & 0.000018 & 0.023833 \\
GRU-MLP/MC-TEM + B vs C-RMTPP-TEMP & 4.845625 & 1.262136e-06 & 0.001725 &     SA-MLP/MC-TO vs GRU-RMTPP-TEM & 4.291839 & 0.000018 & 0.023833 \\
      SA-MLP/MC-TEM + B vs Poisson & 4.811014 & 1.501668e-06 & 0.002051 &   C-LNM-TEMP vs GRU-RMTPP-TEM + B & 4.274534 & 0.000019 & 0.025724 \\
          C-CP-TEMP vs GRU-LNM-TEM & 4.793708 & 1.637267e-06 & 0.002235 &    GRU-MLP/MC-TO vs GRU-RMTPP-TEM & 4.274534 & 0.000019 & 0.025724 \\
 GRU-RMTPP-TEM + B vs C-RMTPP-TEMP & 4.759096 & 1.944617e-06 & 0.002652 &        GRU-LNM-K1 vs SA-MLP/MC-TO & 4.257228 & 0.000021 & 0.027756 \\
       SA-SA/MC-TEM + B vs Poisson & 4.759096 & 1.944617e-06 & 0.002652 &       GRU-LNM-K1 vs GRU-MLP/MC-TO & 4.239922 & 0.000022 & 0.029962 \\
              SA-LNM-K1 vs Poisson & 4.724485 & 2.306997e-06 & 0.003142 &       SA-RMTPP-TEM + B vs Poisson & 4.239922 & 0.000022 & 0.029962 \\
         GRU-LNM-TEM vs C-LNM-TEMP & 4.707179 & 2.511686e-06 & 0.003418 &           C-CP-TEMP vs SA-LNM-TEM & 4.205310 & 0.000026 & 0.034885 \\
        C-CP-TEMP vs GRU-RMTPP-TEM & 4.689873 & 2.733747e-06 & 0.003718 &         C-CP-TEMP vs SA-RMTPP-TEM & 4.205310 & 0.000026 & 0.034885 \\
           C-CP-TEMP vs GRU-LNM-K1 & 4.655261 & 3.235700e-06 & 0.004397 &       GRU-RMTPP-TEM vs C-SA/CM-LE & 4.188005 & 0.000028 & 0.037597 \\
        SA-LNM-TEM vs C-RMTPP-TEMP & 4.603344 & 4.157607e-06 & 0.005646 &       GRU-LNM-TEM vs GRU-SA/MC-TO & 4.170699 & 0.000030 & 0.040540 \\
       C-LNM-TEMP vs GRU-RMTPP-TEM & 4.603344 & 4.157607e-06 & 0.005646 &    C-CP-TEMP vs GRU-SA/MC-TEM + B & 4.153393 & 0.000033 & 0.043699 \\
      SA-RMTPP-TEM vs C-RMTPP-TEMP & 4.603344 & 4.157607e-06 & 0.005646 &          GRU-LNM-K1 vs C-SA/CM-LE & 4.153393 & 0.000033 & 0.043699 \\ \\
\hline 
\end{tabular}
\caption{Pairwise comparisons of all models on the mark NLL using Schaffer's correction.}
\end{table}

\clearpage
\begin{table}[t]
\tiny
\setlength\tabcolsep{1.5pt}
\centering
\begin{tabular}{cccccccc}
\hline \\
                                 Comp. &        Z &            p &       Adj. p &                                 Comp. &        Z &            p &   Adj. p \\ \\
\hline \\
                 GRU-LNM-TO vs Poisson & 8.098149 & 6.661338e-16 & 9.179324e-13 &             SA-LNM-TEM vs SA-RMTPP-TO & 5.012577 & 5.370594e-07 & 0.000677 \\
               C-CP-TEMP vs GRU-LNM-TO & 7.979928 & 1.554312e-15 & 2.140288e-12 &           C-RMTPP-TEMP vs SA-SA/CM-LE & 5.000755 & 5.710634e-07 & 0.000719 \\
                GRU-LNM-TEM vs Poisson & 7.944461 & 1.998401e-15 & 2.749800e-12 &       C-CP-TEMP vs GRU-MLP/MC-TEM + B & 4.988933 & 6.071384e-07 & 0.000764 \\
              C-CP-TEMP vs GRU-LNM-TEM & 7.826240 & 5.107026e-15 & 7.022161e-12 &              GRU-CP-TEM vs GRU-LNM-TO & 4.977110 & 6.454050e-07 & 0.000811 \\
                 SA-LNM-TEM vs Poisson & 7.672553 & 1.687539e-14 & 2.318679e-11 &             C-CP-TEMP vs C-SA/MC-TEMP & 4.977110 & 6.454050e-07 & 0.000811 \\
                SA-CP-TO vs GRU-LNM-TO & 7.660731 & 1.842970e-14 & 2.530398e-11 &             SA-LNM-TO vs GRU-SA/MC-TO & 4.971199 & 6.653998e-07 & 0.000835 \\
               C-CP-TEMP vs SA-LNM-TEM & 7.554332 & 4.218847e-14 & 5.788259e-11 &        GRU-LNM-TEM vs GRU-LNM-TEM + B & 4.941644 & 7.746654e-07 & 0.000971 \\
               SA-CP-TO vs GRU-LNM-TEM & 7.507043 & 6.039613e-14 & 8.280310e-11 &            C-LNM-TEMP vs SA-MLP/CM-TO & 4.941644 & 7.746654e-07 & 0.000971 \\
                SA-CP-TO vs SA-LNM-TEM & 7.235134 & 4.649614e-13 & 6.369971e-10 &          GRU-RMTPP-TEM + B vs Poisson & 4.941644 & 7.746654e-07 & 0.000971 \\
                 C-LNM-TEMP vs Poisson & 7.223312 & 5.073719e-13 & 6.945922e-10 &       GRU-SA/CM-LE + B vs SA-SA/MC-TO & 4.935733 & 7.985028e-07 & 0.000999 \\
               C-CP-TEMP vs C-LNM-TEMP & 7.105091 & 1.202372e-12 & 1.644844e-09 &         SA-CP-TEM vs GRU-SA/CM-LE + B & 4.929822 & 8.230459e-07 & 0.001029 \\
        GRU-LNM-TO vs SA-MLP/CM-LE + B & 6.951404 & 3.616663e-12 & 4.943978e-09 &     SA-CP-TEM + B vs GRU-SA/CM-LE + B & 4.929822 & 8.230459e-07 & 0.001029 \\
            GRU-LNM-TO vs C-RMTPP-TEMP & 6.904115 & 5.051737e-12 & 6.900672e-09 &             SA-LNM-TO vs SA-MLP/CM-LE & 4.929822 & 8.230459e-07 & 0.001029 \\
       GRU-LNM-TEM vs SA-MLP/CM-LE + B & 6.797716 & 1.062905e-11 & 1.450866e-08 &           C-LNM-TEMP vs GRU-MLP/CM-TO & 4.929822 & 8.230459e-07 & 0.001029 \\
                  SA-LNM-TO vs Poisson & 6.797716 & 1.062905e-11 & 1.450866e-08 &         GRU-CP-TEM + B vs GRU-LNM-TEM & 4.918000 & 8.743298e-07 & 0.001089 \\
                SA-CP-TO vs C-LNM-TEMP & 6.785894 & 1.153699e-11 & 1.572492e-08 & GRU-MLP/CM-LE + B vs SA-SA/MC-TEM + B & 4.894356 & 9.862835e-07 & 0.001228 \\
       GRU-LNM-TO vs GRU-MLP/CM-LE + B & 6.762250 & 1.358647e-11 & 1.850477e-08 &        SA-SA/CM-LE + B vs SA-SA/MC-TO & 4.864800 & 1.145724e-06 & 0.001425 \\
           GRU-LNM-TEM vs C-RMTPP-TEMP & 6.750428 & 1.474110e-11 & 2.006263e-08 &          SA-CP-TEM vs SA-SA/CM-LE + B & 4.858889 & 1.180461e-06 & 0.001467 \\
                C-CP-TEMP vs SA-LNM-TO & 6.679495 & 2.397660e-11 & 3.260817e-08 &      SA-CP-TEM + B vs SA-SA/CM-LE + B & 4.858889 & 1.180461e-06 & 0.001467 \\
           GRU-SA/CM-LE + B vs Poisson & 6.632207 & 3.307044e-11 & 4.494272e-08 &          GRU-LNM-TO vs SA-LNM-TEM + B & 4.858889 & 1.180461e-06 & 0.001467 \\
      GRU-LNM-TEM vs GRU-MLP/CM-LE + B & 6.608562 & 3.880696e-11 & 5.269985e-08 &      GRU-MLP/CM-LE + B vs SA-SA/CM-LE & 4.858889 & 1.180461e-06 & 0.001467 \\
            SA-SA/CM-LE + B vs Poisson & 6.561274 & 5.334999e-11 & 7.239594e-08 &           GRU-LNM-TO vs C-MLP/MC-TEMP & 4.847067 & 1.253000e-06 & 0.001552 \\
        SA-LNM-TEM vs SA-MLP/CM-LE + B & 6.525807 & 6.763612e-11 & 9.171458e-08 &             GRU-CP-TEM vs GRU-LNM-TEM & 4.823423 & 1.411153e-06 & 0.001747 \\
         C-CP-TEMP vs GRU-SA/CM-LE + B & 6.513985 & 7.318257e-11 & 9.916238e-08 &        C-CP-TEMP vs GRU-RMTPP-TEM + B & 4.823423 & 1.411153e-06 & 0.001747 \\
            SA-LNM-TEM vs C-RMTPP-TEMP & 6.478519 & 9.262724e-11 & 1.254173e-07 &             GRU-LNM-TO vs C-MLP/CM-LE & 4.823423 & 1.411153e-06 & 0.001747 \\
          GRU-SA/MC-TEM + B vs Poisson & 6.454875 & 1.083085e-10 & 1.465414e-07 &      GRU-SA/CM-LE + B vs GRU-SA/MC-TO & 4.805690 & 1.542189e-06 & 0.001905 \\
          C-CP-TEMP vs SA-SA/CM-LE + B & 6.443053 & 1.170941e-10 & 1.583112e-07 &                    SA-CP-TO vs Hawkes & 4.787957 & 1.684881e-06 & 0.002079 \\
             GRU-LNM-TO vs SA-SA/MC-TO & 6.401675 & 1.536813e-10 & 2.076234e-07 &          SA-MLP/MC-TEM + B vs Poisson & 4.787957 & 1.684881e-06 & 0.002079 \\
               SA-CP-TEM vs GRU-LNM-TO & 6.395764 & 1.597464e-10 & 2.156577e-07 &           SA-LNM-TEM vs GRU-MLP/CM-LE & 4.776134 & 1.786969e-06 & 0.002202 \\
           SA-CP-TEM + B vs GRU-LNM-TO & 6.395764 & 1.597464e-10 & 2.156577e-07 &     SA-MLP/CM-LE + B vs GRU-SA/MC-TEM & 4.770223 & 1.840217e-06 & 0.002265 \\
                 SA-CP-TO vs SA-LNM-TO & 6.360298 & 2.013629e-10 & 2.714372e-07 &               GRU-CP-TO vs GRU-LNM-TO & 4.764312 & 1.894988e-06 & 0.002331 \\
               GRU-SA/CM-LE vs Poisson & 6.360298 & 2.013629e-10 & 2.714372e-07 &      SA-MLP/CM-LE vs GRU-SA/CM-LE + B & 4.764312 & 1.894988e-06 & 0.002331 \\
        C-CP-TEMP vs GRU-SA/MC-TEM + B & 6.336654 & 2.348091e-10 & 3.160530e-07 &      GRU-SA/MC-TEM + B vs SA-SA/MC-TO & 4.758401 & 1.951323e-06 & 0.002396 \\
       SA-LNM-TEM vs GRU-MLP/CM-LE + B & 6.336654 & 2.348091e-10 & 3.160530e-07 &        SA-CP-TEM vs GRU-SA/MC-TEM + B & 4.752490 & 2.009265e-06 & 0.002465 \\
            GRU-LNM-TO vs GRU-SA/MC-TO & 6.271632 & 3.572831e-10 & 4.801885e-07 &    SA-CP-TEM + B vs GRU-SA/MC-TEM + B & 4.752490 & 2.009265e-06 & 0.002465 \\
            GRU-LNM-TEM vs SA-SA/MC-TO & 6.247988 & 4.157741e-10 & 5.583846e-07 &              SA-CP-TO vs GRU-SA/CM-TO & 4.740668 & 2.130146e-06 & 0.002609 \\
              SA-CP-TEM vs GRU-LNM-TEM & 6.242077 & 4.317990e-10 & 5.794743e-07 &       SA-SA/CM-LE + B vs GRU-SA/MC-TO & 4.734757 & 2.193176e-06 & 0.002684 \\
          SA-CP-TEM + B vs GRU-LNM-TEM & 6.242077 & 4.317990e-10 & 5.794743e-07 &                SA-CP-TO vs C-SA/CM-LE & 4.728846 & 2.257996e-06 & 0.002762 \\
             C-CP-TEMP vs GRU-SA/CM-LE & 6.242077 & 4.317990e-10 & 5.794743e-07 &         C-RMTPP-TEMP vs GRU-SA/MC-TEM & 4.722935 & 2.324652e-06 & 0.002841 \\
            GRU-LNM-TO vs SA-MLP/CM-LE & 6.230255 & 4.656777e-10 & 6.235425e-07 &         GRU-LNM-TEM vs SA-LNM-TEM + B & 4.705202 & 2.536150e-06 & 0.003097 \\
           SA-SA/MC-TEM + B vs Poisson & 6.230255 & 4.656777e-10 & 6.235425e-07 &          GRU-LNM-TEM vs C-MLP/MC-TEMP & 4.693380 & 2.687281e-06 & 0.003278 \\
          SA-CP-TO vs GRU-SA/CM-LE + B & 6.194788 & 5.836343e-10 & 7.803190e-07 &       SA-MLP/CM-LE vs SA-SA/CM-LE + B & 4.693380 & 2.687281e-06 & 0.003278 \\
                SA-SA/CM-LE vs Poisson & 6.194788 & 5.836343e-10 & 7.803190e-07 &        SA-CP-TO vs GRU-MLP/MC-TEM + B & 4.669735 & 3.015879e-06 & 0.003673 \\
           SA-CP-TO vs SA-SA/CM-LE + B & 6.123856 & 9.133769e-10 & 1.219358e-06 &        C-CP-TEMP vs SA-MLP/MC-TEM + B & 4.669735 & 3.015879e-06 & 0.003673 \\
           GRU-LNM-TEM vs GRU-SA/MC-TO & 6.117945 & 9.479004e-10 & 1.264499e-06 &            GRU-LNM-TEM vs C-MLP/CM-LE & 4.669735 & 3.015879e-06 & 0.003673 \\
         C-CP-TEMP vs SA-SA/MC-TEM + B & 6.112033 & 9.836953e-10 & 1.311266e-06 &         GRU-LNM-TEM + B vs SA-LNM-TEM & 4.669735 & 3.015879e-06 & 0.003673 \\
              C-CP-TEMP vs SA-SA/CM-LE & 6.076567 & 1.227826e-09 & 1.635465e-06 &           GRU-SA/CM-LE vs SA-SA/MC-TO & 4.663824 & 3.103863e-06 & 0.003768 \\
           GRU-LNM-TEM vs SA-MLP/CM-LE & 6.076567 & 1.227826e-09 & 1.635465e-06 &             SA-CP-TEM vs GRU-SA/CM-LE & 4.657913 & 3.194306e-06 & 0.003875 \\
        C-LNM-TEMP vs SA-MLP/CM-LE + B & 6.076567 & 1.227826e-09 & 1.635465e-06 &         SA-CP-TEM + B vs GRU-SA/CM-LE & 4.657913 & 3.194306e-06 & 0.003875 \\
            C-LNM-TEMP vs C-RMTPP-TEMP & 6.029279 & 1.646931e-09 & 2.188771e-06 &              SA-CP-TO vs C-SA/MC-TEMP & 4.657913 & 3.194306e-06 & 0.003875 \\
         SA-CP-TO vs GRU-SA/MC-TEM + B & 6.017457 & 1.771788e-09 & 2.352935e-06 &          GRU-CP-TEM + B vs SA-LNM-TEM & 4.646091 & 3.382835e-06 & 0.004093 \\
             SA-LNM-TEM vs SA-SA/MC-TO & 5.976079 & 2.285720e-09 & 3.033150e-06 &     GRU-SA/MC-TEM + B vs GRU-SA/MC-TO & 4.628358 & 3.685764e-06 & 0.004456 \\
               SA-CP-TEM vs SA-LNM-TEM & 5.970168 & 2.370093e-09 & 3.142743e-06 &              GRU-CP-TO vs GRU-LNM-TEM & 4.610625 & 4.014604e-06 & 0.004850 \\
           SA-CP-TEM + B vs SA-LNM-TEM & 5.970168 & 2.370093e-09 & 3.142743e-06 &              SA-MLP/MC-TEM vs Poisson & 4.604714 & 4.130335e-06 & 0.004985 \\
              SA-CP-TO vs GRU-SA/CM-LE & 5.922880 & 3.163524e-09 & 4.188506e-06 &            GRU-LNM-TO vs SA-RMTPP-TEM & 4.598803 & 4.249259e-06 & 0.005125 \\
              GRU-SA/MC-TEM vs Poisson & 5.916969 & 3.279293e-09 & 4.338505e-06 &      SA-MLP/CM-LE + B vs SA-SA/MC-TEM & 4.592892 & 4.371460e-06 & 0.005268 \\
       C-LNM-TEMP vs GRU-MLP/CM-LE + B & 5.887413 & 3.922869e-09 & 5.186032e-06 &     SA-MLP/CM-LE vs GRU-SA/MC-TEM + B & 4.586981 & 4.497024e-06 & 0.005414 \\
            SA-LNM-TEM vs GRU-SA/MC-TO & 5.846036 & 5.034255e-09 & 6.650251e-06 &    GRU-MLP/CM-LE + B vs GRU-SA/MC-TEM & 4.581070 & 4.626039e-06 & 0.005565 \\
            GRU-LNM-TO vs SA-MLP/CM-TO & 5.816481 & 6.009951e-09 & 7.933136e-06 &             C-LNM-TEMP vs SA-RMTPP-TO & 4.563336 & 5.034704e-06 & 0.006052 \\
           GRU-LNM-TO vs GRU-MLP/CM-TO & 5.804658 & 6.449733e-09 & 8.507198e-06 &              GRU-CP-TEM vs SA-LNM-TEM & 4.551514 & 5.326118e-06 & 0.006397 \\
            SA-LNM-TEM vs SA-MLP/CM-LE & 5.804658 & 6.449733e-09 & 8.507198e-06 &          C-RMTPP-TEMP vs SA-SA/MC-TEM & 4.545603 & 5.477814e-06 & 0.006573 \\
            C-CP-TEMP vs GRU-SA/MC-TEM & 5.798747 & 6.681207e-09 & 8.799150e-06 &          GRU-SA/CM-LE vs GRU-SA/MC-TO & 4.533781 & 5.793707e-06 & 0.006947 \\
          SA-CP-TO vs SA-SA/MC-TEM + B & 5.792836 & 6.920753e-09 & 9.107711e-06 &       SA-SA/MC-TEM + B vs SA-SA/MC-TO & 4.533781 & 5.793707e-06 & 0.006947 \\
               SA-CP-TO vs SA-SA/CM-LE & 5.757370 & 8.543450e-09 & 1.123464e-05 &         SA-CP-TEM vs SA-SA/MC-TEM + B & 4.527870 & 5.958120e-06 & 0.007132 \\
               SA-SA/MC-TEM vs Poisson & 5.739637 & 9.487979e-09 & 1.246720e-05 &     SA-CP-TEM + B vs SA-SA/MC-TEM + B & 4.527870 & 5.958120e-06 & 0.007132 \\
           GRU-LNM-TEM vs SA-MLP/CM-TO & 5.662793 & 1.489287e-08 & 1.955434e-05 &                SA-SA/CM-TO vs Poisson & 4.527870 & 5.958120e-06 & 0.007132 \\
          GRU-LNM-TEM vs GRU-MLP/CM-TO & 5.650971 & 1.595440e-08 & 2.093218e-05 &             SA-LNM-TO vs SA-MLP/CM-TO & 4.516048 & 6.300441e-06 & 0.007523 \\
         SA-LNM-TO vs SA-MLP/CM-LE + B & 5.650971 & 1.595440e-08 & 2.093218e-05 &         SA-CP-TO vs GRU-RMTPP-TEM + B & 4.504226 & 6.661534e-06 & 0.007947 \\
             C-CP-TEMP vs SA-SA/MC-TEM & 5.621416 & 1.893989e-08 & 2.481126e-05 &            SA-LNM-TO vs GRU-MLP/CM-TO & 4.504226 & 6.661534e-06 & 0.007947 \\
             SA-LNM-TO vs C-RMTPP-TEMP & 5.603683 & 2.098449e-08 & 2.746870e-05 &            SA-SA/CM-LE vs SA-SA/MC-TO & 4.498315 & 6.849424e-06 & 0.008158 \\
              GRU-MLP/MC-TO vs Poisson & 5.597771 & 2.171247e-08 & 2.839991e-05 &              SA-CP-TEM vs SA-SA/CM-LE & 4.492404 & 7.042376e-06 & 0.008380 \\
             C-LNM-TEMP vs SA-SA/MC-TO & 5.526839 & 3.260523e-08 & 4.261504e-05 &          SA-CP-TEM + B vs SA-SA/CM-LE & 4.492404 & 7.042376e-06 & 0.008380 \\
               SA-CP-TEM vs C-LNM-TEMP & 5.520928 & 3.372145e-08 & 4.404021e-05 &          SA-MLP/CM-LE vs GRU-SA/CM-LE & 4.492404 & 7.042376e-06 & 0.008380 \\
           SA-CP-TEM + B vs C-LNM-TEMP & 5.520928 & 3.372145e-08 & 4.404021e-05 &            C-CP-TEMP vs SA-MLP/MC-TEM & 4.486493 & 7.240521e-06 & 0.008594 \\
             GRU-MLP/MC-TEM vs Poisson & 5.503195 & 3.729705e-08 & 4.863535e-05 &              GRU-RMTPP-TEM vs Poisson & 4.468759 & 7.867453e-06 & 0.009331 \\
  SA-MLP/CM-LE + B vs GRU-SA/CM-LE + B & 5.485461 & 4.123917e-08 & 5.373463e-05 &     SA-MLP/CM-LE + B vs GRU-MLP/MC-TO & 4.451026 & 8.546087e-06 & 0.010127 \\
             SA-CP-TO vs GRU-SA/MC-TEM & 5.479550 & 4.264082e-08 & 5.551834e-05 &           GRU-LNM-TEM vs SA-RMTPP-TEM & 4.445115 & 8.784476e-06 & 0.010401 \\
            C-CP-TEMP vs GRU-MLP/MC-TO & 5.479550 & 4.264082e-08 & 5.551834e-05 &          SA-LNM-TEM vs SA-LNM-TEM + B & 4.433293 & 9.280455e-06 & 0.010979 \\
        SA-LNM-TO vs GRU-MLP/CM-LE + B & 5.461817 & 4.712854e-08 & 6.126710e-05 &           SA-LNM-TEM vs C-MLP/MC-TEMP & 4.421471 & 9.803121e-06 & 0.011587 \\
             GRU-LNM-TO vs SA-RMTPP-TO & 5.438173 & 5.382972e-08 & 6.992481e-05 &              C-CP-TEMP vs SA-SA/CM-TO & 4.409649 & 1.035383e-05 & 0.012228 \\
      C-RMTPP-TEMP vs GRU-SA/CM-LE + B & 5.438173 & 5.382972e-08 & 6.992481e-05 &     GRU-MLP/CM-LE + B vs SA-SA/MC-TEM & 4.403738 & 1.064015e-05 & 0.012555 \\
   SA-MLP/CM-LE + B vs SA-SA/CM-LE + B & 5.414529 & 6.145035e-08 & 7.970111e-05 &         GRU-MLP/MC-TO vs C-RMTPP-TEMP & 4.403738 & 1.064015e-05 & 0.012555 \\
            C-LNM-TEMP vs GRU-SA/MC-TO & 5.396796 & 6.784163e-08 & 8.792275e-05 &      GRU-SA/MC-TO vs SA-SA/MC-TEM + B & 4.403738 & 1.064015e-05 & 0.012555 \\
            SA-LNM-TEM vs SA-MLP/CM-TO & 5.390884 & 7.011175e-08 & 9.079471e-05 &             SA-LNM-TEM vs C-MLP/CM-LE & 4.397827 & 1.093402e-05 & 0.012869 \\
           C-CP-TEMP vs GRU-MLP/MC-TEM & 5.384973 & 7.245536e-08 & 9.375724e-05 &           SA-SA/CM-LE vs GRU-SA/MC-TO & 4.368272 & 1.252337e-05 & 0.014727 \\
           SA-LNM-TEM vs GRU-MLP/CM-TO & 5.379062 & 7.487478e-08 & 9.681309e-05 &      SA-MLP/CM-LE vs SA-SA/MC-TEM + B & 4.362360 & 1.286667e-05 & 0.015118 \\
       C-RMTPP-TEMP vs SA-SA/CM-LE + B & 5.367240 & 7.995054e-08 & 1.032961e-04 &    SA-MLP/CM-LE + B vs GRU-MLP/MC-TEM & 4.356449 & 1.321892e-05 & 0.015519 \\
            C-LNM-TEMP vs SA-MLP/CM-LE & 5.355418 & 8.535880e-08 & 1.101982e-04 &         SA-CP-TO vs SA-MLP/MC-TEM + B & 4.350538 & 1.358037e-05 & 0.015930 \\
 SA-MLP/CM-LE + B vs GRU-SA/MC-TEM + B & 5.308130 & 1.107559e-07 & 1.428750e-04 &            C-CP-TEMP vs GRU-RMTPP-TEM & 4.350538 & 1.358037e-05 & 0.015930 \\
              SA-CP-TO vs SA-SA/MC-TEM & 5.302219 & 1.144037e-07 & 1.474664e-04 &      SA-MLP/CM-TO vs GRU-SA/CM-LE + B & 4.350538 & 1.358037e-05 & 0.015930 \\
 GRU-MLP/CM-LE + B vs GRU-SA/CM-LE + B & 5.296308 & 1.181678e-07 & 1.522001e-04 &               GRU-CP-TO vs SA-LNM-TEM & 4.338716 & 1.433174e-05 & 0.016768 \\
            GRU-LNM-TEM vs SA-RMTPP-TO & 5.284485 & 1.260586e-07 & 1.622374e-04 &                  SA-LNM-K1 vs Poisson & 4.338716 & 1.433174e-05 & 0.016768 \\
     C-RMTPP-TEMP vs GRU-SA/MC-TEM + B & 5.260841 & 1.433978e-07 & 1.844096e-04 &     GRU-MLP/CM-TO vs GRU-SA/CM-LE + B & 4.338716 & 1.433174e-05 & 0.016768 \\
  GRU-MLP/CM-LE + B vs SA-SA/CM-LE + B & 5.225375 & 1.738026e-07 & 2.233364e-04 &        GRU-LNM-TO vs SA-RMTPP-TEM + B & 4.326894 & 1.512266e-05 & 0.017648 \\
                     Poisson vs Hawkes & 5.225375 & 1.738026e-07 & 2.233364e-04 &           C-LNM-TEMP vs GRU-MLP/CM-LE & 4.326894 & 1.512266e-05 & 0.017648 \\
      SA-MLP/CM-LE + B vs GRU-SA/CM-LE & 5.213553 & 1.852578e-07 & 2.376858e-04 &           SA-MLP/CM-LE vs SA-SA/CM-LE & 4.326894 & 1.512266e-05 & 0.017648 \\
           GRU-LNM-TO vs GRU-MLP/CM-LE & 5.201731 & 1.974413e-07 & 2.531197e-04 &        GRU-MLP/MC-TEM vs C-RMTPP-TEMP & 4.309161 & 1.638751e-05 & 0.019075 \\
               GRU-SA/CM-TO vs Poisson & 5.178086 & 2.241734e-07 & 2.871662e-04 &       SA-MLP/CM-TO vs SA-SA/CM-LE + B & 4.279606 & 1.872248e-05 & 0.021774 \\
          C-RMTPP-TEMP vs GRU-SA/CM-LE & 5.166264 & 2.388191e-07 & 3.056884e-04 &      GRU-MLP/CM-TO vs SA-SA/CM-LE + B & 4.267784 & 1.974248e-05 & 0.022941 \\
                 C-SA/CM-LE vs Poisson & 5.166264 & 2.388191e-07 & 3.056884e-04 &    GRU-MLP/CM-LE + B vs GRU-MLP/MC-TO & 4.261872 & 2.027211e-05 & 0.023536 \\
             SA-CP-TO vs GRU-MLP/MC-TO & 5.160353 & 2.464844e-07 & 3.150070e-04 &               GRU-RMTPP-TO vs Poisson & 4.232317 & 2.312959e-05 & 0.026830 \\
GRU-MLP/CM-LE + B vs GRU-SA/MC-TEM + B & 5.118976 & 3.071994e-07 & 3.922936e-04 &                C-CP-TEMP vs SA-LNM-K1 & 4.220495 & 2.437664e-05 & 0.028253 \\
                   C-CP-TEMP vs Hawkes & 5.107154 & 3.270477e-07 & 4.173129e-04 &         GRU-LNM-TEM + B vs C-LNM-TEMP & 4.220495 & 2.437664e-05 & 0.028253 \\
         GRU-MLP/MC-TEM + B vs Poisson & 5.107154 & 3.270477e-07 & 4.173129e-04 &          GRU-SA/MC-TEM vs SA-SA/MC-TO & 4.220495 & 2.437664e-05 & 0.028253 \\
              SA-LNM-TO vs SA-SA/MC-TO & 5.101243 & 3.374306e-07 & 4.298866e-04 &            SA-CP-TEM vs GRU-SA/MC-TEM & 4.214584 & 2.502390e-05 & 0.028928 \\
                SA-CP-TEM vs SA-LNM-TO & 5.095332 & 3.481314e-07 & 4.431713e-04 &        SA-CP-TEM + B vs GRU-SA/MC-TEM & 4.214584 & 2.502390e-05 & 0.028928 \\
            SA-CP-TEM + B vs SA-LNM-TO & 5.095332 & 3.481314e-07 & 4.431713e-04 &          GRU-CP-TEM + B vs C-LNM-TEMP & 4.196851 & 2.706521e-05 & 0.031233 \\
         GRU-LNM-TEM + B vs GRU-LNM-TO & 5.095332 & 3.481314e-07 & 4.431713e-04 &       GRU-LNM-TEM vs SA-RMTPP-TEM + B & 4.173207 & 3.003424e-05 & 0.034629 \\
               C-SA/MC-TEMP vs Poisson & 5.095332 & 3.481314e-07 & 4.431713e-04 &            SA-LNM-TEM vs SA-RMTPP-TEM & 4.173207 & 3.003424e-05 & 0.034629 \\
  SA-MLP/CM-LE + B vs SA-SA/MC-TEM + B & 5.083509 & 3.705241e-07 & 4.701951e-04 &     SA-MLP/CM-TO vs GRU-SA/MC-TEM + B & 4.173207 & 3.003424e-05 & 0.034629 \\
          GRU-CP-TEM + B vs GRU-LNM-TO & 5.071687 & 3.943038e-07 & 4.999772e-04 &             SA-CP-TO vs SA-MLP/MC-TEM & 4.167296 & 3.082348e-05 & 0.035447 \\
            SA-CP-TO vs GRU-MLP/MC-TEM & 5.065776 & 4.067394e-07 & 5.153388e-04 &   GRU-MLP/CM-LE + B vs GRU-MLP/MC-TEM & 4.167296 & 3.082348e-05 & 0.035447 \\
             C-CP-TEMP vs GRU-SA/CM-TO & 5.059865 & 4.195529e-07 & 5.311540e-04 &    GRU-MLP/CM-TO vs GRU-SA/MC-TEM + B & 4.161384 & 3.163240e-05 & 0.036314 \\
               C-CP-TEMP vs C-SA/CM-LE & 5.048043 & 4.463584e-07 & 5.646434e-04 &              SA-LNM-TO vs SA-RMTPP-TO & 4.137740 & 3.507431e-05 & 0.040230 \\
          GRU-LNM-TEM vs GRU-MLP/CM-LE & 5.048043 & 4.463584e-07 & 5.646434e-04 &             C-CP-TEMP vs GRU-RMTPP-TO & 4.114096 & 3.886996e-05 & 0.044545 \\
       SA-MLP/CM-LE + B vs SA-SA/CM-LE & 5.048043 & 4.463584e-07 & 5.646434e-04 &              GRU-CP-TEM vs C-LNM-TEMP & 4.102274 & 4.091095e-05 & 0.046843 \\
      C-RMTPP-TEMP vs SA-SA/MC-TEM + B & 5.036221 & 4.748123e-07 & 5.992132e-04 &               SA-CP-TO vs SA-SA/CM-TO & 4.090452 & 4.305337e-05 & 0.049253 \\
     GRU-MLP/CM-LE + B vs GRU-SA/CM-LE & 5.024399 & 5.050118e-07 & 6.368198e-04 &         GRU-SA/MC-TEM vs GRU-SA/MC-TO & 4.090452 & 4.305337e-05 & 0.049253 \\ \\
\hline \\
\end{tabular}
\caption{Pairwise comparisons of all models on the time calibration using Schaffer's correction.}
\end{table}
\end{comment}


\restoregeometry
